Learning Causality for Longitudinal Data

This thesis develops methods for causal inference and causal representation learning (CRL) in high-dimensional, time-varying data. The first contribution introduces the Causal Dynamic Variational Autoencoder (CDVAE), a model for estimating Individual Treatment Effects (ITEs) by capturing unobserved heterogeneity in treatment response driven by latent risk factors that affect only outcomes. CDVAE comes with theoretical guarantees on valid latent adjustment and generalization bounds for ITE error. Experiments on synthetic and real datasets show that CDVAE outperforms baselines, and that state-of-the-art models greatly improve when augmented with its latent substitutes, approaching oracle performance without access to true adjustment variables. The second contribution proposes an efficient framework for long-term counterfactual regression based on RNNs enhanced with Contrastive Predictive Coding (CPC) and InfoMax. It captures long-range dependencies under time-varying confounding while avoiding the computational cost of transformers, achieving state-of-the-art results and introducing CPC into causal inference. The third contribution advances CRL by addressing how latent causes manifest in observed variables. We introduce a model-agnostic interpretability layer based on the geometry of the decoder Jacobian. A sparse self-expression prior induces modular, possibly overlapping groups of observed features aligned with shared latent influences. We provide recovery guarantees in both disjoint and overlapping settings and show that meaningful latent-to-observed structure can be recovered without anchor features or single-parent assumptions. Scalable Jacobian-based regularization techniques are also developed.

==> 1.tex <==
\chapter{Introduction}
\label{chapter:intro}

As traditionally intended, machine learning models aim at recognizing patterns and identifying statistical dependencies for tasks like prediction, classification, and regression \citep{jordan2015machine}. However, these models can \emph{capture} spurious relationships by focusing primarily on correlations. When applied under different conditions, they may mislead, since a statistical association alone does not imply a causal link \citep{pearl2009causality}. 

Causal inference provides a principled framework to capture cause-and-effect relationships \citep{spirtes2010introductionCI, Imbens2015CausalIF, peters2017elements}. In the context of \gls{xai}, there is growing recognition that purely correlation-based explanations can fail to generalize under interventions or distributional shifts \citep{LinardatosXAIReview2021, carloni2025roleCausalityXAI}. Embedding causal assumptions into machine learning workflows strengthens the transparency and trustworthiness of model outputs and leverages scalable algorithms, such as deep neural networks, to handle high-dimensional and time-varying data more effectively \citep{berrevoets2024causal}. At the same time, advances in machine learning have empowered causal inference methods to scale to large, complex datasets, including unstructured data like text and images, overcoming computational bottlenecks of traditional approaches \citep{deshpande2022multiModalSCM, deng2022deepCL}. Together, this synergy between machine learning's computational strengths and causal inference's rigorous foundations paves the way for more robust, interpretable, and reliable data-driven decision making \citep{chernozhukov2018double, ijcai2021p0585, wang2021RobustnessCausality,sanchez2022causal}. 

Causal inference is dedicated to understanding cause‐and‐effect relationships and estimating causal effects between variables \citep{pearl2009causality, Imbens2015CausalIF}. For instance, we might ask: \textit{Does a new drug (the “treatment” \(W\)) lower blood pressure (the “outcome” \(Y\))} ? In a \gls{rct}, patients are randomly assigned to receive the drug or a placebo, ensuring that, on average, nothing else differs between the groups. In observational data, however, patients choose to receive the drug based on characteristics like age, health status, or socioeconomic factors, and the way such choice occurs is unknown, which we commonly refer to as the \emph{unknown assignment mechanism}. These characteristics are called \emph{confounders} (\(X\)) when they influence \(W\) and \(Y\). When confounders are present, comparing treated versus untreated individuals can give a misleading estimate of the treatment's effect \citep{holland1986statistics, pearl2009causality, spirtes2010introductionCI}. For example, if older patients are both more likely to receive the drug and have higher blood pressure, an analysis that ignores age may wrongly conclude that the drug increases blood pressure. 

Although machine learning models excel at capturing complex data dependencies and achieving high predictive performance \citep{lecun2015deep}, predictive modeling alone is inadequate for causal inference from observational data. Observational data capture only factual outcomes and lack randomized treatment assignment, making it difficult to infer causation directly \citep{pearl2009causality, peters2017elements, fernandez2022causal}. Hence, addressing these challenges requires a causal framework. There are two fundamental frameworks for learning causality, \gls{scm} \citep{pearl2009causality} and \gls{po} \citep{rubin2005causal}, which are equivalent in what they can express \citep{pearl2009CIOverview, ibeling2023comparingSCMvsPO}. A causal model is any model that explicitly encodes cause‐and‐effect relations between variables. An \gls{scm} consists of (cf. Chapter \ref{chapter:background}, Section \ref{sect_background:causal_graphs}): 
\begin{inparaenum}[(1)]
\item A \gls{dag} whose nodes represent random variables and whose arrows denote direct causal influence (e.g., "smoking \(\rightarrow\) lung disease").
\item A corresponding set of structural mechanisms, each of which specifies how a variable is generated by its direct causes (its "parents" in the \gls{dag}), together with background noise.
\end{inparaenum}
The graph and the mechanisms jointly define how variables would change under hypothetical interventions and support counterfactual reasoning \citep{pearl2009causality}. In contrast, the \gls{po} approach (cf. Chapter \ref{chapter:background}, Section \ref{sect_background:po_framework_static_def}) defines, for each unit, the outcome that would be observed under each treatment regime (e.g., "the blood‐pressure reading if treated" vs. "if not treated") and defines causal effects as comparisons between these potential outcomes \citep{rubin2005causal}. 

In many applications where individuals may respond differently to the same intervention, such as healthcare, social sciences, and marketing, estimating an \gls{ite} is instrumental. Understanding these heterogeneous treatment effects allows for more personalized and effective interventions. For instance, accurate treatment effect estimation in healthcare can enable clinicians to select optimal treatments tailored to individual patients \citep{shalit2020ITPolicyClinical, atan2018Deep-Treat, mueller2023personalized}. In the social sciences, \gls{ite} estimation can inform targeted interventions that address the specific needs of different population groups \citep{morgan2013handbookSocial, Imbens2015CausalIF}, while in marketing, it allows businesses to refine strategies tailored to particular groups of customers \citep{fang2023alleviating, hair2021dataMarketing}.

\paragraph{Handling Unobserved Heterogeneity in Treatment Effect Estimation for Longitudinal Data}
This thesis focuses on estimating treatment effects within longitudinal data settings, which present several challenges: complex temporal dependencies, time-dependent confounding, and unobserved heterogeneity. If the unobserved sources of heterogeneity are assumed to be confounders, then any naive estimation of the treatment from observed data will be biased. However, the thesis argues that other sets of unobserved features that are not confounders but only explain the response are also crucial if one aims to estimate \gls{ite}. These variables are called \emph{adjustment variables} \citep{pearl2009causality, hassanpour2019DRLCFR, qidong2020new, zhang2021treatment, zheng2024adr}, \emph{risk factors} \citep{zhang2021treatment}, or \emph{effect modifiers} \citep{VanderWeele2007FourTO,vanderweele2012confounding,schouten2024on}. We therefore address this problem as our first contribution in Chapter~\ref{chapter:cdvae} while studying the immediate effect following the application of a treatment that is the \emph{contemporaneous effects} (Assumption~\ref{assp:contemporaneous_effect}). We reframe our problem as follows: 

\begin{question}
\label{question:cdvae}
In longitudinal data, when we are missing baseline covariates that affect only the series of responses, how can we estimate a time-varying treatment effect that is as individual as possible? 
\end{question}

\subparagraph{Significance of the Question~\ref{question:cdvae} in Retail: Example of Saint-Gobain}

\emph{\gls{sgdbf}} is exploring solutions to enhance client satisfaction and operational sustainability. Causal inference is an attractive way to understand client behavior,  leveraging transaction data that records customer interactions, preferences, and purchasing patterns over time. The sequential nature of this data provides an opportunity to infer the causality underlying customer decisions, thereby enabling SGDBF to better understand the effect of the continuing commercial action on the customer purchase behavior and, ultimately, the \gls{roi}. An example of an application involves understanding the impact of commercial visits on client behavior. Here, clients are craftsmen or construction firms, and Saint-Gobain's products are construction materials. Each client group is assigned to a sales representative who schedules in-person visits, sometimes following a phone call, and may visit multiple times within a week. The binary treatment variable (i.e., whether the client received a call or not) affects purchase behavior, which can be quantified in terms of purchase frequency or average purchase amount spent post-visit. Here, a client is considered \emph{treated} if they received at least one visit at each time step, representing a week's time window. As an illustration of Question~\ref{question:cdvae} and considering a time-varying setting where observable variables include client preferences \(\mathbf{X}_t\), the intervention or treatment represented by an in-person visit \(W_t\), and the subsequent outcome, or purchase amount \(Y_t\). However, an unobserved variable, \(\mathbf{U}\), representing the number of current construction projects of the client, introduces an additional challenge: If a client is managing multiple projects simultaneously, receiving a visit may increase their purchase frequency and amount. Conversely, if they have few or no active projects, even multiple commercial visits may fail to incentivize purchases due to a lack of projects to consume the materials.

We, therefore, aim to estimate the effect of treatment \(W_{t+1}\) on \(Y_{t+1}\) given a context history $\mathbf{H}_t$ that includes all records as in Figure~\ref{fig:CG_compressed_contemp}, while also accounting the possible heterogeneity in treatment effect that may be induced by the unobserved variable $\mathbf{U}$.
\begin{figure}[!htbp]
\begin{center}
\includegraphics[scale=0.6]{figures/cdvae/cg_cdvae_compressed.pdf}
\caption{A compressed description of the data generation process behind the causal Question~\ref{question:cdvae}.}
\label{fig:CG_compressed_contemp}
\end{center}
\end{figure}

\subparagraph{Significance of the Question~\ref{question:cdvae} in Precision Medicine} Consider a scenario where we aim to estimate the effect of a medical intervention like chemotherapy \(W_t\) on the volume of a cancerous tumor \(Y_t\). During a time window of medical treatment, one could gather all records on vital measures that were measured as \(\mathbf{X_t}\). However, it is not infrequent in such a medical scenario to have missed essential baseline covariates \(\mathbf{U}\), such as genetic predispositions, lifestyle factors, and pre-existing health conditions, that may influence patients' responses to the treatment. Therefore, the underlying \gls{dgp} could be described compactly in Figure~\ref{fig:CG_compressed_contemp}. As a result, individual response to treatment and, therefore, its efficacy may crucially depend on unobserved adjustment variables \(\mathbf{U}\).

\subparagraph{Related contributions to Question~\ref{question:cdvae}}
\begin{itemize}
    \item \textit{\underline{M El Bouchattaoui}, M Tami, B Lepetit, PH Cournède. Causal dynamic variational autoencoder for counterfactual regression in longitudinal data}. Under review at TMLR 2025.
    \item \textit{\underline{M El Bouchattaoui}, M Tami, B Lepetit, PH Cournède. A non-linear mixed effect model for the estimation of causal effects through time}. The 54th Annual Meeting of the French Statistical Society, 2023, 10 pages.
    \item  \textit{\underline{M El Bouchattaoui}, M Tami, B Lepetit, PH Cournède. CDVAE: Estimating causal effects over time under unobserved adjustment variables. }Colloquium Quarter causality (When Causal Inference meets Statistical Analysis, Paris 2023).
    \item Open source implementation: \url{https://github.com/moad-lihoconf/cdvae}.
\end{itemize}


\paragraph{From Immediate to Long-Term Treatment Effects}
Building on our initial focus on handling unobserved heterogeneity and estimating treatment effects for immediate responses, our second contribution broadens the causal question. Here, we aim to forecast the effect of a sequence of treatments across multiple future time points. We achieve this through careful temporal modeling and architectural design, ensuring a computationally efficient approach to infer long-term treatment effects across various horizons. To summarize, our second contribution answers the following causal question:
\begin{question} 
\label{question:ccpc}
In longitudinal data, assuming no unobserved sources of heterogeneity (whether confounders or risk factors), how can we efficiently estimate the effect of any potential sequence of future treatments (Figure~\ref{fig:CG_compressed_forecast}) on subsequent responses over extended forecasting horizons? 
\end{question}

\begin{figure}[!htbp]
\begin{center}
\includegraphics[scale=0.7]{figures/intro/CG_compressed_forecast.pdf}
\caption{A compressed description of the data generation process behind the causal Question~\ref{question:ccpc}.}
\label{fig:CG_compressed_forecast}
\end{center}
\end{figure}

\subparagraph{Significance of the Question~\ref{question:ccpc} in Retail: Example of Saint-Gobain} In retail, understanding the immediate effect of an intervention, like a promotional campaign or a commercial visit, and its influence over time is essential for long-term ROI and ensuring sustained customer engagement. Being able to assess the long-term effect of a treatment plan is strategic because it enables sales representatives to simulate, on an individual basis, all possible future treatment sequences counterfactually. They can then choose the sequence that maximizes a specific target, such as total or average purchase amount realized following those commercial actions. Using our current notation and following Figure~\ref{fig:CG_compressed_forecast}, the Question\ref{question:ccpc} amounts to assessing the treatment effect of the sequence \((W_{t + 1}, \dots, W_{t + \tau})\) on \(Y_{t+\tau}\) given the history of records $\mathbf{H}_t$.

\subparagraph{Significance of Question~\ref{question:ccpc} in Precision Medicine} Answering this question would allow clinicians to evaluate all possible counterfactual trajectories of patient responses following a treatment strategy \((W_{t + 1}, \dots, W_{t + \tau})\), for example, administering chemotherapy this week, no treatment for the next eight weeks, then radiotherapy in the tenth week, and then choose the best possible treatment path based on the predicted outcome \(Y_{t+\tau}\) for a patient, given their historical records and characteristics \(\mathbf{H}_t\). Such tailored interventions are data-driven and adaptive, meaning that the models could infer updated patient trajectories based on the updated vital signs. 

\subparagraph{Related contribution to Question~\ref{question:ccpc}}
\begin{itemize}
    \item \underline{M El Bouchattaoui}, M Tami, B Lepetit, PH Cournède. Causal Contrastive Learning for Counterfactual Regression Over Time. NeurIPS 2024.
    \item Open source implementation: \url{https://github.com/moad-lihoconf/causal-cpc}.
\end{itemize}

\paragraph{From Treatment Effect Estimation to Discovering Causal Relationships} 

Building on our earlier contributions that focus on estimating treatment effects for specific outcomes, either immediately or over extended horizons, we now shift our attention to the relationships within the dimensions of covariates over time. This final contribution addresses the causal relationships embedded within the covariate dimensions themselves. Specifically, at Saint-Gobain, each time step's covariates capture purchases by product, where each dimension corresponds to the number of purchases made for a particular item. In this context, understanding causal connections between these dimensions over time allows us to gain insight into purchasing behaviors and the pathways that drive them. By studying these causal relationships within the covariate dimensions, we aim to uncover the underlying causal mechanisms that shape purchase patterns, shedding light on how various product purchases influence each other over time. This analysis provides a broader perspective on client behavior, enabling a deeper understanding of purchasing dynamics and effectively informing more targeted strategies for meeting client needs.

Our goal falls, therefore, under the theme of  \gls{crl} \citep{scholkopf2021toward}, whose objective is to uncover high-level latent factors that give rise to complex data. While recent work has made progress in visual or linguistic domains, real-world applications such as retail analytics, healthcare, or behavioral science often involve structured, high-dimensional data evolving over time. In these settings, the high number of observed variables and their entangled dependencies pose a significant barrier to interpretability. Analysts are not only interested in identifying latent causes, but also in understanding how these causes manifest across familiar, fine-grained variables, such as products in retail or diagnoses in healthcare. Yet current \gls{crl} methods offer limited guidance for making these latent factors transparent and actionable. Once a model is trained, it is often unclear what the learned representations mean or how they relate to domain-specific concepts. This lack of interpretability hinders trust, downstream use, and scientific insight. To address this gap, we ask:

\begin{question}
\label{question:crl}
How can we discover causal structure in high-dimensional, evolving data in an interpretable and grounded way, linking latent abstractions to meaningful groupings of observed variables?
\end{question}

\subparagraph{Related contribution to Question~\ref{question:crl}}
\begin{itemize}
    \item \textit{\underline{M El Bouchattaoui}, M Tami, B Lepetit, PH Cournède. Toward a more transparent \gls{crl}, 9th Causal Inference Workshop at UAI 2024.}
    \item Open source implementation: \url{https://github.com/moad-lihoconf/crl_transparency}.
\end{itemize}


\section*{Thesis Roadmap} 
This thesis begins with a foundational exploration of the \gls{po} framework in Chapter \ref{chapter:background}, where we establish core concepts in causal inference, such as \gls{ite}, \gls{cate} and \gls{ate}, using confounders and key identifiability assumptions to address causal inference questions. We then introduce \gls{scm} and causal graphs, setting the stage for \gls{crl}. In Chapter~\ref{chapter:cdvae}, we address estimating treatment effects in settings with unobserved risk factors that influence outcomes over time. Our model, \gls{cdvae}, estimates treatment effects by modeling this unobserved heterogeneity, achieving strong performance on synthetic and semi-synthetic datasets. Extending this approach, Chapter~\ref{chapter:ccpc} presents a novel framework for long-term counterfactual regression using \gls{rnn} with \gls{cpc} and \gls{infomax}. This efficient method captures long-term dependencies without transformers, delivering \gls{sota} results. In Chapter~\ref{chapter:crl}, we address \gls{crl} for high-dimensional, time-varying data, introducing structural sparsity to enhance interpretability by linking latent variables, assumed causal, to observable data. Our method is applied to Saint-Gobain purchase data, showcasing its utility in real-world applications. Finally, Chapter~\ref{chapter:epilogue} summarizes the contributions and discusses implications for advancing causal inference and representation learning in complex, time-varying datasets.







==> 2.tex <==
\chapter{Background}
\label{chapter:background}
The \gls{po} framework is a cornerstone of causal inference, offering a structured approach to defining and estimating causal effects by considering hypothetical outcomes under varying treatment conditions. This chapter introduces the fundamental concepts of potential outcomes and treatments, emphasizing their importance through illustrative examples. The discussion includes the \gls{ite} and the fundamental challenge of causal inference, the inability to observe all potential outcomes for any given individual. Furthermore, we incorporate covariates and examine the role of confounders, introducing key metrics such as the \gls{cate} and \gls{ate}.

The chapter also covers identifiability issues, addressed through assumptions such as the \emph{\gls{sutva}}. We acknowledge complexities introduced by challenges like \emph{spillover effects}, \emph{carryover effects}, and \emph{feedback mechanisms}, which can complicate causal estimation. We also discuss the role of instrumental and adjustment variables, using examples and a simple adjustment-based model to clarify these concepts. An overview of related work on identifiability, ATE, and \gls{cate} in static settings provides a foundation for subsequent discussions on more complex, dynamic environments.

In transitioning to \emph{time-varying} settings, the chapter explores alternative definitions of potential outcomes, as highlighted in our key contributions, such as \gls{cdvae} \citep{bouchattaoui2023CDVAE} and Causal \gls{cpc} \citep{bouchattaoui2024CausalCPC}. We address general definitions and the restrictive assumptions inherent to each model, underscoring the limitations of classical adjustment methods in time-varying contexts. This discussion leads into the identifiability assumptions required for \emph{sequential ignorability} and emphasizes the challenges associated with time-varying treatment regimes.

Finally, the chapter introduces the concept of  \gls{scm} and \emph{causal graphs}, discussing principles such as d-separation and the do-operator. We clarify the distinct yet complementary roles of the \gls{po} framework and \gls{scm} in this thesis: 
\begin{warning}
    \emph{The \gls{po} framework is employed primarily for causal inference, \gls{scm} for causal representation learning, and causal graphs as tools applicable to both approaches}.
\end{warning} 

\section{Potential Outcome Framework: Static setting}
\label{sect_background:po_framework_static}

\subsection{Definition}
\label{sect_background:po_framework_static_def}
The \gls{po} framework, also known as the \emph{Rubin Causal Model} or \emph{Neyman-Rubin Causal Model} \citep{Neyman1923, rubin1974estimating}, is one of the most widely adopted mathematical frameworks in causal inference. This framework provides a rigorous foundation for defining and estimating causal effects by considering hypothetical outcomes that could occur under different treatment conditions.

In causal inference, the main goal is to estimate the effect of an intervention on units such as individuals, organizations, or objects. We are usually interested in how different interventions can lead to different outcomes. For example, medical treatments like chemotherapy or radiotherapy can have distinct effects on the same patient's volume of their cancerous tumour; a commercial campaign with two different contents can have two different engagement/buying effects for the same customer. Moreover, the causal relationship depends not only on the nature and timing of the intervention but also on the specific context of the unit involved, for example, a patient's medical record.

\begin{remark}[Treatment Range]
\label{remark:discrete_treat}
In this thesis, we will consider scenarios where the treatment variable, denoted by $W$, is \emph{discrete} and takes \emph{finite} values within a set $\mathcal{W}$. However, we relax this restriction in causal discovery tasks, allowing variables to originate from a continuous latent space. For discrete treatments, one regime typically corresponds to a passive state (i.e., no treatment or control group), while others correspond to active treatments, which may vary in type, intensity or dosage.
\end{remark}

Let us assume we observe $N$ units. Each pair of a unit and a treatment defines a potential outcome or response, denoted $(i, \omega) \rightarrow Y_i(\omega)$. A potential outcome $Y_i(\omega)$ is said to be \emph{observed} only if the unit $i$ receives treatment $\omega$, i.e., under the event $W_i = \omega$. Importantly, the treatment must precede the observation of the corresponding potential outcome.

Consider the scenario where the treatment is binary, and we observe a finite sample of treatments and responses $\{(W_i, Y_i)\}_{i=1}^N$. The treatment assignment for each unit is defined as follows:
\[
W_i = \begin{cases}
1, & \text{if unit } i \text{ receives the treatment}, \\
0, & \text{if unit } i \text{ receives the control}.
\end{cases}
\]
Each unit $i$ has two potential outcomes: 
\begin{itemize}
\item $Y_i(1)$, the outcome if the unit receives the treatment; and 
\item $Y_i(0)$, the outcome if the unit receives the control. 
\end{itemize}

The causal effect for unit $i$ is the difference between these potential outcomes. This is formally captured by the \gls{ite}:
\[
\tau_i \coloneqq Y_i(1) - Y_i(0).
\]
By definition, for each unit \(i\) we observe only one potential outcome, namely the one corresponding to the observed treatment \(W_i\)  which is \(Y_i(W_i)\), and the counterfactual \(Y_i(1 - W_i)\) remains unobserved. This \emph{fundamental problem of causal inference} \citep{holland1986statistics} means that the individual treatment effect \(\tau_i\) is inherently a missing‐data quantity. We must, therefore, establish connections between observed data and potential outcomes by comparing responses across different units. This necessitates consideration of the \emph{treatment assignment mechanism}, which dictates how treatment is assigned across the population.

Since individual-level causal effects are unobservable, researchers often rely on aggregate measures, such as the \gls{ate}:
\[
\tau \coloneqq \mathbb{E}[Y_i(1) - Y_i(0)],
\]
which captures the expected causal effect of treatment across the entire population. The expectation is taken over the population distribution of units (c.f.  Remark \ref{remark:superpopulation}).

Identifying the \gls{ate} depends on certain assumptions that allow for estimation based on observed data. Implicit in our formulation of potential outcomes is the assumption of \emph{no spillover effect} \citep{Imbens2015CausalIF}, i.e., that the treatment of a unit is the sole determinant of its potential outcome, independent of the treatments assigned to other units. Moreover, the treatment for each unit has a consistent effect, with no variation in efficacy. These ideas are formalized by the \emph{Stable Unit Treatment Value Assumption (\gls{sutva})} \citep{rubin1980randomization}, which consists of two key components:

\begin{assumption}[\gls{sutva}]
\label{assp:sutva}
The \gls{sutva} implies:
\begin{compactenum}
    \item \textbf{No Interference/spillover effect}: The potential outcomes of any unit are unaffected by the treatments assigned to other units, meaning no interference exists between units.
    \item \textbf{Consistency}: The observed outcome for a unit is the same as the potential outcome associated with the treatment it actually received. That is, if $W_i = w$, then $Y_i = Y_i(w)$.
\end{compactenum}
\end{assumption}


The no-interference assumption is critical, though not universally applicable. In real-world scenarios like studying infectious diseases, one unit's potential outcome may be influenced by the treatment status of others, as in the case of immunization effects depending on herd immunity \citep{Imbens2015CausalIF}.

Additional assumptions are necessary to link observed data to potential outcomes to estimate the ATE. One fundamental assumption is \emph{strong ignorability} \citep{Rosenbaum1983TheCR}, which asserts that the treatment assignment, $W$, is independent of the potential outcomes, given a set of observed covariates, $X$. These covariates represent pre-treatment characteristics, i.e., they occur before the treatment and are therefore important for explaining the distribution of $W$.
\begin{warning}
Throughout this thesis, covariates play a central role, mainly as we focus on estimating more individualized treatment effects that vary across subpopulations based on covariate values.  
\end{warning}

\begin{remark}[On the Use of Expectation]
\label{remark:superpopulation}
In causal inference studies, two main perspectives exist for addressing a set of units from a probabilistic standpoint \citep{Imbens2015CausalIF, DingLi2018CIMissingData}. The first considers a \emph{fixed} set of observed units, where all potential outcomes are fixed but partially unknown. In this view, causal effects are defined only for specific units and may not generalize to other sets \citep{holland1986statistics}. The second, adopted in this thesis, assumes the set of units is randomly sampled from an infinite population, referred to as the \emph{super-population} \citep{rubin1974estimating}. This perspective allows for the use of expectation, aligns with standard statistical theory, and offers mathematical convenience. Specifically, it facilitates reasoning about risks and generalization errors, central to machine learning \citep{Vapnik1998, ShalevShwartzBenDavid2014}. By adopting this perspective, we apply principles from statistical learning theory, such as Empirical Risk Minimization, to assess model performance and ensure generalization to new data. While causal inference in fields like social sciences and epidemiology often refers to a finite set of observed units as the "population", we adhere to the statistical theory terminology, using \emph{population} to denote an infinite set. For a finite set, we use the term \emph{sample}.
\end{remark}

In causal inference, we define probability distributions over the space $\mathcal{Y}(0) \times \mathcal{Y}(1) \times \mathcal{W} \times \mathcal{X}$, where $\mathcal{Y}(0)$ and $\mathcal{Y}(1)$ represent the domain ranges of the potential outcomes. For simplicity, we assume these domains are equal and denote the common outcome domain as $\mathcal{Y}$. Therefore, the probability distribution for causal inference is defined over $\mathcal{Y}^2 \times \mathcal{W} \times \mathcal{X}$, which allows us to sample $(Y(0), Y(1), W, X)$ in an independent and identically distributed (i.i.d.) manner.

\begin{remark}
Since all relevant domains are either finite sets or subsets of Euclidean spaces, we assume all probability distributions are absolutely continuous w.r.t the Dirac or Lebesgue measure. As a result, a probability density function, denoted as $p$, exists by the Radon-Nikodym theorem \citep{billingsley2017probability}.
\end{remark}

Thus, individual data points $(Y_i(0), Y_i(1), W_i, X_i)$ are sampled from the joint distribution:
\[
p(Y_i(0), Y_i(1), W_i, X_i) = p(W_i \mid Y_i(0), Y_i(1), X_i) p(Y_i(0), Y_i(1) \mid X_i) p(X_i).
\]

The treatment assignment mechanism is encapsulated in $p(W_i \mid Y_i(0), Y_i(1), X_i)$, which describes how treatment is assigned. Since much of this work assumes a binary treatment, it is often sufficient to study the propensity score, defined as:
$$
e(X_i, Y_i(0), Y_i(1)) \coloneqq p(W_i = 1 \mid Y_i(0), Y_i(1), X_i).
$$
However, because the general definition of the propensity score includes unobserved potential outcomes, we commonly assume the assignment mechanism to be \emph{unconfounded} (also said ignorable). Formally,
\begin{assumption}[Ignorability/unconfoundedness]
\label{assp:ignorability}
The treatment assignment does not depend on the potential outcomes: 
\begin{equation}
\label{eq:ignorability}
\{Y_i(1), Y_i(0)\} \perp\!\!\!\perp W_i \mid X_i.
\end{equation}
\end{assumption}

Under this assumption, the propensity score simplifies to:
\begin{equation}
\label{eq:propensity_static}
    e(X_i) = p(W_i = 1 \mid X_i).
\end{equation}
The \emph{ignorability assumption,} as stated in Equation \ref{eq:ignorability}, ensures that treated and untreated subpopulations are comparable within any homogeneous region of $\mathcal{X}$. To ensure this comparability, it is essential that both treated and control units are present at each level of $X$. This necessity leads to the "overlap" assumption:
\begin{assumption}[Overlap/Positivity]
\label{assp:overlap_static}
For any given context realization $x \in \mathcal{X}$, the probability of observing \emph{any} treatment regime $\omega \in \mathcal{W}$ is strictly positive:
\begin{equation}
p(x) \neq 0 \implies p(W = \omega \mid x) > 0.
\end{equation}
\end{assumption}
These assumptions, namely consistency (\ref{assp:sutva}), overlap (\ref{assp:overlap_static}), and unconfoundedness (\ref{assp:ignorability}), provide the foundation for identifying causal effects that we summarize under the assumption of \emph{strong ignorability}.
\begin{definition}[Strong Ignorability]
\label{assp:strongly_ignorable}
The treatment assignment is considered strongly ignorable if consistency, overlap, and unconfoundedness hold.
\end{definition}
Given strong ignorability, we can relate the conditional expectations of potential outcomes to observable quantities \citep{Imbens2015CausalIF}:
$$
\mathbb{E}[Y_i(\omega) \mid X_i = x] = \mathbb{E}[Y_i \mid W_i = \omega, X_i = x], \quad \omega \in \{0, 1\}.
$$
This relationship enables estimation of the \gls{cate} for units with covariates $X_i = x$:
$$
\tau(x) \coloneqq \mathbb{E}[Y_i \mid W_i = 1, X_i = x] - \mathbb{E}[Y_i \mid W_i = 0, X_i = x].
$$
The overlap assumption ensures that treated and control units exist at each value of $x$, allowing computation of $\tau(x)$. The \gls{ate} is then obtained by averaging $\tau(x)$ over the distribution of $X_i$:
$$
\tau = \mathbb{E}_X\Bigg[ \mathbb{E}\left[Y_i(1) \mid X_i = x\right] - \mathbb{E}\left[Y_i(0) \mid X_i = x\right] \Bigg].
$$
\begin{remark}
In randomized experiments, the experimenter designs the assignment mechanism, specifying how individual treatments are assigned. However, this thesis focuses solely on \underline{observational studies}, where the assignment mechanism \underline{is not controlled} and must be inferred from data, even under strong ignorability, estimating propensity scores is crucial in this process.
\end{remark}

\paragraph{Taxonomy of variables for causal inference} In the field of causal inference, it is crucial to understand the taxonomy of variables to accurately estimate causal effects. This is depicted in Figure \ref{fig:General_Static_CG}. The response variable, \( Y \), represents the outcome we want to explain or predict. The treatment variable, \( W \), is believed to influence \( Y \), and we seek to estimate its causal effect. Confounders, \( X \), are variables that affect both \( W \) and \( Y \), which can potentially bias the causal effect if not properly controlled. In our modeling for \gls{cdvae} (Chapter \ref{chapter:cdvae}), we also consider another important set of variables: adjustment variables, \( U \). These variables affect the response but not the treatment, making them adjustment variables for outcome modeling to yield more precise individual response trajectories. Similarly, instruments, \( I \), are variables that affect the treatment \( W \) but not \( Y \), except indirectly through \( W \). The study of causal inference in the presence of instruments is out of the scope of thesis.
\begin{figure}[!htbp]
\begin{center}
\includegraphics[scale=0.7]{figures/background/General_Static_CG.pdf}
\caption{A general causal graph clarifying the causal links between outcome $Y$, treatment $W$, confounders $X$, adjustment variables $U$ and instruments $I$.}
\label{fig:General_Static_CG}
\end{center}
\end{figure}
\begin{remark}[\gls{cate} vs ATE]
Understanding when to use the \gls{ate} versus the \gls{cate} is crucial in statistical causal inference because it influences the analytical approach and the interpretation of results. The \gls{ate} is used when the treatment effect is presumed to be consistent across an entire population or when making policy decisions that affect everyone. This concept is particularly useful for generalizing findings, as highlighted in foundational works \citep{rubin1974estimating, holland1986statistics}.

On the other hand, the \gls{cate} is vital for examining how treatment effects differ among subpopulations defined by specific covariates like age, gender, or socioeconomic status. The \gls{cate} offers a deeper dive into the nuances of causal relationships, enabling a more tailored analysis in situations where treatment effects are not uniform across all individuals \citep{Rosenbaum1983TheCR}. This approach is especially relevant in sectors such as personalized medicine, where understanding and leveraging the diversity in treatment responses can significantly enhance outcomes \citep{murphy2003OptimTreatRegime}.

Utilizing the \gls{cate} allows for the identification of subgroups that might benefit more from a treatment or, conversely, might be at risk of adverse effects. This strategic insight aids in decision-making and resource distribution, thereby elevating the effectiveness and precision of interventions.
\end{remark}

\subsection{Methods: An Overview}
\label{sect_background:po_framework_static_overview}

\paragraph{Weighting Methods} Weighting methods are widely used in causal inference to adjust for confounding by reweighting the data. This creates a synthetic population where the treatment assignment is independent of covariates. This technique allows for the estimation of causal effects by weighting units inversely proportional to their probability of receiving the treatment or control. One of the key methods in this domain is \emph{\gls{iptw}}, which employs the inverse of the propensity score (Equation \ref{eq:propensity_static}) to weight observations \citep{Rosenbaum1983TheCR}. \gls{iptw} adjusts the sample to create a pseudo-population where the covariates' distribution is balanced between treated and control units, facilitating an unbiased estimation of \gls{ate}. A refinement to \gls{iptw}, proposed by \citet{hirano2001estimation}, involves \emph{propensity score weighting with regression adjustment}, enhancing the estimator's efficiency. This method merges weighting with outcome regression, yielding consistent estimates even when the outcome model is inaccurately specified. 

More recent developments have introduced machine learning-based methods to enhance the accuracy of weighting strategies. \citet{athey2017state} developed the \emph{Generalized Propensity Score} approach, which allows for flexible, nonparametric modeling of the propensity score using random forests \citep{Breiman2001RandomF}. This is particularly useful for dealing with the limitations of parametric models, which may not perform well with high-dimensional covariates. Another method is the \emph{\gls{tmle}}, introduced by \citet{van2006targeted}. \gls{tmle} is a doubly robust estimator that incorporates propensity score weighting with a targeted regression adjustment for the outcome. It offers semiparametric efficiency and ensures valid inference even when the propensity score or outcome model is misspecified.

\paragraph{Matching Methods} Matching methods are a prominent category of causal inference techniques designed to generate balanced treatment and control groups by pairing or grouping units with similar covariates. The objective is to emulate the randomization process, ensuring that treated and control units are comparable on observed covariates. This reduces confounding and enhances the validity of causal effect estimates. 

\emph{Propensity Score Matching (PSM)} stands out as one of the most widely adopted matching techniques. Developed by \citet{Rosenbaum1983TheCR}, PSM pairs treated and control units based on their propensity scores, which reflect the probability of receiving treatment given the covariates. Matching on the propensity score allows PSM to create groups that are balanced on covariates, facilitating unbiased estimation of treatment effects. \citet{austin2011introduction} offers an in-depth review of PSM's benefits and limitations, highlighting that while it significantly reduces bias, its efficacy is contingent on the quality of the propensity score model. \emph{Nearest Neighbor Matching (NNM)} is another widely adopted method, pairing each treated unit with the control unit possessing the closest covariate values or propensity scores. \citet{abadie2006large} enhance NNM by introducing bias-corrected matching estimators that compensate for covariate discrepancies between treated and control units, thereby increasing the precision of treatment effect estimates. \emph{Mahalanobis Distance Matching}, proposed by \citet{rubin1973matching}, employs the Mahalanobis distance for matching treated and control units based on the covariance structure of the covariates. This technique is especially effective when covariates are measured on differing scales, as the Mahalanobis distance accounts for correlations among covariates. \citet{stuart2010matching} extends the discussion to more sophisticated matching methods like \emph{Optimal Matching} and \emph{Genetic Matching}. Optimal Matching aims to minimize the total distance between treated and control units throughout the sample, whereas Genetic Matching leverages an evolutionary algorithm to optimize the balance between the groups. Recent developments have introduced matching methods based on machine learning to enhance flexibility and accuracy in high-dimensional settings. For example, \citet{kallus2018balanced} suggests \emph{Balanced Nearest Neighbor Matching}, which applies a machine learning approach to identify optimal matches that minimize covariate imbalance. 

\paragraph{Regression Adjustment} 
Including covariates in regression models allows for adjusting confounding, isolating the treatment's effect on the outcome. One of the earliest examples of regression adjustment can be found in the work of \citet{cochran1947some}, who proposed using linear regression models to adjust for covariates to estimate a treatment's causal effect. \citet{rubin1973use} expanded on this approach by formalizing regression adjustment within the \gls{po} framework, illustrating how regression can estimate both the \gls{ate} and the \gls{cate}. \gls{glm} broadens the scope of linear regression to accommodate non-normal outcome distributions, such as binary or count data \citep{mccullagh1989GLM}. \gls{glm} are extensively utilized in causal inference studies, especially in epidemiology, where outcomes are often binary events (e.g., disease occurrence). 

A significant advancement in regression adjustment methods is \emph{Doubly Robust Estimation}. Introduced by \citet{robins1995semiparametric}, this method combines outcome regression with propensity score weighting to provide valid treatment effect estimates, even if one of the models (either the outcome model or the propensity score model) is incorrectly specified. \citet{bang2005doubly} demonstrated that doubly robust estimators offer greater robustness to model misspecification than traditional regression methods. \emph{Nonparametric Regression} techniques, such as \emph{Kernel Regression} and \emph{Spline Regression}, allow for flexible modeling of the covariate-outcome relationship without assuming a specific functional form. \citet{abadie2005semiparametric} introduced semiparametric regression models that mix parametric and nonparametric components for more flexible treatment effect modeling. In recent years, regression methods based on machine learning have become popular in causal inference. For example, \citet{Athey2019GeneralizedRF} proposed Generalized Random Forests (GRF), employing regression trees to estimate heterogeneous treatment effects. 

\paragraph{Non-parametric models}
An important class of non-parametric models refers to the extension of random forests \citep{Breiman2001RandomF} to perform causal inference. To this end, causal forests were introduced in \cite{Wager2018EstimationAI, Athey2019GeneralizedRF} as a non-parametric approach to estimate treatment effects in complex settings. To do so, causal forests split the data into two groups based on the treatment assignment and then built separate trees for the treated and untreated groups. The prediction for an individual is then obtained by combining the predictions from the treated and untreated trees. The \gls{cate} is estimated as the difference between the predictions for the treated and untreated groups. 

To develop more robust estimation methods, an emerging technique called \emph{Double Machine Learning} (DML) \citep{chernozhukov2017orthogonal, chernozhukov2018double, Foster2019OrthogonalSL} could provide an unbiased estimate of treatment effects on the condition that either the outcome model or the treatment model is well specified the general method consists of two stages of estimation. In the first step, we fit two predictive tasks, one on the outcome and one on the treatment, and then the two fitted models are combined to perform a second estimation targeting CATE.

\paragraph{Neural Network-Based Approaches} Representation learning \citep{bengio2013representation} has emerged as a powerful strategy for causal inference, particularly useful when dealing with high-dimensional covariates and complex data structures. The goal is to transform the covariates into a lower-dimensional representation that facilitates the estimation of causal effects by reducing the bias due to confounding. This is typically achieved through creating representations where the distributions of treated and control groups are balanced. For instance, \citet{shalit2017estimating} proposed the concept of learning \emph{balancing representations} by minimizing both the prediction error of the outcome and a discrepancy measure between the treated and control distributions in the representation space. They introduced an objective function that combines a supervised loss for outcome prediction with an unsupervised loss for distributional alignment. Building on this concept, \citet{shalit2017estimating} developed the \emph{Counterfactual Regression} (CFR) model, which employs neural networks to learn representations that minimize the distance between the distributions of treated and control units using Integral Probability Metrics (IPMs) \citep{muller1997IPM}, such as the Wasserstein distance or Maximum Mean Discrepancy (MMD) \citep{gretton2012kernel}. By reducing this distance, the model aims to satisfy the unconfoundedness assumption in the representation space, effectively making the treatment assignment independent of the covariates after transformation. Further extending these ideas, \citet{yoon2018ganite} introduced \emph{GANITE}, a Generative Adversarial Network (GAN)-based framework for estimating individualized treatment effects. \emph{Dragonnet}, proposed by \citet{shi2019Dragonnet}, integrated propensity score estimation directly into the representation learning process and jointly learned the representation and the propensity score. Additionally, \citet{hassanpour2019counterfactual} presented \emph{Counterfactual Networks}, which used domain adversarial training to learn representations invariant to treatment assignment while preserving outcome-predictive information. This approach helps mitigate biases due to observed confounding by ensuring that the learned representations do not carry treatment-specific information. \citet{louizos2017causalproxyconf} introduced the \emph{Causal Effect Variational Autoencoder} (CEVAE), which used deep variational inference to model the joint distribution of covariates, treatments, and outcomes. Extension to multi-treatment settings was proposed by \citet{Schwab2018PerfectMatch} where they combined representation learning with optimal transport to balance covariates across multiple treatment groups simultaneously.

As a summary, Table~\ref{tab:comparison_methods} presents a comparative overview of the main causal inference models discussed, grouped by category and highlighting key characteristics and references.
\begin{table}[h!]
\centering
\caption{Comparison of Causal Inference Methods by Category}
\renewcommand{\arraystretch}{2} 
\resizebox{\textwidth}{!}{
\begin{tabular}{|l|l|p{10.5cm}|l|}
\hline
\textbf{Category} & \textbf{Method / Model} & \textbf{Key Characteristics} & \textbf{Reference(s)} \\
\hline
\multirow{4}{*}{Weighting Methods} 
& IPTW & Uses inverse propensity score for weighting; creates pseudo-population &  \cite{Rosenbaum1983TheCR} \\
& Propensity Score + Regression & Combines weighting and regression for robustness & \cite{hirano2001estimation} \\
& Generalized Propensity Score & Uses machine learning for flexible estimation & \cite{athey2017state, Breiman2001RandomF}\\
& \gls{tmle} & Doubly robust; targeted estimation with ML enhancements & \cite{van2006targeted} \\
\hline

\multirow{5}{*}{Matching Methods} 
& Propensity Score Matching (PSM) & Matches on estimated treatment probability & \cite{Rosenbaum1983TheCR} \\
& Nearest Neighbor Matching (NNM) & Pairs treated with nearest control units & \cite{abadie2006large} \\
& Mahalanobis Distance Matching & Accounts for covariate correlation in matching & \cite{rubin1973matching}  \\
& Optimal / Genetic Matching & Minimizes global imbalance; uses optimization algorithms & \cite{stuart2010matching}\\
& Balanced Nearest Neighbor Matching & ML-based flexible matching & \cite{kallus2018balanced} \\
\hline

\multirow{4}{*}{Regression Adjustment} 
& Linear / \gls{glm}  Regression & Adjusts for covariates using parametric models & \cite{cochran1947some} \\
& Doubly Robust Estimation & Combines regression and weighting; robust to model misspecification & \cite{robins1995semiparametric, bang2005doubly} \\
& Semiparametric Regression & Blends linear and nonparametric terms & \cite{abadie2005semiparametric} \\
& Generalized Random Forests (GRF) & Nonparametric, tree-based regression for heterogeneous treatment effects & \cite{Athey2019GeneralizedRF}\\
\hline

\multirow{2}{*}{Non-Parametric Models} 
& Causal Forests & Builds separate trees for treated and control; estimates \gls{cate} & \cite{Wager2018EstimationAI, Athey2019GeneralizedRF} \\
& Double Machine Learning (DML) & Orthogonalizes outcome and treatment models using ML & \cite{chernozhukov2017orthogonal, chernozhukov2018double, Foster2019OrthogonalSL}\\
\hline

\multirow{6}{*}{Neural Network Approaches} 
& Counterfactual Regression (CFR) & Balancing representations via neural networks & \cite{shalit2017estimating} \\
& GANITE & GAN-based model to estimate individual treatment effects & \cite{yoon2018ganite} \\
& Dragonnet & Integrates propensity score estimation within a deep net & \cite{shi2019Dragonnet}  \\
& Counterfactual Networks & Adversarial training to ensure balance and outcome prediction & \cite{hassanpour2019counterfactual} \\
& CEVAE & Uses variational autoencoders to model unobserved confounders & \cite{louizos2017causalproxyconf} \\
& Perfect Match & Optimal transport-based method for multi-treatment settings & \cite{Schwab2018PerfectMatch} \\
\hline
\end{tabular}
}
\label{tab:comparison_methods}
\end{table}



\section{Potential Outcome Framework for Longitudinal data: Main Setting of the Thesis}
\label{sect_background:po_framework_longit}
\subsection{Introduction: Dynamic vs. Time-Varying Treatment Regimes} 
\label{sect_background:po_framework_longit_intro}

\paragraph{Motivation}
In research across various fields, such as healthcare, the primary goal is the discovery of effective treatment regimes or intervention strategies. For instance, in clinical settings, a drug might be effective for one patient yet ineffective or even harmful for another \citep{collins2015new}. Similarly, in business, what works for one customer may fail for another. This heterogeneity rules out a one-size-fits-all approach and motivates the use of \emph{policies}, also known as \emph{Dynamic Treatment Regimes (DTRs)}. Policies/DTRs provide a flexible and personalized approach by utilizing a series of decision rules that facilitate adaptive interventions over time \citep{murphy2003OptimTreatRegime, robins2004optimal}. These rules map an individual's historical data, such as medical records in healthcare or consumer attributes in retail, to specific treatments. For example, a company might develop a series of promotional actions or sales visits customized to a customer's previous interactions with the brand. Decision rules could specify the timing and approach for in-person sales visits based on the customer's past engagement and purchase history \citep{shin2006response}. In precision medicine, the type and dosage of treatments should be adjusted according to a patient's medical records and vital statistics \citep{schulte2014q}. DTRs consist of decision rules aimed at selecting personalized treatments over time, adapting to individuals' changing contexts and responses.

\paragraph{Main challenges}
Understanding cause and effect in complex, dynamic scenarios presents substantial challenges. Responses and evolving factors frequently influence time-varying treatments. For instance, a patient's reaction to initial treatment can affect future treatment choices \cite{vanderLaanPetersen2007}. Other time-varying confounders, such as disease progression or changes in patient behavior, further complicate this situation. Similarly, in marketing, a customer's response to an initial promotion might influence future marketing strategies and other dynamic covariates like customer preferences or external market conditions, which could also impact both treatment and response.

\paragraph{Setup} Within the \gls{po} framework, as described by \cite{robins2009estimation}, we consider a cohort of individuals, also referred to as units, denoted by \( i \in \{1, 2, \dots, N\} \), each observed over \( T \) sequential time steps. For each time step \( t \in \{1, 2, \dots, T\} \), several key variables are tracked:

\begin{itemize}
    \item \textbf{Treatment} \( W_{it} \in \mathcal{W} = \{0, \dots, K-1\} \): This represents the treatment administered to individual \( i \) at time \( t \) which takes \(K\) different values. For example, in a medical context, \( W_{it} \) might represent the administration of radiotherapy to treat a cancerous tumor.
  
    \item \textbf{Outcome} \( Y_{it} \in \mathcal{Y} \subset \mathbb{R} \): This is the response or outcome of interest that we wish to evaluate as a result of the treatment in the case of a cancer patient, \( Y_{it} \) could represent the tumor volume at time \( t \).
  
    \item \textbf{Context} \( \mathbf{X}_{it} \in \mathcal{X} \subset \mathbb{R}^{d_x} \): This denotes the set of covariates or confounders that may influence both the treatment decision and the outcome. The context is represented as a \( d_x \)-dimensional vector that varies over time, for example, in a medical setting, \( \mathbf{X}_{it} \) could include a patient's medical records, vital signs, or other health-related factors that change over time. Both static and dynamic confounders can be concatenated with dynamic variables at each time step and represented as \( \mathbf{X}_{it} \).

    \item \textbf{Partially observed potential outcomes} \( \{Y_{it}(\omega_1, \dots, \omega_t) \mid (\omega_1, \dots, \omega_t) \in \mathcal{W}^t \} \subset \mathcal{Y} \subset \mathbb{R} \): These represent the potential outcomes for an individual \( i \) at time \( t \), conditional on the sequence of treatments \( (\omega_1, \dots, \omega_t) \) received up to that point.
\end{itemize}

We define the \emph{history process} \( \mathbf{H}_{it} \in \mathcal{H}_t \) as the collection of all relevant information up to time \( t \) for an individual \( i \). Formally, this includes the covariates, past treatments, and past outcomes:
\begin{equation}
\label{eq:def_process_hist}
    \mathbf{H}_{it} \coloneqq [\mathbf{X}_{i,\leq t}, W_{i,<t}, Y_{i,<t}].
\end{equation}
This history encapsulates the context \( \mathbf{X}_{it} \), past treatment assignments \( W_{i,<t} \), and past outcomes \( Y_{i,<t} \), which are critical in determining the treatment to be administered at a time \( t \). We now define a dynamic treatment regime.

\begin{definition}[Dynamic Treatment Regimes (DTRs)]
\label{def:DTR}
A DTR \( \pi_{\leq T} \coloneqq (\pi_1, \pi_2, \dots, \pi_T) \) is defined as a sequence of decision rules. Each decision rule \( \pi_t \) specifies the treatment to be assigned at a time \( t \) based on the available history up to that point. Formally, the treatment decision rule is expressed as:
\[
\pi_t: \mathcal{H}_t \rightarrow \mathcal{W}.
\]
This rule assigns a treatment \( W_{it} \) based on the individual's history \( \mathbf{H}_{it} \) at the time \( t \). We can, therefore, define a particular set of potential outcomes under a treatment regime \( \pi_{\leq T} \), where each element is represented as \( Y_t(\pi_{\leq t}) \). \emph{Throughout the thesis, we use “dynamic treatment regime” and “policy” interchangeably.}
\end{definition}

In this thesis, we focus on a type of treatment regime that we call \emph{time-varying}, meaning that the potential treatment at a given time step \( t \) does not dynamically depend on the observed history, specifically:
\begin{assumption}[Time-Varying Treatment Regime]
\label{assp:time_varying_treat}
A treatment regime is considered time-varying when its values change over time but in a \emph{non-dynamic} way, that is, for every time step \( t \), and for every realization of the history process \( \mathbf{h}_{t} \), the decision rule is a constant function, i.e., \( \pi_t(\mathbf{h}_{t}) = \omega_t \).
\end{assumption}

It is for this reason that through the thesis, the potential outcomes are denoted as \( Y_t(\omega_{\leq t}) \), where the potential treatment \( \omega_t \) is pre-specified and does not depend on the individual's observed history  \(\mathbf{H}_{t}\). Instead, each \( \omega_t \) is chosen exogenously from the treatment space \(\mathcal{W}\), independently of the realized history process. 

\begin{example}[Time-varying vs. Dynamic Treatments]
    For an individual, two treatment regimes could be : 
    \begin{inparaenum}[(1)]
    \textbf{Time-varying}: administer radiotherapy on days 1–5 of each 21-day cycle.
    \textbf{Dynamic}: increase dose if interim tumor volume has not fallen by 20\% by day 10. 
    \end{inparaenum}
\end{example}

\begin{remark}[Intermediate Potential Outcomes]
\label{remark:intermediate_pos}
In our work, we are not only interested in estimating the treatment effect at the end/follow-up of a study, i.e., only defining causal effects \gls{wrt} the final potential outcomes \( Y_T(\omega_{\leq T}) \). The fact that we measure "intermediate" outcomes \( Y_1, \dots, Y_{T-1} \) motivates the definition of causal effects as functions of the remaining potential outcomes \( Y_t(\omega_{\leq t}) \). Virtually speaking, at each time step, we have a final outcome measured \( Y_t \), for which we aim to estimate the causal effect, either conditional or averaged through \(\mathbb{E}(Y_t(\omega_{\leq t}) \mid \mathbf{X}_{ \leq t}, Y_{<t} )\) or \(\mathbb{E}(Y_t(\omega_{\leq t}))\), respectively.
\end{remark}

\subsection{Causal Effects in Longitudinal Settings: Definitions and Identification}
The missing data problem is exacerbated in longitudinal settings: at each time step \( t \), we only observe one version of the outcome, while \(K^t-1\) potential outcomes are missing because their corresponding treatment assignments were not chosen. This setting is more challenging than estimating causal effects at the end of a study, where only a total of \( K^T - 1 \) missing potential outcomes exist. For our case (c.f. Remark \ref{remark:intermediate_pos}), the total number of missing outcomes throughout the study is \( \sum_{t=1}^T (K^t - 1) \).

For notational convenience, we denote the following vector form for a sequence of covariates:
\[
\mathbf{X}_{ < t}(\omega_{< t}) \coloneqq (\mathbf{X}_1, \mathbf{X}_2(\omega_1), \mathbf{X}_3(\omega_1, \omega_2), \dots, \mathbf{X}_t(\omega_{< t})).
\]
We have defined "potential covariates" due to the sequential nature of the data. This means that current covariates could potentially be affected by past treatments. Therefore, a rigorous definition of the potential outcome should consider both a potential sequence of treatments and a potential sequence of covariates \citep{robins2004optimal,vansteelandt2014structural} : 
\[
Y_{\leq t}(\omega_{\leq t}, \mathbf{X}_{< t}(\omega_{< t}) ) \coloneqq (Y_1(\omega_1), Y_2(\omega_{1, 2}, \mathbf{X}_{2}(\omega_{1})), \dots, Y_t(\omega_{\leq t}, \mathbf{X}_{< t}(\omega_{< t}))).
\]
To draw causal inference in longitudinal data up to time \(t\), we define a probability distribution over the product space consisting of:
\begin{itemize}
  \item all treatments \(W_{\le t}\) forming the space \(\mathcal{W}^t\),
  \item all potential outcomes
  \[
  \bigl\{Y_s(\omega_{\leq s}) : \omega_{\leq s} \in \mathcal{W}^s \bigr\}_{1 \le s \le t},
  \]
  forming the space
  \[
  \prod_{s=1}^{t} \prod_{\substack{\omega_{\leq s} \in \mathcal{W}^s}} \mathcal{Y}
  = \mathcal{Y}^{\sum_{s=1}^{t} |\mathcal{W}^s|},
  \]
  \item all potential covariates
  \[
  \{\mathbf{X}_1\} \,\cup\, \bigl\{\mathbf{X}_s(\omega_{<s}): \omega_{<s} \in \mathcal{W}^{s-1}\bigr\}_{2 \le s \le t},
  \]
  forming the space
  \[
  \mathcal{X} \times \prod_{s=2}^t \prod_{\substack{\omega_{<s} \in \mathcal{W}^{s-1}}} \mathcal{X}
  = \mathcal{X}^{1 + \sum_{s=2}^{t} |\mathcal{W}^{s-1}|}.
  \]
\end{itemize}

In full generality, the assignment mechanism at time \(t\) takes the form:
\[
p\bigl(W_t \mid \{Y_{\leq t}(\omega_{\leq t})\}_{\omega_{\leq t} \in \mathcal{W}^t},\, \{\mathbf{X}_{\leq t}(\omega_{<t})\}_{\omega_{<t} \in \mathcal{W}^{t-1}},\, W_{<t}\bigr),
\]
which is highly complex due to its dependence on all sequences of potential outcomes and covariates defined up to time \( t \). To simplify this assignment mechanism, we introduce a structural assumption similar to the concept of ignorability in static settings but adapted to longitudinal data. This is referred to as \emph{sequential ignorability} \citep{robins2009estimation}, which assumes that at any time in the study, treatment is conditionally randomized given the history of observed variables:
\begin{assumption}[Sequential Ignorability]
\label{assp:seq_ignorability}
Sequential ignorability holds when, at each time step \( t \), the treatment assignment is sequentially randomized given the observed history process up to time \( t \), formally:
\[
\bigl(
  \{Y_{\leq t}(\omega_{\leq t})\}_{\omega_{\leq t} \in \mathcal{W}^t},\,
  \{\mathbf{X}_{\leq t}(\omega_{< t})\}_{\omega_{< t} \in \mathcal{W}^{t-1}}
\bigr)
\perp\!\!\!\perp
W_t
\;\mid\;
\mathbf{H}_t.
\]
\end{assumption}
Next, we present the consistency assumption to link the observed outcomes and covariates to the potential ones. Specifically, the observed outcome at time \( t \), \( Y_t \), corresponds to the potential outcome \( Y_t(W_{\leq t}) \), and similarly for the covariates \( \mathbf{X}_t \). Formally:
\begin{assumption}[Consistency]
\label{assp:consistency_seq}
For every time step \( t \), and for any sequence of treatments \( \omega_{\leq t} \), the observed outcomes and covariates are equal to the potential outcomes and covariates under that treatment sequence, formally:
\[
W_{ \leq t} = \omega_{\leq t} \implies Y_{t} = Y_{t}(\omega_{\leq t}) \text{ and } \mathbf{X}_{t} = \mathbf{X}_{t}(\omega_{< t}).
\]
\end{assumption}
The consistency assumption \ref{assp:consistency_seq} states that one potential outcome is observed when a specific treatment is observed at any time step. This also implies that there is no interference \emph{across} units, meaning that the treatments other units receive do not affect the potential outcome of other units (Assumption \ref{assp:sutva}). However, it's important to note that without restrictive assumptions, we cannot assume that there is no interference \emph{within} the observations of \underline{the same individual}. This is why, in addition to the announced attributes $\mathbf{X}_{t}$ being potential confounders, the past treatment trajectory $W_{<t}$ also confounds both $Y_{t}$ and $W_{t}$. This assumption applies to all past information $\mathbf{H}_{t}$ up to the current time step $t$ and assumes it to be confounding $Y_{it}$ and $W_{it}$ (Figure \ref{fig:cg_detailed_3steps}).
\begin{figure}
\begin{center}
\includegraphics[scale=0.5]{figures/background/cg_detailed_3steps_NoU.pdf}
\caption{A causal graph is assumed to generate longitudinal data of 3-time steps ($T = 3$). Edges are colored (pink, blue, and red) whenever the causal relation may contribute to confounding treatment and response at any time step $t$.} 

\label{fig:cg_detailed_3steps}
\end{center}
\end{figure}
Now, armed with the sequential ignorability assumption and consistency, the assignment mechanism can be as
\[
p\!\left(W_t \mid
  \{Y_{\leq t}(\omega_{\leq t})\}_{\omega_{\leq t} \in \mathcal{W}^t},\;
  \{\mathbf{X}_{\leq t}(\omega_{< t})\}_{\omega_{< t} \in \mathcal{W}^{t-1}},\;
  W_{<t}
\right)
= p(W_t \mid Y_{< t}, \mathbf{X}_{\leq t}, W_{< t})
= p(W_t \mid \mathbf{H}_t).
\]

Similar to our discussion in the static setting (Section \ref{sect_background:po_framework_static_def}), the Assumption \ref{assp:seq_ignorability} guarantees that within a specific area of the space of \(\mathbf{H}_t\), the groups of individuals who were treated and those who were not can be fairly compared. This kind of "local" comparability is ensured by having both treated and untreated individuals present at each level of \( \mathbf{H}_t \): 
\begin{assumption}[Overlap/Positivity]
\label{assp:overlap_seq}
Given any time step \( t \), and for any possible historical context \( \mathbf{h}_t \), the probability of observing any of the two treatment regimes \( \omega_t \) is strictly positive:
\[
p(\mathbf{h}_t) \neq 0 \implies p(W_t = \omega_{t} \mid \mathbf{h}_t) > 0.
\]
\end{assumption}
\begin{warning}
The causal quantity of interest in the longitudinal setting depends on the scientific objective of the study. In this thesis, we take the viewpoint that the primary causal quantity of interest is the mean of the potential outcomes given the observed covariates (Equation \ref{eq:exp_pot_outc_classic}).
\end{warning}

\begin{definition}[Conditional Expected Potential Outcome]
\label{def:cond_expect_po}
The expected potential outcome at time \( t \), given the history of covariates \( \mathbf{X}_{\leq t} = \mathbf{x}_{\leq t} \) and responses \( Y_{<t} = y_{<t} \), is formalized as:
\begin{equation}
\label{eq:exp_pot_outc_classic}
m_{t}^{\omega_{\leq t}}(\mathbf{x}_{\leq t}, y_{<t}) := \mathbb{E}(Y_{t}(\omega_{\leq t}) \mid \mathbf{X}_{\leq t} = \mathbf{x}_{\leq t}, Y_{<t} = y_{<t}), \quad \omega_{\leq t} \in \mathcal{W}^t.
\end{equation}
\end{definition}

The conditional potential outcome allows us to evaluate the possible counterfactual trajectories of the responses given records for any given potential sequence of treatments. Furthermore, this causal quantity allows us to define another interesting causal quantity, the CATE in the time-varying setting.
\begin{definition}[Time-varying CATE]
\label{def:cate_time_varying}
Given two potential sequences of treatments \(\omega_{\leq t}\) and \(\omega'_{\leq t}\), the time-varying \gls{cate} is defined as
\[
\begin{aligned}
\tau_t(\mathbf{x}_{\leq t}, y_{<t}; \omega_{\leq t}, \omega'_{\leq t})
&\coloneqq \mathbb{E}\bigl[Y_t(\omega_{\leq t}) - Y_t(\omega'_{\leq t})
\,\big|\, \mathbf{X}_{\leq t} = \mathbf{x}_{\leq t},\, Y_{<t} = y_{<t}\bigr] \\[0.8ex]
&= m_t^{\omega_{\leq t}}(\mathbf{x}_{\leq t}, y_{<t})
- m_t^{\omega'_{\leq t}}(\mathbf{x}_{\leq t}, y_{<t}).
\end{aligned}
\]
\end{definition}
Based on this causal quantity, we can define the ATE for the longitudinal data up to time \( t \).
\begin{definition}[Time-varying ATE]
\label{def:ate_time_varying}
Given two potential sequences of treatments \( \omega_{\leq t} \) and \( \omega'_{\leq t} \), the time-varying \gls{ate} is defined as: 
\[
\tau_t(\omega_{\leq t}, \omega'_{\leq t}) \coloneqq \mathbb{E}_{\mathbf{X}_{\leq t}, Y_{<t}} \bigl[\tau_{t}(\mathbf{x}_{\leq t}, y_{<t}; \omega_{\leq t}, \omega'_{\leq t})\bigr]. 
\]
\end{definition}

\paragraph{Why do we focus on estimating conditional potential outcomes?} 
To estimate the CATE, it's necessary to calculate the difference in potential outcomes between a candidate treatment trajectory \( \omega_{\leq t} \) and a potential control trajectory \( \omega_{\leq t}^{(c)} \). However, the control sequence need not be identical for all units (e.g.\ \(\omega^{(c)}_{\le t} = (0,\dots,0)\)). Instead, it can be more informative to compare two counterfactual outcome trajectories corresponding to different treatment sequences \(\omega_{\le t}\) and \(\omega'_{\le t}\), as in the general definition of the time‐varying CATE. Therefore, we adopt an outcome-based approach, where the estimation of \gls{cate} (Definition \ref{def:cate_time_varying}) can be performed in a later stage, tailored to the specific needs of the application. This approach also applies to the time-varying ATE, which similarly relies on comparing two treatment sequences. This later stage of estimation underscores the versatility of our method in applying CATE/ATE:
\begin{itemize}
    \item Deciding which of the two potential treatments is favorable for a given individual by assessing \( \tau_{t}(\mathbf{x}_{\leq t}, y_{<t}; \omega_{\leq t}, \omega'{\leq t}) \).
    \item Deciding on a population level whether it is more favorable to switch treatment from \( \omega_{\leq t}^{\prime} \) to \( \omega_{\leq t} \), depending on \( \tau_t(\omega_{\leq t}, \omega'_{\leq t}) \).
\end{itemize}
\paragraph{Policy learning from counterfactuals}
Additionally, framing our general causal inference task this way allows us to leverage the estimated counterfactual responses to learn a policy—that is, choosing the best possible treatment strategy for a given individual without explicitly estimating \gls{cate} or ATE. For instance, in the case of a cancer dataset, where the response of interest is tumor volume, one could choose the treatment sequence (e.g., chemotherapy, radiotherapy) that minimizes tumor volume. Formally, we learn such a DTR/policy by solving an optimisation problem over a prespecified class $\Pi$ of admissible regimes \citep{murphy2003OptimTreatRegime,robins2004optimal}. For example, the \emph{history-specific} optimal policy is
\[
\pi_{\le t}^\star(\mathbf h_{t})
      \;\in\; \arg\min_{\pi_{\le t} \in \Pi}
      \mathbb E\!\bigl[Y_t(\pi_{\le t})
                       \mid\mathbf X_{\le t} = \mathbf x_{\le t},\; Y_{<t} = y_{<t} \bigr],
\]
which reduces to the pointwise minimization $\min_{\omega_{\le t}} m_t^{\omega_{\le t}}(\mathbf x_{\le t}, y_{<t})$ when $\Pi$ contains only fixed treatment sequences—that is, under the time-varying regime assumption (\ref{assp:time_varying_treat}). 
 
This approach demonstrates the flexibility and adaptability of our method to various research questions and practical applications, enhancing its potential impact and utility. 

The three causal quantities defined so far are identified given the formulated assumptions of sequential ignorability, consistency, and positivity, collectively referred to as the \emph{sequential ignorability assumptions}. We summarize the results in the following proposition.
\begin{proposition}[\citep{robins-time-varying-exposures, robins1999association}]
\label{prop_backround:identif_po_cate_time}
    Given the assumption of sequential ignorability, the conditional potential outcomes are identified as:
    \[
    m_{t}^{\omega_{\leq t}}(\mathbf{x}_{\leq t}, y_{<t}) = \mathbb{E}_{Y_{t} \mid \mathbf{H}_{t}}(Y_{t} \mid \mathbf{H}_{t}  = [\mathbf{x}_{\leq t},  y_{<t}, \omega_{< t}], W_{t} = \omega_{t}).
    \]
   As a result, the time-varying \gls{cate} is identified as
\[
\begin{aligned}
\tau_t(\mathbf{x}_{\leq t}, y_{<t}; \omega_{\leq t}, \omega'_{\leq t})
&= \mathbb{E}_{Y_t \mid \mathbf{H}_t}\bigl(Y_t \,\big|\, \mathbf{H}_t = [\mathbf{x}_{\leq t}, y_{<t}, \omega_{<t}],\, W_t = \omega_t\bigr) \\[0.8ex]
&\quad - \mathbb{E}_{Y_t \mid \mathbf{H}_t}\bigl(Y_t \,\big|\, \mathbf{H}_t = [\mathbf{x}_{\leq t}, y_{<t}, \omega'_{<t}],\, W_t = \omega'_t\bigr).
\end{aligned}
\]
    The time-varying \gls{ate} is identified as:

\begin{equation*}
\begin{split}
\tau_t(\omega_{\leq t}, \omega'_{\leq t}) 
&= \mathbb{E}_{(\mathbf{X}_{\leq t}, Y_{<t})} \left[ 
    \mathbb{E}_{Y_{t} \mid \mathbf{H}_{t}} \left(
        Y_t \,\middle|\, \mathbf{H}_t = [\mathbf{x}_{\leq t}, y_{<t}, \omega_{<t}],\, W_t = \omega_t
    \right)
\right] \\
&\quad - \mathbb{E}_{(\mathbf{X}_{\leq t}, Y_{<t})} \left[ 
    \mathbb{E}_{Y_{t} \mid \mathbf{H}_{t}} \left(
        Y_t \,\middle|\, \mathbf{H}_t = [\mathbf{x}_{\leq t}, y_{<t}, \omega'_{<t}],\, W_t = \omega'_t
    \right)
\right].
\end{split}
\end{equation*}
\end{proposition}

\subsection{Modeling Challenges}
\label{intro:model_challenges_time}
\paragraph{Causal feedback} 
For longitudinal data, feedback refers to the idea that previous treatments may impact an intermediate variable, which in turn affects future treatments. In the literature, these intermediate variables are typically confounders, leading to what is often called \emph{treatment-confounder feedback} \citep{robins1997causalNested, AssoCausaMSM1999, robins2000MSM}. However, in this thesis, we consider a more complex scenario where we also assume the existence of \emph{treatment-response feedback}. Both types of causal feedback are depicted in Figure \ref{fig:cg_detailed_3steps}. To understand the importance of causal feedback in longitudinal data, let's consider a simple model of the time-varying outcome \(Y_t\):
\begin{equation}
Y_t = \gamma Y_{t-1} + \beta W_t + \beta_1 W_{t-1} +  \mathbf{\alpha}^\top \mathbf{X}_t + \epsilon_t,
\end{equation}
where \( \epsilon_t \) is an error term independent of \( Y_{< t}, W_{\leq t},\mathbf{X}_{\leq t} \).
Assuming consistency, we can write the following model for the potential outcomes:
\begin{equation}
Y_t(\omega_{\leq t}) = \gamma Y_{t-1}(\omega_{< t}) + \beta \omega_t + \beta_1 \omega_{t-1} +  \mathbf{\alpha}^\top \mathbf{X}_t(\omega_{< t}) + \epsilon_t.
\end{equation}
Since we consider the history process \( \mathbf{H}_t \) to confound the treatment \( W_t \) and outcome \( Y_t \), we observe both \emph{treatment-confounder feedback} through the term $\mathbf{X}_t(\omega_{< t})$ and \emph{treatment-response feedback} through the term $Y_{t-1}(\omega_{< t})$. These two types of feedback occur because we are considering the \emph{carryover effect}:

\begin{definition}[Carryover Effect]
 \label{def:carryover_effect}
A \emph{carryover effect} (or \emph{lagged effect}) refers to any additional influence that treatments administered at one or more previous time points (\(W_{t-1}, W_{t-2}, \dots\)) exert on the outcome \(Y_t\) \emph{beyond} the direct, immediate effect of \(W_t\).
\end{definition}

Here, the carryover effect manifests because the past treatment \(W_{t-1}\) affects \(Y_t\) directly and also \underline{indirectly} through the feedback paths
\[
W_{t-1} \to Y_{t-1} \to Y_t
\quad \text{and} \quad
W_{t-1} \to \mathbf{X}_t \to Y_t.
\]
When conditioning on \(Y_{t-1}\) and \(\mathbf{X}_t\), we introduce \emph{post-treatment bias} \citep{rosenbaum1984PostTreatBias, robins1997causalNested, robins1999MSMBinaryOutc} because they are both affected by \(W_{t-1}\). Consequently, we cannot consistently estimate the parameter \(\beta_1\).
 
One might argue that removing conditioning on \( Y_{t-1} \) and \( \mathbf{X}_t \) could allow for consistent estimation of \( \beta_1 \). However, doing so would violate sequential ignorability (\ref{assp:seq_ignorability}), and therefore the treatment effect \( \beta \), associated with \( W_t \), cannot be consistently estimated due to missing confounders—resulting in \emph{omitted variable bias} \citep{EmpiricistCompanion, cinelli2020making} in the case of our linear regression model.

The simple model we presented is commonly called a \emph{fixed effect model} \citep{blackwell2018make, imbens2024causal}, and it cannot handle causal feedback. However, if one is only interested in \gls{cte}, that is we assume : 
\begin{assumption}[Contemporaneous Treatment Effect (CTE)]
\label{assp:contemporaneous_effect}
We restrict ourselves to measuring only the CTE, i.e., the effect related to the current treatment variable \( W_t \). The potential trajectory of treatments up to \( t-1 \), \( \omega_{< t} \), is assumed to be consistent with the \textbf{observed} history of treatments, i.e., \(  W_{< t} = \omega_{< t} \). Therefore, the potential outcomes of interest at each time step \( t \) are \( \{Y_t(W_{< t}, \omega)\}_{\omega \in \mathcal{W}} \).
\end{assumption}
The potential outcomes can then be written as 
\begin{equation}
Y_t(W_{< t}, \omega_{t}) = \gamma Y_{t-1}(W_{< t}) + \beta \omega_t + \beta_1 W_{<t-1} +  \mathbf{\alpha}^\top \mathbf{X}_t(W_{< t}) + \epsilon_t.
\end{equation}
which, by consistency assumption, is reduced to 
\begin{equation}
Y_t(W_{< t}, \omega_{t}) = \gamma Y_{t-1}+ \beta \omega_t + \beta_1 W_{<t-1} +  \mathbf{\alpha}^\top \mathbf{X}_t + \epsilon_t,
\end{equation}
and the causal parameter $\beta$ can be estimated consistently. It is therefore common and convenient in the case of Assumption \ref{assp:contemporaneous_effect} to denote the potential outcome \(Y_t( \omega_{t})\) as it would be the case in Chapter \ref{chapter:cdvae}. 

\paragraph{Controlling for Confounding Bias} 
Since conditioning for confounding variables in outcome models cannot fully address the estimation of causal effects in a sequence of variables, even standard methods discussed in static settings, such as matching \cite{Abadie2004ImplementingME,Austin2011AnIT}, stratification \citep{Frangakis2002PrincipalSI,Imbens2015CausalIF}, or classical weighting methods \citep{Rosenbaum1983TheCR,DAgostino1998PropensitySM}, may fall short. To this end, \emph{\gls{msm}} (cf. Section \ref{sect_background:po_framework_longit_overview}) were introduced to estimate time-dependent causal effects in the presence of time-dependent confounders \citep{robins-time-varying-exposures,robins1999MSMBinaryOutc,robins2000MSM}. \gls{msm} provides consistent estimates of causal effects for time-varying treatments through IPTW. This method accounts for time-dependent confounding by assigning each subject a weight based on the inverse probability of receiving the treatment, given their covariates. Intuitively, this creates a pseudo-population where each individual is duplicated as many times as the inverse of their weight. In this pseudo-population, weighted time-dependent confounders are balanced over time.

\subsection{Literature Overview: The Challenge of Missing Confounders}
\label{sect_intro:review_miss_conf}
\paragraph{Unit Fixed Effects Regression Models}
Unit fixed effects models are a widely used approach for addressing \emph{time-invariant unobserved confounders} in longitudinal data, particularly in econometrics, political science, and social sciences \citep{beck2001time, wilson2007lot, hsiao2007panel, wooldridge2010econometric, bell2015explaining, clark2015should}. These models adjust for individual-specific characteristics that do not change over time by including unit-specific intercepts, capturing the unobserved characteristics of each individual. This allows researchers to control for factors that affect the outcome but are not directly observed or measured. The general form of the \gls{po} model can be, for example, written as:
\[
Y_t(W_{< t}, \omega_{t}) = \alpha_0 + \gamma Y_{t-1} + \beta \omega_t + \beta_1 W_{<t-1} +  \mathbf{\alpha}^\top \mathbf{X}_t + \epsilon_t,
\]
where $\alpha_0$ represents the \emph{unit-specific effect} and is typically viewed as a function $h$ of unobserved confounders, $\mathbf{U}$, that does not change over time, $\alpha_0 = h(\mathbf{U})$. This approach allows for the implicit control of these confounders through the unit-specific intercepts. However, as noted before, this method can introduce post-treatment bias when dynamic causal feedback paths are present, making it less suitable for models where past outcomes or covariates affect current treatments \citep{imai2019should}.

A natural extension of this model is the \emph{two-way fixed effects model} \citep{de2020two-wayFixEffects, callaway2021DiDTimePeriods, sant2020doubly, goodman2021difference, arkhangelsky2021double, athey2017state}, which incorporates a time-specific effect, $\lambda_t$, to account for unobserved heterogeneity that varies across time but is constant across individuals:
\[
Y_t(W_{< t}, \omega_{t}) = \alpha_0 + \lambda_t + \gamma Y_{t-1} + \beta \omega_t + \beta_1 W_{<t-1} +  \mathbf{\alpha}^\top \mathbf{X}_t + \epsilon_t.
\]
Traditional two-way fixed effects models operate under the assumption of homogeneous treatment effects across individuals, which limits their applicability in scenarios where treatment effects may vary. To address this limitation,\citet{callaway2021DiDTimePeriods} developed methodologies for estimating group-specific treatment effects, allowing for heterogeneity in treatment effects across different subpopulations. Building on this work, \citet{arkhangelsky2021double} proposed a doubly-robust linear estimator which maintains unbiasedness under two conditions: either when the two-way linear model holds in the presence of observed covariates, or when a set of assumption on treatment assignment are satisfied. 

\subparagraph{Modeling Group-Based Unobserved Heterogeneity}
As per unobserved heterogeneity that varies across groups, \emph{group-based approaches} have been developed which cluster units into groups with shared characteristics, allowing researchers to control for unobserved heterogeneity across groups rather than individuals. \citet{bonhomme2015grouped} pioneered this method with their \emph{grouped heterogeneity models}, which cluster units into latent groups based on both observed and unobserved characteristics. These models have been successfully applied in policy evaluation, where grouping units based on unobserved characteristics, such as economic conditions or regional factors, helps isolate the effects of an intervention \citep{bonhomme2015grouped}. \citet{su2016IdentifLatentStructPanel} extended this approach by developing methods to handle \emph{latent group structures} in large datasets, making it possible to identify unobserved heterogeneity in panel data with high-dimensional covariates. 

\paragraph{Interactive Panel Models}
Interactive fixed effects models extend two-way fixed effects models by allowing for interactions between units and time periods through latent factors. These models, introduced by \citep{bai2009panel}, are particularly useful in addressing \emph{time-varying unobserved confounders}, which are prevalent in longitudinal data settings such as macroeconomic studies or public health interventions. Interactive fixed effects models enhance the ability to capture more complex patterns in the data by incorporating unobserved factors that vary across units and over time \citep{bai2009panel}. Interactive panel data is part of a broader class of general factor models for which synthetic control has been extensively studied \citep{abadie2010synthetic, arkhangelsky2019synthetic, chernozhukov2019inference, ben2021augmented}.

\paragraph{Instrumental variables for panel data}
Despite the extensive focus on instrumental variables (IVs) for addressing unmeasured confounding in static settings \citep{hernan2006instruments, imbens2014instrumental, Imbens2015CausalIF, hartford2017deepIV, Athey2019GeneralizedRF, syrgkanis2019HTEInstru, wang2022ConfoundedInstru, cheng2023causalCondInstru}, their application in the context of time-varying data with missing confounders has been relatively underexplored in the literature. Early contributions by \citet{angrist1996identification} introduced the potential outcomes framework in IV settings, demonstrating how IV estimands could be interpreted as local average treatment effects (LATE) for specific subpopulations. Building on this, \citet{michael2024instrumental} proposed a weighted IV estimator for \gls{msm}, incorporating time-varying IVs to adjust for unobserved confounders dynamically. This estimator is particularly useful for complex longitudinal data as it generates stabilized weights that simultaneously account for treatment and confounders over time. \citet{sun2018semiparametric} tackled data missing not at random (MNAR) using IVs, providing a semiparametric framework capable of robust estimation, even when the missing data mechanism is non-ignorable. 

\paragraph{Proximal Causal Learning (PCI)}
The PCI leverages proxy variables—measured covariates that serve as imperfect surrogates for unmeasured confounders, which allows for the identification of causal effects even when the standard \emph{no unmeasured confounding} assumption fails \citep{MiaoProxyUnmeasuredConf2016,tchetgen2020introduction}. These proxies facilitate the recovery of causal effects by solving inverse problems via bridge functions and the g-formula \citep{MiaoProxyUnmeasuredConf2016}. Initially developed for point exposures, PCI has been extended to dynamic treatment regimes and time-varying treatments \citep{tchetgen2020introduction,zhang2024IdentifDTRProxies}. 

\subparagraph{Proximal Causal Inference in Dynamic Treatment Settings}
In dynamic treatment settings, PCI employs time-varying proxies to overcome hidden confounders across multiple time points. For example, \citet{zhang2024IdentifDTRProxies} have shown that utilizing two independent proxy variables at each time point can identify the joint distribution of counterfactual outcomes. This approach aids in estimating optimal dynamic treatment regimes even with unmeasured confounding, extending the utility of the proximal g-formula. This formula generalizes Robins' g-formula for time-varying treatments, as discussed in \citep{tchetgen2020introduction}. Moreover, the proximal inverse probability-weighted (PIPW) estimator, described in \citet{ying2022proximalSurvCurv}, improves standard IPW methods by including proxy variables to adjust for hidden confounders. This allows for estimating survival curves and other longitudinal outcomes without assuming ignorability. Proximal doubly robust (PDR) estimators, which maintain consistency even when models for either confounders or outcomes are incorrectly specified, have also been proposed \citep{ying2023PCILongitStudy}. Despite its advantages, PCI faces practical challenges in identifying suitable proxies that satisfy relevance and completeness conditions \citep{tchetgen2020introduction, zhang2024IdentifDTRProxies}. Estimating bridge functions and solving nested inverse problems can also be computationally intensive. 


\paragraph{The Deconfounding Approach}
In genetic studies, latent, unobserved confounding factors; like population structure, complicate causal inference by inducing spurious associations between genotypes and phenotypes. To address this challenge, \cite{tran2018implicit} propose a method based on \emph{implicit causal models} which incorporate implicit density functions, implemented via neural networks, allowing them to capture nonlinear relationships and gene-population interactions. \citet{ranganath2018multiple} formalize a general framework for causal inference in the presence of unmeasured confounding. They introduce two key assumptions
\begin{inparaenum}[(i)]
    \item \emph{shared confounding}: all treatments are influenced by a common set of latent variables. 
    \item \emph{independence given shared confounders}: conditioning on these latent variables renders the treatments conditionally independent.
\end{inparaenum}
To estimate the unobserved confounders, they construct an \emph{information-regularized estimator}, which balances two competing goals: preserving the shared confounding structure while ensuring that the independence condition is not violated. Expanding on this line of thought, \cite{wang2019blessings} articulate the \emph{theory of the deconfounder}. Their central insight is that when many causes are observed jointly, the combined pattern of their assignments contains information about the latent confounders. They showed that it is possible to construct a latent variable, via a probabilistic factor model, that captures the influence of unobserved confounders. Conditioning on this variable permits unbiased estimation of treatment effects. The deconfounder framework has found practical applications beyond genetics. In recommendation systems, it enables more accurate predictions by adjusting for hidden user traits that simultaneously influence item exposure and preferences \citep{DeconfoundedRecommender2018}. In healthcare, \citet{zhang2019medicalDeconf} applied the deconfounder to observational studies using electronic health records to correct for unmeasured confounding in treatment effect estimation.

\subparagraph{Deconfounding in Temporal Settings}
Researchers have extended the deconfounder approach to dynamic and time-series contexts, where treatments and confounders evolve over time. \cite{Bica2020TimeSDecounf} introduce the \emph{Time Series Deconfounder}, which uses a \gls{rnn} with multitask outputs to build a temporal factor model. At each time step, the model infers latent variables that account for hidden confounders and ensures that assigned treatments are conditionally independent given these variables. This framework enables estimating treatment effects even in the presence of multiple time-varying confounders. Building on this idea, \cite{kuzmanovic2021deconfounding} propose the \emph{Deconfounding Temporal Autoencoder} (DTA), designed for longitudinal data with noisy proxies of hidden variables. The DTA architecture combines a \gls{lstm} autoencoder with a causal regularization penalty, learning a latent representation that substitutes for unmeasured confounders. Once this embedding is learned, an outcome model is conditioned on it to estimate \gls{cate}.

\subparagraph{Deconfounding Continuous-Time Settings}
In settings with continuous treatments and irregularly sampled data, \cite{cao2023estimating} adapt the deconfounding framework using neural differential equations. Their model constructs a latent factor process via a stochastic controlled differential equation, augmented by a Lipschitz-constrained convolutional operator. \cite{hatt2024sequential} focus on sequential treatment settings where a single intervention is administered at each time step, and unobserved confounders remain stable. They model treatment assignment as a first-order Markov process, conditioned on observed covariates and latent variables. By inferring these latent variables, modeled via a Gaussian process, they restore conditional independence and enable \gls{cate} estimation.

\subparagraph{Substitute Adjustment and the Limits of Deconfounding}
Recently, \citet{adams2024substitute} distinguished their work from the original deconfounder theory, particularly regarding causal interpretations and the methodology used for adjustments. While the deconfounder, as introduced by \citet{wang2019blessings}, emphasizes adjusting for latent variables to estimate causal parameters under the assumption of unobserved confounding, \citet{adams2024substitute} argued for a broader approach termed "\emph{Substitute Adjustment}." This method does not rely on strict causal assumptions but estimates adjusted regression parameters using inferred latent variables. This approach abstracts from causal interpretations, making the method applicable in a broader context where causal claims may not be strictly held.

As a summary, Table~\ref{tab:missing_confounders_comprehensive} presents a comparative overview of the main models discussed, grouped by category, main characteristics, and references.
\begin{table}[h!]
\centering
\caption{Comprehensive Overview of Methods Addressing Missing Confounders in Longitudinal Data}
\label{tab:missing_confounders_comprehensive}
\resizebox{0.9\textwidth}{!}{
\begin{tabular}{|p{2.8cm}|p{3.5cm}|p{6.2cm}|p{2.3cm}|}
\hline
\textbf{Category} & \textbf{Method / Model} & \textbf{Key Features} & \textbf{References} \\
\hline

\multirow{3}{=}{\textbf{Fixed Effects Models}} 
& Unit Fixed Effects & Controls time-invariant unobserved confounders using unit intercepts. Prone to post-treatment bias. & \citep{hsiao2007panel, wooldridge2010econometric} \\
& Two-Way Fixed Effects& Time fixed effects; Treatment effects are homogeneous.& \citep{callaway2021DiDTimePeriods, arkhangelsky2021double} \\
& Grouped Heterogeneity Models & Units clustered into latent groups; shared unobserved factors across groups.& \citep{bonhomme2015grouped, su2016IdentifLatentStructPanel} \\
\hline

\multirow{2}{=}{\textbf{Interactive Panel Models}} 
& Interactive Fixed Effects & Latent factors vary over units and time; captures time-varying confounding. & \citep{bai2009panel} \\
& Generalized Synthetic Control & Combines factor models and synthetic control; robust for high-dimensional confounding. & \citep{xu2017generalized} \\
\hline

\multirow{4}{=}{\textbf{Instrumental Variable Methods}} 
& IV for \gls{msm} & Weighted IV estimator for marginal structural models with time-varying IVs. & \citep{michael2024instrumental} \\
& IVs for MNAR Data & Semi-parametric IV estimator. & \citep{sun2018semiparametric} \\
\hline

\multirow{4}{=}{\textbf{Proximal Causal Inference (PCI)}} 
& Proximal G-Formula & Uses proxies and bridge functions to recover causal effects without ignorability. & \citep{tchetgen2020introduction, MiaoProxyUnmeasuredConf2016} \\
& PIPW Estimator & Proxy-based inverse probability weighting for survival analysis. & \citep{ying2022proximalSurvCurv} \\
& Proximal DR Estimator & Doubly robust estimator under proxy-based confounding. & \citep{ying2023PCILongitStudy} \\
\hline

\multirow{6}{=}{\textbf{Latent Variable / Deconfounder Models}} 
& Implicit Causal Models & Neural density estimators for unobserved confounding in genetics. & \citep{tran2018implicit} \\
& Shared Confounding Estimator & Assumes common latent confounders across multiple treatments. & \citep{ranganath2018multiple} \\
& The Deconfounder & Factor model for multiple causes; estimates substitute confounders. & \citep{wang2019blessings} \\
& Medical Deconfounder & EHR-based treatment effect estimation with latent confounder modeling. & \citep{zhang2019medicalDeconf} \\
& Time Series Deconfounder & RNN-based factor model for time-varying unobserved confounders. & \citep{Bica2020TimeSDecounf} \\
& DTA  & Proxy-driven autoencoder for \gls{cate} in time-series settings. & \citep{kuzmanovic2021deconfounding} \\
& Gaussian Process Factor Model & Uses GP over time to infer latent confounders in sequential treatments. & \citep{hatt2024sequential} \\
& Neural Diff. Equation Model & Latent confounders in continuous-time data via stochastic diff. eqs. & \citep{cao2023estimating} \\
\hline

\textbf{Alternative Adjustment} 
& Substitute Adjustment & Does not assume causal structure; recovers latent variables to adjust regression. & \citep{adams2024substitute} \\
\hline

\end{tabular}
}
\end{table}




\subsection{Literature Overview: Methods verifying our Causal assumptions}
\label{sect_background:po_framework_longit_overview}
In this section, we review the models that follow the same assumptions as our work in Chapters \ref{chapter:cdvae} and \ref{chapter:ccpc}, that is, they assume sequential ignorability (\ref{assp:seq_ignorability}), work under binary or discrete treatments (Remark \ref{remark:discrete_treat}), and perform counterfactual regression, i.e, estimate the conditional counterfactual response (Definition \ref{def:cond_expect_po} and Proposition \ref{prop_backround:identif_po_cate_time}). 

These models aim to estimate the effects of a given treatment sequence on the outcome over a prediction horizon \( \rho \), given the patient's treatment history and covariates at time \( t \). Formally, we model:
\[
\mathbb{E}\left[Y_{t+\rho} \mid W_{t, t+\rho-1}, \mathbf{H}_t\right] = g\left(\rho, W_{t: t+\rho-1}, \mathbf{H}_t\right)
\]
where \( g \) is a non-linear function. The goal is to predict the future outcome \( Y_{t+\rho} \) based on the patient's treatment sequence \(W_{t: t+\rho-1}\) and covariate history \( \mathbf{H}_t \).

\paragraph{\gls{msm}}  To control for time-dependent confounding, \gls{msm} adjusts for the bias introduced by time-varying covariates through the use of \emph{stabilized weights} \citep{robins2000MSM}:
\begin{equation}
    \label{eq:SW_orig}
    \mathrm{SW}(t, \rho)  = \prod_{s=t}^{t+\rho-1} \frac{\prod_{k=0}^{K-1} p\left(W_s=k \mid W_{ <s} \right)}{\prod_{k=0}^{K-1} p\left(W_s=k \mid W_{ <s}, \mathbf{X}_{\leq s}\right)}
\end{equation}
where \( p(\cdot) \) is the conditional probability mass function for discrete treatments, or the density function for continuous treatments, and \( K \) represents the number of treatment variables (e.g., chemotherapy, radiotherapy). The stabilized weights are computed by comparing the treatment probability given the patient's history \( \mathbf{H}_t \) with the treatment probability given only on past treatments \( W_{<t} \) (Numerator of Equation \ref{eq:SW_orig}).
We estimate the propensity weights using logistic regression:
\begin{align*}
p\bigl(W_t = k \mid W_{<t}\bigr)
&= \sigma\!\left(
      \sum_{j=0}^{K-1} \alpha_{j,k}
      \left(\sum_{s=1}^{t-1}\mathds{1}_{\{W_s = j\}}\right)
    \right),\\
p\bigl(W_t = k \mid \mathbf{H}_t\bigr)
&= \sigma\!\left(
      \sum_{j=0}^{K-1}\phi_{j,k}
      \left(\sum_{s=1}^{t-1}\mathds{1}_{\{W_s = j\}}\right)
      + \beta_1 \mathbf{X}_t + \beta_2 \mathbf{X}_{t-1}
    \right),
\end{align*}
where \( (\alpha_{j,k})_{0 \leq j,k \leq K-1}, (\phi_{\star})_{0 \leq j,k \leq K-1}, (\beta_1,\beta_2 ) \) are regression coefficients and \( \sigma(\cdot) \) is the Sigmoid function. The model then uses the weighted regression to estimate the outcome at time \( t + \rho \):
\begin{equation*}
g\bigl(\rho,\,W_{t:t+\rho-1},\,\mathbf{H}_t\bigr)
= \sum_{k=0}^{K-1}\delta_k
  \left(\sum_{s=t}^{t+\rho-1}\mathds{1}_{\{W_s = k\}}\right)
  + \boldsymbol{\eta}_1^\top\mathbf{X}_t
  + \boldsymbol{\eta}_2^\top\mathbf{X}_{t-1},
\end{equation*}

where \( (\delta_{k})_{0 \leq k \leq K-1} \) and \( \boldsymbol{\eta}_{1}, \boldsymbol{\eta}_{2} \) are regression coefficients, representing the effects of the treatments and covariates, respectively.

\paragraph{\gls{rmsm}}
The RMSM \citep{lim2018RMSN} generalizes the standard \gls{msm} by enabling highly non-linear modeling of the dynamics between covariates and treatments using a \gls{rnn} architecture. The model uses stabilized weights for the regression loss based on the \gls{iptw}, which is generalized to handle multiple treatment assignments, censored data, and continuous dosages. \citet{lim2018RMSN} suggested adding a second weighting term to the stabilized weight of  \gls{msm} in Equation\ref{eq:SW_orig} to account for censoring:
\[
SW^*(t, \rho) = \prod_{s=t}^{t+\rho} \frac{f\left(C_s = 0 \mid \mathcal{T} > s, W_{<s}\right)}{f\left(C_s = 0 \mid \mathcal{T} > s, \mathbf{X}_{<s}, W_{< s}\right)},
\]
where \( C_n = 1 \) represents censoring of the trajectory, and \( \mathcal{T} \) is the time of its occurrence. The stabilized weights are truncated at their 1st and 99th percentile values and normalized by their mean for each individual \(i\):
\[
\tilde{\mathrm{SW}}_i^*  = \frac{\mathrm{SW}_i^*(t, \rho)}{\frac{1}{T_i} \sum_{t=1}^{T_i} \mathbb{E}( \mathrm{SW}^*(t, \rho))},
\]
where \( T_i \) is the number of observations per patient. These two stabilized weights are used to balance the individual regression loss over a time horizon \(\rho\) as follows:
\[
\mathcal{L}_{Y}= \mathrm{SW}_i(t, \rho) \times\tilde{SW}_i^*(t, \rho) \times  \left\|Y_{t+\rho-1} - g\left(\rho, \omega_{t: \rho-1}, \mathbf{H}_t\right)\right\|^2. 
\]

\subparagraph{Model Architecture}
The \gls{rmsm} framework defines six neural networks:
\begin{itemize}
    \item \textbf{Four propensity networks}: These RNN-based models compute the numerators and denominators of the two stabilized weights. Each network uses a Sigmoid output with binary cross-entropy loss for binary treatments, Softmax for categorical treatments, and a Variational \gls{rnn} for continuous dosages.

    \item \textbf{Two prediction networks}:
    \begin{inparaenum}[(1)]
        \item \textbf{Encoder}: A \gls{lstm} processes the individual's covariate and treatment history, learning a hidden representation at each time step. 
        \item \textbf{Decoder}: Given an intended treatment plan and hidden representation, the decoder predicts outcomes across future time steps. 
    \end{inparaenum}
\end{itemize}

\paragraph{\gls{crn}}
In \cite{bica2020estimatingCRN}, the authors proposed \gls{crn}, a model that employs \emph{domain adversarial training} \citep{li2018deepdomain, schoenauer2019multidomain,ganin2016domain} to mitigate bias instead of weighting.  Let \( q_{\theta_W}(\cdot \mid  \Phi\left(\mathbf{H}_t\right) ) \) be the treatment classifier and \( G_Y\left(\Phi\left(\mathbf{H}_t; \theta_R\right); \theta_Y\right) \) be the outcome prediction network where \( \Phi(\cdot) \) is the representation function parameterized by \( \theta_R \). The treatment loss \( \mathcal{L}_{W}\left(\theta_R, \theta_{W}\right) \) and outcome loss \( \mathcal{L}_{Y}\left(\theta_R, \theta_Y\right) \) are defined as:
\[
\mathcal{L}_{W}\left(\theta_R, \theta_{W}\right) = -
 \log q_{\theta_W}(W_{t+1} \mid \Phi\left(\mathbf{H}_t ; \theta_R\right)), 
\]
\[
\mathcal{L}_{Y}\left(\theta_R, \theta_Y\right) = \left\|Y_{t+1} - G_Y\left(\Phi\left(\mathbf{H}_t ; \theta_R\right), \theta_Y\right)\right\|^2.
\]
The model aims to maximize the treatment loss and minimize the outcome regression loss to achieve a balanced representation, adversarially. The overall training loss is
\[
\mathcal{L}\left(\theta_R, \theta_Y, \theta_{W}\right) = \mathcal{L}_{Y}\left(\theta_R, \theta_Y\right) - \lambda \mathcal{L}_{W}\left(\theta_R, \theta_{W}\right),
\]
where \( \lambda \) is a hyperparameter that balances the contributions of the two loss functions. The adversarial training follows the approach of \cite{ganin2016domain}, using a gradient reversal layer on the discriminator network, allowing the model to minimize the overall loss using backpropagation while maintaining treatment invariance.

\paragraph{Causal Transformer}  
\citet{Melnychuk2022CausalTF} proposed a transformer-based architecture, the Causal Transformer, for estimating counterfactual outcomes over time. The model processes sequential data using three specialized transformer subnetworks that separately encode time-varying covariates \( \mathbf{X}_{\leq t} \), past treatments \( W_{<t} \), and past outcomes \( Y_{< t} \). The model computes a representation \(\Phi_t = \Phi\left(\mathbf{H}_t; \theta_R\right)\) via an architecture that comprises the following three subnetworks:
\begin{inparaenum}[(1)]
    \item \textbf{Covariate Network}: Encodes the sequence of observed covariates \( \mathbf{X}_{\leq t} \).
    \item \textbf{Treatment Network}: Encodes the sequence of prior treatments \( W_{<t} \).
    \item \textbf{Outcome Network}: Encodes the sequence of prior outcomes \( Y_{< t} \).
\end{inparaenum}

Each of these networks uses:
\begin{inparaenum}[(1)]
    \item \textbf{Masked Multi-head Self-Attention}: To ensure that no future information is seen during the encoding of past data.
    \item \textbf{Shared Trainable Positional Encoding}: To retain temporal relationships.
\end{inparaenum}

\subparagraph{Training} The CT employs a custom end-to-end training procedure based on the \gls{cdc} loss, designed to reduce confounding bias:
The loss consists of two components:
\begin{itemize}
\item Factual Outcome Loss:
\[
\mathcal{L}_{Y}(\theta_Y, \theta_R) = \left\| Y_{t+1} - G_Y(\mathbf{\Phi}_t, W_t; \theta_Y) \right\|^2.
\]
\item \gls{cdc} Loss:
\[
\mathcal{L}_{conf}(\theta_W, \theta_R) = -\sum_{j=1}^{K} 1[W_t = j] \log G_W(\mathbf{\Phi}_t; \theta_W).
\]
Here, \( G_W \) predicts treatment assignments, and the \gls{cdc} loss encourages \( \mathbf{\Phi}_t \) to remain non-predictive of the treatment \( W_t \).
\end{itemize}
The overall objective function is:
\[
\hat{\theta}_Y, \hat{\theta}_R
= \arg \min_{\theta_Y,\, \theta_R}
\bigl\{
  \mathcal{L}_Y(\theta_Y, \theta_R)
  + \alpha\,\mathcal{L}_{\mathrm{conf}}(\theta_W, \theta_R)
\bigr\},
\]
\[
\hat{\theta}_W
= \arg \min_{\theta_W}
\mathcal{L}_W(\theta_R, \theta_W).
\]
The CT is trained with an end-to-end learning approach, implementing techniques such as masked cross- and self-attention to ensure that the model learns from historical data while preventing look-ahead bias.

\paragraph{G-Net} 
Unlike previous discussed models, which are designed for \underline{time-varying treatment regimes}, G-Net \citep{Li2021GNetAR} is primarily designed for counterfactual prediction in \underline{dynamic treatment regimes} (c.f. Definition \ref{def:DTR}). It is a sequential, \gls{rnn}-based model, which is built on the g-calculus, also called g-computation or g-formula \citep{ROBINS1986-G-formula, robins1997causalNested, vansteelandt2014structural}. 

G-calculus is a general identification result introduced by \citet{ROBINS1986-G-formula} that expresses any conditional counterfactual responses (or full distribution) under dynamic treatment rules entirely in terms of observable conditional densities. In its general form, g-calculus can be presented as in the following proposition:
\begin{proposition}[G-calculus  \citep{ROBINS1986-G-formula}]
\label{prop:g_calculus_dtr}
Assume the standard assumptions of consistency, positivity, and sequential ignorability (Assumptions \ref{assp:consistency_seq}, \ref{assp:overlap_seq}, \ref{assp:seq_ignorability}). Fix a counterfactual forecasting horizon $\rho\!>\!0$ and let $\pi_{t:t+\rho-1}
      :=\bigl(
           \pi_t,\dots,\pi_{t+\rho-1}
         \bigr)$ be the collection of decision rules that operate between time~$t$ and $t+\rho-1$ as in Definition \ref{def:DTR}.  The conditional counterfactual response at the horizon $\rho$ can be expressed as
\begin{equation}
\label{eq:g_calculus_dtr}
\begin{split}
&\mathbb{E}\bigl[Y_{t+\rho}\bigl(\pi_{t:t+\rho-1}\bigr)
  \;\bigm|\;\mathbf{H}_t=\mathbf{h}_t\bigr]\\
&=
\int_{\mathcal X^{\rho-1}}\!\!
\int_{\mathcal Y^{\rho-1}}
\mathbb{E}\Bigl[
  Y_{t+\rho}
  \;\bigm|\;
  \mathbf{H}_t=\mathbf{h}_t,\, 
  \mathbf{X}_{t+1:t+\rho-1}=\mathbf{x},\, 
  Y_{t+1:t+\rho-1}=y,\\
&\qquad
  W_{t:t+\rho-1}
    =\pi_{t:t+\rho-1}(\mathbf{h}_t,\mathbf{x},y)
\Bigr]\\
&\quad\times
\prod_{j=t+1}^{t+\rho-1}
  p\Bigl(
    \mathbf{x}_j,\,y_j
    \;\bigm|\;
    \mathbf{H}_t=\mathbf{h}_t,\, 
    \mathbf{X}_{t+1:j-1}=\mathbf{x}_{t+1:j-1},\, 
    Y_{t+1:j-1}=y_{t+1:j-1},\\
&\qquad
    W_{t:j-1}
      =\pi_{t:j-1}(\mathbf{h}_t,\mathbf{x}_{t+1:j-1},y_{t+1:j-1})
  \Bigr)
\,d\mathbf{y}\,d\mathbf{x}\,.
\end{split}
\end{equation}

\end{proposition}

The utility of Proposition \ref{prop:g_calculus_dtr} is that it allows the conditional counterfactual response to be rewritten as a forward simulation that iteratively plugs in the conditional distributions of future covariates and outcomes $\{\mathbf{X}_{t+j}, Y_{t+j} \}_{1 \le j \le \rho-1}$ given the entire past $\mathbf{H}_{t}$.  After fitting the conditional distributions \( p_{\theta_{W}}(W_t\mid\mathbf{H}_t),\;
    p_{\theta_{X}}(\mathbf{X}_{t+1}\mid\mathbf{H}_t),\;
    p_{\theta_Y}(Y_{t+1}\mid\mathbf{H}_t, W_t)\) on the observed data, one can: first overwrite future treatments with a policy \(\pi\), and second, roll the simulation forward to obtain Monte-Carlo draws of the conditional counterfactual response. An estimation  with g-calculus  \(\mathbb{E}\bigl[Y_{t+\rho}\bigl(\pi_{t:t+\rho-1}\bigr)
  \;\bigm|\;\mathbf{H}_t=\mathbf{h}_t\bigr]\) can therefore be described by the Algorithm \ref{alg:gcomp}.

\begin{algorithm}
\caption{Monte Carlo g-computation}
\label{alg:gcomp}
\begin{algorithmic}[1]
  \REQUIRE Longitudinal data $\{\{\mathbf{H}_t^{(i)}, W_t^{(i)}, Y_t^{(i)}\}_{t=1}^{T}, i=1,\dots,n\}$
  \REQUIRE Horizon $\rho$
  \REQUIRE Dynamic policy $\pi = \{\pi_s\}_{s=t}^{t+\rho-1}$
  \REQUIRE Number of (Monte-Carlo) simulation paths $N_{MC}$
  \ENSURE Estimate $\hat\mu_{t,\rho}^{\pi}(\mathbf{h}_t)
        = \mathbb{E}[Y_{t+\rho}(\pi)\mid\mathbf{H}_t=\mathbf{h}_t]$
  
  \STATE \textbf{Stage 1: Model fitting}
  \STATE Estimate conditional laws:
  \begin{align*}
    p_{\theta_{W}}(W_t\mid\mathbf{H}_t),\;
    p_{\theta_{X}}(\mathbf{X}_{t+1}\mid\mathbf{H}_t),\;
    p_{\theta_Y}(Y_{t+1}\mid\mathbf{H}_t, W_t)
  \end{align*}
  by maximizing the joint log-likelihood on observed data.
  
  \STATE \textbf{Stage 2: Forward simulation (g-calculate)}
  \FOR{$n \in \{1, \dots, N_{MC}\}$}
    \STATE Initialize history: $\mathbf{H}_t^{(n)} \gets \mathbf{h}_t$
    \FOR{$s \in \{t, \dots, t+\rho-1\}$}
      \STATE Set treatment by policy: $W_s^{(n)} \gets \pi_s(\mathbf{H}_s^{(n)})$
      \STATE Sample next covariates: $\mathbf{X}_{s+1}^{(n)} \sim p_{\theta_{X}}(\cdot\mid\mathbf{H}_s^{(n)})$
      \STATE Sample next outcome: $Y_{s+1}^{(n)} \sim p_{\theta_Y}(\cdot\mid\mathbf{H}_s^{(n)}, W_s^{(n)})$
      \STATE Update history:
      \begin{align*}
        \mathbf{H}_{s+1}^{(n)} \gets \mathbf{H}_s^{(n)} \cup \{\mathbf{X}_{s+1}^{(n)}, W_s^{(n)}, Y_{s+1}^{(n)}\}
      \end{align*}
    \ENDFOR
  \ENDFOR

  \STATE \textbf{Stage 3: Causal estimand}
  \STATE Compute:
  \[
    \hat\mu_{t,\rho}^{\pi}(\mathbf{h}_t)
    = \frac{1}{N_{MC}} \sum_{n=1}^{N_{MC}} Y_{t+\rho}^{(n)}
  \]
  \RETURN $\hat\mu_{t,\rho}^{\pi}(\mathbf{h}_t)$
\end{algorithmic}
\end{algorithm}

G-Net is \gls{rnn}-based realization of Algorithm \ref{alg:gcomp} where similar to Causal transformers and CRN, a representation \(\Phi_t\) of the process history \(\mathbf{H}_t\) is learned through an \gls{lstm} which is used to learned conditional densities  \(p_{\theta_{W}}(W_t\mid\Phi_t),\;
    p_{\theta_{X}}(\mathbf{X}_{t+1}\mid\Phi_t),\;
    p_{\theta_Y}(Y_{t+1}\mid\Phi_t, W_t)\). Everything is trained end-to-end by the negative log-likelihood of the triples $(W_t,\mathbf X_{t+1},Y_{t+1}) $.

Since we only treat time-varying treatment regimes similar to RMSM, CRN, and Causal Transformers, the g-calculus could be adapted to this case by replacing a policy with a sequence of potential treatments:

\begin{corollary}
\label{corr:g_calculus_time_var_tr}
Assume we are operating under a time-varying treatment regime following Assumption \ref{assp:time_varying_treat}. Given the same assumption as in the Proposition \ref{prop:g_calculus_dtr}, the conditional counterfactual response at the horizon $\rho$ for a fixed treatment plan $\omega_{t:t+\rho-1}\!=\!(\omega_t,\dots,\omega_{t+\rho-1})\in\mathcal W^{\rho}$ is expressed as
\begin{equation}
\label{eq:g_calculus_time_var_tr}
\begin{split}
&\mathbb{E}\bigl[Y_{t+\rho}\bigl(\omega_{t:t+\rho-1}\bigr)
  \;\bigm|\;
  \mathbf{H}_t=\mathbf{h}_t\bigr]\\
&=
\int_{\mathcal X^{\rho-1}}\!\!
\int_{\mathcal Y^{\rho-1}}
\mathbb{E}\Bigl[
  Y_{t+\rho}
  \;\bigm|\;
  \mathbf{H}_t=\mathbf{h}_t,\,
  \mathbf{X}_{t+1:t+\rho-1}=\mathbf{x},\,
  Y_{t+1:t+\rho-1}=y,\\
&\qquad
  W_{t:t+\rho-1}
    =\omega_{t:t+\rho-1}
\Bigr]\\
&\quad\times
\prod_{j=t+1}^{t+\rho-1}
  p\Bigl(
    \mathbf{x}_j,\,y_j
    \;\bigm|\;
    \mathbf{H}_t=\mathbf{h}_t,\,
    \mathbf{X}_{t+1:j-1}=\mathbf{x}_{t+1:j-1},\,
    Y_{t+1:j-1}=y_{t+1:j-1},\\
&\qquad
    W_{t:j-1}
      =\omega_{t:j-1}
  \Bigr)
\,d\mathbf{x}\,dy\,.  
\end{split}
\end{equation}

\end{corollary}

\section{Causal graphs}
\label{sect_background:causal_graphs}
In this section, we define a causal graph mathematically. Establishing the formalism of such an object is crucial for this thesis because, although we adopt the \gls{po} framework in the first two contributions to reason about causal inference, having a graphical understanding of causal assumptions allows us to simplify conditional probabilities by leveraging the graphical structure between variables. On the other hand, the notion of a causal graph is fundamental in the third contribution, as we no longer reason about specific treatments and responses but instead focus on how the variables constituting the time-varying confounders \(\mathbf{X}_t\) interact with each other. Since these confounder variables are often high-dimensional and sparse, such as vectors representing baskets of purchased products (cf. Chapter \ref{chapter:intro}, Section \ref{sect_crl:intro}), the modern machine learning approach is to model them using neural network-based representations, as done in the first two contributions. This naturally raises the question of whether one can learn representations of confounders such that the latent variables are \emph{causal}, meaning they exhibit causal relationships among themselves both instantaneously (within each time slice) and over time (across time slices). This field of study is commonly called \emph{causal representation learning} (CRL) \citep{scholkopf2021toward}.  

It is worth mentioning that different causal modeling frameworks exist for reasoning about the causal learning problem. The two most common frameworks are causal graphical models (CGMs) and \gls{scm}. Causal Bayesian networks are another term used to refer to CGMs \citep{spirtes2001causation}.  

The first and necessary building block for defining a causal graphical model is to establish what we mean by a causal relationship between two arbitrary random variables.  

\begin{definition}[Causal Effect \citep{scholkopf2022statistical}]  
\label{def:causal_effect}  
A random variable \(X_1\) is said to have a causal effect on a random variable \(X_2\) if there exist two values \(x_1 \neq x'_1\) such that the distribution of \(X_2\) after \emph{intervening} on \(X_1\) and setting it to \(x_1\) differs from the distribution of \(X_2\) after setting \(X_1\) to \(x'_1\).  
\end{definition}  

A crucial component in defining a causal effect is the notion of \emph{intervention}, which refers to an action upon the cause \(X_1\). This bears the same intuition as the nature of treatment in the potential outcome framework. However, one still needs to formally define what an intervention entails when dealing with causal graphs, which naturally leads to the discussion of the \emph{do-operator}.  

A causal graphical model is, first and foremost, a directed graphical model in the classical sense \citep{lauritzen1996graphicalmodels, koller2009probabilisticgraph} that is acyclic; i.e., every causal effect “propagates” from earlier to later variables, and no variable can (directly or indirectly) be its own ancestor, thereby enforcing the principle that causes precede their effects. However, unlike standard directed graphical models, the directed edges in a causal graphical model carry a \emph{causal interpretation}: a directed edge signifies a causal effect, as stated in Definition \ref{def:causal_effect}. Formally:

\begin{definition}[CGM]
\label{def:CGM_CBN}
A Causal Graphical Model (CGM) \( \mathcal{M}=(G,p) \) over \( n \) random variables \( X_1,\dots,X_n \) is a tuple consisting of:  
\begin{itemize}
    \item A directed acyclic graph (DAG) \( G \), where directed edges (\( X_j\rightarrow X_i \)) represent a direct causal effect of \( X_j \) on \( X_i \), as in Definition \ref{def:causal_effect}.
    \item A probability distribution \( p(X_1, \dots, X_n) \) that is \emph{Markovian} \gls{wrt} \( G \), meaning it factorizes as:
\end{itemize}
\begin{equation}
\label{eq:cf}
p(X_1, \dots, X_n)=\prod_{i=1}^n p(X_i \mid Pa(X_i))
\end{equation}
where \( Pa(X_i) \coloneqq \{X_j : (X_j\rightarrow X_i) \in G\} \) is the set of parents (i.e., direct causes) of \( X_i \) in the graph \( G \).  
\end{definition}

Assuming \( p(X_1, \dots, X_n) \) admits a strictly positive density \gls{wrt} a product measure (e.g a product of Lebesgue and counting measures depending on whether \(X_i\) is continuous or discrete) so that the conditional probability distribution \( p(X_i \mid Pa(X_i))\) is well defined for every \(i \in \{1,\dots,n\}\) and for every possible choice of the set \(Pa(X_i)\)\citep{Lauritzen1990}, the Markov factorization is equivalent to what is known as the \emph{local directed Markov condition} \citep{spirtes2010introduction}, which is a purely probabilistic graphical property. 

\begin{definition}[Local Directed Markov Condition]
\label{def:causalMarkov}
A distribution \( p \) satisfies the local directed Markov condition \gls{wrt} a \gls{dag} \( G \) if every variable is conditionally independent of its non-descendants in \( G \), given its parents in \( G \).  
\end{definition}

For example, if we are given a probability distribution over three variables \(p(X_1, X_2, X_3)\) such that
\[
p(X_1, X_3 \mid X_2) = p(X_1 \mid X_2)\, p(X_3 \mid X_2),
\]
and we assume a \gls{dag} of the form
\[
X_1 \longleftarrow X_2 \longrightarrow X_3,
\]
then \(p\) satisfies the local directed Markov condition because \(X_1\), given its parent \(X_2\), is conditionally independent of its non-descendant \(X_3\), i.e.,
\[
X_1 \indep X_3 \mid X_2.
\]
The same property holds for \(X_3\) by symmetry.

Under the condition of strict positive density for \( p(X_1, \dots, X_n) \), the Markov factorization is also equivalent to another important graphical criterion extensively used in causal inference: \emph{d-separation}. To formally define d-separation, we first introduce the concept of a \emph{path} being \emph{blocked} in a graph.  
\begin{definition}[Path]
A path \(\pi = (X_1, \dots, X_p)\) in a DAG \(G\) is a sequence of distinct nodes connected by edges, regardless of their orientation, that is, for \(i\neq j\), \(X_i \neq X_j\) and 
\[
X_j\rightarrow X_i \text{ or } X_i\rightarrow X_j.
\]
\end{definition}

\begin{definition}[Blocking a Path]
\label{def:blocking_path}
A path \(\pi = (X_1, \dots, X_p)\) is said to be blocked given a set of observed nodes \(\mathbf{O}\) if there exists a node \(X_i\) in the path such that:
\begin{itemize}
    \item \(X_i\) is a common parent, i.e., \(X_{i-1} \longleftarrow X_i \longrightarrow X_{i+1}\), and \(X_i \in \mathbf{O}\).
    \item \(X_i\) is part of a cascade structure, i.e., \(X_{i-1} \longrightarrow X_i \longrightarrow X_{i+1}\) or \(X_{i-1} \longleftarrow X_i \longleftarrow X_{i+1}\), and \(X_i \in \mathbf{O}\).
    \item \(X_i\) is a collider, i.e., \(X_{i-1} \longrightarrow X_i \longleftarrow X_{i+1}\), but \(X_i \notin \mathbf{O}\) and no descendant of \(X_i\) is in \(\mathbf{O}\).
\end{itemize}
\end{definition}

For example, let's consider the path \(  X_1 \longrightarrow X_2 \;\longleftarrow\; X_3 \longrightarrow X_4 \longrightarrow X_5
\) and let  \(\mathbf O\subseteq\{X_2,\,X_3,\,X_4\}\), then:
\begin{itemize}
  \item At \(X_2\): the structure \(X_1 \;\to\; X_2 \;\leftarrow\; X_3\) makes \(X_2\) a \emph{collider}; it is blocked if \(X_2\notin \mathbf O\).
  \item At \(X_3\): the structure \(X_2 \;\leftarrow\; X_3 \;\to\; X_4\) makes \(X_3\) a \emph{fork}; it is blocked if \(X_3\in \mathbf O\).
  \item At \(X_4\): the structure \(X_3 \;\to\; X_4 \;\to\; X_5\) makes \(X_4\) a \emph{chain}; it is blocked if \(X_4\in \mathbf  O\).
\end{itemize}

\textbf{All conditioning blocking sets:} the path is blocked by \(\mathbf O\) precisely when \emph{at least one} of the following holds:
\begin{itemize}
  \item \emph{Collider at \(X_2\) is blocked}: \(X_2\notin \mathbf O\).
  \item \emph{Fork at \(X_3\) is blocked}: \(X_3\in \mathbf O\).
  \item \emph{Chain at \(X_4\) is blocked}: \(X_4\in \mathbf O\).
\end{itemize}

Equivalently, every subset \(\mathbf O\) except the one that contains \(X_2\) and contains neither \(X_3\) nor \(X_4\) will block the path.  Thus, the seven blocking sets are:
\begin{center}
\begin{tabular}{ll}
\toprule
Set \(O\) & Blocks via \\
\midrule
\(\emptyset\)               & \(X_2\) (collider; \(X_2\notin \mathbf O\)) \\
\(\{X_3\}\)                & \(X_2\) or \(X_3\) \\
\(\{X_4\}\)                & \(X_2\) or \(X_4\) \\
\(\{X_3,X_4\}\)            & \(X_2\), \(X_3\), or \(X_4\) \\
\(\{X_2,X_3\}\)            & \(X_3\) \\
\(\{X_2,X_4\}\)            & \(X_4\) \\
\(\{X_2,X_3,X_4\}\)        & \(X_3\) or \(X_4\) \\
\bottomrule
\end{tabular}
\end{center}
\paragraph{Non–blocking set:} The only subset that does \emph{not} block is \(\mathbf O = \{X_2\}\), since it “unblocks” the collider at \(X_2\) and contains neither \(X_3\) nor \(X_4\).

\begin{definition}[D-separation]
\label{def:d-sep}
Let \( A, B, C \) be non-overlapping sets of nodes in a graph \( G \). \( A \) and \( B \) are \emph{d-separated} given \( C \) if all paths connecting \( a \in A \) and \( b \in B \) are blocked by \( C \), meaning the paths are inaccessible when conditioning on \( C \).  
\end{definition}

One key application of d-separation is simplifying conditional probability dependencies based on the graphical relationships between variable sets \( A, B, C \).

\begin{proposition}
\label{prop:prod_prob_d-sep}
If the sets of nodes \( A \) and \( B \) are d-separated given \( C \), then:
\[
p(A, B \mid C) = p(A \mid C) p(B \mid C).
\]
\end{proposition}

\begin{corollary}
\label{corollary:simplify_cond_prob_d-sep}
If the sets of nodes \( A \) and \( B \) are d-separated given \( C \), then the conditional probability \( p(A \mid B, C) \) simplifies to \( p(A \mid C) \), meaning it is sufficient to condition only on the set of nodes blocking the paths between \( A \) and \( B \).
\end{corollary}

The global directed Markov condition is based on the d-separation property and is defined as follows:  

\begin{definition}[Global Directed Markov Condition]  
\label{def:global_markov_cond}  
A probability distribution \( p \) is said to satisfy the global directed Markov condition if, for any disjoint sets of variables \( A, B, C \), d-separation of \( A \) and \( B \) given \( C \) in \( G \) implies that \( A \) is conditionally independent of \( B \) given \( C \) in \( p \).  
\end{definition}  

When a graphical model is endowed with a causal interpretation, as in the case of CGM in Definition \ref{def:CGM_CBN}, the local directed Markov condition becomes a key property that links causal relationships in a causal graph to conditional probabilities. This property is known as the \emph{Causal Markov Condition} \citep{spirtes2001causation}. To define it formally, we first introduce the notion of a causally sufficient set of variables in a graph.  

\begin{definition}[Causally Sufficient Set]  
\label{def:caus_suff_set}  
A set of variables \( \mathbf{O}\) in a causal graph \( G \) is said to be causally sufficient if there is no variable \( X \) in \( \bar{\mathbf{O}} \) that is a common cause of at least two variables in \( A \).  
\end{definition}  
In other words, a set of variables is causally sufficient if it includes all common causes of the variables within the set. For example, if a DAG has the form
\[
X_1 \longrightarrow X_2 \;\longleftarrow\; X_3 \longrightarrow X_4 \longrightarrow X_5,
\]
then the set \(\{X_1, X_2, X_4\}\) is not causally sufficient because it misses a common parent of two variables within the set, \(X_2\) and \(X_4\), which is \(X_3\). The set \(\{X_1, X_2, X_3, X_4\}\) is therefore causally sufficient.

We can now define the Causal Markov Condition.

\begin{definition}[Causal Markov Condition]  
\label{def:causal_markov_cond}
Let \( \mathcal{M} = (G, p) \) be a CGM over \( n \) random variables \( X_1, \dots, X_n \). The causal graph is said to satisfy the Causal Markov Condition if the set of variables \( \{X_1, \dots, X_n\} \) is causally sufficient and the distribution \( p(X_1, \dots, X_n) \) satisfies the local directed Markov condition (cf. Definition \ref{def:causalMarkov}).  
\end{definition}  
The utility of the Causal Markov Condition lies in its ability to express the joint probability distribution of the system variables \( X_1, \dots, X_n \). If a variable, say \( X_j \), is externally manipulated to follow a new mechanism \( p^*(X_j \mid Pa(X_j)) \), then one only needs to replace the original mechanism \( p(X_j \mid Pa(X_j)) \) with its altered version \( p^*(X_j \mid Pa(X_j)) \) in the Markov factorization according to the graph \( G \):  

\begin{equation}
\label{eq:do_proba}
    p(X_1, \dots, X_n \mid do(X_j \sim p^*(X_j \mid Pa(X_j)))) \coloneqq p^*(X_j \mid Pa(X_j)) \prod_{i=1, i\neq j}^n p(X_i \mid Pa(X_i)).
\end{equation}

Here, we use the \emph{do-notation} to emphasize that \( X_j \) has been actively intervened upon rather than passively observed. As a result, the conditioning sign in the \gls{lhs} of Equation \ref{eq:do_proba} does not represent classical probabilistic conditioning.  

It is common for the variable \( X_j \) to be assigned a particular value, say \( x_j \), typically denoted as \( do(X_j=x_j) \). In this case, we replace \( p(X_j \mid Pa(X_j)) \) with the Dirac distribution \( \delta(X_j = x_j) \), and the interventional probability becomes:  

\begin{equation}
\label{eq:do_atomic}
    p(X_1, \dots, X_n \mid do(X_j = x_j)) = \delta(X_j = x_j) \prod_{i=1, i\neq j}^n p(X_i \mid Pa(X_i)).
\end{equation}

\gls{scm} represents another causal modeling framework that still relates to causal graphs but differs in its functional nature: direct causes (parents) influence their effects (children) through directed functional relationships:
\begin{definition}[Structural Causal Model]
\label{def:SCM}
An \gls{scm} is a causal model represented by a tuple \( M = \langle \Xi_n, \mathbb{X}_n, \mathbb{F}, p_{\Xi_n} \rangle \), where:
\begin{enumerate}
    \item \(\Xi_n \coloneqq \{ \xi_1, \dots, \xi_n \}\) is the set of exogenous noise variables that capture factors not explicitly represented in the model.
    \item \(\mathbb{X}_n \coloneqq \{ X_1, \dots, X_n \} \) represents the set of observed variables in the model, also referred to as endogenous variables. These variables are determined by \(\Xi_n\) and \(\mathbb{X}_n\) itself through functional dependencies.
    \item \(\mathbb{F} \coloneqq \{ f_1, f_2, \dots, f_n \} \) is the set of structural functions such that:
\[
    X_i := f_i\left(Pa(X_i), \xi_i\right), \quad i=1, \dots, n
 \]
where \(Pa(X_i) \subset \mathbb{X}_n -\{X_i\}\).
    \item \(p_{\Xi_n}\) refers to the joint probability distribution over the noise terms \(p_{\Xi_n}(\xi_1, \dots, \xi_n)\).
\end{enumerate}
\end{definition}

From the definition of an \gls{scm}, there is a strong connection with causal graphs. Given the structure of an \gls{scm}, we can define an associated causal graph as follows:  

\begin{definition}[Induced Causal Graph]
\label{def:inducedgraph}
The causal graph $G$ induced by an \gls{scm} \( M = \langle \Xi_n, \mathbb{X}_n, \mathbb{F}, p_{\Xi_n} \rangle \) is the directed graph with nodes $ \mathbb{X}_n$ and a directed edge from each node in $Pa(X_i)$ to $X_i$ for all $i \in \{1, \dots, n\}$.
\end{definition}

According to the induced causal graph, we must eliminate any possible cycles in the graph to ensure that the probability distribution over the observed variables \( \mathbb{X}_n \) is uniquely defined. We therefore assume the acyclicity of the induced causal graph:  

\begin{assumption}[Acyclicity]\label{ass:acyclicity}
The induced graph \( G \) of an \gls{scm} \( M \) is assumed to be a directed acyclic graph (DAG).
\end{assumption}

To ensure that the probability distribution over the observed variables \( \mathbb{X}_n \), as induced by the \gls{scm} model, admits a Markov factorization according to its induced causal graph, we further assume that the exogenous noise variables are independent:  

\begin{assumption}[Causal Sufficiency / No Hidden Confounders]
\label{ass:causalsufficiency}
The exogenous noise variables \( \Xi_n \) are jointly independent, i.e.,  
\[
p_{\Xi_n}(\xi_1, \dots, \xi_n) = p_{\xi_1}(\xi_1) \times \dots \times p_{\xi_n}(\xi_n).
\]
\end{assumption}

The causal sufficiency assumption is equivalent to stating that the set of observed causal variables is causally sufficient according to Definition \ref{def:caus_suff_set}. Moreover, this assumption is often referred to as the \emph{no hidden confounders} assumption, since the presence of an unobserved common cause of variables within \( \mathbb{X}_n \) would violate causal sufficiency. Specifically, if a common cause of variables in \( \mathbb{X}_n \) is not itself part of \( \mathbb{X}_n \), then \( \mathbb{X}_n \) would not be causally sufficient, leading to dependencies among the exogenous noise variables and violating the assumed independence of \( \Xi_n \).

An important consequence of acyclicity and causal sufficiency is that the causal conditionals associated with the causal graph can now be defined as the push-forward of the noise distribution \( p_{\Xi_n} \) through the functional dependencies \( \mathbb{F} \):  
\[
p(X_i \mid Pa(X_i)) \coloneqq p_{\xi_i}(f_{Pa(X_i)}^{-1}(X_i)) \quad \text{for} \quad i=1,\dots,n,
\]
where \( f_{Pa(X_i)}^{-1}(X_i) \) denotes the preimage of \( X_i \) under the mapping \( f_i \), given the values of \( Pa(X_i) \).


==> 3.tex <==
\chapter{Causal Dynamic Variational Autoencoder}
\label{chapter:cdvae}
\section{Introduction}
\label{sect_cdvae:intro}
Estimating \gls{ite} helps us understand how individuals uniquely respond to the same treatment, enabling more personalized and effective decision-making. For example, in healthcare, two patients receiving the same drug might experience considerably different outcomes due to underlying genetic or lifestyle differences \citep{atan2018Deep-Treat, shalit2020ITPolicyClinical, mueller2023personalized}. The exact curriculum might yield more remarkable improvement for one student than another in education, depending on background factors like socioeconomic status \citep{morgan2013handbookSocial, Imbens2015CausalIF}. Likewise, in marketing, identical promotions might drive purchases in one customer segment but not another \citep{hair2021dataMarketing, fang2023alleviating}.

\emph{Longitudinal data} arise naturally in these domains. Consider, for instance, a medical dataset recording blood pressure, treatments (e.g., vasopressors), and vitals for each patient at regular intervals. Or a retail dataset tracking weekly customer purchases following commercial campaigns. Each longitudinal data describe a sequence of treatments, covariates, and responses causally interacting through time. As discussed in Section \ref{intro:model_challenges_time} and \ref{sect_intro:review_miss_conf}, this setting brings unique challenges:
\begin{inparaenum}[(1)]
    \item \emph{Time-dependent confounding}: Confounders influenced by past treatment can impact subsequent treatments and responses \citep{platt2009time};
    \item \emph{Selection bias}: Time-varying covariates exhibit imbalanced distributions across treatment regimes, which should be accounted for to estimate treatment effects accurately \citep{robins2000MSM, schisterman2009overadjustment, lim2018RMSN};
    \item \emph{Long-term dependencies}: A treatment effect may unfold over extended periods, requiring models to capture complex long-range interactions between covariates, treatments, and responses \citep{choi2016retain, pham2017predicting};  
    \item \emph{Missing covariates}: Some variables crucial for predicting outcomes—like genetic predispositions or environmental exposures—introduce bias and less personalized treatment effect estimation unless properly accounted for.  
\end{inparaenum}

\paragraph{Assumptions over Confounders and Existing Approaches}  
The existing literature primarily addresses the first three challenges under the assumption of \emph{sequential ignorability} (\ref{assp:seq_ignorability}), where all confounders, whether static or time-varying, are fully observed. Methods such as \gls{msm} \citep{robins-time-varying-exposures}, \gls{rmsm} \citep{lim2018RMSN}, \gls{crn} \citep{bica2020estimatingCRN}, G-Net \citep{Li2021GNetAR}, \gls{ct} \citep{Melnychuk2022CausalTF}, and our model Causal \gls{cpc} \citep{bouchattaoui2024CausalCPC} have been developed based on this assumption (cf. Section \ref{sect_background:po_framework_longit_overview}, Chapter \ref{chapter:background}). When the fourth challenge—missing covariates—is addressed, it is often in the form of \emph{missing confounders}, violating sequential ignorability. Existing approaches (cf. Section \ref{sect_intro:review_miss_conf}) either condition on \emph{observed proxies} of confounders to infer a latent representation of the unobserved confounders \citep{MeasbiasproxyConf, MiaoProxyUnmeasuredConf2016, louizos2017causalproxyconf, LuChengCMAproxynConf20121} or apply the \emph{deconfounding technique}, which involves imposing a factor model over the treatment assignment to mitigate hidden confounding \citep{lopezmultipletreatments, ranganath2018multiple, wang2019blessings, zhang2019medicalDeconf, Bica2020TimeSDecounf, hatt2024sequential}.  

\paragraph{Our Focus} In contrast to missing confounders, we study for the first time the presence of \emph{unobserved static adjustment variables}—factors that influence only the outcome sequence and remain \emph{time-invariant}. In a medical context, these could include genetic factors, environmental conditions, or lifestyle attributes that impact treatment response but are not directly observed \citep{sadowski2024characterizing}. The absence of such variables can lead to a loss of heterogeneity in the estimated treatment effect. This phenomenon can also be understood through the lens of \emph{population structure}, which arises from distinct subgroups within a population that share characteristics such as geography, socioeconomic status, or cultural practices. Having knowledge of, or being able to infer accurately, population structure allows for a more precise estimation of \gls{ite} by capturing variations in treatment responses across subgroups. In genomics \citep{laird2011fundamentalsgenetics, peter2020genetic}, for instance, such a structure arises due to evolutionary or migration histories. Moreover, population structure often acts as an \emph{effect modifier} \citep{hernan_whatif_2020}, altering treatment effects across subgroups without directly influencing treatment assignment \citep{hyun2024increased}. By accounting for such effect modifiers through stratified or interaction analyses, treatment effects can be estimated more accurately, even in randomized trials \citep{schochet2024design}. 

In this work, we specifically address the challenge of missing covariates by focusing on estimating the contemporaneous treatment effect (\ref{assp:contemporaneous_effect})—the effect of the current treatment on the subsequent response. The potential trajectory of treatments up to \( t-1 \), \( \omega_{< t} \), is assumed to be consistent with the observed history of treatments, i.e., \( \omega_{< t} = W_{< t} \). Therefore, the potential outcomes of interest at each time step \( t \) are \( \{Y_t(W_{< t}, \omega)\}_{\omega \in \mathcal{W}} \).

\begin{remark}[Carryover Effect and CTE]
\label{remark:carryover_effect}
Although we target the contemporaneous treatment effect in the \gls{cdvae} model, we do not formally assume the no carryover effect (Definition \ref{def:carryover_effect}), i.e., that past treatments do not affect current outcomes. This would imply that given any two potential treatment sequences \( \omega_{\leq t} \) and \( \omega'_{\leq t} \), such that \( \omega_t = \omega'_t \), then \( Y_t(\omega_{\leq t}) = Y_t(\omega'_{\leq t}) \), which is different from our Assumption \ref{assp:contemporaneous_effect}.
\end{remark}

We consider the \gls{ite} as an \emph{\gls{acate}}, where the \gls{cate} depends not only on the confounding variables but also on adjustment variables. We aim to achieve \emph{near-oracle performance} in treatment effect estimation by leveraging the learned representation of unobserved adjustment variables. Specifically, we prove that for all baselines satisfying sequential ignorability, treatment effect estimation is substantially improved when these models are augmented with the learned representation of unobserved adjustment variables produced by our model—ultimately delivering performance that approaches the oracle scenario, where the true unobserved adjustment variables are directly fed into the baselines. Extensive experiments on synthetic data and semi-synthetic data derived from real-world datasets such as \gls{mimic}-III \citep{johnson2016mimic} validate our approach.


\paragraph{Our Approach}  
We treat the unobserved adjustment variables as latent variables and leverage a probabilistic modeling approach based on the \emph{Dynamic Variational Autoencoder (DVAE)} framework \citep{Girin2021DynamicalVAReview} to estimate the \gls{acate}, where we augment the CATE with the learned representation of unobserved adjustment variables, which we term \emph{substitutes}. We address the covariate imbalance induced by selection bias in longitudinal data using a weighted empirical risk minimization strategy, where the weights are a function of the propensity scores. Additionally, we derive a generalization bound for the error in estimating \gls{acate} and use its approximation as a loss function for our model, which we refer to as \emph{Causal DVAE (CDVAE)}. To account for potential population structure induced by unobserved adjustment variables, we define a flexible prior over the latent variables using a learnable \gls{gmm}. We ensure the causal validity of the learned substitutes by imposing a finite-order \gls{cmm} on the response series. The causal validity follows from our proof that, once the finite-order \gls{cmm} holds, the learned substitutes account for all relevant adjustment variables (Theorem \ref{thm:valid_Z}) and that the \gls{acate} leveraging the substitutes is identifiable. To experimentally support the theoretical analysis, we discuss the relevance of all CDVAE components through an ablation study. 

Furthermore, since we adopt a probabilistic approach, we represent the substitute for unobserved adjustment variables as a \emph{stochastic} latent variable. Consequently, the choice of the substitute given individual longitudinal data is not unique.  As a novel contribution, we study Causal DVAE in the \emph{near-deterministic regime}, where we reduce the variance of the responses (outputs of the Causal DVAE) to near zero. This process indirectly pushes the covariance matrix of the substitutes toward zero, preventing their distribution from becoming overly diffuse. An intuitive consequence of this approach is that any sampled substitute of the adjustment variables yields the same treatment effect as the mean substitute. We demonstrate that as the response variance approaches zero, the treatment effect remains consistent regardless of the specific instance of the substitutes. The near-deterministic regime of VAEs has not been previously explored in the context of causal inference, making this a novel contribution. To draw an analogy, in the deconfounding literature \citep{lopezmultipletreatments, ranganath2018multiple, wang2019blessings, zhang2019medicalDeconf, Bica2020TimeSDecounf, hatt2024sequential}, substitutes—referring to learned representations of missing confounders—are theoretically assumed to follow a Dirac posterior. This enables deterministic selection and facilitates treatment effect identifiability. However, the training of these models is based on a non-degenerate posterior, creating a disconnect between theoretical assumptions and practical implementation. Our approach bridges this gap by achieving near-deterministic behavior while maintaining a probabilistic framework.
 
We also examine the classical approach of mixed-effect modeling for treatment effect estimation, which uses \textit{random effects} to capture individual-level variation and account for latent heterogeneity \citep{fitzmaurice2012applied, Demidenko2013MixedMT}. While these models address unobserved heterogeneity by incorporating random intercepts or slopes, our modeling  goes further by learning representations of unobserved variables and seamlessly integrating them into the \gls{ite} estimation pipeline. This comparison highlights a shared objective: both approaches aim to mitigate unobserved heterogeneity to enhance the precision of treatment effect estimates. 

Our \emph{contributions} can be summarized as follows: 
\begin{itemize}
    \item We propose a principled approach to infer a latent representation of unobserved adjustment variables (Section \ref{sect_cdvae:causal_dvae}).
    \item We prove the theoretical validity of the learned adjustment variables by modeling the response series as a finite-order conditional Markov process, ensuring that \gls{ite} conditioned on learned substitutes are identifiable (Section \ref{sect_cdvae:CMM}).
    \item We study for the first time the near-deterministic regime of VAEs for causal inference and show that reducing the variance of response predictions enforces consistency in treatment effect estimation, even under stochastic modeling of adjustment variables (Section \ref{sect_cdvae:cdvae_near_det}).
    \item Numerical experiments confirm the effectiveness of \gls{cdvae} in estimating \gls{ite}, showing that our method consistently outperforms \gls{sota} baselines (Section \ref{sect_cdvae:experiments}), as further analyzed through an ablation study.
    \item We show that for \gls{sota} baselines, augmenting their input covariates with the inferred representation of adjustment variables given by \gls{cdvae} substantially enhances their accuracy in estimating \gls{ite} (Section \ref{sect_cdvae:experiments}) and even provide near-oracle performances.
\end{itemize}


\section{Related Work}
\paragraph{Causal Inference in Time-Varying Settings.} In Section \ref{sect_background:po_framework_longit_overview}, we extensively covered \gls{msm} \citep{robins2000MSM} and their role in addressing time-varying confounders in causal inference through IPTW \citep{robins-time-varying-exposures}. Despite their utility, \gls{msm} encounter challenges related to high-variance estimates and the need for a good specification of the treatment assignment mechanism, especially in complex scenarios. \gls{msm} are often integrated with g-computation \citep{vansteelandt2014structural} and Structured Nested Mean Models \citep{robins1997causalNested}, particularly in epidemiology. We also discussed recent advancements utilizing neural network-based models, such as the \gls{rmsm} \citep{lim2018RMSN}, employing RNNs for enhanced modeling of propensity and outcomes, and the \gls{crn} \citep{bica2020estimatingCRN}, which adopts adversarial domain training to mitigate bias in the presence of time-varying confounders. Additionally, we examined the G-Net \citep{Li2021GNetAR} and the \gls{ct} \citep{Melnychuk2022CausalTF}, highlighting their contributions to multi-timestep counterfactual prediction through g-computation and adversarial training, respectively. Although the contribution of the next Chapter \ref{chapter:ccpc} (Causal \gls{cpc}) targets the long-term counterfactual regression, we include it in this chapter's experiments as a complementary baseline. Causal \gls{cpc} leverages temporal dynamics through contrastive predictive coding and information maximization and learns a balanced representation using an adversarial training strategy (cf. Chapter \ref{chapter:ccpc} for a full description).

\begin{warning}
While the aforementioned models have made significant strides in causal inference for time-varying settings, our approach laid by CDVAE enhances these methods by incorporating inferred adjustment variables into the modeling process. By augmenting the input covariates of these \gls{sota} models with our inferred representations, we achieve a more accurate estimation of \gls{ite} and improve the overall robustness of causal inference in longitudinal data.   
\end{warning}

\paragraph{Combining Weighting and Representation Learning}
A key driver for developing representation learning in causal inference is to address covariate imbalance in high-dimensional settings. These methods aim to achieve balance in the learned feature space to mitigate covariates shift. Combining weighting methods, such as those proposed by \cite{zubizarreta2015stable, li2018balancing, johansson2018learningweighted, hassanpour2019counterfactual}, with representation-based causal inference, offers a promising approach to address the challenges faced by representation learning in the context of causal inference. These methods demonstrate how properly designed weights can alleviate the difficulties associated with representation learning techniques. However, a trade-off exists between covariate balance and predictive performance: \emph{overly strict balancing can lead to the loss of valuable features and exacerbate bias in estimating treatment effects \citep{assaad2021counterfactual, zhang2020learning}.} On the other hand, \cite{zhang2020learning} and \cite{johansson2019support} highlighted that such regularization might lead to a loss of ignorability in the representation and suggested learning representations in which context information remains preserved but where treatment groups overlap. To this end, \cite{assaad2021counterfactual} introduced the Balancing Weights Counterfactual Regression (BWCFR) method, which aims to achieve balance \emph{within the reweighted covariate} representations instead of directly balancing the covariates representations. \cite{assaad2021counterfactual} argues that BWCFR provides bounds on the degree of imbalance as a function of the propensity model and offers theoretical guarantees for estimating the \gls{cate} using the overlapping weight. \cite{johansson2022generalization} built on the previous work on sampling weighting for counterfactual regression and representation learning \citep{johansson2016learning, shalit2017estimating, kallus2020deepmatch, jung2020learningWERM, assaad2021counterfactual}, and provided a comprehensive theory for weighted risk minimization for \gls{cate} for a learned representation from the data. 
\begin{remark}
In this work, we extend the weighted empirical risk minimization framework, which has been primarily developed for static settings, to the longitudinal context. Our approach focuses on contemporaneous treatments rather than sequences of interventions (see Assumption \ref{assp:contemporaneous_effect}). This distinction allows us to naturally adapt these methods to time-varying data without introducing unnecessary complexity. While these extensions are straightforward, they offer important practical insights by maintaining the balance between covariates across time points, even as treatment effects evolve. 
\end{remark}

\paragraph{Probabilistic Modeling in Causal Inference}
In scenarios where confounders are unobserved but proxy variables are available, probabilistic models were used to infer a representation for the unobserved confounding given the proxy variables \citep{MeasbiasproxyConf, MiaoProxyUnmeasuredConf2016, louizos2017causalproxyconf, LuChengCMAproxynConf20121}. While our work assumes the presence of observed confounding, it draws inspiration from the theory of deconfounding \citep{lopezmultipletreatments, ranganath2018multiple, wang2019blessings}, and its recent extensions to time-varying settings. The idea behind the deconfounding is to impose a factor model over the treatment assignment, where each cause becomes conditionally independent given latent variables that serve as substitutes for the unobserved confounders. \cite{Bica2020TimeSDecounf} extended the application of the deconfounding method to sequential settings with multiple treatments, aiming to infer time-varying confounders. They assumed that the joint distribution of treatments at each time step, conditioned on learned substitutes and observed confounders, could be decomposed into the product of the conditional distribution of each treatment. For the case of a single treatment per time step, \cite{hatt2024sequential} assumed a conditional Markov model over the treatment sequences given the sequence of confounders and the latent variables to be inferred. However, extending the deconfounder theory to longitudinal settings does not guarantee the consistency assumption required for identifying the ATE. \cite{wang2019blessings} proposed a theory of identification that relies on the assumption that the operation on the latent variables follows a Dirac distribution, allowing for a certain construction of the substitute confounder. In contrast, \cite{Bica2020TimeSDecounf} utilizes variational dropout to construct the substitute, and \cite{hatt2024sequential} adopts variational inducing point-based inference for a Gaussian process latent variable model extended to the sequential setting.

\begin{warning}
In this work, we aim to demonstrate that the core idea of the factor model can be applied to learn valid substitutes for unobserved adjustment variables in the time-varying domain. Unlike previous deconfounder works, we show that assuming a higher-order conditional Markov model for the series of responses is sufficient to infer a valid representation of static adjustment variables. 
\end{warning}

\section{Problem Definition}
\label{sect_cdvae:problem_def}
This work adopts the \gls{po} framework for longitudinal data developed in Section \ref{sect_background:po_framework_longit_intro}. We consider a binary treatment variable and narrow the scope of \gls{po} to align with the \gls{cte} hypothesis, as outlined in Assumption \ref{assp:contemporaneous_effect}. Consequently, we express the counterfactual outcomes as \( Y_t(W_{< t}, \omega) \), simplified to \( Y_t(\omega) \) within this chapter for ease of notation.

Given the \gls{cte} assumption (\ref{assp:contemporaneous_effect}) and the binary nature of treatments, the \gls{cate} $\tau_{t}(\mathbf{x}_{\leq t}, y_{<t}; \omega_{\leq t}, \omega'_{\leq t})$ (Definition \ref{def:cate_time_varying}) can be simplified to:
\[
\tau_{t}(\mathbf{x}_{\leq t}, y_{<t}; \omega_{\leq t}, \omega'_{\leq t}) = \tau_{t}(\underbrace{\mathbf{x}_{\leq t}, y_{<t}, \omega_{< t}}_{\mathbf{h}_{t}}; \omega_{t}, \omega'_{t} ) = \mathbb{E}(Y_t(\omega_{t}) - Y_t(\omega'_{t}) \mid \mathbf{H}_{t} = \mathbf{h}_{t}),
\]
assuming that $\omega_{< t} = \omega'_{<t}$ by \gls{cte} is consistent with the observed history process $\mathbf{H}_{t}=\mathbf{h}_{t}$, i.e., $W_{<t} = \omega_{< t}$ by the \gls{cte} assumption. Since the treatment is binary, we adopt the convention where the value 0 refers to control and 1 refers to applying the treatment of interest. This allows us to define the \gls{cate} as
\[
\tau_{t}(\mathbf{h}_{t}; \omega_{t}, \omega'_{t}) = \tau_{t}(\mathbf{h}_{t}) = \mathbb{E}(Y_t(1) - Y_t(0) \mid \mathbf{H}_{t} = \mathbf{h}_{t}),
\]
which represents the difference between the expected potential outcomes at a time $t$, given the context history $\mathbf{H}_{t} = \mathbf{h}_{t}$.  The sequential ignorability assumption defined in Section \ref{assp:seq_ignorability} allows for the identification of \gls{cate}:
\begin{equation}
\tau_t(\mathbf{h}_t) = \mathbb{E}(Y_{t}| \mathbf{H}_t = \mathbf{h}_t, W_{t} = 1) - \mathbb{E}(Y_{t}| \mathbf{H}_t = \mathbf{h}_t, W_{t} = 0).
\label{eq:CATE_Identifiability}
\end{equation}
So far, we expressed the CATE as a function of the confounding history \(\mathbf{H}_t\). Now, assuming we \textbf{observe adjustment variables} $\mathbf{U}$ and aim to estimate a heterogeneous treatment effect depending on both $\mathbf{H}_{t}$ and $\mathbf{U}$. We define the \emph{Augmented CATE (ACATE)} as follows:
\begin{equation}
\label{eq:def_acate}
\tau_{t}(\mathbf{h}_{t}, \mathbf{u}) \coloneqq \mathbb{E}(Y_t(1) - Y_t(0) \mid \mathbf{H}_{t}= \mathbf{h}_{t}, \mathbf{U} =  \mathbf{u}).
\end{equation} 
The assumed risk factors $\mathbf{U}$ affect the response series but not the treatment as in the diagram of Figure \ref{fig:CG_compressed}. The fact that the adjustment variables do not confound treatment and response at any time step makes the assumed ignorability of treatment given history context sufficient to identify the \gls{acate}, i.e.,
\begin{equation}
\label{eq:acate_identif_U}
\tau_{t}(\mathbf{h}_{t}, \mathbf{u}) = \mathbb{E}(Y_{t}| \mathbf{H}_t = \mathbf{h}_t, \mathbf{U}= \mathbf{u}, W_{t} = 1)
- \mathbb{E}(Y_{t}| \mathbf{H}_t = \mathbf{h}_t, \mathbf{U}= \mathbf{u}, W_{t} = 0)
\end{equation}

\begin{figure}[ht]
    \centering
    \includegraphics[scale=0.6]{figures/cdvae/cg_cdvae_compressed.pdf}
    \caption{
        A simplified representation of the \gls{dgp} at time $t$. 
        Edges between $Y_{<t}$, $W_{<t}$, and $\mathbf{X}_{<t}$ are omitted for simplicity.
    }
    \label{fig:CG_compressed}
\end{figure}

\begin{intuitionbox}
\paragraph{Inference problem} Deriving the \gls{acate} becomes straightforward when both confounding and adjustment variables are fully observed. However, when \( \mathbf{U} \) is missing, unobserved heterogeneity in the treatment effect arises, leading to incomplete or biased conclusions about treatment effects. This raises the following key inference question: \textit{Under what conditions can a substitute \( \mathbf{Z} \) for the unobserved adjustment variables \( \mathbf{U} \) ensure the identifiability of the \gls{acate} by replacing \( \mathbf{U} \) with \( \mathbf{Z} \), specifically guaranteeing that the following equality \( \color{red}{(i)} \) holds?}  
\begin{equation}
    \begin{aligned}
     \tau_{t}(\mathbf{h}_{t}, \mathbf{z}) &=   \mathbb{E}(Y_t(1) - Y_t(0) \mid \mathbf{H}_{t}= \mathbf{h}_{t}, \mathbf{Z} =  \mathbf{z})\\
    &\overset{\color{red}{(i)}}{=}  \mathbb{E}(Y_{t}| \mathbf{H}_t = \mathbf{h}_t, \mathbf{Z}= \mathbf{z}, W_{t} = 1)
- \mathbb{E}(Y_{t}| \mathbf{H}_t = \mathbf{h}_t, \mathbf{Z}= \mathbf{z}, W_{t} = 0) \\
    \end{aligned}
    \label{eq:acate_with_Z}
\end{equation}
\end{intuitionbox}

\section{Mixed Effect Modeling and Heterogeneous Treatment Effect: A Unifying View}
To motivate our modeling approach, consider a study of vitamin D supplementation, represented by the treatment indicator \(W\),  on frailty $Y$ \citep{bray2018VitDeffect, cai2022VitDeffects}, with financial resources $\mathbf X$ as a confounder. For example, individuals with more economic resources may be more likely to afford and take vitamins. Observing data at multiple time points (e.g., monthly) allows us to use a causal graph to describe these relationships, as illustrated in Figure \ref{fig:dynamic_model_with_U}. 
\begin{figure}
     \centering
    \includegraphics[scale=0.7]{figures/cdvae/cg_mixed_effect_ex_.pdf}
    \caption{A causal graph describing panel data for the Vitamin D problem. }
  \label{fig:dynamic_model_with_U}
\end{figure}
The \gls{cate} can be defined, under the ignorability assumption of\ref{assp:ignorability} as:
$$\tau(\mathbf H_{t}) \coloneqq \mathbb{E}(Y_{t} \mid W_{t} = 1, \mathbf H_{t}) - \mathbb{E}(Y_{t} \mid W_{t} = 0,\mathbf H_{t}).$$
This equation shows that treatment effects can vary based on financial resources. However, consider the impact of vitamin D on frailty for younger versus older individuals. Age $U$ can significantly affect the treatment response, as younger individuals may metabolize vitamin D more effectively. Therefore, we use \gls{acate} (similar to Equation \ref{eq:def_acate}) as a treatment effect estimation that includes the age variable:
\begin{equation}
\label{eq:tau_X_U}
\tau(\mathbf H_{t},\mathbf U) \coloneqq \mathbb{E}(Y_{t} \mid W_{t} = 1,\mathbf H_{t},\mathbf U) - \mathbb{E}(Y_{t} \mid W_{t} = 0, \mathbf H_{t}, \mathbf U).
\end{equation}
Including $U$ improves prediction precision. When $U$ \emph{is unobserved}, mixed-effect models \citep{fitzmaurice2012applied, Demidenko2013MixedMT} help address this by accounting for random effects, which can be seen as proxies for unobserved factors like age. For illustrative purposes, we specify a mixed-effect model for the outcome variable:
\[
\label{eq:y_re_dynamic}
\scalebox{0.8}{%
$\mathbb{E}(Y_{t} \mid W_{t}, \mathbf X_{\leq t}, Y_{<t}, \alpha^{(1)}, \alpha^{(2)}) = \gamma_1Y_{t-1} + \gamma_2Y_{t-2} + \underbrace{(\beta_1 Y_{t-1} + (\beta_2 + \alpha^{(1)})X_{t} + \alpha^{(2)})}_{\text {\gls{acate}}}W_t + \beta_3X_{t}.$}
\]
Here, $\boldsymbol  \alpha = (\alpha^{(1)}, \alpha^{(2)})$ are \emph{random} effects, usually modeled with a Gaussian distribution $\mathcal{N}(0, \Sigma)$. \(\beta_1\) and \(\beta_2\) are unknown but \emph{fixed} effects. Having the two types of effects is what makes such modeling a mixed-effect model \citep{Demidenko2013MixedMT}. \(\gamma_1\)  and \(\gamma_2\) are also fixed unknown parameters. An interesting observation from Equation \ref{eq:y_re_dynamic} is that not all adjustment variables are necessarily present in the \gls{acate}. The past response $Y_{t-1}$ serves as an observed adjustment variable for $Y_{t}$ and modifies \gls{acate} when it changes through the parameter \(\beta_1\). On the other hand, $Y_{t-2}$ is still an adjustment variable but does not modify the effect \gls{acate} when it changes. This behavior summarizes  the concept of effect modification \citep{causainf_whatIf, VanderWeele2007FourTO}, where certain variables change the treatment effect when conditioned on them.

Random effects \(\boldsymbol  \alpha\) serve as a compact way to represent unobserved heterogeneity. This could be the case of factors such as age that are not directly recorded but nevertheless modify each subject’s response trajectory. For expositional clarity, let's adopt the guiding viewpoint that these random effects are random variables, measurable with respect to the unobserved sources of heterogeneity. Consequently, we can express $ \boldsymbol  \alpha  = \boldsymbol  \alpha(\mathbf U) \coloneqq (\alpha^{(1)}(\mathbf U), \alpha^{(2)}(\mathbf U))$, with $\alpha^{(1)}, \alpha^{(2)}: \mathcal{U} \xrightarrow{} \mathbb{R}$, two arbitrary unknown mappings. By substituting random parameters with $\mathbf U$ and incorporating mappings, we refine the model:
\[\mathbb{E}(Y_{t} \mid \mathrm{Pa}(Y_{t})) \coloneqq \gamma_1Y_{t-1} + \gamma_2Y_{t-2} + \underbrace{(\beta_1Y_{t-1} + (\beta_2 + \alpha^{(1)}(\mathbf U)))X_{t} + \alpha^{(2)}(\mathbf U))}_{\text {\gls{acate} }}W + \beta_3 \mathbf X_{t}.
\label{eq:model_pa_y}
\]
Here, $\mathrm{Pa}(Y) = \{W_{t},\mathbf X_{\leq t}, Y_{<t}, \mathbf U\}$ are the parent variables of $Y_t$.  Our method of inferring unobserved risk variables parallels non-linear mixed-effects models \citep{Demidenko2013MixedMT}. By viewing random effects as arising from unobserved risk factors, we may refer to these risk factors as random effects with slight terminology adjustments.

\paragraph{Methodology} Our approach aligns with Bayesian network concepts \citep{peters2017elements} and mixed-effects modeling. Rather than directly learning random parameters, we propose learning a representation of unobserved $\mathbf U$ and mapping $\alpha(.)$. Using neural networks \citep{Girin2021DynamicalVAReview}, we model complex non-linear dependencies and interactions among covariates, treatments, and inferred risk factors. Estimating the \gls{acate} with unobserved variables involves the following methodology:
\begin{compactenum}
\item Learn a representation $\mathbf{Z}$ of unobserved sources of variation.
\item Model the mapping $\alpha(.)$ using flexible neural networks to capture complex relationships.
\item Perform counterfactual regression, conditioning the treatment effect on representation $\mathbf{Z}$ and the observed context history.
\end{compactenum}

\section{Causal DVAE}
\label{sect_cdvae:causal_dvae}

\subsection{When does a Latent Representation Act as a Valid Substitute for Unobserved Adjustment Variables?}
\label{sect_cdvae:CMM}
To address the issue of unobserved risk factors $\mathbf{U}$ in our problem (as defined in Section \ref{sect_cdvae:problem_def}), we treat \(\mathbf{Z}\) as a latent variable to be learned from the observed data distribution \(p(\mathbf{X}_{\leq T}, W_{\leq T}, Y_{\leq T})\) within a probabilistic model defined over the conditional responses as follows:
\begin{assumption}[CMM($p$): Conditional Markov Model of order $p$]
\label{assp:cmm_y}
We say that a latent variable $\mathbf{Z}$ follows a Conditional Markov Model of order $p$, written \(\mathbf{Z} \sim CMM(p)\), if there exists a fixed order \( p \in \mathbb{N}^* \) and a parameter vector \( \theta \) such that the response distribution factorizes as:  
\[
p_\theta(y_{\leq T} , \mathbf{z} \mid  \mathbf{x}_{\leq T}, \omega_{\leq T}) = p(\mathbf{z})\prod_{t = 1}^T p_\theta\left(y_t \mid y_{t-1:t-p}, \mathbf{x}_{\leq t}, \omega_{\leq t}, \mathbf{z}\right).
\]
For \( t < 1 \), we set \( y_t = \emptyset \) by convention.
\end{assumption}

The fact that \(\mathbf{Z}\) is set only with a prior in Assumption \ref{assp:cmm_y} mimics the role of \(\mathbf{U}\) because \(\mathbf{U}\) consists of static adjustment variables that are parentless, as illustrated in the causal graph (Figure \ref{fig:CG_compressed}). The bounded memory assumption over the sequence of responses, that is, the direct causal effect of past responses on future ones stops at an arbitrary order \(p\), is a technical condition ensuring the causal validity of \(\mathbf{Z}\) as in the Theorem \ref{thm:seq_ign_augmented} where we demonstrate the sequential ignorability property when augmenting the history process with \(\mathbf{Z}\), replicating the same result as if the true adjustment variables \(\mathbf{U}\) were available. All the proofs are deferred to Appendix \ref{appendix_cdvae:proofs}.

\begin{theoremBox}[Sequential Ignorability with Augmented History]
\label{thm:seq_ign_augmented}
Let $\mathbf{Z}$ be a latent variable verifying CMM($p$). Assume the response domain $\mathcal{Y}$ is a Borel subset of a compact interval. Therefore, sequential ignorability holds when augmenting the history process with $\mathbf{Z}$: 
$$Y_{t}(\omega) \indep  W_{t}| \mathbf{H}_{t} = \mathbf{h}_{t},\mathbf{Z}= \mathbf{z}\quad \forall (\omega,\mathbf{h}_{t},\mathbf{z}),$$
where $\mathbf{H}_{t}$ represents the history process up to time $t$. 
\end{theoremBox}


The ignorability result of Theorem \ref{thm:seq_ign_augmented} is the first step into answering the inference problem of \ref{sect_cdvae:problem_def} as it allows us to establish the identifiability of the \gls{acate} when $\mathbf{Z}$ replaces the true unobserved variable $\mathbf{U}$ in Equation \ref{eq:acate_identif_U}, summarized in the following corollary:

\begin{corollary}[Identifiability of \gls{acate} with $\mathbf{Z}$]
\label{corollary:acate_identif_U}
Let $\mathbf{Z}$ be a latent variable satisfying CMM($p$). The Augmented CATE, when augmented with $\mathbf{Z}$ instead of $\mathbf{U}$ as defined in \eqref{eq:acate_identif_U}, is identifiable. Specifically:
 \begin{equation}
 \tau_{t}(\mathbf{h}_{t}, \mathbf{z}) = \mathbb{E}(Y_{t}| \mathbf{H}_t = \mathbf{h}_t, \mathbf{Z}= \mathbf{z}, W_{t} = 1) - \mathbb{E}(Y_{t}| \mathbf{H}_t = \mathbf{h}_t, \mathbf{Z}= \mathbf{z}, W_{t} = 0) 
 \end{equation}
\end{corollary}

As a result, Corollary \ref{corollary:acate_identif_U} addresses the identifiability problem and its conditions as raised in Section \ref{sect_cdvae:problem_def}: A \gls{cmm} of arbitrary order over the conditional distribution of responses, along with a mild regularity condition on the response domain as stated in Theorem \ref{thm:seq_ign_augmented}, constitutes a sufficient condition to ensure the identifiability of the \gls{acate}. To further emphasize the relevance of \(\mathbf{Z} \sim CMM(p)\), we show that any two substitutes satisfying \(CMM(p)\) must necessarily be related through a measurable map given the entire process history \(\mathbf{H}_T\):

\begin{theoremBox}
\label{thm:valid_Z}
Let \(\mathbf{Z}\) be a latent variable such that \(\mathbf{Z} \sim CMM(p)\), and assume the domain \(\mathcal{Y}\) is a Borel subset of a compact interval. Then, any static adjustment variable that influences the entire series of responses in the panel must be measurable with respect to \((\mathbf{Z}, \mathbf{H}_T)\).
\end{theoremBox}

\begin{figure}[h!]
    \centering
    \includegraphics[width=0.6\linewidth]{figures/cdvae/proof_sketch_valid_Z.pdf}
    \caption{A simplified causal graph for the sketch of the proof for Theorem \ref{thm:valid_Z}. We do not represent $W_{\leq t}, \mathbf{X}_{\leq t}$ for simplicity.}
    \label{fig:cg_proof_meas}
\end{figure}

\textbf{Intuition behind \(\mathrm{CMM}(p)\).} We provide an intuition behind the \(\mathrm{CMM}(p)\) assumption by sketching a proof of Theorem~\ref{thm:valid_Z} using d-separation properties, assuming the data generation process follows the graph depicted in Figure~\ref{fig:cg_proof_meas}. Let \(\mathbf{Z}'\) be an unobserved risk variable independent of \(\mathbf{Z}\), as illustrated in Figure~\ref{fig:cg_proof_meas}. Given that \(\mathbf{Z} \sim \mathrm{CMM}(p)\) and for \(m > p\), \(Y_t\) and \(Y_{t-m}\) are d-separated given
\[
\bigl\{Y_{t-1:t-m+1}, \mathbf{Z}, W_{\leq t}, \mathbf{X}_{\leq t}\bigr\},
\]
implying
\[
Y_t \indep Y_{t-m} \mid Y_{t-1:t-m+1},\, \mathbf{Z},\, W_{\leq t},\, \mathbf{X}_{\leq t}.
\]
Now, suppose \(\mathbf{Z}'\) influences the entire series of responses similarly to \(\mathbf{Z}\). In this case, \(\mathbf{Z}'\) acts as a common parent for both \(Y_t\) and \(Y_{t-m}\), creating a path
\[
Y_{t-m} \leftarrow \mathbf{Z}' \rightarrow Y_t
\]
that cannot be blocked by conditioning on
\[
\bigl\{Y_{t-1:t-m+1}, \mathbf{Z}, W_{\leq t}, \mathbf{X}_{\leq t}\bigr\}.
\]
Consequently,
\[
Y_t \notindep Y_{t-m} \mid Y_{t-1:t-m+1},\, \mathbf{Z},\, W_{\leq t},\, \mathbf{X}_{\leq t},
\]
which contradicts the implications of the conditional Markov assumption.

\subsection{Definition of the probabilistic model}
\label{subsect_cdvae:def_cdvae_model}
We define in the section the probabilistic model to learn a substitute \(\mathbf{Z}\), building on the DVAE approach. We break down the approach into three steps, where we first deal with selection bias (Step 1), then we incorporate the inductive bias of population structure and define a GMM over the substitutes (Step 2).  Finally, we define the suitable \gls{elbo} to be maximized (Step 3).  

\label{step:def_cdvae_model_1}
\paragraph{Step 1: Handling Selection Bias} In a purely factual setting, modeling data with a DVAE involves maximizing:
\vspace{-5pt} 
\[
\begin{aligned}
\log p_{\theta}\bigl(y_{\leq T} \mid \mathbf{x}_{\leq T}, \omega_{\leq T}\bigr)
&= \sum_{t=1}^{T} \log p_{\theta}\bigl(y_t \mid y_{<t}, \mathbf{x}_{\leq t}, \omega_{\leq t}\bigr) \\[1.2ex]
&= \sum_{t=1}^{T} \log p_{\theta}\bigl(y_t \mid \mathbf{h}_t, \omega_t\bigr).
\end{aligned}
\]
based on the observed data distribution. However, this model cannot perform counterfactual regression—switching treatment assignment during inference to estimate counterfactual responses—nor does it allow for causal inference. This limitation arises in observational studies where treatment assignment is typically non-random and depends on observed covariates, resulting in a selection bias. We adopt the importance sampling strategy to reduce the selection bias by reweighing the likelihood of the factual model \citep{shimodaira2000WeightedLL}. The key idea is to assign weights $\{\alpha(\mathbf{h}_{t}, \omega_t)\}_{t=1}^{T}$ to units in the population such that the resulting distribution in a given treatment regime matches that of the entire population. Therefore, we seek to maximize the likelihood \(L\) defined as
\[
L \coloneqq \sum_{t=1}^{T} \mathbb{E}_{\mathbf{H}_t, W_t} \biggl[
    \alpha(\mathbf{H}_t, W_t)\,
    \mathbb{E}_{Y_t \mid \mathbf{H}_t, W_t}\bigl(
        \log p_{\theta}(y_t \mid \mathbf{H}_t, W_t)
    \bigr)
\biggr].
\]

A more convenient formulation expresses \(L\) as an expectation over all individual-level panel series
\[
\mathcal{D}_T \coloneqq \{Y_{\leq T}, \mathbf{X}_{\leq T}, W_{\leq T}\}
= \mathbf{H}_T \cup \{Y_T, W_T\}:
\]
\begin{equation}
\label{eq:weighted_ll}
L = \sum_{t=1}^{T} \mathbb{E}_{\mathcal{D}_T} \biggl[
    \alpha(\mathbf{H}_t, W_t)\,
    \log p_{\theta}\bigl(Y_t \mid \mathbf{H}_t, W_t\bigr)
\biggr].
\end{equation}

We define a \emph{conditional} DVAE model by specifying the conditional generative model \(p_{\theta}(y_{\leq T}, \mathbf{z} \mid \mathbf{x}_{\leq T}, \omega_{\leq T})\), which is decomposed as follows:
\[
p_{\theta}(y_{\leq T}, \mathbf{z} \mid \mathbf{x}_{\leq T}, \omega_{\leq T})
= \prod_{t=1}^{T} p_{\theta}\bigl(y_t \mid y_{<t}, \mathbf{x}_{\leq t}, \omega_{\leq t}, \mathbf{z}\bigr)\, p(\mathbf{z}).
\]

\label{step:def_cdvae_model_2}
\paragraph{Step 2: Incorporating Population Structure} 
To account for an eventual population structure induced by unobserved adjustment variables, we place a Gaussian mixture prior over the latent variable \(\mathbf{Z}\), with \(K\) components:
\begin{equation} 
\label{eq:prior_Z_gmm}
p(\mathbf{z}) = \sum_{c=1}^{K} \pi_{c} \mathcal{N}(\mathbf{z}|\mu_c, \Sigma_c).
\end{equation}
This prior corresponds to first generating a cluster index \(C \sim \mathrm{Cat}(\boldsymbol{\pi})\), followed by \(\mathbf{Z} \mid C \sim \mathcal{N}(\mu_C, \Sigma_C)\). Here, \(\boldsymbol{\pi}\) represents the probability distribution over cluster assignments, satisfying
\[
\sum_{c=1}^K \boldsymbol{\pi}_c = 1,
\]
with \(\mathrm{Cat}(\boldsymbol{\pi})\) denoting the categorical distribution parameterized by \(\boldsymbol{\pi}\).Each cluster \(c\) is associated with a learnable Gaussian distribution of mean \(\mu_c\) and covariance \(\Sigma_c\). The complete generative model becomes
\begin{equation}
\label{eq:gen_model_complete}
p_{\theta}\bigl(y_{\leq T}, \mathbf{z}, c \mid \mathbf{x}_{\leq T}, \omega_{\leq T}\bigr)
= \prod_{t=1}^{T} p_{\theta}\bigl(y_t \mid y_{<t}, \mathbf{x}_{\leq t}, \omega_{\leq t}, \mathbf{z}\bigr)\, p(\mathbf{z} \mid c)\, p(c).
\end{equation}

We approximate the true posterior over \((\mathbf{z}, c)\) using a factorized variational distribution
\begin{equation}
\label{eq:approx_posterior_facto}
q_{\phi}(\mathbf{z}, c \mid \mathcal{D}_T)
= q_{\phi_z}\bigl(\mathbf{z} \mid \mathcal{D}_T\bigr)\,
  q_{\phi_c}\bigl(c \mid \mathcal{D}_T\bigr),
\end{equation}
where \(\phi = \phi_z \cup \phi_c\) collects the variational parameters. The following theorem characterizes the corresponding variational bound.
\begin{theoremBox}[Weighted ELBO Decomposition]
\label{thm:elbo_def}
Under the generative model defined by Equation \ref{eq:gen_model_complete} and the approximate posterior factorization of Equation \ref{eq:approx_posterior_facto}, the weighted likelihood in Equation \ref{eq:weighted_ll} can be decomposed as:
\begin{equation}
L = \mathbb{E}_{\mathcal{D}_T} \left[ \mathrm{ELBO_0}(\mathcal{D}_T; \theta, \phi) \right] + \mathbb{E}_{\mathcal{D}_T}\left[\Delta_0(\mathcal{D}_T; \theta, \phi)\right],
\end{equation}
where the individual gap term \(\Delta_0\) is given by:
\begin{equation}
\label{eq:indiv_gap}
    \Delta_0(\mathcal{D}_T; \theta, \phi) \coloneqq \sum_{t = 1}^{T} \alpha(\mathbf{h}_t, \omega_t) D_{KL}(q_{\phi}(\mathbf{z}, c \mid \mathcal{D}_T) \parallel p_{\theta}(\mathbf{z}, c \mid \mathcal{D}_T)),
\end{equation}
and the individual ELBO termed \(\mathrm{ELBO_0}\) is expressed as:
\begin{align}
\mathrm{ELBO_0}(\mathcal{D}_T; \theta, \phi) &=  \sum_{t = 1}^{T} \mathbb{E}_{\mathbf{Z} \sim q_{\phi_z}(\cdot \mid \mathcal{D}_T)} \left[ \alpha(\mathbf{h}_t, \omega_t) \log p_{\theta}(y_{t} \mid \mathbf{h}_t, \omega_t, \mathbf{Z}) \right] \label{eq:elbo_orig}\\
&- \left( \sum_{t = 1}^{T} \alpha(\mathbf{h}_t, \omega_t) \right) \left\{ D_{KL}(q_{\phi_z}(\mathbf{z} \mid \mathcal{D}_T) \parallel p(\mathbf{z}))  + \mathbb{E}_{\mathbf{Z} \sim q_{\phi_z}(\cdot \mid \mathcal{D}_T)} D_{KL}(q_{\phi_c}(c \mid \mathcal{D}_T) \parallel p(c \mid \mathbf{Z}) ) \right\}. \notag 
\end{align}
\end{theoremBox}

The individual gap \(\Delta_0\) is a positive term that quantifies the inaccuracy of the variational approximation of \( L \) using \(\mathrm{ELBO_0}\) Equation \ref{eq:elbo_orig}. The ELBO term, $\mathrm{ELBO}_0$, comprises three components:  \begin{inparaenum}[(1)]
\item A weighted sum of the conditional log-likelihoods of the responses (reconstruction term).  
\item A \gls{kl} divergence between the approximate posterior of the continuous latent variables \( q_{\phi_z}(\cdot \mid \mathcal{D}_T) \), which serve as substitutes for adjustment variables, and the prior \(p(\mathbf{z})\).  
\item A \gls{kl} divergence between the approximate posterior of the discrete latent \( q_{\phi_c}(\cdot \mid \mathcal{D}_T) \) and the true conditional posterior \(p(\mathbf{C} \mid \mathbf{Z} )\), averaged over \( q_{\phi_z}(\cdot \mid \mathcal{D}_T) \).  
\end{inparaenum} 
The decoupling of these two approximate posteriors arises from the assumed factorization over the joint approximate posterior as in Equation \ref{eq:approx_posterior_facto}.

\begin{remark}
In a DVAE, the inference model \(q_\phi\bigl(\mathbf{z} \mid \mathcal{D}_T\bigr)\) approximates the true posterior \(p_\theta\bigl(\mathbf{z} \mid \mathcal{D}_T\bigr)\). Although this structure is not always followed in applications \citep{Bayer2014STORN, krishnan2015DKF, Li2018DisentangledSA, han2021disentangledRecWass, bai2021cContrastDisentSeq}, it is preferable that the approximate posterior mirrors the true one when simplified using d-separation. However, the true posterior cannot be simplified due to the data’s generation process and dynamics. For instance, omitting conditioning on the entire sequence of treatments and covariates is invalid since \(\{\mathbf{Z}\}\) and \(\{\mathbf{X}_{\leq T}, W_{\leq T}\}\) are not d-separated given \(\{Y_{\leq T}\}\). For example, in the chain
\[
W_{t-1} \rightarrow Y_t \leftarrow \mathbf{Z},
\]
\(Y_t\) acts as a collider and belongs to \(\{Y_{\leq T}\}\).
\end{remark}

\label{step:def_cdvae_model_3}
\paragraph{Step 3: Addressing the Discrete Latent Variable \(C\)}  
The approximate posterior \(q_{\phi}(\mathbf{z}, c \mid \mathcal{D}_T)\) involves both continuous and discrete latent variables, \(\mathbf{z}\) and \(c\), respectively. Training deep generative models with discrete latent variables presents challenges due to difficulties in reparameterization and handling high cardinality, even when using classical approaches like Gumbel-Softmax \citep{jang2016categorical, tucker2017rebar, huijben2022review}. To avoid designing an additional inference network for \(q_{\phi_c}(c \mid \mathcal{D}_T)\) and the associated computational cost, we follow \citet{Vade, falck2021multi} and define a \emph{Bayes-optimal posterior} for the discrete latent variable. Specifically, we leverage the decomposition of Equation \ref{eq:approx_posterior_facto} and choose \(q_{\phi_c}(c \mid \mathcal{D}_T)\) in such a way that the third term in the ELBO of Equation \ref{eq:elbo_orig} is minimized by definition:
\begin{equation}
\label{eq:opt_problem_VaDE}
\min_{q_{\phi_c}(\cdot \mid \mathcal{D}_T)} \mathbb{E}_{\mathbf{Z} \sim q_{\phi_z}(\cdot \mid \mathcal{D}_T)} D_{KL}(q_{\phi_c}(c \mid \mathcal{D}_T) \parallel p(c \mid \mathbf{Z})).
\end{equation}
The minimal value of this optimization problem is
\begin{equation}
    \min_{q_{\phi_c}(\cdot \mid \mathcal{D}_T)} \mathbb{E}_{\mathbf{Z} \sim q_{\phi_z}(\cdot \mid \mathcal{D}_T)} D_{KL}(q_{\phi_c}(\cdot \mid \mathcal{D}_T) \parallel p(\cdot \mid \mathbf{Z})) = -\log \mathrm{Const}(q_{\phi_z}(\cdot \mid \mathcal{D}_T)), 
\end{equation}
where \(\mathrm{Const}(q_{\phi_z}(\cdot \mid \mathcal{D}_T))\) is a constant that depends only on the approximate posterior over the continuous latents:
\[
\mathrm{Const}(q_{\phi_z}(\cdot \mid \mathcal{D}_T)) = \sum_{c=1}^K \exp(\mathbb{E}_{\mathbf{Z} \sim q_{\phi_z}(\cdot \mid \mathcal{D}_T)} \log p(c \mid \mathbf{Z})).
\]
The minimizer is given by:
\begin{equation}
\label{eq:bayes_opt_posterior}
    \mathbf{\pi}(c \mid q_{\phi_z}(\cdot \mid \mathcal{D}_T)) = \frac{\exp(\mathbb{E}_{\mathbf{Z} \sim q_{\phi_z}(\cdot \mid \mathcal{D}_T)} \log p(c \mid \mathbf{Z}))}{\mathrm{Const}(q_{\phi_z}(\cdot \mid \mathcal{D}_T))}.
\end{equation}
Moreover, the minimal value is:
\begin{equation}
\label{eq:min_VaDE_trick}
    \min_{q_{\phi_c}(\cdot \mid \mathcal{D}_T)} \mathbb{E}_{\mathbf{Z} \sim q_{\phi_z}(\cdot \mid \mathcal{D}_T)} D_{KL}(q_{\phi_c}(\cdot \mid \mathcal{D}_T) \parallel p(c \mid \mathbf{Z})) = -\log Z(q_{\phi_z}(\cdot \mid \mathcal{D}_T)).
\end{equation}
Thus, we update the original \(\mathrm{ELBO}_0\) in Equation \ref{eq:elbo_orig} to obtain a \emph{modified} ELBO by replacing \(q_{\phi_c}(\cdot \mid \mathcal{D}_T)\) with the minimizer \(\mathbf{\pi}(c \mid q_{\phi_z}(\cdot \mid \mathcal{D}_T))\) and plugging in the minimal value from Equation \ref{eq:min_VaDE_trick}:
\begin{equation}
\label{eq:welbo_def}
\begin{split}
\mathrm{ELBO}(\mathcal{D}_T; \theta, \phi) &=  \sum_{t = 1}^{T} \mathbb{E}_{\mathbf{Z} \sim q_{\phi_z}(\cdot \mid \mathcal{D}_T)} 
\left[ \alpha(\mathbf{h}_t, \omega_t) \log p_{\theta}(y_{t} \mid \mathbf{H}_t, W_t, \mathbf{Z}) \right] \\
&- \left[\sum_{t = 1}^{T}\alpha(\mathbf{h}_t, \omega_t)\right] \left\{D_{KL}(q_{\phi_z}(\cdot \mid \mathcal{D}_T) \parallel p(\mathbf{z})) - \log Z(q_{\phi_z}(\cdot \mid \mathcal{D}_T))\right\}.
\end{split}
\end{equation}

As a result, the modified ELBO is computationally more efficient than the original one, as it bypasses the need for applying a reparameterization trick to discrete latent variables and eliminates the necessity of training over specific parameters \(\phi_c\), all while remaining a valid lower bound for the weighted likelihood \(L\). This validity holds since Theorem \ref{thm:elbo_def} applies to any arbitrary approximate posterior \(q_{\phi_c}(\cdot \mid \mathcal{D}_T)\), and in particular, to \(\mathbf{\pi}(c \mid q_{\phi_z}(\cdot \mid \mathcal{D}_T))\), which is the minimizer of Equation \ref{eq:opt_problem_VaDE}. We henceforth use \(\phi\) to denote \(\phi_z\). 


\subsection[CDVAE in the near deterministic regime]{\gls{cdvae} in the near deterministic regime}
\label{sect_cdvae:cdvae_near_det}
In this section, we explore the behavior of Causal DVAE in the \emph{near-deterministic regime}, where the variance of the generative model approaches zero. We examine how this regime affects inference and causal identifiability, demonstrating that it leads to a non-diffuse posterior suitable for treatment effect estimation. 

\paragraph{Model Setup}  For the remainder of our discussion, we define the DVAE model parameters as $\mathcal{M}_{vae} = \{\theta, \phi\}$ and assume the approximate posterior to be Gaussian \(q_{\phi}(\mathbf{z} \mid \mathcal{D}_T) \sim \mathcal{N}(\mathbf{z}|\mu_{\mathbf{z}}, \Sigma_{\mathbf{z}})\), where the mean is defined as $\mu_{\mathbf{z}}= f_{\mu_{\mathbf{z}}}(\mathcal{D}_T; \phi)$, and the covariance matrix is given by $\Sigma_{\mathbf{z}} = S_{\mathbf{z}}S_{\mathbf{z}}^\top$, with $S_{\mathbf{z}} = f_{S_{\mathbf{z}}}(\mathcal{D}_T; \phi)$. Moreover, we assume the conditional generative model to be Gaussian such that:
\begin{equation}
\label{eq:proba_yt_gaussian}
p_{\theta}(y_{t} \mid y_{<t}, \mathbf{x}_{\leq t}, \omega_{\leq t}, \mathbf{z}) = \mathcal{N}(f_t(\mathbf{h}_{t}, \omega_t, \mathbf{z}; \theta), \sigma^2),
\end{equation}
with $\sigma > 0$, a spatially and temporally uniform scale parameter.

\paragraph{Motivation} In probabilistic modeling, our inference model for the substitute adjustment variable is \emph{stochastic}. However, to calculate \gls{ite} for each individual, we need to choose a unique instance of the latent variable representation. Otherwise, infinite \gls{ite} could be generated by sampling repeatedly from \(q_{\phi_z}(\cdot \mid \mathcal{D}_T)\). A natural choice for this deterministic representation is the \emph{mean} of the posterior. Yet, because we sample from the approximate posterior during training rather than using the mean, it is essential to prevent the posterior from becoming \emph{overly diffuse} (i.e. it has high variance with no sharp peak)—ensuring that the mean remains valid during causal inference. Previous studies \citep{dai2018diagnosingvae, takida2022preventingoversmoothing} show that operating in the \emph{near-deterministic regime} of the VAE decoder—where $\sigma \to 0^+$—leads the encoder’s covariance matrix toward zero, resulting in near-deterministic behavior. We, therefore, explore the near-deterministic regime in our Causal DVAE by controlling the decoder’s variance to induce a non-diffuse, stable posterior distribution suitable for causal inference in the latent space.

\paragraph{Side Benefit: Preventing Posterior Collapse}
A well-known challenge in training VAEs is \emph{posterior collapse}, where the approximate posterior converges to the uninformative prior, making the latent space irrelevant \citep{bowman2015generating, sonderby2016ladder, higgins2017betavae, dai2018diagnosingvae, fu2019cyclical, lucas2019dontblameElbo, wang2021PosteriorNonIdentif, takida2022preventingoversmoothing}. A notable advantage of the near-deterministic regime is its ability to \emph{avoid posterior collapse} within the latent space, a benefit demonstrated in \emph{static VAEs} \citep{lucas2019dontblameElbo, takida2022preventingoversmoothing}. Specifically, \cite{takida2022preventingoversmoothing} showed that the decoder’s output variance and covariance could influence the latent space by causing over-smoothing by affecting the gradient regularization strength, which in turn leads to posterior collapse. By controlling variance in the near-deterministic regime, we mitigate this collapse and preserve meaningful latent representations.

We advance the study of \emph{dynamic} VAE models by investigating their behavior in the near-deterministic regime within the context of causal inference. This work is the first to explore dynamic VAEs in this regime for causal applications, addressing a gap in the literature, as such behavior has yet to be thoroughly examined, even in non-causal, factual settings.

We prove that in our framework, replacing the original lower bound $\mathrm{ELBO_0}(\mathcal{D}_T; \theta, \phi)$ with the modified $\mathrm{ELBO}(\mathcal{D}_T; \theta, \phi)$ still ensures the existence of a parameterization under which the approximate likelihood of responses converges to the true likelihood. Specifically, Theorem \ref{thm:vaes_to_truell} demonstrates that, for a sequence of inference and generative models parameterized by \(\sigma\), the gap between the modified and true importance-weighted likelihoods asymptotically approaches zero.  

\begin{theoremBox}[Asymptotic Likelihood Recovery]
\label{thm:vaes_to_truell}
Suppose $d_{\mathbf{z}} \leq T$. There exists a family of autoencoders $\{\phi_{\sigma}, \theta_{\sigma}\}_{\sigma > 0}$ such that 
\[
\lim_{\sigma \to 0^+} p_{\theta_{\sigma}}(y_{\leq T} \mid \mathbf{x}_{\leq T}, \omega_{\leq T}) = p(y_{\leq T} \mid \mathbf{x}_{\leq T}, \omega_{\leq T}),
\]
and when operating under the Bayes-optimal posterior over the discrete latent, i.e.,  
\[
q_{\phi}(c \mid \mathcal{D}_T) = \pi(c \mid q_{\phi}(\cdot \mid \mathcal{D}_T)),
\]  
the gap \(\Delta(\mathcal{D}_T; \theta_{\sigma}, \phi_{\sigma})\) between the modified ELBO (Equation \ref{eq:welbo_def}) and the true weighted likelihood \(L\) (Equation (\ref{eq:weighted_ll})) satisfies  
\[
\Delta(\mathcal{D}_T; \theta_{\sigma}, \phi_{\sigma}) = \mathrm{ELBO}(\mathcal{D}_T; \theta_{\sigma}, \phi_{\sigma}) - L(\mathcal{D}_T; \theta_{\sigma}),
\]
and converges to zero:  
\[
\lim_{\sigma \to 0^+}  \Delta(\mathcal{D}_T; \theta_{\sigma}, \phi_{\sigma}) = 0.
\]
\end{theoremBox}
This result generalizes prior findings for static VAEs \citep{dai2018diagnosingvae} to the more complex dynamic setting with GMM priors and weighted objectives. It also addresses an oversight in \cite{dai2018diagnosingvae} regarding the proof of gap convergence. 

More importantly, we establish a critical property in our setting within the near-deterministic regime: the causal effect remains asymptotically consistent whether one uses an arbitrary realization of the latent variable \(\mathbf{z}\) or the posterior mean \(\mu_{\mathbf{z}}\). Theorem \ref{thm:sigma_to_0} formalizes this insight as follows:
\begin{theoremBox}[Realization-Invariant Causal Consistency]
\label{thm:sigma_to_0}
For a fixed $\sigma > 0$, let a parametrization of Causal DVAE \(\mathcal{M}_{vae}^*(\sigma) = \{\theta_{\sigma}^*, \phi_{\sigma}^*\}\) be an optimal solution to the ELBO defined in Equation \ref{eq:welbo_def}. Then, \underline{for any} substitute realization \(\mathbf{z} \in \mathbb{R}^{d_z}\), the conditional expected outcome satisfies the following consistency in the near-deterministic regime:
\begin{equation}
    \lim_{\sigma \to 0^+} \mathbb{E}_{\mathcal{M}_{vae}^*(\sigma)}\left[ Y_t \mid \mathbf{H}_{t}, W_t = \omega, \mathbf{Z}= \mathbf{z} \right] 
    = \lim_{\sigma \to 0^+} \mathbb{E}_{\mathcal{M}_{vae}^*(\sigma)}\left[ Y_t \mid \mathbf{H}_{t}, W_t = \omega, \mathbf{Z}= \mu_{\mathbf{z}} \right].
\end{equation}
As a result of Corollary \ref{corollary:acate_identif_U}, the Augmented \gls{cate} satisfies the same consistency in the near-deterministic regime:
\begin{equation}
    \lim_{\sigma \to 0^+} \tau_{\mathcal{M}_{vae}^*(\sigma)}(\mathbf{H}_{t}, \mathbf{z}) 
    = \lim_{\sigma \to 0^+} \tau_{\mathcal{M}_{vae}^*(\sigma)}(\mathbf{H}_{t}, \mu_{\mathbf{z}}).
\end{equation}
\end{theoremBox}
Theorem \ref{thm:sigma_to_0} demonstrates that as the variance parameter \(\sigma\) of the generative model approaches zero, both the expected outcome and the estimated causal effect remain consistent, regardless of whether one relies on an arbitrary realization of the latent variable \(\mathbf{z}\) or its posterior mean \(\mu_{\mathbf{z}}\). Such consistency ensures that, in the near-deterministic regime, the causal effect is robust to the specific realization of the latent variable. 

\section{Generalization Bound over Treatment Effect Estimation and Derivation of Model Loss}
\label{sect_cdvae:gen_bound_tot_loss}
We establish in this section a theoretical generalization bound for the error in estimating \gls{acate}, which serves as a foundation for deriving the training loss of \gls{cdvae}. We begin by defining a suitable representation function to address the high dimensionality of the history \(\mathbf{H}_t\). Next, we introduce a weighted risk minimization framework that ensures a covariates' balance between treatment groups. We then derive a generalization bound for treatment effect estimation, relating the error in estimating \gls{acate} to the model’s weighted risk. Finally, we construct the \gls{cdvae} training objective by integrating these theoretical insights into a structured loss function.

\paragraph{Step 1: Representation Learning} In causal inference with high-dimensional covariates, increasing the number of covariates makes it challenging to satisfy the overlap assumption, as ensuring that all units have a non-zero probability of receiving each treatment becomes harder. This "curse of dimensionality" leads to greater imbalance between treated and control groups. While including more covariates can reduce bias from unobserved confounders, it may increase bias due to poor overlap, compromising the reliability of causal effect estimations. Additionally, high-dimensional models make causal effect estimation more prone to increased variance \citep{ning2020robustHD,d2021overlapHD}. To address these challenges and given the high-dimensional nature of the context history $\mathbf{H}_t$, we introduce a representation function $\Phi$ that reduces dimensionality while retaining essential information in a latent space, allowing causal inference in a lower-dimensional setting, mitigating issues associated with high dimensionality.

We assume $\Phi$ is invertible to prevent information loss in the latent space. In fact, if we formulate our sequential ignorability assumptions over the original space, then there is no guarantee the same assumptions should hold in the representation space for any general function $\Phi$. It is possible to lose information related to confounders after the transformation $\Phi$, so ignorability cannot hold anymore. As a result, the treatment effect becomes unidentifiable. To this end, we need to ensure identifiability assumptions over the latent space, namely sequential ignorability and overlap, i.e.:
\begin{equation*}
    Y_{t}(\omega) \indep  W_{t}| \Phi(\mathbf{H}_{t}), \quad p(W_t=\omega|\Phi(\mathbf{h}_{t}))>0 \quad, \forall (\omega,\mathbf{h}_{t}).
\end{equation*}
\begin{remark}
\label{remark:from_ft_to_f_Phi}
Following Eq. (\ref{eq:proba_yt_gaussian}), the generative model for the responses is defined as \(Y_t = f_t(\mathbf{H}_t, W_t, \mathbf{Z}) + \epsilon_t \), where \( \epsilon_t \sim \mathcal{N}(0, \sigma^2) \) is the error term. A common modeling \citep{johansson2016learning, shalit2017estimating, shi2019Dragonnet, johansson2022generalization} approach for \( f_t \) is to assume  
\[
f_t(\mathbf{H}_t, W_t, \mathbf{Z}) \coloneqq W_t f_{t,1}(\mathbf{H}_t, \mathbf{Z}) + (1 - W_t) f_{t,0}(\mathbf{H}_t, \mathbf{Z}),
\]  
where \( f_{t,0} \) and \( f_{t,1} \) denote the mappings to the response under each treatment regime \( W_t \in \{0,1\} \).  

The representation function \( \Phi \) over \( \{\mathbf{H}_t\}_{t=1}^{T} \) produces lower-dimensional vectors \( \{\mathbf{r}_t\}_{t=1}^{T} \), living in a space \( \mathcal{R} \subset \mathbb{R}^r \). Instead of defining \underline{time-dependent} generative functions \( f_t \), we define a single hypothesis function  
\[
f: \mathcal{R} \times \mathcal{W} \times \mathbb{R}^{d_{\mathbf{z}}} \rightarrow \mathcal{Y},
\]  
such that:  
\[
 Y_t = f(\Phi(\mathbf{H}_t), W_t, \mathbf{Z}) + \epsilon_t = W_t f_{1}(\Phi(\mathbf{H}_t), \mathbf{Z}) + (1-W_t) f_{0}(\Phi(\mathbf{H}_t), \mathbf{Z}) + \epsilon_t.
\]
\end{remark}

By assuming the invertibility of $\Phi$, we can show that such conditions hold in the latent space if they hold in the original space. We summarize the result in the following proposition:
\begin{proposition}
Let $\Phi$ be a representation function according to Remark \ref{remark:from_ft_to_f_Phi}.  then $Y_{t}(\omega) \indep  W_{t}| \Phi(\mathbf{H}_{t})$ holds if and only if $Y_{t}(\omega) \indep  W_{t}| \mathbf{H}_{t}$. Moreover,  $p(W_t=\omega|\Phi(\mathbf{h}_{t}))>0$ holds if and only if $p(W_t=\omega|\mathbf{h}_{t})>0$.
\end{proposition}

In practice and for the remainder of the work, the outcome and propensity models share the same representation $\Phi(\mathbf{H}_t)$, encouraging it to capture information predictive of both treatment and response. While invertibility is theoretically assumed to maintain identifiability, implementation does not enforce it. Instead, the focus is on ensuring that $\Phi(\mathbf{H}_t)$ is predictive across treatment regimes, with regularization used to balance $\Phi(\mathbf{H}_t)$ across the two treatment regimes \( W_t \in \{0,1\} \) using the Wasserstein distance \citep{gretton2012kernel}, similar to \cite{shalit2017estimating, lim2018RMSN, bica2020estimatingCRN, assaad2021counterfactual, Melnychuk2022CausalTF, johansson2022generalization}.

\paragraph{Step 2: Weighted Risk Minimization} 
To integrate causal inference into the DVAE framework, we employ weighted risk minimization techniques \citep{kallus2020deepmatch, johansson2022generalization}. First, we justify the choice of weights \(\alpha(\mathbf{H}_t, W_t)\) used in the definition of the weighted ELBO in Section~\ref{subsect_cdvae:def_cdvae_model}. In general, these weights can be any arbitrary mapping
\[
\alpha: \mathbf{H}_t \times \mathcal{W} \to \mathbb{R}^+
\]
such that
\[
\mathbb{E}_{\mathbf{H}_t \mid W_t = \omega}\bigl[\alpha(\mathbf{H}_t, \omega)\bigr] = 1
\quad \text{for all} \quad \omega \in \mathcal{W},
\]
meaning the weights \(\alpha(\mathbf{h}_t, \omega)\) induce a weighted probability \emph{target distribution} \(g\) over the population such that
\[
g(\mathbf{h}_t \mid W_t = \omega)
\coloneqq \alpha(\mathbf{h}_t, \omega)\, p(\mathbf{h}_t \mid W_t = \omega).
\]
Intuitively, the weights either \emph{stretch} or \emph{shrink} each observed unit so that learning occurs on a \emph{new synthetic population} whose covariates follow the distribution \(g\). Choosing an appropriate weighting strategy \(\alpha(\mathbf{h}_t, \omega)\) is crucial for achieving covariate balance between treatment groups, i.e.,
\[
g(\mathbf{h}_t \mid W_t = 1) = g(\mathbf{h}_t \mid W_t = 0).
\]

We use \emph{overlap weights} \cite{li2018balancing, assaad2021counterfactual}, defined as
\[
\alpha(\mathbf{h}_t, \omega)
\propto
\frac{
    e\bigl(\Phi(\mathbf{h}_t)\bigr)\,\bigl(1 - e\bigl(\Phi(\mathbf{h}_t)\bigr)\bigr)
}{
    \omega\, e\bigl(\Phi(\mathbf{h}_t)\bigr)
    + (1 - \omega)\,\bigl(1 - e\bigl(\Phi(\mathbf{h}_t)\bigr)\bigr)
},
\]
where \(e(\Phi(\mathbf{h}_t)) = p(W_t = 1 \mid \Phi(\mathbf{h}_t))\) is the propensity score in the representation space.

Overlap weights emphasize units with propensity scores near \(0.5\), focusing on regions where treated and control groups overlap most, which enhances comparability and improves covariate balance. This approach reduces variance by down-weighting units with extreme propensity scores, mitigating instability from excessively large weights, and leading to more reliable and efficient causal effect estimates \citep{li2018balancing}.

We now define the \emph{weighted population risk} for a given treatment regime \( W_t = \omega \) : we measure the expected risk for a given \( (f, \Phi) \) at time \( t \) over the weighted population distributed according to \( g \), as:
\[    
R_{t, g}^{\omega}(f, \Phi) \coloneqq \mathbb{E}_{\mathbf{H}_t \mid W_t} \left[ \alpha(\mathbf{H}_t, W_t) \, \ell_{f, \Phi}(\mathbf{H}_t, W_t) \mid W_t = \omega \right],
\]
where \( \ell_{f, \Phi}(\mathbf{h}_t, \omega) \) is the expected pointwise loss which averages prediction error over the encoder’s posterior and potential outcomes:
\begin{equation}
\label{eq:expected_pt_loss}
\ell_{f, \Phi}(\mathbf{h}_t, \omega) \coloneqq \mathbb{E}_{\mathbf{Z} \sim q_{\phi}(\mathbf{Z} \mid \mathcal{D}_{\leq t-1})} \, \mathbb{E}_{Y_t(\omega) \mid \mathbf{H}_t, \mathbf{Z}} \left[ L\left( Y_t(\omega), f\left( \Phi(\mathbf{H}_t), \mathbf{Z}, W_t \right) \right) \mid  \mathbf{H}_t=\mathbf{h}_t, \mathbf{Z} \right].
\end{equation}

In the definition of the expected pointwise loss, we respect the temporal order by conditioning the approximate posterior of the continuous latents only on the longitudinal data up to time step \( t \). In line with our probabilistic modeling in Section \ref{subsect_cdvae:def_cdvae_model} and the distributional assumptions in Section \ref{sect_cdvae:cdvae_near_det}, we define the loss as the negative log-likelihood:
\[
L\left( Y_t(\omega), f\left( \Phi(\mathbf{H}_t), \mathbf{Z}, W_t \right) \right) = -\log \mathcal{N}\left(Y_t(\omega); f\left( \Phi(\mathbf{H}_t), \mathbf{Z}, W_t \right), \sigma^2\right).
\]

\paragraph{Step 3: Generalization Bound} Our aim during training is to minimize the factual quantities $\{R_{t, g}^{\omega}(f, \Phi)\}_{t=1}^{T}$ to reduce the error in estimating treatment effects. To formalize and theoretically justify this objective, we establish a generalization bound for the \gls{pehe} \citep{hill2011bayesian}, which accounts for our weighted population risks $\{R_{t, g}^{\omega}(f, \Phi)\}_{t=1}^{T}$. \gls{pehe} measures the mean squared error (MSE) between the true and estimated \gls{acate} at time $t$ as \footnote{Note that $p_{\theta}(\mathbf{H}_t, \mathbf{Z}) = p(\mathbf{Z} \mid \mathcal{D}_{\leq t-1}) \, p(\mathbf{H}_t)$ because $\mathbf{X}_t$ is d-separated from $\mathbf{Z}$ given $\mathcal{D}_{\leq t-1} = [Y_{\leq t-1}, \mathbf{X}_{\leq t-1}, W_{\leq t-1}]$.}
\[
\epsilon_{\mathrm{PEHE}_t}
= \mathbb{E}_{\mathbf{H}_t} 
  \mathbb{E}_{\mathbf{Z} \sim q_{\phi}\bigl(\mathbf{Z} \mid \mathcal{D}_{\leq t-1}\bigr)}
  \biggl[
    \bigl( \tau(\mathbf{H}_t, \mathbf{Z}) 
    - \hat{\tau}_{f, \Phi}(\mathbf{H}_t, \mathbf{Z}) \bigr)^2
  \biggr].
\]

where $\tau(\mathbf{H}_t, \mathbf{Z})$ is the true \gls{ite} and $\hat{\tau}_{f, \Phi}(\mathbf{H}_t, \mathbf{Z})$ is the estimated \gls{ite} using hypothesis $f$ and representation $\Phi$, as defined in the outcome model in Remark \ref{remark:from_ft_to_f_Phi}.

Similarly, we define the weighted \gls{pehe} with respect to the target distribution \( g \):
\[
\epsilon_{\text{PEHE}_{t, g}} =  \mathbb{E}_{\mathbf{H}_t \sim g}\mathbb{E}_{\mathbf{Z} \sim q_{\phi}(\mathbf{Z} \mid \mathcal{D}_{\leq t-1})} \left[ \left( \tau(\mathbf{H}_t, \mathbf{Z}) - \hat{\tau}_{f, \Phi}(\mathbf{H}_t, \mathbf{Z}) \right)^2 \right].
\]
We provide an upper bound for the weighted \gls{pehe} for \gls{cdvae} similar to \citet{assaad2021counterfactual}. This bound consists of three key components: the weighted factual prediction error, a term capturing the discrepancy between treatment and control distributions in the confounders representation space, and a term that accounts for the variance of the generative model over responses.

\begin{theoremBox}[Generalization Bound for Weighted \gls{pehe}]
\label{thm:pehe_wbound}
Let \(\mathcal{M}_{\mathrm{VAE}}(\sigma) = \{\theta_{\sigma}, \phi_{\sigma}\}\) be the VAE model defined in Section~\ref{subsect_cdvae:def_cdvae_model}. For a given class of functions \(G\), assume there exists a constant \(B_{\Phi}\) such that \(\ell_{f,\Phi} / B_{\Phi} \in G\). Assume the representation \(\Phi\) is invertible. Then, the error in estimating the treatment effect at time \(t\) for a weighted population is upper bounded by
\begin{equation}
\label{eq:bound_pehe}
\begin{aligned}
\epsilon_{\mathrm{PEHE}_{t, g}}
\leq\, &2\sigma^2 \biggl\{
    R^{\omega=1}_{t, g}\bigl(f, \Phi\bigr)
    + R^{\omega=0}_{t, g}\bigl(f, \Phi\bigr) \\[0.8ex]
    &\quad + B_{\Phi}\, \mathrm{IPM}_{G}\bigl(g_{\Phi}(\cdot \mid W_t=1),\, g_{\Phi}(\cdot \mid W_t=0)\bigr)
    - \log(2\pi\sigma^2)
\biggr\},
\end{aligned}
\end{equation}
where \(g_{\Phi}(r)\) is the distribution induced by \(\Phi\) in the representation space \(\mathcal{R}\). The \gls{ipm} \citep{muller1997IPM, sriperumbudur2009integral} measures the dissimilarity between distributions.

Assuming strict overlap in treatment assignment, where \( \delta \in (0, 0.5) \) such that \( \delta < e(\mathbf{h}_t) < 1 - \delta \), then there exists constants \(A_{t,g}, B_{t,g}\)  such that the unweighted \gls{pehe} \( \epsilon_{\mathrm{PEHE}_{t}} \) is bounded:
\[
A_{t,g} \cdot \epsilon_{\text{PEHE}_{t,g}}(\hat{\tau}) \leq \epsilon_{\text{PEHE}_{t}}(\hat{\tau}) \leq B_{t,g} \cdot \epsilon_{\text{PEHE}_{t,g}}(\hat{\tau}).
\label{eq:bound_pehe_strict_delta}
\]
\end{theoremBox}
The representation discrepancy in \ref{eq:bound_pehe} quantifies the distributional imbalance between treatment groups, measured using IPMs like the Wasserstein distance or Maximum Mean Discrepancy \citep{gretton2012kernel}. The connection between \( \epsilon_{\mathrm{PEHE}_{t}} \) and \( \epsilon_{\mathrm{PEHE}_{t,g}} \) indicates that minimizing the weighted \gls{pehe} can also minimize \( \epsilon_{\mathrm{PEHE}_{t}} \), thereby enhancing the reliability of \gls{ite} estimation across the original population.   

To justify the pertinence of our probabilistic model defined in Section \ref{subsect_cdvae:def_cdvae_model}, we show in the following how maximizing the likelihood term in the ELBO of Equation \ref{eq:welbo_def} implies minimization of the risks \( R^{\omega = 1}_{t, g}\left(f, \Phi \right) \) and \( R^{\omega = 0}_{t, g}\left(f, \Phi \right) \).

\begin{proposition}[ELBO–Risk Connection]
\label{prop:approx_factual_risk}
Assume \underline{stationarity} of the approximated posterior of \(\mathbf{Z}\) given sub-longitudinal data; that is, there exists \(t_0\) such that for all \(t \geq t_0\),
\[
q_\phi\bigl(\mathbf{Z} \mid \mathcal{D}_t\bigr) \approx q_\phi\bigl(\mathbf{Z} \mid \mathcal{D}_T\bigr).
\]
Given a finite sample batch
\[
\mathcal{B} = \bigl\{\mathcal{D}_{iT} = \{W_{it}, Y_{it}, \mathbf{X}_{it}\}_{t=1}^{T} : i = 1, \dots, |\mathcal{B}|\bigr\},
\]
we have the following approximation:
\begin{equation}
\label{eq:approx_recons_welbo}
\begin{aligned}
&\sum_{t = t_0}^{T} \mathbb{E}_{\mathbf{Z} \sim q_\phi(\cdot \mid \mathcal{D}_T)}
\biggl[
\alpha(\mathbf{H}_t, W_t)\,
\log p_\theta\bigl(Y_t \mid \mathbf{H}_t, W_t, \mathbf{Z}\bigr)
\biggr] \\[1.2ex]
&\quad \approx -\frac{1}{|\mathcal{B}|} \sum_{t = t_0}^{T}
\biggl\{n_1^{(t)} R^{\omega=1}_{t, g}\bigl(f, \Phi\bigr)
+ n_0^{(t)} R^{\omega=0}_{t, g}\bigl(f, \Phi\bigr)\biggr\},
\end{aligned}
\end{equation}
with
\[
R^{\omega}_{t, g}\bigl(f, \Phi\bigr)
\approx -\frac{1}{n_\omega^{(t)}}
\sum_{\substack{i \in \mathcal{B} \\ W_{it}=\omega}}
\mathbb{E}_{\mathbf{Z} \sim q_\phi(\mathbf{Z} \mid \mathcal{D}_{iT})}
\biggl[
\alpha(\mathbf{H}_{it}, \omega)\,
\log p_\theta\bigl(Y_{it} \mid \mathbf{H}_{it}, \omega, \mathbf{Z}\bigr)
\biggr],
\]
where \(n_\omega^{(t)}\) represents the number of instances in the batch \(\mathcal{B}\) for which \(W_{it} = \omega\).
\end{proposition}
As a result, maximizing the ELBO in Equation \ref{eq:welbo_def} not only maximizes the weighted conditional likelihood over responses (the "reconstruction term") but also, as shown in Equation \ref{eq:approx_recons_welbo}, minimizes the weighted population risk. This, in turn, decreases the generalization bound in Theorem \ref{thm:pehe_wbound}, reducing the error in treatment effect estimation. To further reduce this error, we include the \gls{ipm} term from Theorem \ref{thm:pehe_wbound}, regularizing the ELBO of Equation \ref{eq:welbo_def} with the \gls{ipm} term at each time step: 
\[
\mathcal{L}_{\mathrm{IPM}}(\theta_{\omega}, \Phi) \coloneqq \sum_{t=1}^T \mathrm{IPM}_{G} \left( g_{\theta_{\omega}, \Phi}(\cdot \mid W_t = 1), \, g_{\theta_{\omega}, \Phi}(\cdot \mid W_t = 0) \right).
\]

where \(\theta_{\omega}\) are the parameters of the propensity score model $e_{\theta_{\omega}}(\Phi(.))$. 
\begin{intuitionbox}
\paragraph{Intuition: Stationarity of the inferred latent variables}
We further justify the core assumption made in Proposition~\ref{prop:approx_factual_risk}. The representation learning for the adjustment variables is achieved by approximating the posterior \(p_\theta(\mathbf{z} \mid \mathcal{D}_T)\) with \(q_\phi(\mathbf{z} \mid \mathcal{D}_T)\). Here, the missing baseline covariates are inferred by analyzing \emph{all longitudinal data} \(\{y_{\leq T}, \mathbf{x}_{\leq T}, \omega_{\leq T}\}\). However, since these covariates are \emph{static} and \emph{pre-response} variables, we should, ideally, be able to infer the exact substitute from a shorter longitudinal dataset \(\{y_{\leq T'}, \mathbf{x}_{\leq T'}, \omega_{\leq T'}\}\) where \(T' < T\), or from any temporal slice \(\{y_{t_1:t_2}, \mathbf{x}_{t_1:t_2}, \omega_{t_1:t_2}\}\) with \(t_2 > t_1\). Thus, ensuring a form of stationarity in our posterior approximation is crucial.

To understand the importance of this property, consider estimating the \gls{ate} for longitudinal data at time \(t\):
\[
\tau_t \coloneqq \mathbb{E}\bigl(Y_t(1) - Y_t(0)\bigr)
= \mathbb{E}_{\mathbf{Z}, \mathbf{H}_t}\biggl[
    \mathbb{E}_{Y_t \mid \mathbf{Z}, \mathbf{H}_t, W_t}\bigl(Y_t \mid \mathbf{Z}, \mathbf{H}_t, W_t=1\bigr)
    - \mathbb{E}_{Y_t \mid \mathbf{Z}, \mathbf{H}_t, W_t}\bigl(Y_t \mid \mathbf{Z}, \mathbf{H}_t, W_t=0\bigr)
\biggr].
\]

To compute \(\tau_t\), we need to marginalize the conditional response over the joint distribution of covariates and latent adjustment variables, \(p(\mathbf{h}_t, \mathbf{z}) = p(\mathbf{z} \mid \mathcal{D}_{\leq t})\, p(\mathbf{h}_t)\). Because we model \(p_\theta(\mathbf{z} \mid \mathcal{D}_T)\), which depends on the \emph{entire} history, there is, in general, no guarantee that
\[
p(\mathbf{z} \mid \mathbf{h}_t) \approx p_\theta(\mathbf{z} \mid \mathcal{D}_T).
\]
\end{intuitionbox}

As a consequence of the stationarity assumption in Proposition \ref{prop:approx_factual_risk}, we introduce a penalty term in the form of the Wasserstein distance between consecutive posterior distributions \(q_{\phi}(\mathbf{z}|\mathcal{D}_t)\) and \(q_{\phi}(\mathbf{z}|\mathcal{D}_{t-1})\), penalizing significant variations as the data history grows. To preserve the model’s capacity to capture time-varying dependencies, we begin regularization from \(t_0 \gg 0\), typically \(t_0 = \frac{T}{2}\):  
\[
\mathcal{L}_{\mathrm{DistM}}(\phi) \coloneqq \sum_{t=t_0}^T \mathbb{E}_{\mathcal{D}_{t}} W(q_{\phi}(\mathbf{z} \mid \mathcal{D}_{t}), q_{\phi}(\mathbf{z} \mid \mathcal{D}_{t-1})).
\]
Assuming a Gaussian approximate posterior, the Wasserstein distance simplifies to  
\[
\mathcal{L}_{\mathrm{DistM}}(\phi) = \sum_{t=t_0}^T  \mathbb{E}_{\mathcal{D}_{t}}||\mu_{\mathbf{z}}(\mathcal{D}_{t}) - \mu_{\mathbf{z}}(\mathcal{D}_{t-1})||_2^2 + \mathbb{E}_{\mathcal{D}_{t}}||S_{\mathbf{z}}(\mathcal{D}_{t}) - S_{\mathbf{z}}(\mathcal{D}_{t-1})||^2_{F},
\]
where the penalty regularizes the first and second moments of the posterior distribution as the data history grows.  

\paragraph{Step 4: Total Loss Function and Training Strategy}  
The overall loss for the CDVAE model combines the $\mathrm{ELBO}$ from Equation \ref{eq:welbo_def} with two additional terms: \(\mathcal{L}_{\mathrm{IPM}}\), which reduces covariate imbalance at each time step and addresses residual imbalance not corrected by weighting, and \(\mathcal{L}_{\mathrm{DistM}}\), which captures the global, static nature of adjustment variables. To push the Causal DVAE toward a near-deterministic regime, we treat the variance parameter \(\sigma\) as learnable and fit it using the following loss function:  

\begin{equation}
\label{eq:tot_loss}
\mathcal{L}_{\mathrm{tot}}(\theta, \theta_{\omega}, \phi, \Phi, \sigma) = -\mathrm{ELBO}(\theta, \phi, \Phi, \sigma) + \lambda_{\mathrm{IPM}} \mathcal{L}_{\mathrm{IPM}}(\theta_{\omega}, \Phi) + \lambda_{\mathrm{DistM}} \mathcal{L}_{\mathrm{DistM}}(\phi).
\end{equation}

Since the loss \(\mathcal{L}_{\mathrm{tot}}\) depends on the treatment parameters \(\theta_{\omega}\), as the weighted \(\mathrm{ELBO}\) is also a function of the propensity scores, we introduce an additional loss function \(\mathcal{L}_{W}\), a binary cross-entropy loss to predict treatment from confounders representation. To optimize CDVAE, we adopt an adversarial training strategy, simultaneously minimizing \(\mathcal{L}_{\mathrm{tot}}\) with respect to \(\theta, \phi, \Phi,\) and \(\sigma\), while minimizing \(\mathcal{L}_{W}\) with respect to \(\theta_{\omega}\) (c.f. Algorithm \ref{alg:cdvae_training}):  
\[
\begin{cases}
\displaystyle
\min_{\theta,\, \phi,\, \Phi,\, \sigma}
\mathcal{L}_{\mathrm{tot}}\bigl(\theta, \theta_{\omega}, \phi, \Phi, \sigma\bigr), \\[1.5ex]
\displaystyle
\min_{\theta_{\omega}}
\mathcal{L}_{W}\bigl(\theta_{\omega}, \Phi\bigr).
\end{cases}
\]
The adversarial nature of the training arises because, in one optimization step, we learn the representation \(\Phi\) to predict the response while applying an \gls{ipm} regularization to ensure balance between the weighted covariates. In the subsequent optimization step, for a fixed representation, we train the treatment classifier to predict the treatment. We use the Wasserstein distance as a specific case of \gls{ipm}, with details on its computation provided in Algorithm \ref{alg:wasserstein_distance}.

\paragraph{\gls{cdvae}: Model Specification and Architecture}
\label{sect_cdvae:CDVAE_archi}
We use a three-head neural network architecture for \gls{cdvae} to learn a shared representation between outcome and treatment models inspired by \cite{shi2019Dragonnet}. This architecture consists of two prediction heads for potential outcomes and one for treatment (Appendix \ref{appendix_cdvae:extended_archi_CDVAE}). We use a \gls{gru} \citep{cho2014GRU} to learn a representation \(\Phi(\mathbf{h}_{t+1})\) of the context history. The input of the outcome model  \(f_{\theta_{y}}\) is the shared representation \(\Phi(\mathbf{h}_{t+1})\) and a sampled substitute \(\mathbf{z}\) from  \(q_{\phi}(\mathbf{z} \mid \mathcal{D}_T) \). The outcome model \(f_{\theta_{y}}\) is represented by two non-linear functions \(f_{\theta_{y}^1}\) and \(f_{\theta_{y}^0}\) for treatment assignments \(1\) and \(0\), respectively. The third head is a binary classifier \(f_{\theta_{\omega}}\) estimating the propensity score. The inference model (encoder) \(q_\phi\left(\mathbf{z} \mid y_{\leq T}, \mathbf{x}_{\leq T}, \omega_{\leq T}\right)\) is modeled by an GRU, producing a hidden state that represents the sequence. Two non-linear mappings, \(\mu_{\phi_2}\) and \(\Sigma_{\phi_3}\), learn the mean and diagonal covariance matrix in the latent space.

\section{Experiments}
\label{sect_cdvae:experiments}

\paragraph{Baselines} In all our experiments, we compare \gls{cdvae} against the relevant baselines: \gls{rmsm}, \gls{crn}, G-Net, \gls{ct}, and Causal \gls{cpc}. Each baseline is evaluated in three different configurations:  
\begin{inparaenum}
    \item The "base approach," where models are trained using only static and time-varying confounders.  
    \item The "substitute approach," where models are augmented with substitutes for the unobserved adjustment variables, obtained from \gls{cdvae} and represented by the mean of the approximated posterior.  
    \item The "oracle approach," where models are trained with the true adjustment variables.  
\end{inparaenum}

\section{Algorithmic Details} 
\label{appendix_cdvae:Algorithmic_details}
In this section, we provide the algorithmic details for \gls{cdvae}. First, we describe the approximation of the \gls{ipm} term used in Equation \ref{eq:tot_loss}. The \gls{ipm} term aims to reduce covariate imbalance between the treatment and control groups by quantifying the dissimilarity between their distributions.  To calculate the IPM, we use the Sinkhorn-Knopp algorithm \citep{sinkhorn1967diagonal} and the Wasserstein distance computation algorithm (Algorithm 3 in \cite{cuturi2014fastWass}). The Wasserstein distance computation (Algorithm \ref{alg:wasserstein_distance}) calculates the pairwise distances between data points and constructs a kernel matrix using a regularization parameter. It then computes the row and column marginals based on the weights assigned to each data point. The Sinkhorn-Knopp algorithm (Algorithm \ref{alg:sinkhorn_knopp}), integrated within the Wasserstein distance computation, is used to compute the optimal transport matrix. Finally, the Wasserstein distance is obtained by summing the products of the optimal transport matrix and the pairwise distances.  Computing the Wasserstein distance at each time step and for every batch is computationally expensive. To accelerate training, we compute it for a subsample of the time indices, sampled randomly at each batch. Empirically, this approach is sufficient for maintaining model performance. Specifically, we sample 10\% of the time indices at each batch, corresponding to \(m = \left\lfloor\frac{T}{10}\right\rfloor\) time steps, as shown in Algorithm \ref{alg:cdvae_training}.
\begin{algorithm}
\caption{Sinkhorn-Knopp Algorithm}
\label{alg:sinkhorn_knopp}
\begin{algorithmic}[1]
  \REQUIRE Kernel matrix $K \in \mathbb{R}^{n_t \times n_c}$
  \REQUIRE Row marginal vector $a \in \mathbb{R}^{n_t}$, Column marginal vector $b \in \mathbb{R}^{n_c}$
  \ENSURE Optimal transport matrix $T \in \mathbb{R}^{n_t \times n_c}$
  \STATE Initialize transport matrix $T^{(0)}$ with all entries set to $1$
  \STATE Set iteration counter $k \gets 0$
  \WHILE{not converged}
    \STATE Update row scaling vector $u \in \mathbb{R}^{n_t}$
    \STATE $u_i \gets \frac{a_i}{\sum_{j=1}^{n_c} K_{ij} T^{(k)}_{ij}}$
    \STATE Update column scaling vector $v \in \mathbb{R}^{n_c}$
    \STATE $v_j \gets \frac{b_j}{\sum_{i=1}^{n_t} K_{ij} T^{(k)}_{ij}}$
    \STATE Update transport matrix $T^{(k+1)}$
    \STATE $T^{(k+1)}_{ij} \gets \frac{u_i K_{ij} v_j}{\sum_{i'=1}^{n_t} \sum_{j'=1}^{n_c} u_{i'} K_{i'j'} v_{j'}}$
    \STATE Increment iteration counter $k \gets k + 1$
    \IF{convergence criterion met}
      \STATE \textbf{Return} $T^{(k+1)}$
    \ENDIF
  \ENDWHILE
\end{algorithmic}
\end{algorithm}

\begin{algorithm}
\caption{Weighted Wasserstein Distance Computation}
\label{alg:wasserstein_distance}
\begin{algorithmic}[1]
  \REQUIRE Batch $\mathcal{B} = \{\{\omega_{it}, y_{it}, \mathbf{x}_{it}\}_{t=1}^{T}, i=1,\dots,|\mathcal{B}|\}$
  \REQUIRE Representation learner $\Phi$
  \REQUIRE Weights vectors $\alpha_{\Phi}(\mathbf{h}_t, \omega)$
  \REQUIRE Regularization parameter $\lambda$
   
   \FOR{$t \in \{1, 2, \dots, T\}$}
     \STATE Compute $n_t^{(t)} \gets \sum_{i \in \mathcal{B}} W_{it}$, $n_c^{(t)} \gets \sum_{i \in \mathcal{B}} (1 - W_{it})$
     \STATE Compute pairwise distances matrix $M \in \mathbb{R}^{n_t^{(t)} \times n_c^{(t)}}$ \COMMENT{$M_{ij}^{(t)} = \|\mathbf{H}_{it} - \mathbf{H}_{jt}\|_{L_2}$, $\forall i,j \in \mathcal{B}$; $W_{it} =1$ and $W_{jt} =0$}
     \STATE Initialize kernel matrix $K \in \mathbb{R}^{n_t^{(t)} \times n_c^{(t)}}$ such that $K_{ij}^{(t)} \gets e^{-\lambda M_{ij}^{(t)}}$
     \STATE Compute row marginal vector $a^{(t)} \in \mathbb{R}^{n_t}$ such that $a_i^{(t)} \gets \frac{\alpha_{\Phi}(\mathbf{h}_{it}, 1)}{\sum_{k=1, W_{kt} =1} \alpha_{\Phi}(\mathbf{h}_{it}, 1)}$
     \STATE Compute column marginal vector $b^{(t)} \in \mathbb{R}^{n_c}$ such that $b_j^{(t)} \gets \frac{\alpha_{\Phi}(\mathbf{h}_{it}, 0)}{\sum_{k=1, W_{kt} =0} \alpha_{\Phi}(\mathbf{h}_{it}, 0)}$
     \STATE Compute optimal transport matrix $T^{(t)} \in \mathbb{R}^{n_t^{(t)} \times n_c^{(t)}}$: 
     \STATE \hspace{1cm} $T^{(t)} \gets \text{Sinkhorn-Knopp}(K^{(t)}, a^{(t)}, b^{(t)})$
     \STATE Compute Wasserstein distance $D_t \gets \sum_{i=1}^{n_t} \sum_{j=1}^{n_c} T_{ij}^{(t)} M_{ij}^{(t)}$
   \ENDFOR
   \STATE \textbf{Return} $\sum_{t=1}^{T} D_t$
\end{algorithmic}
\end{algorithm}

\begin{algorithm}
\caption{Pseudo-code for training \gls{cdvae}}
\label{alg:cdvae_training}
\begin{algorithmic}[1]
\REQUIRE Training Data $\mathcal{D}_T = \{\{w_{it}, y_{it}, \mathbf{x}_{it}\}_{t=1}^{T}, i=1,\dots,n\}$
\REQUIRE \gls{cdvae} parameters $\phi$, $\theta_y$, $\theta_{\omega}$, $\Phi$, $\sigma$, Optimizer parameters

\FOR{$p \in \{1, \dots, \text{epoch}_{\text{max}}\}$}
    \FOR{batch $\mathcal{B} = \{\{w_{it}, y_{it}, \mathbf{x}_{it}\}_{t=1}^{T}, i=1,\dots,|\mathcal{B}|\}$}
        \STATE Compute approximate posterior $q_\phi(z \mid y_{\leq T}, \mathbf{x}_{\leq T}, \omega_{\leq T})$
        \STATE Sample latent variables $z$ from $q_\phi(z \mid y_{\leq T}, \mathbf{x}_{\leq T}, \omega_{\leq T})$
        \STATE Compute representation \(\Phi(\mathbf{H}_t)\) for \(t=1,\dots, T\).
        \STATE Compute \(\mathrm{ELBO}(\theta, \phi, \Phi, \sigma)\).
        \STATE Compute \(\mathcal{L}_{\mathrm{DistM}}(\phi)\).
        \STATE Choose $t_{1}, \dots, t_{m} \sim \mathcal{U}([1, T]) $ compute \gls{ipm}  term as :
    \[
        \mathcal{L}_{\mathrm{IPM}} = \sum_{i=1}^m \mathrm{IPM}_{G} \left( g_{\theta_{\omega}, \Phi}(\cdot \mid W_{t_i} = 1), \, g_{\theta_{\omega}, \Phi}(\cdot \mid W_{t_i} = 0)\right)
        \]
        \STATE Compute total loss \( \mathcal{L}_{\mathrm{tot}} = \mathrm{ELBO}(\theta, \phi, \Phi, \sigma) + \lambda_{\mathrm{IPM}} \mathcal{L}_{\mathrm{IPM}}(\theta_{\omega}, \Phi) + \lambda_{\mathrm{DistM}} \mathcal{L}_{\mathrm{DistM}}(\phi).\)
        \STATE Update parameters related to the total loss
    
        $$[\theta, \phi, \Phi, \sigma] \leftarrow  [\theta, \phi, \Phi, \sigma ]- \mu  \left( \frac{\partial \mathcal{L}_{\mathrm{tot}}(\theta, \theta_{\omega}, \phi, \Phi, \sigma)}{\partial [\theta, \phi, \Phi, \sigma] }  \right  ) $$
        \STATE Compute binary cross-entropy loss for the propensity network \(\mathcal{L}_{W}(\theta_{\omega}, \Phi).\) and update parameters
        $$\theta_{\omega}  \leftarrow  \theta_{\omega} - \mu_{W}  \left( \frac{\partial  \mathcal{L}_{W}(\theta_{\omega}, \Phi)}{\partial \theta_{\omega}}  \right  ) $$
    \ENDFOR
\ENDFOR
\STATE \textbf{Return} Trained \gls{cdvae} model
\end{algorithmic}
\end{algorithm}


\section{Models hyperparameters}
\label{sect_cdvae:hyperparams_details}

\paragraph{Hyperparameter Selection} 
All models are fine-tuned using a grid search over hyperparameters, including architecture and optimizer settings. Model selection is based on the mean squared error (MSE) of factual outcomes on a validation set, which is also used as the criterion for early stopping. More details are in Appendix \ref{appendix_cdvae:hyperparams_details}. We use PyTorch \citep{Paszke2019PyTorchAI} and PyTorch Lightning \citep{Falcon_PyTorch_Lightning_2019} to implement \gls{cdvae} and all baselines. For hyperparameter selection, we fine-tune models using a random grid search. \gls{cdvae} is optimized using the weighted reconstruction error as the selection criterion. We do not use a metric related to the quality of estimating \gls{ite}, as this would not be applicable in real-world scenarios where \gls{ite} are unavailable. Designing a suitable criterion for causal cross-validation or hyperparameter tuning in causal models remains an open problem. Various proxies are used in the literature, including loss over factual outcomes \citep{lim2018RMSN, hassanpour2019DRLCFR, bica2020estimatingCRN, Bica2020TimeSDecounf}, one nearest-neighbor imputation for counterfactual outcomes \citep{shalit2017estimating, johansson2022generalization}, influence functions \citep{alaa2019validating}, rank-preserving causal cross-validation \citep{schuler2018comparison}, and Robinson residual decomposition \citep{nie2021quasi,lu2020reconsidering}. Since we aim to select the best regularization parameters ($\lambda_{IPM}$, $\lambda_{MM}$) along with other \gls{cdvae}-related parameters, we avoid using total loss as it may bias ($\lambda_{IPM}$, $\lambda_{MM}$) toward small values. Instead, we use the weighted reconstruction error for fine-tuning. Similarly, Causal \gls{cpc}, \gls{ct}, \gls{crn}, and \gls{rmsm} are fine-tuned using loss over the factual response.  We report in Appendix \ref{appendix_cdvae:hyperparams_details} the search space of hyperparameters for all baselines.

\subsection{Adapting Baselines to Our Causal Settings} 
\label{sect_cdvae:adapat_baselines} 
All the considered baselines do not assume the observation of adjustment variables; however, they only consider time-varying and static confounders. It is not straightforward to incorporate adjustment variables into these models when observed. Naively augmenting their input with adjustment variables and treating them as static confounders often results in suboptimal performance or even worse outcomes compared to excluding the adjustment variables altogether. This is primarily due to two reasons: 
\begin{inparaenum}
\item Most baselines concatenate static confounders with time-varying ones at each time step. When high-dimensional adjustment variables are included, this dramatically increases the number of parameters, leading to overfitting. 
\item When comparing different versions of the same baseline, it is important to ensure comparable complexity represented by the number of learnable parameters (Table \ref{tab:models_complexities}).
\item Models such as \gls{crn}, \gls{ct}, and Causal \gls{cpc} learn a balanced representation. Including adjustment variables naively as input may bias the learned representation towards these variables, as they are inherently balanced. 
\end{inparaenum}

To ensure fair experimentation, we adapt the baselines as follows:
\begin{itemize}
    \item \textbf{\gls{crn}, \gls{ct}, and Causal \gls{cpc}:} Instead of solely feeding the balanced representation to the outcome network, we augment it with static adjustment variables, similar to the \gls{cdvae} design, where the representation \(\Phi(\mathbf{H}_t)\) is augmented with substitutes \(\mathbf{Z}\).
    \item \textbf{G-Net:} Adjustment variables are only used to augment the representation fed to the outcome model, not the representation used to reconstruct the current covariates \(\mathbf{X}_t\).
    \item \textbf{\gls{rmsm}:} Stabilized weights are learned solely as a function of \(\mathbf{H}_t\), while the adjustment variables are concatenated with the representation of \(\mathbf{H}_t\).
\end{itemize}

\begin{table}[ht]
    \caption{Trainable parameters in thousands (k) for baselines in all configurations for the synthetic and semi-synthetic \gls{mimic}-III data.}
    \label{tab:models_complexities}
    \centering
    \resizebox{.5\textwidth}{!}{ 
    \begin{tabular}{|p{4cm}|p{2cm}|p{2cm}|} \hline 
        Model & Params (k), synthetic data & Params (k), \gls{mimic}-III data \\ \hline 
        \gls{cdvae} & 11.5 & 5.7 \\ \hline 
        Causal \gls{cpc} (base) & 6.7 & 5.3 \\  
        Causal \gls{cpc} (with substitute) & 7.1 & 5.7 \\ 
        Causal \gls{cpc} (oracle) & 14.3 & 7.5 \\ \hline 
        CT (base) & 18.7 & 16.3 \\  
        CT (with substitute) & 18.9 & 16.7 \\ 
        CT (oracle) & 26 & 18.7 \\ \hline 
        G-Net (base) & 21.2 & 4.1 \\  
        G-Net (with substitute) & 21.5 & 4.3 \\  
        G-Net (oracle) & 28.5 & 5.7 \\ \hline 
        \gls{crn} (base) & 8.3 & 3.5 \\  
        \gls{crn} (with substitute) & 8.5 & 3.7 \\ 
        \gls{crn} (oracle) & 14.2 & 4.9 \\ \hline 
        \gls{rmsm} (base) & 14 & 6.7 \\  
        \gls{rmsm} (with substitute) & 15.3 & 6.9 \\  
        \gls{rmsm} (oracle) & 20.9 & 8.0 \\ \hline
    \end{tabular}%
    }
\end{table}


\subsection{Synthetic Data Sets}
\paragraph{Generation} 
We simulate a longitudinal dataset of time-length \(T=75\) by generating the time-varying variables autoregressively. Specifically, the confounders \(\mathbf{X}_t\) at each time step \(t\) are generated in \(\mathbb{R}^{d_x}\) with \(d_x = 100\), and the dynamics are specified through an autoregression of order \(p=8\) plus a regression over the past treatment trajectory. Each dimension \(j \in \{1,\dots,d_x\}\) of \(\mathbf{X}_t\) is defined as
\[
\begin{aligned}
\mathbf{X}_t^{(j)}
&= \frac{1}{p}\sum_{k=1}^p \gamma_k^{X,(t,j)}\,\mathbf{X}_{t-k}^{(j)}
+ \frac{1}{p}\sum_{k=1}^p \gamma_k^{XW,(t,j)}\, W_{t-k}
+ \epsilon_{t,j}^X,
\end{aligned}
\]
with
\[
\gamma_k^{X,(t,j)} \sim \mathcal{N}(0,1), \quad
\gamma_k^{XW,(t,j)} \sim \mathcal{N}(0,1), \quad
\epsilon_t^X :=
\bigl[\epsilon_{t,1}^X,\dots,\epsilon_{t,d_x}^X\bigr]^\top
\sim \mathcal{N}(0,\Sigma_x).
\]

To ensure dependence between confounders, the vector error \(\epsilon_t^X\) is generated by a Gaussian distribution with a non-diagonal covariance matrix
\[
\Sigma_x
= \rho\,\mathbf{1}_{d_x}\mathbf{1}_{d_x}^\top
+ (1-\rho)\,\sigma^2 I_{d_x},
\]
where \(\rho=0.5\) and \(\sigma^2=0.3\).

The treatment \(\omega_t\) is generated using a Bernoulli distribution with probability \(\sigma(\pi_t)\) defined by a logistic model to simulate the assignment mechanism. Here, \(\sigma(\cdot)\) denotes the sigmoid function:
\[
\pi_t = \frac{1}{p}\sum_{k=1}^p \gamma_k^{W,t}W_{t-k}
+ \frac{1}{d_xp}\sum_{k=1}^p \langle \gamma_k^{WX,t},\mathbf{X}_{t-k}\rangle
+ \frac{1}{p}\sum_{k=1}^p \gamma_k^{WY,t}Y_{t-k}
+ \epsilon_W.
\]
To ensure the variation of imbalance between treatment and control groups through time, we simulate the regression parameters as follows: 
\begin{equation*}
\begin{aligned}
\gamma_{k}^{W, t}, \, \gamma_{k}^{WY, t} 
&\sim \mathcal{N}\bigl(\sin(t / \pi), \, 0.01^2\bigr), \\[0.5ex]
\gamma_{k}^{WX, t} 
&\sim \mathcal{N}\bigl(\sin(t / \pi), \, 0.01^2\bigr)^{\otimes d_x}, \\[0.5ex]
\epsilon_W 
&\sim \mathcal{N}(0, \, 0.01^2).
\end{aligned}
\end{equation*}
We generate treatment assignment as 
\begin{equation*}
W_t \sim \operatorname{Bernoulli}(\sigma(\pi_t)).
\end{equation*}
To specify the outcome model, we first generate the unobserved adjustment variables \(\mathbf{U} \in \mathbb{R}^{d_u}\) with \(d_u = 100\) using a Gaussian mixture of three distributions:
\[
\mathbf{U} \sim \frac{1}{K}\sum_{i=1}^K \mathcal{N}\bigl(\mu_i, \Sigma_u\bigr),
\]
where \(\mu_1, \dots, \mu_K \sim \mathcal{U}\bigl([-10, 10]\bigr)^{\otimes d_u}\), \(\Sigma_u = 0.2\,\mathrm{diag}(\mathbf{1}_{d_u})\), and \(K=8\).
Finally, we write the expression of the two potential outcomes as a function of the context history. The chosen specification is motivated by the classic mixed-effect approach. We introduce the random effects to have an individual reaction to the change in a covariate $\mathbf{X}_{t,j}$, and we model it by the Hadamard product between the covariate vector and the unobserved adjustment vector. The observed response is defined following the consistency assumption \ref{assp:consistency_seq}:
\begin{equation*}
    Y_t =  Y_t(1) W_t + Y_t(0)(1-W_t)
\end{equation*}
\begin{equation*}
Y_t(\omega) = \frac{1}{d_{U}}\langle  \gamma_{\omega}^{YU}, \mathbf{U}    \rangle  \sum_{k = 1}^{p}W_{t-k} + \frac{1}{d_xp}\sum_{k = 1}^{p}\langle \gamma_{k, \omega}^{YX,t}, \mathbf{X}_{t-k}\rangle + \frac{1}{p}\sum_{k = 1}^{p}\gamma_{k, \omega}^{Y,t}Y_{t-k} +  \epsilon_Y
\end{equation*}
\[
\gamma_{k, \omega}^{YX, t} \sim \mathcal{N}\bigl(\gamma_{\omega}^{YX}, 0.01^2\bigr), \ 
\gamma_{\omega}^{YU} \sim \mathcal{N}\bigl(\gamma_{\omega}^{YU}, 0.01^2\bigr),
\]
\[
\gamma_{k, \omega}^{Y, t} \sim \mathcal{N}\bigl(\gamma_{\omega}^{Y}, 0.1^2\bigr), \ 
\epsilon_Y \sim \mathcal{N}(0, 0.01^2).
\]
With \(\gamma_{1}^{YX}, \gamma_{1}^{Y} = 0.0, 0.2\) and \(\gamma_{0}^{YX}, \gamma_{0}^{Y} = 0.2, 0.1\) and \(\gamma_{0}^{YU} = 0.1\) while \(\gamma_{1}^{YU}\) is varied generate multiple datasets with different modifications levels of treatment effect induced by \(\mathbf{U}\). The experiment is conducted with 5000 samples for training, 500 for validation, and 1000 for testing.

\paragraph{Controlling the Effect of Unobserved Adjustment Variables} 
To assess the impact of unobserved variables \(\mathbf{U}\), we vary the parameter \(\gamma_{(1)}^{YU}\) which determines the contribution of \(\mathbf{U}\) in generating \(Y_t(1)\). By design, \(Y_t(1)\) increases with \(\gamma_{(1)}^{YU}\), and the parameter \(\gamma_{(1)}^{YX}\) is varied within the range \([0, 2.5]\) with a step size of \(0.25\), and we generate a longitudinal dataset at each level of \(\gamma_{(1)}^{YX}\). We report the mean and standard deviation over 10 different seeds of \gls{pehe} in estimating the one-step-ahead \gls{acate}, i.e., \(\epsilon_{\mathrm{PEHE}_{T+1}}\), over the test individuals (smaller is better).

\begin{figure}[ht]
  \centering

    \begin{subfigure}[b]{0.49\textwidth}
    \centering
    \includegraphics[width=8cm, height=4cm]{figures/cdvae/perf_arsim_Causal_Transformer.pdf}
    \caption{Performance of Causal Transformer with CDVAE Comparison}
    \label{fig:perf_sim_ct}
  \end{subfigure}
  \hfill
  \begin{subfigure}[b]{0.49\textwidth}
    \centering
    \includegraphics[width=8cm, height=4cm]{figures/cdvae/perf_arsim_CausalCPC.pdf}
    \caption{Performance of Causal CPC with CDVAE Comparison}
    \label{fig:perf_sim_ccpc}
  \end{subfigure}%
  
  \vspace{0.5cm} 

  \begin{subfigure}[b]{0.49\textwidth}
    \centering
    \includegraphics[width=8cm, height=4cm]{figures/cdvae/perf_arsim_CRN.pdf}
    \caption{Performance of CRN with CDVAE Comparison}
    \label{fig:}
  \end{subfigure}
  \hfill
  \begin{subfigure}[b]{0.49\textwidth}
    \centering
    \includegraphics[width=8cm, height=4cm]{figures/cdvae/perf_arsim_G-Net.pdf}
    \caption{Performance of G-Net with CDVAE Comparison}
    \label{fig:perf_sim_gnet}
  \end{subfigure}

  \vspace{0.5cm} 
  \begin{subfigure}[b]{0.49\textwidth}
    \centering
    \includegraphics[width=8cm, height=4cm]{figures/cdvae/perf_arsim_RMSN.pdf}
    \caption{Performance of RMSN with CDVAE Comparison}
    \label{fig:perf_sim_rmsn}
  \end{subfigure}
\caption{Evolution of PEHE in estimating ACATE for synthetic data across increasing levels of heterogeneity induced by adjustment variables $\mathbf{U}$. }
  \label{fig:perf_sim_combined}
\end{figure}
\paragraph{Results} The Figure \ref{fig:perf_sim_combined} shows the performances of all models given the three possible configurations (base, substitute and oracle). First, the error in estimating the \gls{acate} increases substantially as the coefficient \(\gamma_{(1)}^{YU}\) increases because the contribution of the unobserved static variables becomes considerably more important in the writing of the potential outcomes. However, \gls{cdvae} notably displays a slower increase in error and superior performance in all data configurations. Second, the errors decrease across all levels of unobserved heterogeneity when the baselines are provided with the substitutes learned features by \gls{cdvae}, highlighting the superiority of the substitute approach assisted by \gls{cdvae} over the base one. As expected, a baseline in the oracle approach generally performs better than with substitutes, especially at higher values of \(\gamma_{(1)}^{YU}\), while the substitute approach provides near-oracle performance. Extended results are provided in Appendix \ref{appendix_cdvae:arsim_extended_results}. 


\subsection[Semi-Synthetic MIMIC-III Data]{Semi-Synthetic \gls{mimic}-III Data}
We adapt to our setting a semi-synthetic dataset constructed by \cite{Melnychuk2022CausalTF} based on the \gls{mimic}-III dataset \citep{johnson2016mimic}. The covariates are high-dimensional and include several vital measurements recorded in intensive care units. We investigate the effect of vasopressor treatments on blood pressure in patients. The static covariates in the dataset (gender, ethnicity, and age) are included in the data construction as adjustment variables for the response (blood pressure). We conduct our experiments with 1400 patients for training, 200 patients for validation, and 400 patients for testing.

A cohort of 2,000 patients is extracted from the \gls{mimic}-III dataset, with the simulation setup proposed by \cite{Melnychuk2022CausalTF} extending the model introduced in \cite{schulam2017reliable}. Let \(d_y\) denote the dimension of the outcome variable. For multiple outcomes, untreated outcomes, denoted as \(\mathbf{Z}_t^{j,(i)}\) for \(j=1, \ldots, d_y\), are generated for each patient \(i\) in the cohort. The generation process is defined as:  
\begin{equation}
\mathbf{Z}_t^{j,(i)} = \underbrace{\alpha_S^j \mathbf{B}\text{-spline}(t) + \alpha_g^j g^{j,(i)}(t)}_{\text{endogenous}} + \underbrace{\alpha_f^j f_Z^j\left(\mathbf{X}_t^{(i)}\right)}_{\text{exogenous}} + \underbrace{\varepsilon_t}_{\text{noise}},
\end{equation}
where the B-spline \(\mathbf{B}\text{-spline}(t)\) models the endogenous component, \(g^{j,(i)}(\cdot)\) is sampled independently for each patient from a Gaussian process with a Matérn kernel, and \(f_Z^j(\cdot)\) is sampled from a Random Fourier Features (RFF) approximation of a Gaussian process.  

To introduce confounding into the assignment mechanism, current time-varying covariates are incorporated via a random function \(f_Y^l\left(\mathbf{X}_t\right)\) and the average of a subset of the previous \(T_l\) treated outcomes, \(\bar{A}_{T_l}\left(\overline{\mathbf{Y}}_{t-1}\right)\). For \(d_a\) binary treatments \(\mathbf{A}_t^l\), where \(l=1, \ldots, d_a\), the treatment assignment mechanism is modeled as:  
\begin{equation*}
\begin{aligned}
    p_{\mathbf{A}_t^l} &= \sigma\left(\gamma_A^l \bar{A}_{T_l}\left(\overline{\mathbf{Y}}_{t-1}\right) + \gamma_X^l f_Y^l\left(\mathbf{X}_t\right) + b_l\right), \\
    \mathbf{A}_t^l &\sim \operatorname{Bernoulli}\left(p_{\mathbf{A}_t^l}\right),
\end{aligned}
\end{equation*}
where \(\sigma(\cdot)\) denotes the sigmoid function.  

Static features \(\mathbf{U}\), such as gender and ethnicity, which are categorical, are one-hot encoded. A random Singular Value Decomposition (SVD) transformation \(f_E(\cdot)\) is then applied to \(\mathbf{U}\), retaining all singular components. Subsequently, treatments are applied to the untreated outcomes using the following expression:  
\begin{equation}
E^j(t) = \sum_{i=t-w^l}^t \frac{\min_{l=1, \ldots, d_a} \mathbb{1}_{\left[\mathbf{A}_i^l=1\right]} p_{\mathbf{A}_i^l} \beta_{lj} + \left|\sum_{k=1}^{d_U} f_E(U)_k\right|}{\left(w^l-i\right)^2},
\end{equation}
where \(w^l\) is the treatment window.  

The final outcome combines the treatment effect and the untreated simulated outcome:
\begin{equation}
Y^j_t = Z^j_t + E^j(t).
\end{equation}
Similar to the synthetic data experiment, we evaluate all baselines using three approaches (base, with substitutes, and oracle), and report the \gls{pehe} in estimating the one-step-ahead \gls{acate} for a patient trajectory.

\paragraph{Results} Figure \ref{fig:perf_mimic} reports the mean and standard deviation of \gls{pehe} for \gls{cdvae} and all baselines across all configurations. Similar to the synthetic data results, the base approach always performs worse than the substitute and oracle approaches. However, the substitute approach substantially enhances performance compared to the base approach, highlighting the relevance of the substitutes learned by \gls{cdvae}. Across all configurations, \gls{cdvae} achieves the best performance compared to all baselines. Extended results are provided in Appendix \ref{appendix_cdvae:mimic_extended_results}.

\begin{figure}%[t]
\begin{center}
\includegraphics[width=0.6\linewidth]{figures/cdvae/perf_mimic_combined.pdf}
\caption{Results on the \gls{mimic}-III data reported by \gls{pehe} and organized following the three possible configurations. Smaller is better.}
\label{fig:perf_mimic}
\end{center}
\end{figure}

\section{Discussion}
\paragraph{Ablation Study}  
To experimentally validate the design of \gls{cdvae}, we perform an ablation study by exploring several model configurations: the full \gls{cdvae} model with all components; \gls{cdvae} without the \gls{ipm} term (\(\lambda_{\mathrm{IPM}} = 0\)); \gls{cdvae} without the distribution matching term (\(\lambda_{\mathrm{DistM}} = 0\)); \gls{cdvae} without both the \gls{ipm}  term and distribution matching term (\(\lambda_{\mathrm{IPM}} = 0, \lambda_{\mathrm{DistM}} = 0\)); \gls{cdvae} without the \gls{ipm}  term and weighting (\(\lambda_{\mathrm{IPM}} = 0\), w/o weighting); \gls{cdvae} (\(\lambda_{\mathrm{IPM}} = 0, \lambda_{\mathrm{DistM}} = 0\), w/o weighting); and \gls{cdvae} with a fixed variance parameter (\(\sigma = 1\)). We follow the same experimental protocol as in prior experiments, conducting the ablation for the synthetic dataset across all heterogeneity levels induced by \(\gamma_{(1)}^{YU}\) and for the semi-synthetic \gls{mimic}-III dataset. Across all configurations, the full \gls{cdvae} consistently outperforms the other models. Furthermore, removing individual components results in progressively higher errors, as shown in Tables \ref{tab:ablation_perf_sim} and \ref{tab:ablation_perf_mimic}. Interestingly, the configurations (\(\lambda_{\mathrm{IPM}} = 0, \lambda_{\mathrm{DistM}} = 0\), without weighting) and (\(\sigma = 1\)) either perform comparably to or worse than the second-best model, Causal \gls{cpc}, on both the synthetic dataset and the \gls{mimic}-III dataset. 
\begin{table} 
    \caption{\gls{cdvae} ablation study conducted on the semi-synthetic \gls{mimic}-III data reported by \gls{pehe}. Smaller is better.}
    \label{tab:ablation_perf_mimic}
    \centering
    \resizebox{0.5\textwidth}{!}{
    \begin{tabular}{|c|c|} 
    \hline
    Model      & $\mathrm{PEHE}$ \\ \hline 
    \textbf{\gls{cdvae} (ours)} & \textbf{17.63$\pm$0.25}\\
    \hline
    \textbf{\gls{cdvae} ($\lambda_{\mathrm{IPM}}=0$)} & 18.38$\pm$0.26\\
    \hline
     \textbf{\gls{cdvae} ($\lambda_{\mathrm{DistM}}=0$)} & 18.21$\pm$0.26\\
     \hline
     \textbf{\gls{cdvae} ($\sigma=1$)} & 20.50$\pm$1.04\\
    \hline
    \textbf{\gls{cdvae} ($\lambda_{\mathrm{IPM}}=0, \lambda_{\mathrm{DistM}}=0$)} & 18.45$\pm$0.23\\
     \hline
    \textbf{\gls{cdvae} ($\lambda_{\mathrm{IPM}}=0$, w/o weighting)} & 18.97$\pm$0.28\\
    \hline
    \textbf{\gls{cdvae} ($\lambda_{\mathrm{IPM}}=0, \lambda_{\mathrm{DistM}}=0$, w/o weighting)} & 19.23$\pm$0.28\\
    \hline
    \end{tabular}%
    }
\end{table}

\begin{table}[!htbp]
 \caption{Results on the synthetic data reported by \gls{pehe}. Smaller is better.}
 \label{tab:ablation_perf_sim}
 \centering
\renewcommand{\arraystretch}{1.5} 
\resizebox{\textwidth}{!}{
\begin{tabular}{|c|c|c|c|c|c|c|c|c|c|c|c|} 
\hline
Model       & $\gamma_{(1)}^{YU} = 0$ & $\gamma_{(1)}^{YU} = 0.25$ & $\gamma_{(1)}^{YU} = 0.5$ & $\gamma_{(1)}^{YU} = 0.75$ & $\gamma_{(1)}^{YU} = 1$ & $\gamma_{(1)}^{YU} = 1.25$ & $\gamma_{(1)}^{YU} = 1.5$ & $\gamma_{(1)}^{YU} = 1.75$ & $\gamma_{(1)}^{YU} = 2$ & $\gamma_{(1)}^{YU} = 2.25$ & $\gamma_{(1)}^{YU} = 2.5$ \\ \hline 

\textbf{\gls{cdvae} (ours)} & \textbf{0.43$\pm$0.02}& \textbf{0.50$\pm$0.03}& \textbf{0.96$\pm$0.09}& \textbf{1.57$\pm$0.08}& \textbf{1.90$\pm$0.10}&  \textbf{2.35$\pm$0.18}& \textbf{3.57$\pm$0.17}& \textbf{4.80$\pm$0.20}& \textbf{6.84$\pm$0.20}& \textbf{7.64$\pm$0.48}& \textbf{9.03$\pm$0.50}\\
 \hline
\textbf{\gls{cdvae} ($\lambda_{\mathrm{IPM}}=0$)}& 0.48$\pm$0.02& 0.57$\pm$0.03& 1.12$\pm$0.01& 1.80$\pm$0.15 & 2.23$\pm$0.12& 2.53$\pm$0.15  & 3.88$\pm$0.13& 5.23$\pm$0.11& 7.37$\pm$0.21& 7.95$\pm$0.12& 9.32$\pm$0.36\\ \hline

\textbf{\gls{cdvae} ($\lambda_{\mathrm{DistM}}=0$)}& 0.46$\pm$0.02& 0.57$\pm$0.03& 1.10$\pm$0.02& 1.78$\pm$0.13& 2.18$\pm$0.13& 2.64$\pm$0.18& 3.95$\pm$0.15& 5.20$\pm$0.12& 7.14$\pm$0.13& 8.08$\pm$0.14&9.25$\pm$0.19\\\hline

\textbf{\gls{cdvae} ($\sigma=1$)}& 0.81$\pm$0.40& 0.66$\pm$0.07& 2.17$\pm$0.53& 5.73$\pm$1.51& 9.27$\pm$3.27& 10.67$\pm$2.02& 12.66$\pm$2.16& 14.28$\pm$4.23& 15.63$\pm$4.04& 18.23$\pm$5.71&17.19$\pm$5.71\\\hline

\textbf{\gls{cdvae} ($\lambda_{\mathrm{IPM}}=0, \lambda_{\mathrm{DistM}}=0$)}& 0.48$\pm$0.02& 0.57$\pm$0.03& 1.16$\pm$0.07& 1.84$\pm$0.17& 2.33$\pm$0.12& 2.66$\pm$0.14& 4.05$\pm$0.10& 5.36$\pm$0.13& 7.48$\pm$0.12& 8.20$\pm$0.13&9.40$\pm$0.24\\\hline

\textbf{\gls{cdvae} ($\lambda_{\mathrm{IPM}}=0$, w/o weighting)}& 0.50$\pm$0.01& 0.60$\pm$0.01& 1.20$\pm$0.03& 1.90$\pm$0.11& 2.31$\pm$0.10& 2.66$\pm$0.13& 3.99$\pm$0.16& 5.30$\pm$0.19& 7.51$\pm$0.12& 8.21$\pm$0.15&9.41$\pm$0.23\\\hline

\textbf{\gls{cdvae} ($\lambda_{\mathrm{IPM}}=0, \lambda_{\mathrm{DistM}}=0$, w/o weighting)}& 0.50$\pm$0.02& 0.62$\pm$0.02& 1.27$\pm$0.03& 1.98$\pm$0.10& 2.39$\pm$0.09& 2.85$\pm$0.14& 4.19$\pm$0.13& 5.59$\pm$0.13& 7.61$\pm$0.15& 8.41$\pm$0.14&9.78$\pm$0.21\\\hline
\end{tabular}%
}
\end{table}


\begin{figure}[ht]
  \centering
  \begin{subfigure}[b]{0.45\textwidth}
    \centering
    \includegraphics[width=8cm, height=4cm]{figures/cdvae/perf_arsim_y_sigma.pdf}
    \caption{Synthetic data.}
  \label{fig:perf_arsim_y_sigma}
  \end{subfigure}%
  \hfill
  \begin{subfigure}[b]{0.45\textwidth}
     \centering
    \includegraphics[width=8cm, height=4cm]{figures/cdvae/perf_mimic_y_sigma.pdf}
    \caption{\gls{mimic}-III.}
  \label{fig:perf_mimic_y_sigma}
  \end{subfigure}%
  \caption{Evolution of variance parameter update during training for synthetic data (left) for each level of \(\gamma_{(1)}^{YU}\) and \gls{mimic}-III (right) averaged over 10 random initializations}
\end{figure}

\paragraph{On the Near-Deterministic Behavior of \gls{cdvae}}  
For the theoretical results in Section \ref{sect_cdvae:cdvae_near_det} to hold, it is necessary to verify whether the variance parameter \(\sigma\), as a learnable parameter, indeed decreases toward zero during training. In all experiments, \(\sigma\) is initialized at one, and we show in Figure \ref{fig:perf_arsim_y_sigma} its behavior during training on the synthetic dataset across all levels of \(\gamma_{(1)}^{YU}\), as well as on the \gls{mimic}-III dataset in Figure \ref{fig:perf_mimic_y_sigma}. In all cases, the variance parameter stably decreases toward zero, validating the near-deterministic regime at the end of training. This supports the consistency result related to the treatment effect established in Theorem \ref{thm:sigma_to_0}.

\paragraph{\gls{cdvae} Robustness to the Number of Components in the Prior} 
We demonstrate that the number of components \(K\) in the Gaussian mixture prior does not substantially affect the PEHE. The chosen value, selected via random search, is \(K=7\), while the ground truth is \(K=8\). To test robustness, we evaluate CDVAE with values below and above this baseline, namely \(K=2, 5, 8, 11\). For the semi-synthetic MIMIC-III dataset, the true number of components is unknown, and the value selected via grid search is \(K=5\). To test robustness, we also evaluate \(K=2, 8, 11, 14\). Figure \ref{fig:ablation_arsim_n_clusters} shows the evolution of errors for the synthetic data across levels of \(\gamma_{(1)}^{YU}\) for different values of \(K\). While there are slight differences in performance means for CDVAE with varying \(K\), almost all error bars overlap across all levels of \(\gamma_{(1)}^{YU}\). The same observations hold for MIMIC-III, as depicted in Figure \ref{fig:ablation_mimic_n_clusters}. This highlights the robustness of CDVAE to the choice of \(K\) for the prior and its low sensitivity compared to the components analyzed in the ablation study.

\begin{figure}[ht]
  \centering
  \begin{subfigure}[b]{0.45\textwidth}
    \centering
    \includegraphics[width=8cm, height=4cm]{figures/cdvae/ablation_arsim_n_clusters.pdf}
    \caption{Synthetic data.}
  \label{fig:ablation_arsim_n_clusters}
  \end{subfigure}
  \hfill
  \begin{subfigure}[b]{0.45\textwidth}
     \centering
    \includegraphics[width=8cm, height=4cm]{figures/cdvae/ablation_mimic_n_clusters.pdf}
    \caption{\gls{mimic} data.}
  \label{fig:ablation_mimic_n_clusters}
  \end{subfigure}%
  \caption{Results of \gls{cdvae} when varying the number of components \(K\) of the prior for the synthetic data (left) and \gls{mimic}-III (right) reported by \gls{pehe}. Smaller is better. }
\end{figure}


\paragraph{Bayesian Model Assessment of \gls{cdvae}}  
We assess the quality of the conditional response fitting in our variational framework through a posterior predictive check \citep{RubinPostPredC1984,meng1994posterior,gelman1995bayesianDA} and similar to \citet{Bica2020TimeSDecounf, hatt2024sequential}. For each time step \(t\), let \(\mathbf{y}_{t}^{\mathrm{obs}} \coloneqq \{y_{i,t}\}_{i=1}^{N_{\mathrm{val}}}\) represent the observed responses in the validation dataset. We generate \(S\) replicated datasets of responses \(\mathbf{y}_{t}^{\mathrm{rep}}(s) \coloneqq \{y_{i,t}^{\mathrm{rep}}(s)\}_{i=1}^{N_{\mathrm{val}}}\) for \(s = 1, \dots, S\), such that for each individual \(i\) in the validation dataset, we draw \(S\) samples of latent substitutes \(\mathbf{z}_i(1), \dots, \mathbf{z}_i(S) \sim q_{\phi}(\cdot \mid \mathcal{D})\). The approximate posterior serves as a proxy for the true (inaccessible) posterior \(p(\mathbf{z} \mid \mathcal{D})\). Replicated responses are then generated from the fitted conditional distribution:  
\(
Y_{t}^{\mathrm{rep}}(s) \sim Y_t \mid y_{<t}, \mathbf{x}_{\leq t}, \omega_{\leq t}, \mathbf{z}_i(s).
\)

To compare the observed and replicated data, we define a statistic \(\mathbb{T}\) based on the conditional log-likelihood:  
\[
\mathbb{T}(\mathbf{y}_{t}^{\mathrm{obs}}) \coloneqq \frac{1}{N_{\mathrm{val}}} \sum_{i=1}^{N_{\mathrm{val}}} \log p_{\theta}(y_{i,t} \mid \mathbf{h}_{it}, \omega_{i,t}, \mathbf{z}_{i}(s)),
\]
and for replicated responses:
\(
\mathbb{T}(\mathbf{y}_{t}^{\mathrm{rep}}(s)) \coloneqq \frac{1}{N_{\mathrm{val}}} \sum_{i=1}^{N_{\mathrm{val}}} \log p_{\theta}(y_{i,t}^{\mathrm{rep}}(s) \mid \mathbf{h}_{it}, \omega_{i,t}, \mathbf{z}_{i}(s))
\). We then define a posterior predictive p-value as:
\[
p = \Pr(\mathbb{T}(\mathbf{y}_{t}^{\mathrm{rep}}(s)) > \mathbb{T}(\mathbf{y}_{t}^{\mathrm{obs}})),
\]
which is approximated as:
\[
p \approx \frac{1}{S} \sum_{s=1}^{S} \mathbbm{1}\{\mathbb{T}(\mathbf{y}_{t}^{\mathrm{rep}}(s)) > \mathbb{T}(\mathbf{y}_{t}^{\mathrm{obs}})\}.
\]
We compare these p-values over time to assess how closely the distribution of the conditional responses matches the distribution of the replicated responses. If the model accurately captures the conditional response distribution given the substitutes, the test statistics for the replicated data should be close to those for the observed data, ideally resulting in a p-value equal to 0.5. Figures \ref{fig:perf_arsim_p_values} and \ref{fig:perf_mimic_p_values} show the temporal evolution of the p-values for both the synthetic data and semi-synthetic MIMIC-III. In general, all the p-values fluctuate inside the interval \([0.41,0.59]\) except for the synthetic dataset with \(\gamma_{(1)}^{YU}=0.0\) because \(\mathbf{U}\) no longer modifies the potential outcomes \((Y_t(1))_{t \geq 1}\). Interestingly, the bias in the p-values (Figure \ref{fig:perf_arsim_p_values}) decreases as \(\gamma_{(1)}^{YU}\) increases because CDVAE is designed to capture substantial heterogeneity in the responses due to the unobserved adjustment variables.  
\begin{figure}[ht]
  \centering
  \begin{subfigure}[b]{0.45\textwidth}
    \centering
    \includegraphics[width=8cm, height=4cm]{figures/cdvae/perf_arsim_p_values.pdf}
    \caption{Synthetic data}
  \label{fig:perf_arsim_p_values}
  \end{subfigure}%
  \hfill
  \begin{subfigure}[b]{0.45\textwidth}
     \centering
    \includegraphics[width=8cm, height=4cm]{figures/cdvae/perf_mimic_p_values.pdf}
    \caption{\gls{mimic}-III}
  \label{fig:perf_mimic_p_values}
  \end{subfigure}%
  \caption{Evolution of \gls{cdvae} posterior predictive p-values for synthetic (left) and semi-synthetic \gls{mimic}-III data (right). We report the average for 10 random initializations at each time step.}
\end{figure}

\paragraph{Connection to the Deconfounder Theory}
Our approach can also provide a remedy for a key inconsistency in the deconfounder theory \citep{lopezmultipletreatments,ranganath2018multiple, wang2019blessings, wang2019blessingsreply}. Crucially, while the inference model for the latent confounder is probabilistic, leading to a distribution over the substitute confounder, the theory assumes that the posterior distribution collapses into a Dirac delta distribution, implying certainty in the confounders' estimation. This assumption simplifies the theoretical framework but introduces a fundamental incoherence between the stochastic nature of the inference models and the deterministic assumption in the theory \citep{d2019comment,imai2019comment, D'AmourMulti-Cause2019}. There is a significant theoretical-application gap: In theory, the deconfounder assumes that the substitute confounder is estimated with certainty, while in practice, inference models are \emph{stochastic} \citep{zhang2019medicalDeconf, Bica2020TimeSDecounf, hatt2024sequential}, and the latent confounder is described by a distribution, introducing uncertainty.   
Our use of near-deterministic VAEs indirectly controls the posterior variance, finding a compromise where the posterior remains less diffuse yet not fully deterministic. This approach enables a more precise estimation of the substitute confounder without assuming perfect certainty, addressing an inherent inconsistency. Applying this method within deconfounder theory holds independent interest beyond this works’s scope. Future research could explore integrating these improvements into the deconfounder framework, with near-deterministic VAEs for substitute confounders inference to bridge theory and practice. 

\paragraph{Comparing our approach to the deconfounder} Unlike the deconfounder, our method does not require the consistency assumption for identifying treatment effects. Whereas the deconfounder framework models unobserved covariates as confounders affecting both treatment and outcome, we treat these unobserved covariates as adjustment variables, thus bypassing the need for the consistency assumption.

\paragraph{Estimating \texorpdfstring{$p(Y_{t}(\omega))$}{p(Yt(omega))}}
In causal inference, when unobserved confounders are present, the conditional distribution of potential outcomes plays a critical role. If the adjustment variables $\mathbf{U}$ are observed, the potential outcome can be represented as:
\[
p(Y_{t}(\omega)) = p(Y_t \mid \mathbf{h}_t, W_t = \omega) = \int p(y_t \mid \mathbf{h}_t, W_t = \omega, \mathbf{U} = \mathbf{u}) p(\mathbf{u} \mid \mathbf{h}_t, W_t = \omega) d\mathbf{u}.
\]
Due to the structural assumptions over the causal graph, the treatments $W_t$ and covariates $\mathbf{X}_t$ are d-separated from $\mathbf{U}$ given $\mathbf{H}_t$, implying:
\[
p(\mathbf{u} \mid \mathbf{h}_t, W_t = \omega) = p(\mathbf{u} \mid \mathcal{D}_{t-1}),
\]
where the conditional potential outcome is identifiable, but estimating it requires sampling from the posterior distribution of the adjustment variables, $p(\mathbf{u} \mid \mathcal{D}_{t-1})$.

When $\mathbf{U}$ is not observed, let $\mathbf{Z}$ be a latent variable satisfying the CMM(p). Under what conditions does the following equality hold?
\begin{equation}
    \begin{aligned}
    \int p(y_t \mid \mathbf{h}_t, W_t = \omega, \mathbf{Z} = \mathbf{z}) p(\mathbf{z} \mid \mathcal{D}_{t-1}) \, d\mathbf{z} 
    &\overset{(*)}{=} \int p(y_t \mid \mathbf{h}_t, W_t = \omega, \mathbf{U} = \mathbf{u}) p(\mathbf{u} \mid \mathcal{D}_{t-1}) \, d\mathbf{u} \\
    &= p(Y_{t}(\omega) \mid \mathbf{h}_t).
    \end{aligned}
    \label{eq:p_Y_from_z_to_y}
\end{equation}
This equation addresses the potential risk of non-uniqueness in the \gls{cmm} assumption, which could lead to varying values on the left-hand side (LHS) of Equation \ref{eq:p_Y_from_z_to_y}. However, our framework differs from the traditional deconfounder framework. Here, the identification of the conditional potential outcome \(p(Y_t \mid \mathbf{h}_t)\) occurs \emph{independently} of the latent variables, as sequential ignorability holds without requiring conditioning on them. The \gls{cmm} assumption, under the condition \(\mathbf{Z} \indep \mathbf{X}_{\leq T}, W_{\leq T}\), ensures that no confounding backdoor paths are introduced by conditioning on \(\mathbf{Z}\). Thus, using \(\mathbf{Z}\) as a substitute for \(\mathbf{U}\) presents no identifiability or consistency issues. This conclusion also extends to the marginal distribution of potential outcomes, formally shown through a copula argument, as in \cite{D'AmourMulti-Cause2019}.
\begin{equation}
\begin{aligned}
p(Y_{t}(\omega)) &= \int p(Y_{t}(\omega) \mid \mathbf{H}_t =  \mathbf{h}_t) p(\mathbf{h}_t) d\mathbf{h}_t, \\
p(Y_{t}(\omega)) &= \int p(Y_{t} \mid \mathbf{H}_t =  \mathbf{h}_t, W_t = \omega) p(\mathbf{h}_t) d\mathbf{h}_t, \\
p(Y_{t}(\omega)) &= \int p(y_{\leq t}, \mathbf{x}_{\leq t}, \omega_{\leq t}) \frac{p(\mathbf{h}_t)}{p(\mathbf{h}_t, \omega_t)} d\mathbf{h}_t, \\
p(Y_{t}(\omega)) &= \int \int p(y_{\leq t}, \mathbf{z} \mid \mathbf{x}_{\leq t}, \omega_{\leq t}) p(\mathbf{x}_{\leq t}, \omega_{\leq t}) \frac{p(\mathbf{h}_t)}{p(\mathbf{h}_t, \omega_t)} d\mathbf{h}_t d\mathbf{z}, \\
&= \int \int c(y_{\leq t}, \mathbf{z} \mid \mathbf{x}_{\leq t}, \omega_{\leq t}) p(y_t \mid \mathbf{h}_t, \omega_t) p(\mathbf{z} \mid \mathbf{x}_{\leq t}, \omega_{\leq t}) p(\mathbf{h}_t) d\mathbf{h}_t d\mathbf{z}.
\end{aligned}
\end{equation}
The copula \(c(y_{\leq t}, \mathbf{z} \mid \mathbf{x}_{\leq t}, \omega_{\leq t})\) is restricted by the CMM(p) assumption. This constraint differs significantly from the deconfounder theory, where factor models often separate multiple treatments or treatment sequences and impose no such restrictions on the outcome model. Therefore, identifying potential outcomes in the deconfounder framework requires additional assumptions, as discussed in \cite{wang2019blessings, wang2019blessingsreply}. However, our framework enforces conditional separation of responses given past sequences of treatments and covariates, implying independence between the latent variables and treatment sequences.

Finally, in practice, how can we estimate \(p(Y_{t}(\omega))\)? We express this as:
\begin{equation}
\begin{aligned}
p(Y_{t}(\omega)) &= \int p(y_{t} \mid \mathbf{H}_t =  \mathbf{h}_t, W_t = \omega) p(\mathbf{h}_t) d\mathbf{h}_t, \\
&= \int \int  p(y_{t} \mid \mathbf{h}_t, \omega, \mathbf{z}) p(\mathbf{z} \mid \mathbf{h}_t, \omega) p(\mathbf{h}_t) d\mathbf{h}_t d\mathbf{z}, \\
&= \int \int p(y_{t} \mid \mathbf{h}_t, \omega, \mathbf{z}) p(\mathbf{z} \mid \mathcal{D}_{t-1}) p(\mathbf{h}_t) d\mathbf{h}_t d\mathbf{z}, \\
&\approx \int \int p_{\theta}(y_{t} \mid \mathbf{h}_t, \omega, \mathbf{z}) q_{\phi}(\mathbf{z} \mid \mathcal{D}_{T}) p(\mathbf{h}_t) d\mathbf{h}_t d\mathbf{z}.
\end{aligned}
\end{equation}

Here, \(p_{\theta}(y_{t} \mid \mathbf{h}_t, \omega, \mathbf{z})\) is modeled by the outcome model (decoder), while \(q_{\phi}(\mathbf{z} \mid \mathcal{D}_{T})\) is the approximate posterior distribution of the latent variables, estimated using the observed sequence of data.

\paragraph{Capturing "bad variables"}
We examine whether the substitute adjustment variables \(\mathbf{Z}\) can inadvertently capture "bad variables," that is, variables that may introduce bias into the estimation of causal effects. One potential source of bias arises from M-colliders (Figure \ref{fig:m_collider}). If the substitute adjustment variables \(\mathbf{Z}\) capture information not only about the true adjustment variables \(\mathbf{U}\), but also about a collider variable \(\mathbf{M}\), this could result in \(\mathbf{Z} \not\perp W_{\leq T}\). 

\begin{figure}[ht]
\begin{center}
\includegraphics[scale=0.5]{figures/cdvae/m_colliders.pdf}
\caption{An example of an M-collider structure, where the variable \(V\) influences both the treatment and the response, as indicated by the dashed arrows.}
\label{fig:m_collider}
\end{center}
\end{figure}

The key concern is whether \(\mathbf{Z}\) could “blindly” capture information from the sequence of responses or treatments. Such cases may lead to open collider paths like
\[
\mathbf{U} \rightarrow Y_t \leftarrow W_{\leq t}
\quad \text{or} \quad
\mathbf{U} \rightarrow Y_t \leftarrow \mathbf{X}_{\leq t}.
\]
These scenarios would violate the assumption that \(\mathbf{Z} \perp W_{\leq t}\) and \(\mathbf{Z} \perp \mathbf{X}_{\leq t}\). In essence, including colliders in the substitute adjustment variables can open “backdoor” paths, leading to biased treatment effect estimates. To prevent this, it is essential to ensure that the substitute variables \(\mathbf{Z}\) do not inadvertently encode information about colliders that affect both the treatments and the responses.

\paragraph{Conclusion}  
In this work, we proposed CDVAE, a novel framework for estimating treatment effects in high-dimensional, time-varying settings. By leveraging variational inference with robust regularization techniques, we introduced a principled approach to infer latent adjustment variables while ensuring identifiability and mitigating covariate imbalance. Our framework demonstrated theoretical guarantees for generalization and treatment effect consistency in the near-deterministic regime of VAEs—an overlooked property in the causal inference literature. Extensive empirical evaluations support the effectiveness of CDVAE on both synthetic and semi-synthetic datasets. Future work could focus on extending this framework to:  
\begin{inparaenum}
    \item dynamic treatment regimes (Definition \ref{def:DTR}, Chapter \ref{chapter:background}), for example, by incorporating the g-calculus (Proposition \ref{prop:g_calculus_dtr});
    \item providing generalization bounds for treatment effects when they depend on a sequence of treatments \citep{lewis2021doubledebiased, vankadara2022causal, oh2022generalizationDTR, csillag2024generalization};
    \item exploring theoretically the bias-variance trade-off in the estimation of treatment effects in the near-deterministic regime.  
\end{inparaenum}




==> 4.tex <==
\chapter{Causal Contrastive Predictive Coding}
\label{chapter:ccpc}

\section{Introduction}
\label{sect_ccpc:intro}
It is vital in real-world applications to estimate potential responses, i.e., responses under hypothetical treatment strategies. Individuals show diverse responses to the same treatment, emphasizing the need to quantify individual response trajectories. This enables personalized interventions, enhancing decision-making efficacy. In medical contexts, precise response estimation enables tailored treatments for patients \citep{atan2018Deep-Treat, shalit2020ITPolicyClinical, mueller2023personalized}. This chapter focuses on \emph{counterfactual regression over time}, estimating responses under hypothetical treatment plans based on individual records, including past covariates, responses, and treatment sequences up to the current prediction time \citep{robins2000MSM, robins-time-varying-exposures}. We have seen some of the challenges (Chapter \ref{chapter:background} and \ref{chapter:cdvae}) we need to address in the time-varying setting, which are \emph{time-dependent confounding}, \emph{selection bias}, and \emph{long-term dependencies}. As mentioned in Sections \ref{sect_background:po_framework_longit_overview} and \ref{sect_cdvae:intro}, RMSNs \citep{lim2018forecasting}, CRN \citep{bica2020estimatingCRN}, and G-Net \cite{Li2021GNetAR}, have tackled these causal inference challenges. However, their reliance on \gls{rnn} limits their ability to capture long-term dependencies. Recent studies like Causal Transformer \citep{Melnychuk2022CausalTF} propose better integrating transformers to represent temporal dynamics. Rather than viewing this as a limitation of \gls{rnn}, we see it as an opportunity to emphasize their strengths. We design specific architectures for counterfactual regression over large horizons, avoiding complex, hard-to-interpret models like transformers. Our approach leverages the computational efficiency of \gls{rnn}, incorporating \emph{Contrastive Predictive Coding (CPC)} \citep{oord2018representation, henaff2020data} for learning data history representations. This enhances model performance while maintaining efficiency, offering a compelling alternative to transformer-based approaches. Furthermore, we usually formulate identification assumptions of counterfactual responses over the original process history space, namely sequential ignorability, overlap, and consistency for longitudinal data (Assumptions \ref{assp:seq_ignorability}, \ref{assp:overlap_seq}, \ref{assp:consistency_seq}). However, these assumptions may not hold in the representation space for arbitrary functions. Since identification often involves conditional independence, it applies when using an invertible representation function. Current models for time-varying settings \citep{lim2018forecasting, bica2020estimatingCRN, Melnychuk2022CausalTF} do not enforce representation invertibility. To address this, instead of adding complexity with a decoder, we \emph{implicitly} push the history process to be "reconstructable" from the encoded representation by maximizing Mutual Information (MI) between representation and input, following the \emph{Information Maximization (InfoMax)} principle \cite{linsker1988selforga}, akin to Deep \gls{infomax} \cite{DeepInfoMax2019}. We summarize these main design differences between the baselines and Causal \gls{cpc} in Table \ref{tab_ccpc:overview_benchmark}. 

\begin{table}[htbp]
    \centering
    \caption{Summary of concurrent methods contrasted against Causal \gls{cpc} across design aspects.}
    \renewcommand{\arraystretch}{1.2} 
    \setlength{\tabcolsep}{3pt}       
    \small                            
    \begin{tabular}{|p{2cm}|p{2cm}|p{1.8cm}|p{1.8cm}|p{1.8cm}|p{2cm}|p{2cm}|p{2cm}|}
    \hline
    Model & Backbone & Tailored to long-term forecast? & Learning of long-term dependencies & Use of contrastive learning & Prediction of counterfactuals & Handling selection bias & Invertibility of representation \\
    \hline
    \textbf{Causal \gls{cpc} (ours)} & \gls{gru} & Yes & \gls{cpc} & Yes & Autoregressive & Balanced representation & Yes, contrasts representation with input \\
    \hline
    \textbf{Causal Transformer} & 3 Transformers & Yes & Transformers & N/A & Autoregressive & Balanced representation & N/A \\
    \hline
    \textbf{G-Net} & \gls{lstm} & No & N/A & N/A & Autoregressive & G-Computation & Current covariates $\mathbf{X}_t$ \\
    \hline
    \textbf{CRN} & \gls{lstm} & No & N/A & N/A & Autoregressive & Balanced representation & N/A \\
    \hline
    \textbf{RMSN} & \gls{lstm} & No & N/A & N/A & Autoregressive & Weighting & N/A \\
    \hline
    \textbf{MSM} & Logistic+linear model & No & N/A & N/A & Autoregressive & Weighting & N/A \\
    \hline
    \end{tabular}
    \label{tab_ccpc:overview_benchmark}
\end{table}


\section{Contributions}
\label{sect_cccp:contrib}

Our approach is inspired by \emph{self-supervised learning} using \gls{mi} objectives \citep{DeepInfoMax2019}. We aim to maximize \gls{mi}  between different views of the same input, introducing counterfactual regression over time through \gls{cpc} to capture long-term dependencies. Additionally, we propose a tractable lower bound to the original \gls{infomax} objectives for more efficient representations. This is challenging due to the sequential nature and high dimensionality, marking a novelty. We demonstrate the importance of regularization terms via an ablation study. Previous work leveraging contrastive learning for causal inference applies only to the static setting with no theoretical grounding \citep{infomax_static2022}. To our knowledge, we frame for the first time the representation balancing problem from an information-theoretic perspective and show that the suggested adversarial game (Theorem \ref{thm:blancing_iclub}) yields theoretically balanced representations using the \gls{club} of \gls{mi}  \citep{cheng2020club}, computed efficiently. Key innovations of our Causal \gls{cpc} model include:
\begin{itemize}
    \item We showcase the capability of leveraging \gls{cpc} to capture long-term dependencies in the process history using \gls{infonce} \citep{gutmann2010nce, gutmann2012nce, oord2018representation}, an unexplored area in counterfactual regression over time where its integration into process history modeling is not straightforward in causality (Table \ref{tab_ccpc:overview_benchmark}).
    \item We enforce input reconstruction from representation by contrasting the representation with its input. Current baselines generally overlook such quality (c.f. Table \ref{tab_ccpc:overview_benchmark}), yet it ensures retaining confounding information which prevents biased counterfactual estimation.
    \item Applying \gls{infomax} to process history while respecting its dynamic nature is challenging. We provide a tractable lower bound to the original \gls{infomax} problem, bringing theoretical insights into the tightness.    
    \item We suggest minimizing an upper bound on \gls{mi} between representation and treatment to make the representation non-predictive of the treatment, using the \gls{club} of \gls{mi}  \citep{cheng2020club}. This novel information-theoretic perspective results in a theoretically balanced representation across all treatment regimes.    
    \item By using a simple \gls{gru} layer \citep{cho2014GRU} as the model backbone, we demonstrate that well-designed regularizations can outperform more complex models like transformers.
\end{itemize}
Finally, our experiments on synthetic data (cancer simulation \citep{PK-PD}) and semi-synthetic data based on real-world datasets (\gls{mimic}-III \citep{johnson2016mimic}) show the superiority of Causal \gls{cpc} at accurately estimating counterfactual responses.

\section{Related Work}
\label{sect_ccpc:related_work}

\paragraph{Counterfactual Regression Over Time} We compare Causal \gls{cpc} primarily to MSMs, RMSNs, CRN, G-Net, and CT. These models, like ours, assume \emph{sequential ignorability} \citep{robins-time-varying-exposures}. Several alternative models operate under different assumptions, often addressing the presence of unobserved confounders. Some of these models build on deconfounding theory \citep{lopezmultipletreatments, ranganath2018multiple, wang2019blessings}, which recent works have extended to time-varying settings. Deconfounding involves imposing a factor model on treatment assignment, where each treatment becomes conditionally independent, given latent variables that act as proxies for unobserved confounders. Examples of this approach include \cite{Bica2020TimeSDecounf, hatt2021sequential, cao2023estimating}. Other models assume the presence of proxy variables, inferring a representation of unobserved confounders through probabilistic models based on these proxies \citep{veitch2020adapting, LuChengCMAproxynConf20121, kuzmanovic2021deconfounding}. Unlike our setting, which follows the sequential ignorability assumption, many models adopt a data-generating process similar to that in \citep{Soleimani2017TreatmentResponseMF, soleimani2017scalable, qian2021synctwin}. These methods, often non- or semi-parametric, tend to either ignore static covariates or handle them linearly, leading to computational inefficiencies and scalability issues. Nevertheless, some non- or semi-parametric approaches—such as \cite{schulam2017reliable, seedat2022continuous,de2022predicting, hizli2023causal}—align with our causal assumptions but extend them to continuous time, treating sequential ignorability in a continuous setting. Additionally, models like \cite{JiangCF-GODE2023} incorporate continuous-time and assume interactions between units, where an individual’s outcome depends on both their treatment and the treatments of others. \cite{berrevoets2021disentangled}, focusing on binary treatment sequences, requires a stronger version of sequential ignorability—conditional on current covariates—. In contrast, our model assumes a weaker version, conditioning on the entire history of covariates to account for long-lasting confounding effects.  Furthermore, \cite{chen2023multi} focuses solely on binary treatments and targets estimating the average treatment effect on the treated. The authors assume a specific treatment regime where individuals enter a post-treatment state after a defined time period. This assumption is restrictive compared to our framework, which allows for complex, individualized treatment assignment mechanisms and non-binary treatments, where treatment values fluctuate over time. As a result, \cite{chen2023multi} is incompatible with our causal assumptions. Other methods, like \cite{wu2023counterfactual}, address high-dimensional counterfactual generation based on time-varying treatment plans under the same sequential ignorability assumption. However, they are not designed for causal forecasting over multiple time steps, as required in our setting. Similarly, \cite{frauen2023estimating} focuses on estimating the average causal effect and is not suited for predicting individual treatment effects or conditional counterfactual responses, as it targets marginal counterfactual expectations via g-computation.

In contrast, we introduce a contrastive learning approach to capture long-term dependencies while maintaining a simple model and ensuring high computational efficiency in training and prediction. We demonstrate that simple models with well-designed regularization terms can still achieve high prediction quality. Additionally, previous works \citep{robins-time-varying-exposures, robins2000MSM, lim2018RMSN, Li2021GNetAR, Melnychuk2022CausalTF} did not consider the role of invertible representation in improving counterfactual regression. Here, we introduce an \gls{infomax} regularization term to make our encoder easier to invert. 

\paragraph{\gls{infomax} Principle} The \gls{infomax} principle aims to learn a representation that maximizes \gls{mi}  with its input \citep{linsker1988selforga, bell1995information}. Estimating \gls{mi}  for high-dimensional data is challenging and is often addressed by maximizing a simple and tractable lower bound on \gls{mi}  \citep{DeepInfoMax2019, VarBoundsMI2019, liang2023factorizedCL}. Another approach involves maximizing \gls{mi}  between two lower-dimensional representations of different views of the same input \citep{bachman2019learning, henaff2020data, tian2020contrastive, Tschannen2020OnMIMAX}, offering a more practical solution. We adopt this strategy by dividing our process history into two views, past and future (c.f. Figure \ref{fig:ccpc_archi}), and maximizing a tractable lower bound on \gls{mi}  between them, encouraging a "reconstructable" representation of the process history. To our knowledge, the only work applying an \gls{infomax} approach to counterfactual regression, albeit in static settings, is \cite{infomax_static2022}. They propose maximizing \gls{mi}  between an individual's representation and a global representation, aggregating information from all individuals into a single vector. However, the global representation lacks clarity and interpretability, raising uncertainties about its theoretical underpinnings in capturing confounders. Furthermore, there's a lack of theoretical analysis on how minimizing \gls{mi}  between individual and treatment-predictive representations could yield a treatment-invariant representation. As a novelty, we extend the \gls{infomax} principle to longitudinal data, providing a theoretical guarantee of learning balanced representations. 

\textbf{Self-Supervised Learning and Mutual Information} In the self-supervised learning paradigm, Deep \gls{infomax} \citep{DeepInfoMax2019} employs \gls{mi} computation between input images and representations, emphasizing its maximization to enhance reconstruction quality. Additionally, local \gls{mi} calculations between the representation and local features contribute to encoding more intricate patterns shared across data patches. The strategy of maximizing average \gls{mi} between the representation and local regions, such as patches, significantly improves downstream task performance. Notably, global \gls{mi} assumes a more prominent role in reconstructing the complete input given the representation.

\gls{cpc} aligns with the MI-based approach seen in Deep \gls{infomax}, emphasizing the maximization of \gls{mi} between global and local representation pairs. Distinct from Deep \gls{infomax}, \gls{cpc} processes local features sequentially, constructing partial "summary features" to predict specific local features in the future. Classical self-supervised paradigms often focus on tasks like classification or reconstruction-based objectives, leading to distinct preferences for maximizing \gls{mi} in either local or global information. However, integrating both procedures becomes imperative in scenarios involving downstream tasks like counterfactual regression over time. Our proposed Causal \gls{cpc} is strategically designed to align with these intuitions.

Several other methods share similarities with \gls{cpc}, such as Contrastive Multiview Coding \citep{tian2020contrastive}, which emphasizes maximizing \gls{mi} between representations of different views of the same observation. Augmented Multiscale Deep \gls{infomax} \citep{bachman2019learning}, akin to \gls{cpc}, makes predictions across space but differs by predicting representations across layers in the model. Instance Discrimination \cite{zhao2020makes} also encourages learning representations capable of discriminating between individual examples in the dataset. Still, our preference for \gls{cpc} arises from its adaptability in processing sequential features in an ordered and autoregressive manner. This aligns seamlessly with the requirements of our specific context, especially when dealing with counterfactual regression over time.


\section{Problem Formulation}
\label{sect_ccpc:prob_formulation} 
\paragraph{Setup} In the \gls{po} framework \citep{rubin2005causal}, and following \cite{robins2009estimation}, we extend the treatment variable to be discrete (unlike the binary treatment in \gls{cdvae}) and broaden the \gls{po} scope compared to \gls{cdvae} (Chapter \ref{chapter:cdvae}) to consider  the lagged treatment effect:  

\begin{assumption}[Lagged Treatment Effect]
\label{assp:lagged_effect}
We focus our causal framework on examining causal quantities defined with respect to potential outcomes given a lag of \( \rho \) time steps, rather than the entire sequence of treatments. In mathematical terms, this can be represented as \( \{Y_t(W_{\leq t - \rho}, \omega_{t-\rho+1:t})\}_{\omega_{t-\rho+1:t} \in \mathcal{W}^{\rho}} \). This approach relaxes the contemporaneous treatment effect assumption in the \gls{cdvae} model (Chapter \ref{chapter:cdvae}), as it defines counterfactual trajectories of responses over sequences of potential outcomes rather than a single one. On the other hand, the lagged treatment effect assumption enables us to establish a framework for \textbf{causal forecasting}, i.e., estimating causal quantities over time beyond the scope of the observed longitudinal study. Specifically, we can consider the longitudinal study as observed data up to time \( t' = t - \rho \), and then investigate future causal quantities defined as a function of \( \{Y_{t' + \rho}(W_{\leq t'}, \omega_{t'+1:t'+\rho})\}_{\omega_{t'+1:t'+\rho} \in \mathcal{W}^{\rho}} \). \textbf{This is the main setting of our second contribution (Causal \gls{cpc})}.
\end{assumption}

As a result of Assumption \ref{assp:lagged_effect} and for any time step \(t + \rho\), we treat the longitudinal study as observed data up to time \( t\) and investigate future causal quantities defined by 
\[
\{Y_{t + \rho}(W_{\leq t}, \omega_{t+1:t+\rho})\}_{\omega_{t+1:t+\rho} \in \mathcal{W}^{\rho}}.
\]
\begin{figure}
     \centering
    \includegraphics[width = 0.50\textwidth, height = 0.20\textheight]{figures/causal_cpc/cg_compressed_ccpc.pdf}
    \caption{Causal graph over $\mathbf{H}_{t+1}$. For simplicity, we represent past treatments as $W_{ \leq t}$ such that each element in that sub-sequence confounds the next treatment and response $W_{t+1}$ and $Y_{t+1}$. Idem for $Y_{ \leq t}$ and $\mathbf{X}_{ \leq t}$. The static covariates $\mathbf{V}$ are assumed to affect all the time-varying variables. We omit the representation of exogenous noise for simplicity. Interactions between $W_{ \leq t}$ , $\mathbf{X}_{ \leq t}$, and $Y_{ \leq t}$ were also omitted for simplicity.}
  \label{fig:causal_graph}
\end{figure}

As described in Section \ref{sect_background:po_framework_longit_intro}, we track a cohort of individuals (units) \(i \in \{1,2,\dots, N\}\) over \(t_{max}\) time steps. At each time \(t \in \{1,2,\dots,t_{max}\}\), we observe:
\begin{inparaenum}[(1)]
    \item \emph{Discrete treatment} \(W_{it} \in \mathcal{W} = \{0,1, \dots, K-1\}\),
    \item \emph{Outcome of interest} \(Y_{it} \in \mathcal{Y} \subset \mathbb{R}\),
    \item \emph{Time-varying context} \(\mathbf{X}_{it} \in \mathcal{X} \subset \mathbb{R}^{d_x}\), a \(d_x\)-dimensional vector of confounders, and
    \item \emph{Static confounders} \(\mathbf{V} \in \mathcal{V} \subset \mathbb{R}^{d_v}\).
\end{inparaenum} We define the history up to time \(t+1\) as \(\mathbf{H}_{t+1} = [\mathbf{V}, \mathbf{X}_{\leq t+1}, W_{\leq t}, Y_{\leq t}]\), capturing all information before assigning treatment \(W_{t+1}\). This process is illustrated in the causal graph in Figure \ref{fig:causal_graph} where all of the past observed data encompassed in $\mathbf{H}_{t+1}$ confounds future treatments and responses, $W_{t+1}, W_{t+2}, \dots, W_{t_{max}}$ and $Y_{t+1}, Y_{t+2}, \dots, Y_{t_{max}}$, which create long-term dependencies. The fact that the covariates \(\mathbf{X}_{\leq t+1}\) are affected by the  treatments \(W_{\leq t}\) creates time-dependent confounding. The static covariates \(\mathbf{V}\) are assumed to be affecting all of the time-varying variables. Since we suppose sequential ignorability, no possible exogenous noises are affecting both treatments and responses. 

\paragraph{Goal} Given a training dataset \(\{\mathbf{H}_{i,t+1}, i=1,\dots, N \}\) sampled from the empirical distribution \(\mathbb{P}_{\mathbf{H}_{t+1}}\), we address the causal inference problem:

\emph{How can we efficiently estimate counterfactual responses up to time \(t + \rho\), where \(\rho \geq 1\) is the prediction horizon for a potential treatment sequence \(\omega_{t+1:t+\rho} = (\omega_{t + 1}, \dots, \omega_{t + \rho})\), given history \(\mathbf{H}_{t+1}\)?}

The goal is to estimate the causal quantity \(m_{t}^{W_{\leq t}, \omega_{t+1:t+\rho}}(\mathbf{x}_{\leq t}, y_{<t})\) (Equation \ref{eq:exp_pot_outc_classic}). By Assumption \ref{assp:lagged_effect} of the lagged treatment effect and sequential ignorability (Assumption \ref{assp:seq_ignorability}), we obtain the following identification result (Proposition \ref{prop_backround:identif_po_cate_time}):
\begin{align*}
m_{t}^{W_{\leq t}, \omega_{t+1:t+\rho}}(\mathbf{x}_{\leq t}, y_{<t}) 
    &= \mathbb{E}(Y_{t+\rho}(\omega_{t+1:t+\rho})\mid \mathbf{H}_{t+1}) \\
    &= \mathbb{E}\left(Y_{t+\rho}\mid \mathbf{H}_{t+1}, W_{t+1:t+\rho} = \omega_{t+1:t+\rho}\right),
\end{align*}

where \(\mathbb{E}(Y_{t+\rho}(\omega_{t+1:t+\rho})\mid \mathbf{H}_{t+1})\) is the expected outcome at time \(t + \rho\), conditioned on the history \(\mathbf{H}_{t+1}\) and treatment sequence \(\omega_{t+1:t+\rho}\).
\section[Causal CPC]{Causal \gls{cpc}}
\label{sect_ccpc:causal_cpc_def}
\subsection{Representation Learning}
\paragraph{Contrastive Predictive Coding}  Using contrastive learning, we illustrate how to efficiently learn a representation of the process history $\mathbf{H}_{t}$. Causal forecasting across multiple horizons requires representations with high variability predictability within $\mathbf{H}_{t}$. In short-term prediction, we aim to capture low-level information and exploit local signal smoothness. For long-term prediction, shared information between history and future points decreases over time, necessitating a more global structure. Capturing long-term dependencies and slow-varying features is crucial in our setting.

To achieve this, we learn a representation of $\mathbf{H}_t$ that predicts future frames over multiple time steps.
For each prediction horizon \(j\in\{1,\dots,\rho\}\) we define the future frames as
\[
  \mathbf F_{t+j}
  \;:=\;
  \bigl[\mathbf V,\;\mathbf X_{t+j},\;W_{t+j-1},\;Y_{t+j-1}\bigr]
  \;\in\;
  \mathcal U\subset\mathbb R^{d_v+d_x+K+1}.
\]

\noindent\textbf{Step\,1: local encoding.} First, local features are extracted by encoding the frames \((\mathbf F_{t})_{1 \le t \le T-\rho}\)
Let
\[
  \Phi_{\theta_1}:\;
  \mathbb R^{d_v+d_x+K+1}\;\longrightarrow\;\mathbb R^{d_z}
\]
be a component-level encoder.  At a time~\(t\) we obtain the local feature vector
\[
  \mathbf Z_t
  \;\coloneqq\;
  \Phi_{\theta_1}\! (\mathbf F_{t})
  \;=\;
  \Phi_{\theta_1}\! \bigl( \bigl[\mathbf V,\mathbf X_t,W_{t-1},Y_{t-1}\bigr] \bigr).
\]

\noindent\textbf{Step\,2: autoregressive summarisation.}
Collect the sequence \( \mathbf Z_{1:t}=(\mathbf Z_1,\dots,\mathbf Z_t) \). A GRU-based autoregressive map
\[
  \Phi_{\theta_2}^{\mathrm{AR}}:\;
  (\mathbb R^{d_z})^{t}\;\longrightarrow\;\mathbb R^{d_c}
\]
produces the \emph{context representation}
\[
  \mathbf C_t^{\mathrm{enc}}
  \;\coloneqq\;
  \Phi_{\theta_2}^{\mathrm{AR}}\!\bigl(\mathbf Z_{1:t}\bigr).
\]

\noindent\textbf{Composite representation function.}
The overall representation of the process history is therefore the composition
\[
  \Phi_{\theta_1,\theta_2}
  \;\coloneqq\;
  \Phi_{\theta_2}^{\mathrm{AR}}\circ\Phi_{\theta_1},
  \qquad
  \Phi_{\theta_1,\theta_2}(\mathbf H_t)=\mathbf C_t^{\mathrm{enc}},
\]
where \(\Psi_{\theta_1}(\mathbf H_t):=\bigl(\psi_{\theta_1}(\mathbf V,\mathbf X_s,W_{s-1},Y_{s-1})\bigr)_{s=1}^{t}\) applies the frame encoder to each step (c.f. left side of Figure \ref{fig:ccpc_archi}).

To train the model, we use a contrastive loss that encourages the context $\mathbf{C}_t^{\mathrm{enc}}$ to predict future local features $\mathbf{Z}_{t+1}, \dots, \mathbf{Z}_{t+\rho}$ while distinguishing them from the features of other individuals within the same training batch. This is done by minimizing the \gls{infonce} loss $\mathcal{L}^{(InfoNCE)}_j$ for each horizon $j$:
\begin{equation}
\label{eq:infonce_loss_cpc}
\mathcal{L}^{(InfoNCE)}_j(\theta_1, \theta_2, \Gamma_j) \coloneqq -\mathbb{E}_{\mathcal{B}} \left[ \log \frac{\exp(T_j(\mathbf{F}_{t+j}, \mathbf{C}_t^{\mathrm{enc}}))}{\sum_{l=1}^{|\mathcal{B}|} \exp(T_j(\mathbf{F}_{l,t+j},\mathbf{C}_t^{\mathrm{enc}}))} \right],
\end{equation}
where $\mathcal{B}$ is a batch containing individual histories, and $\Gamma_j$ is a weight matrix. The discriminator \(T_j(\cdot, \cdot)\) classifies the correct future feature among negative samples from other individuals:
\begin{equation}
\label{eq:discrim_cpc}
\begin{aligned}
T_j\bigl(\mathbf{F}_{t+j}, \Phi_{\theta_1, \theta_2}(\mathbf{H}_t)\bigr)
&\coloneqq \Phi_{\theta_1}(\mathbf{F}_{t+j})^\top \Gamma_j \mathbf{C}_t^{\mathrm{enc}} \\[0.8ex]
&= \mathbf{Z}_{t+j}^\top \Gamma_j \mathbf{C}_t^{\mathrm{enc}} \\[0.8ex]
&= \mathbf{Z}_{t+j}^\top \hat{\mathbf{Z}}_{t+j}.
\end{aligned}
\end{equation}
In practice, the projection of $\mathbf{C}_t^{\mathrm{enc}}$ on the matrix $\Gamma_j$  yields a prediction $\mathbf{\hat{Z}}_{t+j}$ whose quality is measured by the dot product with the true future local feature $\mathbf{Z}_{t+j}^\top \mathbf{\hat{Z}}_{t+j}$. Minimizing the \gls{infonce} loss $\mathcal{L}^{(InfoNCE)}_j$ provides a lower bound on the \gls{mi} between the context and future features $I(\mathbf{F}_{t+j}, \mathbf{C}_{t})$ \citep{oord2018representation}:
\begin{equation}
 \label{eq:LB_MI_InfoNCE}
  \log(|\mathcal{B}|) - \mathcal{L}^{(InfoNCE)}_j  \leq I(\mathbf{F}_{t+j}, \mathbf{C}_{t}).
\end{equation}
For multiple forecasting horizons $j = 1, 2, \dots, \rho$, we learn long-term dependencies by minimizing the \gls{infonce} loss across all horizons:
\begin{equation}
\label{eq:cpc_loss}
\mathcal{L}^{CPC}(\theta_1, \theta_2, \{\Gamma_j\}_{j=1}^{\rho}) \coloneqq \frac{1}{\rho} \sum_{j=1}^{\rho} \mathcal{L}^{(InfoNCE)}_j(\theta_1, \theta_2, \Gamma_j).
\end{equation}

Thus, minimizing $\mathcal{L}^{CPC}$ maximizes the \emph{shared information} between the context and future components as shown in  Equation (\ref{eq:MI_lb_avg}), pushing the model to capture the global structure of the process over large horizons—crucial for counterfactual regression across multiple time steps:
\begin{equation}
\label{eq:MI_lb_avg}
 \log(|\mathcal{B}|) - \mathcal{L}^{CPC} \leq \frac{1}{\rho} \sum_{j=1}^{\rho} I(\mathbf{F}_{t+j}, \mathbf{C}_{t}) .
\end{equation}
\paragraph{\gls{infomax} Principle} We introduce a regularization term to make the context representation of the process history $\mathbf{H}_{t}$ "reconstructable." We leverage the \gls{infomax} principle to maximize the \gls{mi}  between $\mathbf{H}_{t}$ and the context $\mathbf{C}_t^{\mathrm{enc}}$. However, we avoid computing the contrastive loss between $\mathbf{C}_t^{\mathrm{enc}}$ and $\mathbf{H}_t$ for two main reasons. First, $\mathbf{H}_{t}$ is a high-dimensional sequence, making the loss computation very demanding. Secondly, we are still interested in incorporating inductive bias toward capturing global dependencies, this time by pushing any subsequence to be predictive of any future subsequence within $\mathbf{H}_t$. Hence, we divide the process history into two non-overlapping views, $\mathbf{H}_t^h\coloneqq\mathbf{F}_{1:t_0}$, $\mathbf{H}_t^f\coloneqq\mathbf{F}_{t_0+1:t}$ representing a \emph{historical subsequence} and a \emph{future subsequence} of frames within the process history $\mathbf{H}_{t}$, with $t_0$ randomly chosen per batch. We then maximize the \gls{mi} between the representations of these views, $\mathbf{C}_t^{\mathrm{enc},h}$ and $\mathbf{C}_t^{\mathrm{enc},f}$, resulting in a lower bound to the \gls{infomax} objective as formulated below:
\begin{proposition}
\label{prop:lb_infomax}
Let \( \mathbf C_t^{\mathrm{enc},h} = \Phi_{\theta_1,\theta_2}\!\bigl(\mathbf H_t^{\,h}\bigr)\) and \(  \mathbf C_t^{\mathrm{enc},f} = \Phi_{\theta_1,\theta_2}\!\bigl(\mathbf H_t^{\,f}\bigr) \) be the encodings of the two non-overlapping
subsequences described above. Then
\[
  I\!\bigl(\mathbf C_t^{\mathrm{enc},h},
           \mathbf C_t^{\mathrm{enc},f}\bigr)
  \;\le\;
  I\!\bigl(\mathbf H_t,
           (\mathbf C_t^{\mathrm{enc},h},
            \mathbf C_t^{\mathrm{enc},f})\bigr).
\]
\end{proposition}

We provide an intuitive discussion of the inequality by providing an exact writing of the gap in Proposition \ref{prop:lb_infomax}: 
\begin{theoremBox}
\label{thm:tightness_lb_info}
\begin{align}
I\!\bigl(\mathbf H_t;\,(\mathbf C_t^{\mathrm{enc},h},
                        \mathbf C_t^{\mathrm{enc},f})\bigr)
\;-\;
I\!\bigl(\mathbf C_t^{\mathrm{enc},h},
         \mathbf C_t^{\mathrm{enc},f}\bigr)
  &=
    I\!\bigl(\mathbf H_t;\mathbf C_t^{\mathrm{enc},f}\mid
              \mathbf C_t^{\mathrm{enc},h}\bigr)
    \nonumber\\
  &\quad+\;
    \mathbb E_{\mathbf h_t\sim P_{\mathbf H_t}}
      \,\mathbb E_{\mathbf c_t^{f}\sim
                   P_{\mathbf C_t^{f}\mid\mathbf h_t}}
      \Bigl[
        D_{\mathrm{KL}}\!\bigl(
          P_{\mathbf C_t^{h}\mid\mathbf h_t}
          \,\big\Vert\,
          P_{\mathbf C_t^{h}\mid\mathbf c_t^{f}}
        \bigr)
      \Bigr].
\label{eq:tightness_lb_infomax}
\end{align}
\end{theoremBox}
Both terms on the RHS of Equation (\ref{eq:tightness_lb_infomax}) are positive, providing an alternative proof to Proposition \ref{prop:lb_infomax}. When equality holds, it implies \( I(\mathbf{H}_t; \mathbf{C}_t^{\mathrm{enc},f} \mid \mathbf{C}_t^{\mathrm{enc},h}) = 0 \), indicating that \(\mathbf{H}_t\) is independent of \(\mathbf{C}_t^{\mathrm{enc},f}\) given \(\mathbf{C}_t^{\mathrm{enc},h}\). This suggests that \(\mathbf{C}_t^{\mathrm{enc},h}\) retains sufficient information from \(\mathbf{H}_t\) that is predictive of \(\mathbf{C}_t^{\mathrm{enc},f}\). The symmetry of \gls{mi}  also leads to the occurrence of the second term on the RHS when conditioning on \(\mathbf{C}_t^{\mathrm{enc},f}\). The equality in Proposition \ref{prop:lb_infomax} implies \( \mathbb{P}_{\mathbf{C}_{t}^h \mid \mathbf{h}_t} = \mathbb{P}_{\mathbf{C}_{t}^h \mid \mathbf{c}_{t}^f } \), suggesting that \(\mathbf{C}_t^{\mathrm{enc},f}\) efficiently encodes its subsequence while sharing maximum information with \(\mathbf{C}_t^{\mathrm{enc},h}\).

By considering the proposed variant of the \gls{infomax} principle, we can compute a contrastive bound to $I(\mathbf{C}_t^{\mathrm{enc},h}, \mathbf{C}_t^{\mathrm{enc},f})$ more efficiently, as the random vectors reside in a low-dimensional space thanks to the encoding. We define a contrastive loss using \gls{infonce} similar to  Equation (\ref{eq:infonce_loss_cpc}): 
\begin{equation}
\label{eq:infomax_loss_cpc}
\mathcal{L}^{(InfoMax)}(\theta_{1},\theta_{2}, \eta)  \coloneqq -\mathbb{E}_{\mathcal{B}} \left[ \log \frac{\exp(T_{\eta}(\mathbf{C}_t^f, \mathbf{C}_t^h))}{\sum_{l = 1}^{|\mathcal{B}|} \exp(T_{\eta}(\mathbf{C}_{l,t}^f, \mathbf{C}_t^h))} \right].
\end{equation}
We use a non-linear discriminator $T_{\eta}$ parametrized by $\eta$ (detailed in Appendix \ref{appendix_ccpc:archi_ccpc}). The representation of the past subsequence $\mathbf{C}_t^{h}$ is mapped to a prediction of the future subsequence $\mathbf{\hat{C}}_t^{f}\coloneqq F_{\eta}(\mathbf{C}_t^h)$ and $T_{\eta} = \mathbf{C}_t^{f^{\top}} \mathbf{\hat{C}}_t^f$.

Theorem \ref{thm:tightness_lb_info} and Proposition \ref{prop:lb_infomax} justify using the loss in  Equation (\ref{eq:infomax_loss_cpc}) by showing that our \gls{infomax} simplification provides a valid lower bound; this is because the contrastive loss in Equation (\ref{eq:infomax_loss_cpc}) verifies
\begin{equation}
\log(|\mathcal{B}|) - \mathcal{L}^{(InfoMax)} \leq I(\mathbf{C}_t^h, \mathbf{C}_t^f) \leq I(\mathbf{H}_t, (\mathbf{C}_t^h, \mathbf{C}_t^f)).
\end{equation}
The “mental model” behind our regularization term comes from the \gls{mi}
\[
I\bigl(\mathbf{H}_t; (\mathbf{C}_t^h, \mathbf{C}_t^f)\bigr)
= H(\mathbf{H}_t) - H\bigl(\mathbf{H}_t \mid (\mathbf{C}_t^h, \mathbf{C}_t^f)\bigr),
\]
which can be written using entropy.

Since the entropy term \(H(\mathbf{H}_t)\) is constant and parameter-free, minimizing the conditional entropy
\[
H\bigl(\mathbf{H}_t \mid (\mathbf{C}_t^h, \mathbf{C}_t^f)\bigr) \geq 0
\]
ensures that \(\mathbf{H}_t\) is almost surely a function of \((\mathbf{C}_t^h, \mathbf{C}_t^f)\) (Appendix~\ref{appendix: zero_cond_H}, Proposition~\ref{prop:zero_cond_H}). When \gls{mi} is maximized, the theoretical existence of such a function suggests that the learned context \(\mathbf{C}_t^{\mathrm{enc}}\) can decode and reconstruct \(\mathbf{H}_t\).

\paragraph{\gls{infonce} and \gls{dgp} inversion} 
Beyond the idea of reconstruction, it was shown that the \gls{infonce} objective implicitly learns to invert the data's generative model under mild assumptions \citep{zimmermann2021contrastive}. Recent works \citep{daunhawer2023identifiability, liu2024revealing} extend this insight to multi-modal settings, which can reframe our \gls{infomax} problem: $\mathbf{H}_t^h$ and $\mathbf{H}_t^f$ can be seen as two coupled modalities, allowing us to identify latent generative factors up to some mild indeterminacies (e.g., rotations, affine mappings). We anticipate that multi-modal causal representation learning could be extended to our longitudinal setting, where minimizing our \gls{infomax} objective, in the limit of infinite data, will effectively invert the data generation process up to a class of indeterminacies that we conjecture to be broader and under weaker assumptions than those in current causal representation learning literature, given our focus is on causal inference rather than the identification of causal latent variables. 

To initiate a formal basis for this claim, suppose the true data-generating process is given by $\mathbf{H}_{t} = g(\mathbf{Z}_t)$, where $\mathbf{Z}_t$ represents the true latent factors. In the sequential context, we assume that the same function $g$ generates the two historical subsequences:
\[
\mathbf{H}_t^f = g(\mathbf{z}_t^f), \quad \mathbf{H}_t^h = g(\mathbf{z}_t^h)
\]
We assume a general dependency of the form:
\[
p(\mathbf{z}_t^f \mid \mathbf{z}_t^h ) = \frac{Q(\mathbf{z}_t^f)}{Z(\mathbf{z}_t^h)} \exp(-d(\mathbf{z}_t^f, \mathbf{z}_t^h))
\]
With $d(.,.)$ is a metric as in \cite{matthes2023towards}. With $\mathbf{\Phi}$ being an encoder, we use the \gls{infomax} regularization term as follows:
\[
\mathcal{L}^{(InfoMax)}(\mathbf{\Phi}, d, \mathcal{B}) := -\mathbb{E}_{\mathcal{B}} \left[ \log \frac{\exp(-d(\mathbf{\Phi}(\mathbf{H}_t^f), \mathbf{\Phi}(\mathbf{H}_t^h)))}{\sum_{l = 1}^{|\mathcal{B}|} \exp(-d(\mathbf{\Phi}(\mathbf{H}_{l,t}^f), \mathbf{\Phi}(\mathbf{H}_t^h)))} \right]
\]
According to \cite{matthes2023towards}, under mild regularity conditions, if the encoder $f$ minimizes $\mathcal{L}^{(InfoMax)}$, then $h = g \circ f$ is a scaled permutation matrix. This result suggests that when the encoder achieves a minimizer for $\mathcal{L}^{(InfoMax)}$, the encoder function $f$ closely approximates an invertible transformation of $g$. From a causal inference perspective, if $Y_{it}(\omega_{it}) \indep W_{it} \mid \mathbf{H}_{it}$ and $\mathbf{H}_{it} = g(\mathbf{Z}_{it})$, then an invertible function $g \circ f$ ensures that:
\[
Y_{it}(\omega_{it}) \indep W_{it} \mid g \circ f (\mathbf{H}_{it})
\]
Thus, $Y_{it}(\omega_{it}) \indep W_{it} \mid g(\mathbf{C}_{it}^{\mathrm{enc}})$ and since $g$ is invertible, we have:
\[
Y_{it}(\omega_{it}) \indep W_{it} \mid \mathbf{C}_{it}^{\mathrm{enc}}
\]
This demonstrates that the representation $\mathbf{C}_{it}^{\mathrm{enc}}$ retains the essential independence structure, facilitating accurate counterfactual inference.
\subsection{Balanced representation learning}
\paragraph{Motivation}
Our goal is counterfactual regression, specifically estimating
\[
\mathbb{E}\bigl(Y_{t+\rho}(\omega_{t+1:t+\rho}) \mid \mathbf{H}_{t+1}\bigr).
\]
For simplicity, with \(\rho = 1\), we estimate the potential outcome for a given treatment \(W_{t+1} = \omega_{t+1}\), where \(W_{t+1} \in \{0,1,\dots,K-1\}\), expressed as
\[
\mathbb{E}\bigl(Y_{t+1}(\omega_{t+1}) \mid \mathbf{H}_{t+1}\bigr),
\]
which, under standard assumptions, is identified as
\[
\mathbb{E}\bigl(Y_{t+1}(\omega_{t+1}) \mid \mathbf{H}_{t+1}\bigr)
= \mathbb{E}\bigl(Y_{t+1} \mid \mathbf{H}_{t+1}, W_{t+1} = \omega_{t+1}\bigr).
\]

The RHS can be estimated from data as
\[
\mathbb{E}\bigl(Y_{t+1} \mid \mathbf{H}_{t+1}, W_{t+1}\bigr)
= f(\mathbf{H}_{t+1}, W_{t+1}).
\]
Since only one treatment is observed per individual at each time step, \(W_{i,t+1} = \omega_{i,t+1}\), a fitted model \(\hat{f}\) generates counterfactual responses by switching treatments
\[
\hat{f}\bigl(\mathbf{h}_{i,t+1}, \omega_{t+1}'\bigr), \quad \text{where} \ \omega_{t+1}' \neq \omega_{t+1}
\]
(e.g., chemotherapy vs. radiotherapy). 

The challenge is that \(\mathbf{H}_{t+1}\) and \(W_{t+1}\) are not independent, introducing potential bias in counterfactual estimation \citep{robins1999association}, leading to covariate shift or selection bias. To address this, we learn a representation \(\Phi(\mathbf{H}_{t+1})\) that enforces distributional balance during decoding.

\paragraph{Setup} To mitigate selection bias, we leverage the context representation \( \mathbf{C}_t^{\mathrm{enc}} \) of \( \mathbf{H}_t \) and introduce two sub-networks: one for response prediction and one for treatment prediction, both using a mapping of the context representation:
\[
    \mathbf{\Phi}_t = \mathrm{SELU}(\mathrm{Linear}(\mathbf{C}_t^{\mathrm{enc}})) = \Phi_{\theta_R}(\mathbf{H}_t),
\]
where SELU represents the Scaled Exponential Linear Unit \citep{klambauer2017self}, and \( \theta_R \) denotes all parameters of the representation learner, i.e., \( \theta_R = [\theta_1, \theta_2] \). Following \citep{bica2020estimatingCRN, Melnychuk2022CausalTF}, our objective is to learn a representation that accurately predicts outcomes while remaining \emph{distributionally balanced} across all possible treatment choices \( W_t = 0,1,\dots, K-1 \). To achieve this, we frame the problem as an adversarial game: one network learns to predict the next treatment from the representation, while a regularization term ensures that the representation is non-predictive of the treatment.
\begin{landscape}
\begin{figure}[htbp]
    \centering
    \includegraphics[width=0.9\linewidth]{figures/causal_cpc/causal_cpc.pdf}
    \caption{Causal \gls{cpc} architecture: The left shows the encoder, which learns context \(\mathbf{C}_t^{\mathrm{enc}}\) from process history \(\mathbf{H}_t\), with \gls{cpc} and \gls{infomax} objectives used for pretraining. The right shows the decoder, which autoregressively predicts the future outcome sequence from \(\mathbf{C}_t^{\mathrm{enc}}\).}
    \label{fig:ccpc_archi}
\end{figure}
\end{landscape}

\paragraph{Factual response prediction} Since we intend to predict counterfactual responses for \(\rho\) steps ahead in time, we train a decoder to predict the factual responses \(Y_{t+1}, \dots, Y_{t+\rho}\) given the sequence of treatments \((W_{t+1}, \dots, W_{t+\rho})\). We minimize the negative conditional likelihood
\[
\begin{aligned}
\mathcal{L}_Y(\theta_R, \theta_Y)
&= -\log p_{\theta_Y}\bigl(y_{t+1:t+\rho} \mid \mathbf{\Phi}_t, \omega_{t+1:t+\rho}\bigr) \\[0.8ex]
&= -\sum_{j=1}^{\rho} \log p_{\theta_Y}\bigl(y_{t+j} \mid y_{t+1:t+j-1}, \mathbf{\Phi}_t, \omega_{t+1:t+j}\bigr).
\end{aligned}
\]

We denote \(\mathcal{I}_t^j \coloneqq [Y_{t+1:t+j-1}, \mathbf{\Phi}_t, W_{t+1:t+j}]\) and assume a Gaussian distribution for the conditional responses
\[
Y_{t+j} \mid \mathcal{I}_t^j \sim \mathcal{N}\bigl(G_Y(\mathcal{I}_t^j), \sigma^2\bigr),
\]
where \(G_Y\) models the mean of the conditional response (see right side of Figure~\ref{fig:ccpc_archi}). The response sequence is estimated autoregressively using a GRU-based decoder without teacher forcing \citep{williams1989learning} to ensure model training's consistency with testing in real-world scenarios (Figure~\ref{fig:ccpc_archi} and Algorithm~\ref{alg:dec_training}).

\paragraph{Treatment prediction} We learn a treatment prediction sub-network parameterized by $\theta_W$ that takes as input the representation $\mathbf{\Phi}_{t+1}$ and predicts a distribution \( q_{\theta_W}(\omega_{t+1} \mid \mathbf{\Phi}_{t+1}) \) over the treatment \( W_{t+1} \) by minimizing the negative log-likelihood,
\[
\mathcal{L}_{W} = -\log q_{\theta_W}(\omega_{t+1} \mid \mathbf{\Phi}_{t+1}).
\]
To assess the quality of the representation in predicting the treatment, the gradient from \( \mathcal{L}_{W} \) only updates the treatment network parameters \( \theta_W \) and is not backpropagated through the response of the parameters for the representation \( \mathbf{\Phi}_{t+1} \) (Algorithm \ref{alg:dec_training}).

\paragraph{Adversarial learning} To create an adversarial game, we update the representation learning parameters, and in the next step, the treatment network \( q_{\theta_W}(\cdot \mid \mathbf{\Phi}_{t+1}) \) with adverse losses such that the representation \( \mathbf{\Phi}_{t+1} \) becomes invariant with respect to the assignment of \( W_{t+1} \). Different from \gls{sota} models (as highlighted in related work) and in line with our information guidelines principles, learning a balanced representation \( \mathbf{\Phi}_{t+1} \) amounts to ensuring \( \mathbf{\Phi}_{t+1} \indep W_{t+1} \), which is equivalent to \( I(\mathbf{\Phi}_{t+1}, W_{t+1}) = 0 \). Hence, we minimize the \gls{mi}  as a way to confuse the treatment classifier. Specifically, we minimize an upper bound on \( I(\mathbf{\Phi}_{t+1}, W_{t+1}) \), namely the \gls{club} of \gls{mi}  \citep{cheng2020club}.
\begin{equation}
\begin{aligned}
I_{\text{CLUB}}(\Phi(\mathbf{H}_t), W_{t+1}; q_{\theta_W}) &\coloneqq  \mathbb{E}_{\mathbb{P}_{(\Phi(\mathbf{H}_t), W_{t+1})}} 
\left[ \log q_{\theta_W}(W_{t+1} \mid \Phi(\mathbf{H}_{t+1})) \right] \\
&\quad - \mathbb{E}_{\mathbb{P}_{\Phi(\mathbf{H}_t)}}\mathbb{E}_{\mathbb{P}_{W_{t+1}}} 
\left[ \log q_{\theta_W}(W_{t+1} \mid \Phi(\mathbf{H}_{t+1})) \right].
\end{aligned}
\label{eq:ICLUB}
\end{equation}
We use the objective in  Equation (\ref{eq:ICLUB}) to update the representation learner $\Phi(.)$ \citep{brakel2017learning, DeepInfoMax2019}. This update aims to minimize the discrepancy between the conditional likelihood of treatments for units sampled from $\mathbb{P}_{(\mathbf{H}_t, W_{t+1})}$ and the conditional likelihood of treatments under the assumption of independent sampling from the product of marginals $\mathbb{P}_{\mathbf{H}_{t+1}} \otimes \mathbb{P}_{W_{t+1}}$. In practice, we generate samples from the product of marginals by shuffling the treatment $W_{t+1}$ across the batch dimension similar to \cite{brakel2017learning, DeepInfoMax2019}.

When minimizing $\mathcal{L}_W$, $q_{\theta_W}(\omega_{t+1}\mid \mathbf{\Phi}_{t+1})$ gets closer to the true conditional distribution $p(\omega_{t+1}\mid \mathbf{\Phi}_{t+1})$, and, in this case, the objective in Equation (\ref{eq:ICLUB}) provides an upper bound of the \gls{mi}  between representation and treatment. We formalize the intuition by adapting the result of \cite{cheng2020club}:

\begin{theoremBox}\citep{cheng2020club} Let $q_{\theta_W}(\mathbf{\Phi}_{t+1}, \omega_{t+1})  \coloneqq q_{\theta_W}(\omega_{t+1}|\mathbf{\Phi}_{t+1})p(\mathbf{\Phi}_{t+1})$ be the joint distribution induced by $q_{\theta_W}(\omega_{t+1}|\mathbf{\Phi}_{t+1})$ over the representation space of $\mathbf{\Phi}_{t+1}$. If:
\begin{equation*}
\scalebox{0.9}{$
D_{KL}(p(\mathbf{\Phi}_{t+1}, \omega_{t+1})||q_{\theta_W}(\mathbf{\Phi}_{t+1}, \omega_{t+1})) 
\leq D_{KL}(p(\mathbf{\Phi}_{t+1}) p(\omega_{t+1})||q_{\theta_W}(\mathbf{\Phi}_{t+1}, \omega_{t+1})),
$}
\end{equation*}  
then $I(\mathbf{\Phi}_{t+1}, W_{t+1}) \leq I_{CLUB}(\mathbf{\Phi}_{t+1}, W_{t+1}; q).$
\label{thm:ICLUB_bound}
\end{theoremBox}
Based on Theorem \ref{thm:ICLUB_bound}, our adversarial training is interpretable and can be explained as follows: the treatment classifier seeks to minimize $\mathbb{E}_{\mathbb{P}_{(\mathbf{H}_t, W_{t+1})}}\left[\mathcal{L}_W\right]$, which is equivalent to minimizing Kullback-Leibler divergence 
\[
D_{KL}(p(\mathbf{\Phi}_{t+1}, \omega_{t+1})||q_{\theta_W}(\mathbf{\Phi}_{t+1}, \omega_{t+1})). 
\]

Therefore, $q_{\theta_W}(\mathbf{\Phi}_{t+1}, \omega_{t+1})$ could get closer to $p(\mathbf{\Phi}_{t+1}, \omega_{t+1})$ than, ultimately, to $p(\mathbf{\Phi}_{t+1}) p(\omega_{t+1})$, as we train the network to predict $W_{t+1}$ from $\mathbf{\Phi}_{t+1}$. In this case, and by Theorem \ref{thm:ICLUB_bound}, $I_{CLUB}$ provides an upper bound on the MI. Hence, in a subsequent step, we minimize $I_{CLUB}$ w.r.t the representation parameters, minimizing the \gls{mi} $I(\mathbf{\Phi}_{t+1}, W_{t+1})$ and achieving balance. We theoretically formulate such behavior by proving in the following theorem that, at the Nash equilibrium of this adversarial game, the representation is exactly balanced across the different treatment regimes provided by $W_{t+1}$.
\begin{theoremBox}
\label{thm:blancing_iclub}
Let \(t \in \{1, 2, \dots, t_{\max}\}\), \(\Phi = \Phi_{\theta_R}\), and \(q = q_{\theta_W}\) be, respectively, any representation and treatment network. Let \(\mathbb{P}_{\Phi(\mathbf{H}_t)}\) denote the probability distribution over the representation space, and \(\mathbb{P}_{\Phi(\mathbf{H}_t)\mid W_{t+1}}\) its conditional counterpart. Then, there exist \(\Phi^*\) and \(q^*\) such that
\[
\begin{aligned}
\Phi^*
&= \arg\min_{\Phi} I_{\mathrm{CLUB}}\bigl(\Phi(\mathbf{H}_t), W_{t+1}; q^*\bigr), \\[1.5ex]
q^*
&= \arg\max_{q} \mathbb{E}_{\mathbb{P}_{\Phi^*(\mathbf{H}_t)}}
\bigl[\log q\bigl(W_{t+1} \mid \Phi^*(\mathbf{H}_t)\bigr)\bigr].
\end{aligned}
\]

Such an equilibrium holds if and only if
\[
\mathbb{P}_{\Phi(\mathbf{H}_t)\mid W_{t+1}=0}
= \mathbb{P}_{\Phi(\mathbf{H}_t)\mid W_{t+1}=1}
= \dots
= \mathbb{P}_{\Phi(\mathbf{H}_t)\mid W_{t+1}=k-1},
\]
almost surely.
\end{theoremBox}
Since we target multi-timestep forecasting, covariate balancing in the representation space extends beyond \( t+1 \). For simplicity, we presented it for \( t+1 \), but in practice, the adversarial game applies the balancing across all forecasting horizons (Algorithm \ref{alg:dec_training}). The theorem also holds for other horizons by replacing \( \Phi(\mathbf{H}_t) \) with \( \Phi(\mathbf{H}_{t + j -1}) \) and \( W_{t+1} \) with \( W_{t+j} \), for $2 \leq j \leq \rho$.

\subsection[Causal CPC Training]{Causal \gls{cpc} Training} 
The Causal \gls{cpc} model is trained in two stages:
\paragraph{Encoder pretraining:} We first learn an efficient representation of the process history \( \mathbf{C}_t^{\mathrm{enc}}\) by minimizing loss:
\begin{equation*}
\mathcal{L}_{enc} = \mathcal{L}^{CPC}(\theta_{1}, \theta_{2}, \{\Gamma_j\}_{j=1}^{\rho}) + \mathcal{L}^{(InfoMax)}(\theta_{1}, \theta_{2}, \gamma).
\end{equation*}
We train the encoder using only the contrastive terms, as outlined in Algorithm \ref{alg:enc_pretraining}. Our primary objective is to ensure that, for each time step $t$, the process history $\mathbf{H}_{t}$ is predictive of future local features $\mathbf{Z}_t$. However, calculating the \gls{infonce} loss for a batch across all possible time steps $t=0, \dots, t_{\text{max}}$ can be computationally demanding.

To address this, we adopt a more efficient approach by uniformly sampling a single time step $t$ per batch. Subsequently, the corresponding process history $\mathbf{H}_{t}$ is contrasted. The sampled $\mathbf{H}_{t}$ is then employed as input for the \gls{infomax} objective and randomly partitioned into future $\mathbf{H}_t^f$ and past $\mathbf{H}_t^h$ sub-processes.

\begin{algorithm}
    \caption{Pretraining of the encoder}
    \label{alg:enc_pretraining}
    \begin{algorithmic}[1] 
        \REQUIRE Encoder parameters $\theta_{1,2,3}$, learning rate $\mu$
        \STATE \textbf{Input:} data $\{\mathbf{H}_{i, t_{\max}}, i=1,\dots, N \}$
        
        \FOR{$p \in \{1, \dots,\mathrm{epoch}_{\max}\}$}
            \FOR{$\mathcal{B}=\{ \mathbf{H}_{i, t_{\max}}, i=1,\dots, |\mathcal{B}| \}$}
                \STATE $\mathbf{Z}_t = \Phi_{\theta_1}([\mathbf{X}_{t}, W_{t-1}, Y_{t-1}])$ for $t=0, \dots, t_{\max}$.
                
                \COMMENT{Contrastive Predictive Coding (CPC) Objective}
                \STATE Choose $t \sim \mathcal{U}([1, t_{\max}-1])$.
                \STATE Compute $\mathbf{C}_t^{\mathrm{enc}} = \Phi_{\theta_{1},\theta_{2}}(\mathbf{H}_{t})$.
                \STATE Compute $\mathcal{L}^{\mathrm{CPC}}(\theta_{1},\theta_{2}, \{\Gamma_j\}_{j=1}^{\rho})$.
                
                \COMMENT{Information Maximization (InfoMax) Objective}
                \STATE Choose $t_0 \sim \mathcal{U}([1, t])$.
                \STATE Compute $\mathbf{C}_t^{\mathrm{enc},h}=\Phi_{\theta_{1},\theta_{2}}(\mathbf{H}_t^h), \mathbf{C}_t^{\mathrm{enc},f}=\Phi_{\theta_{1},\theta_{2}}(\mathbf{H}_t^f)$.
                \STATE Compute $\mathcal{L}^{(\mathrm{InfoMax})}(\theta_{1},\theta_{2}, \gamma)$.
                
                \COMMENT{Update Parameters}
                \STATE Update parameters:
                $$
                \theta_{1,2,3} \leftarrow \theta_{1,2,3} - \mu \left( \frac{\partial \mathcal{L}^{\mathrm{CPC}}}{\partial \theta_{1,2,3} } + \frac{\partial \mathcal{L}^{(\mathrm{InfoMax})}}{\partial \theta_{1,2,3} } \right )
                $$
            \ENDFOR
        \ENDFOR
        \STATE \textbf{Return}: Trained encoder.
    \end{algorithmic}
\end{algorithm}

\paragraph{Decoder training:} After pretraining, we fine-tune the encoder by optimizing the factual outcome and treatment networks in the adversarial game from Theorem \ref{thm:blancing_iclub}. Formally:
\begin{equation*}
\begin{aligned}
\min_{\theta_{R},\, \theta_{Y}} \, \mathcal{L}_{\mathrm{dec}}(\theta_{R}, \theta_{Y}, \theta_{W})
&= \mathcal{L}_Y(\theta_{R}, \theta_{Y})
+ I_{\mathrm{CLUB}}\bigl(\Phi_{\theta_{R}}(\mathbf{H}_t), W_{t+1}; q_{\theta_{W}}\bigr), \\[1.5ex]
\min_{\theta_{W}} \, \mathcal{L}_{W}(\theta_{W}, \theta_{R})
&= -\mathbb{E}_{\Phi_{\theta_{R}}(\mathbf{H}_t)}
\bigl[\log q_{\theta_{W}}\bigl(W_{t+1} \mid \Phi_{\theta_{R}}(\mathbf{H}_t)\bigr)\bigr].
\end{aligned}
\end{equation*}
The decoder is trained autoregressively without teacher forcing, using the encoder’s output as input (Algorithm \ref{alg:dec_training}). We apply a lower learning rate to the encoder than the decoder’s untrained components. This implies that for each time step $t$, our GRU-based decoder should predict the future sequence of treatments' responses $\hat{Y}_{t+1:t+\rho}$ with its hidden state initialized to the representation $\mathbf{\Phi}_t$ of the historical process up to time $t$.

To enhance training efficiency, instead of predicting $\hat{Y}_{i,t+1:t+\rho}$ for all individuals $i$ in a batch and for all possible time steps $t$, we randomly select $m$ time indices $t_{i,1}, \dots, t_{i,m}$ for each individual $i$. From these indices, we compute future treatment response sequences $\hat{Y}_{i,t_{i,1}+1:t_{i,1}+\rho}, \dots, \hat{Y}_{i,t_{i,m}+1:t_{i,m}+\rho}$. We found that it is enough to train while selecting randomly 10\% of the time steps.

\begin{algorithm}
    \caption{Training of the decoder}
    \label{alg:dec_training}
    \begin{enumerate}
        \item \textbf{Input:} data $\{\mathbf{H}_{i, t_{\max}}\}_{i=1}^{N}$; pretrained encoder parameters $\theta_{1,2,3}$ (including $\theta_R$); decoder parameters $\theta_{4}, \theta_{Y}, \theta_{W}$; learning rates $\mu_{\mathrm{enc}}, \mu_W, \mu_Y$; prediction horizon $\rho$; number of random time indices $m$.
        
        \item \textbf{For} $p = 1$ to $\mathrm{epoch}_{\max}$ \textbf{do}:
        \begin{enumerate}
            \item Sample a mini-batch $\mathcal{B} \subset \{\mathbf{H}_{i, t_{\max}}\}_{i=1}^{N}$.
            
            \item \textbf{Encoding phase (forward pass):}
            \begin{enumerate}
                \item For all $i \in \{1,\dots,|\mathcal{B}|\}$ and $t = 0,\dots,t_{\max}$, compute
                \[
                    \mathbf{C}_{i, t} = \mathrm{encoder}(\mathbf{H}_{i, t}), 
                    \qquad
                    \boldsymbol{\Phi}_{i,t} = \boldsymbol{\Phi}_{\theta_R}(\mathbf{H}_{i,t}).
                \]
            \end{enumerate}
            
            \item \textbf{Decoding and prediction phase:}
            \begin{enumerate}
                \item For each $i = 1,\dots,|\mathcal{B}|$:
                \begin{enumerate}
                    \item Sample $t_{i,1}, \dots, t_{i,m} \sim \mathcal{U}\big(\{1, \dots, t_{\max}-\rho\}\big)$.
                    \item For each $t \in \{t_{i,1}, \dots, t_{i,m}\}$, compute
                    \[
                        \hat{Y}_{i,t+1:t+\rho},\;
                        \hat{W}_{i,t+1:t+\rho},\;
                        \boldsymbol{\Phi}_{i,t+1:t+\rho-1}
                        = \mathrm{decoder}\!\left(
                            \boldsymbol{\Phi}_{i,t},\,
                            \mathbf{V}_i,\,
                            W_{i,t},\,
                            Y_{i,t},\,
                            W_{i,t+1:t+\rho}
                        \right).
                    \]
                \end{enumerate}
            \end{enumerate}
            
            \item \textbf{Loss calculation:} compute
            \[
                \mathcal{L}_{\mathrm{dec}}(\theta_{R}, \theta_{Y}, \theta_{W}), 
                \qquad
                \mathcal{L}_{W}(\theta_{W}, \theta_{R}).
            \]
            
            \item \textbf{Parameter updates (sequential optimization):}
            \begin{enumerate}
                \item Update encoder parameters $\theta_{1,2,3}$ (via $\theta_R$):
                \[
                    \theta_{1,2,3} \leftarrow \theta_{1,2,3} 
                    - \mu_{\mathrm{enc}} 
                    \frac{\partial \mathcal{L}_{\mathrm{dec}}(\theta_{R}, \theta_{Y}, \theta_{W})}
                           {\partial \theta_{1,2,3}}.
                \]
                
                \item Update decoder and outcome parameters $\theta_{4}$, $\theta_{Y}$:
                \[
                    \theta_{4} \leftarrow \theta_{4} 
                    - \mu_{Y} 
                    \frac{\partial \mathcal{L}_{\mathrm{dec}}(\theta_{R}, \theta_{Y}, \theta_{W})}
                           {\partial \theta_{4}},
                    \qquad
                    \theta_{Y} \leftarrow \theta_{Y} 
                    - \mu_{Y} 
                    \frac{\partial \mathcal{L}_{\mathrm{dec}}(\theta_{R}, \theta_{Y}, \theta_{W})}
                           {\partial \theta_{Y}}.
                \]
                
                \item Update treatment parameters $\theta_{W}$:
                \[
                    \theta_{W} \leftarrow \theta_{W} 
                    - \mu_{W} 
                    \frac{\partial \mathcal{L}_{W}(\theta_{W}, \theta_{R})}
                           {\partial \theta_{W}}.
                \]
            \end{enumerate}
        \end{enumerate}
        
        \item \textbf{Return} the trained decoder (and updated encoder).
    \end{enumerate}
\end{algorithm}

\section{Experiments}
\label{sect_ccpc:experiments}
We compare Causal \gls{cpc} with \gls{sota} baselines: MSMs \cite{robins2000MSM}, RMSN \cite{lim2018RMSN}, CRN \cite{bica2020estimatingCRN}, G-Net \cite{Li2021GNetAR}, and CT \cite{Melnychuk2022CausalTF}. All models are fine-tuned via a grid search over hyperparameters, including architecture and optimizers. Model selection is based on mean squared error (MSE) on factual outcomes from a validation set, and the same criterion is used for early stopping. 

All models were implemented using PyTorch \citep{Paszke2019PyTorchAI} and PyTorch Lightning \citep{Falcon_PyTorch_Lightning_2019}. In contrast to the approach in \cite{Melnychuk2022CausalTF}, we employed early stopping for all models. The stopping criterion was the Mean Squared Error over factual outcomes for a dedicated validation dataset. Specifically, for the Causal \gls{cpc} encoder, the stopping criterion was determined by the encoder's validation loss. While all models in the benchmark were trained using the Adam optimizer \citep{kingma2014adam}, we opted for training Causal \gls{cpc} (encoder plus decoder without the treatment subnetwork) with AdamW \citep{loshchilov2017AdamW} due to its observed stability during training. Similar to the common practice in training GAN discriminators, the treatment subnetwork was optimized using SGD with momentum \citep{sutskever2013importance}. The CT employed the Exponential Moving Average (EMA) \citep{yaz2018} of parameters to enhance training stability. However, this technique was not applied to Causal \gls{cpc}, as experimental evidence suggested only marginal improvements. Weight decay was set to zero for all models. Details on hyperparameters selection per model are provided in Appendix \ref{appendix_ccpc:huperparams_details}. We set $\sigma = 0.05$ throughout our experiments.

\subsection{Experiments with Synthetic Data}
\paragraph{Tumor Growth} 
We use the PharmacoKinetic-PharmacoDynamic (PK-PD) model \cite{PK-PD} to simulate responses of non-small cell lung cancer patients, following previous works \citep{lim2018RMSN, bica2020estimatingCRN, Melnychuk2022CausalTF}. In this simulation, we model the evolution of tumor volume, denoted as $V(t)$, in discrete time, with $t$ representing the number of days since diagnosis:
$$
V(t) = \left(1 + \underbrace{\Lambda \log \left(\frac{K}{V(t-1)}\right)}_{\text{Tumor Growth}} - \underbrace{\kappa_c C(t)}_{\text{Chemotherapy}} - \underbrace{\left(\kappa_{rd} Rd(t) + \upsilon Rd(t)^2\right)}_{\text{Radiation}} + \underbrace{e_t}_{\text{Noise}}\right) V(t-1)
$$
Here, the model parameters $\Lambda, K, \kappa_c, \kappa_{rd}, \upsilon$ are sampled for each patient based on prior distributions from \cite{PK-PD}. Additionally, $Rd(t)$ represents the radiation dose applied at time $t$, and $\mathrm{C}(t)$ denotes the drug concentration. 

We introduce confounding into the radiotherapy/chemotherapy treatment assignment by making it dependent on the evolution of the tumor volume. Treatment is simulated using a Bernoulli distribution with probability $\sigma(\pi_t)$, where:
$$
\pi_t = \frac{\gamma}{D_{\max}}\left(\bar{D}(t) - \delta\right)
$$
Here, $\bar{D}(t)$ represents the average tumor diameter over the last 15 days, and $D_{\max}=13~\mathrm{cm}$ is the maximum tumor diameter. The parameter $\delta$ is set to $\delta=D_{\max}/2$. The parameter $\gamma$ controls the level of time-dependent confounding; a higher value of $\gamma$ gives more weight to the history of tumor diameter in treatment assignment. 

We evaluate our approach on simulated counterfactual trajectories, varying the confounding level via the parameter \( \gamma \). Unlike \cite{Melnychuk2022CausalTF}, who used larger datasets (10,000 for training, 100 for validation, 1,000 for testing), we use a smaller, more challenging dataset (1,000 for training, 100 for validation, 500 for testing) to reflect real-world data limitations. Similar to \citet{bica2020estimatingCRN, Melnychuk2022CausalTF}, counterfactual trajectories are generated with a single treatment per trajectory while the treatment slides over the forecasting range to generate multiple trajectories. We set the prediction horizon to 10 and evaluate two training sequence lengths, 60 and 40, with covariates of dimension 4.

\begin{figure}[ht]
  \centering
  \begin{subfigure}[b]{0.3\textwidth}
    \centering
    \includegraphics[width=\linewidth]{figures/causal_cpc/prf_cancer_sim_gamma1.pdf}
    \caption{$\gamma =1$, sequence length 60}
    \label{fig:gamma1_seq60}
  \end{subfigure}
  \hfill
  \begin{subfigure}[b]{0.3\textwidth}
    \centering
    \includegraphics[width=\linewidth]{figures/causal_cpc/prf_cancer_sim_gamma2.pdf}
    \caption{$\gamma =2$, sequence length 60}
    \label{fig:gamma2_seq60}
  \end{subfigure}
  \hfill
  \begin{subfigure}[b]{0.3\textwidth}
    \centering
    \includegraphics[width=\linewidth]{figures/causal_cpc/prf_cancer_sim_gamma3.pdf}
    \caption{$\gamma =3$, sequence length 60}
    \label{fig:gamma3_seq60}
  \end{subfigure}
  
  \vspace{0.5cm} 

  \begin{subfigure}[b]{0.3\textwidth}
    \centering
    \includegraphics[width=\linewidth]{figures/causal_cpc/prf_cancer_sim_seq40_gamma1.pdf}
    \caption{$\gamma =1$, sequence length 40}
    \label{fig:gamma1_seq40}
  \end{subfigure}%
  \hfill
  \begin{subfigure}[b]{0.3\textwidth}
    \centering
    \includegraphics[width=\linewidth]{figures/causal_cpc/prf_cancer_sim_seq40_gamma2.pdf}
    \caption{$\gamma =2$, sequence length 40}
    \label{fig:gamma2_seq40}
  \end{subfigure}%
  \hfill
  \begin{subfigure}[b]{0.3\textwidth}
    \centering
    \includegraphics[width=\linewidth]{figures/causal_cpc/prf_cancer_sim_seq40_gamma3.pdf}
    \caption{$\gamma =3$, sequence length 40}
    \label{fig:gamma3_seq40}
  \end{subfigure}
\caption{Evolution of error \gls{nrmse} in estimating counterfactual responses for cancer simulation data. Top: training sequence length 60. Bottom: training sequence length 40. In both cases, $\rho=10$. MSM is excluded due to high prediction errors.}
  \label{fig:combined_cancer_sim}
\end{figure}

\paragraph{Results} We tested all models on the cancer simulation data across three confounding levels, \( \gamma = 1, 2, 3 \). Figures \ref{fig:gamma1_seq60}, \ref{fig:gamma2_seq60} and \ref{fig:gamma3_seq60} show the evolution of \gls{nrmse} over counterfactual tumor volume as the prediction horizon increases. Causal \gls{cpc} consistently outperforms all baselines at larger horizons, demonstrating its effectiveness in long-term predictions. This confirms the quality of \( \mathbf{C}_{t} \) in predicting future components across multiple time steps, capturing the global structure of the process as discussed in  Equation (\ref{eq:MI_lb_avg}). We report in Table \ref{tab:benchmark_few_data_cancer} the detailed counterfactual errors for Causal \gls{cpc} and baselines over the cancer simulation dataset, which are responsible for Figure \ref{fig:combined_cancer_sim}.

\begin{table}[!htbp]
\centering
\caption{Results on the synthetic data set with training sequence length 60: mean$\pm$standard deviation of \gls{nrmse}. The best value for each metric is given in bold: smaller is better.}
\label{tab:benchmark_few_data_cancer}
\resizebox{\textwidth}{!}{
\begin{tabular}{|c|c|c|c|c|c|c|c|c|c|c|}
\hline  
\multicolumn{11}{|c|}{$ \gamma =1$} \\
\hline
Model & $\rho = 1$ & $\rho = 2$& $\rho = 3$& $\rho = 4$& $\rho = 5$& $\rho = 6$& $\rho = 7$& $\rho = 8$& $\rho = 9$ & $\rho = 10$\\ 
\hline  
\textbf{Causal \gls{cpc} (ours)} & \textbf{0.83$\pm$ 0.06}& \textbf{0.86 $\pm$ 0.09}& \textbf{0.94$\pm$ 0.09}& \textbf{0.97$\pm$ 0.08}& \textbf{1.03$\pm$ 0.10}& \textbf{1.07 $\pm$ 0.10}& \textbf{1.12$\pm$ 0.10}& \textbf{1.17 $\pm$ 0.09}& \textbf{1.22$\pm$ 0.08}& \textbf{1.26$\pm$ 0.08}\\
\hline  
\textbf{Causal Transformer} & 0.99$\pm$ 0.13& 0.92 $\pm$ 0.14& 0.98$\pm$ 0.14& 1.05$\pm$ 0.15& 1.11 $\pm$ 0.18 & 1.11 $\pm0.11$& 1.21 $\pm$ 17& 1.26$\pm$ 0.16& 1.31 $\pm$ 0.005& 1.35$\pm$ 0.16\\ 
\hline 
 \textbf{G-Net} & 0.91$\pm$0.15& 1.1$\pm$0.16& 1.24$\pm$0
16& 1.33$\pm$0.17& 1.40$\pm$0.18& 1.47$\pm$0.19& 1.52$\pm$0.18& 1.57$\pm$0.22& 1.63$\pm$0.22&1.7$\pm$0.25\\ \hline 
 \textbf{CRN}    & 0.84$\pm$0.10& 0.83$\pm$0.09& 0.92$\pm$0.10& 1.00$\pm$0.11& 1.09$\pm$0.12& 1.17$\pm$0.14& 1.25$\pm$0.16& 1.32$\pm$0.18& 1.37$\pm$0.23&1.43$\pm$0.26\\ \hline 
 \textbf{RMSN}   & 0.99$\pm$0.13& 0.91$\pm$0.04& 1.30$\pm$0.65& 1.43$\pm$0.76& 1.56$\pm$0.83& 1.66$\pm$0.88& 1.73$\pm$0.91& 1.77$\pm$0.89& 1.81$\pm$0.88&1.84$\pm$0.86\\ \hline 
 \textbf{MSM}   & 1.20$\pm$0.10& 1.83$\pm$0.26& 2.07$\pm$0.44& 2.38$\pm$0.44& 2.54$\pm$0.45& 2.90$\pm$0.37& 3.01$\pm$.38& 3.06$\pm$0.36& 3.08$\pm$0.36&3.08$\pm$0.36\\\hline 
\multicolumn{11}{|c|}{$ \gamma = 2$} \\
\hline
\textbf{Causal \gls{cpc} (ours)} & 1.16$\pm$ 0.22& \textbf{0.91 $\pm$ 0.10}& \textbf{0.95 $\pm$ 0.13}& \textbf{1.00 $\pm$ 0.15}& \textbf{1.07$\pm$ 0.19}& \textbf{1.17 $\pm$ 0.24}& \textbf{1.27 $\pm$ 0.25}& \textbf{1.38 $\pm$ 0.28}& \textbf{1.49 $\pm$ 0.30}& \textbf{1.60 $\pm$ 0.34}\\ \hline  

\textbf{Causal Transformer} & 1.24$\pm$0.20& 1.13$\pm$0.15& 1.27$\pm$021& 1.36$\pm$0.28& 1.44$\pm$0.29& 1.55$\pm$0.27& 1.64$\pm$0.28& 1.69$\pm$0.20& 1.74$\pm$0.28& 1.77 $\pm$ 0.29\\ 
\hline
 \textbf{G-Net}& \textbf{1.05$\pm$0.21}& 1.05$\pm$0.08& 1.26$\pm$0.16& 1.38$\pm$0.23& 1.48$\pm$0.27& 1.57$\pm$0.31& 1.64$\pm$0.33& 1.70$\pm$0.36& 1.75$\pm$0.39&1.8$\pm$0.42\\\hline
 \textbf{CRN}& 1.25$\pm$0.25& 1.08$\pm$0.06& 1.14$\pm$0.12& 1.21$\pm$0.17& 1.30$\pm$ 0.21& 1.41$\pm$0.25& 1.54$\pm$0.32& 1.67$\pm$0.41& 1.8$\pm$0.51&1.92$\pm$0.63\\\hline
 \textbf{RMSN}& 1.47$\pm$0.27& 1.33$\pm$0.25& 1.30$\pm$0.23& 1.33$\pm$0.24& 1.38$\pm$0.26& 1.45$\pm$0.28& 1.52$\pm$0.31& 1.60$\pm$0.25& 1.67$\pm$0.38&1.75$\pm$0.42\\\hline
 \textbf{MSM}& 1.43$\pm$0.27& 2.22$\pm$0.53& 2.67$\pm$0.63& 2.98$\pm$0.70& 3.19$\pm$0.74& 3.33$\pm$0.77& 3.41$\pm$0.79& 3.44$\pm$0.25& 3.45$\pm$0.78&3.34$\pm$0.77\\\hline
 \multicolumn{11}{|c|}{$ \gamma = 3$} \\
 \hline
  \textbf{Causal \gls{cpc} (ours)} & 1.37$\pm$0.31& \textbf{1.16$\pm$0.27}& \textbf{1.26$\pm$0.30}& \textbf{1.38$\pm$0.35}& \textbf{1.53$\pm$0.40}& \textbf{1.69$\pm$0.47}&\textbf{ 1.84$\pm$0.52}& \textbf{2.00$\pm$0.51}& 2.14$\pm$0.61& 2.28$\pm$0.66\\ 
   \hline
 \textbf{Causal Transformer} & 1.36$\pm$0.32& 1.42$\pm$0.36& 1.62$\pm$0.46& 1.78$\pm$0.53& 1.89$\pm$0.58& 2.01$\pm$0.63& 2.13$\pm$0.66& 2.22$\pm$0.69& 2.31$\pm$0.69& 2.37$\pm$0.73\\ 
\hline
\textbf{G-Net} &\textbf{ 1.14$\pm$0.24}& 1.22$\pm$0.15& 1.54$\pm$0.26& 1.77$\pm$0.33& 1.94$\pm$0.36& 2.09$\pm$0.40& 2.23$\pm$0.43& 2.34$\pm$0.47& 2.44$\pm$0.52& 2.52$\pm$0.56\\ 
\hline
 \textbf{CRN}& 1.46$\pm$0.29& 1.54$\pm$0.38& 1.70$\pm$0.48& 1.79$\pm$0.53& 1.86$\pm$0.92& 1.92$\pm$0.58& 1.98$\pm$0.59& 2.04$\pm$0.61& \textbf{2.10$\pm$0.63}&\textbf{2.16$\pm$0.64} \\\hline
 
\textbf{RMSN}& 1.22$\pm$0.26& 1.28$\pm$0.29& 1.43$\pm$0.40& 1.56$\pm$0.48& 1.70$\pm$0.53& 1.83$\pm$0.57& 1.95$\pm$0.59& 2.06$\pm$0.61& 2.14$\pm$0.61&2.21$\pm$0.61\\\hline
  
 \textbf{MSM} & 1.70$\pm$0.35& 2.73$\pm$0.88& 3.22$\pm$1.03& 3.25$\pm$1.12& 3.71$\pm$1.18& 3.85$\pm$1.22& 3.91$\pm$1.23& 3.95$\pm$1.24& 3.96$\pm$1.24&3.94$\pm$1.23\\\hline
 \end{tabular}
 }
\end{table}

In the more challenging case where the maximum sequence length is 40 (Figures \ref{fig:gamma1_seq40}, \ref{fig:gamma2_seq40} and \ref{fig:gamma3_seq40}), the error evolution remains similar to Figure \ref{fig:gamma1_seq60}, \ref{fig:gamma2_seq60} and \ref{fig:gamma3_seq60}. Our model maintains its advantage, outperforming most baselines in long-term forecasting. However, Causal \gls{cpc} does not outperform other models in short-term forecasting, a consistent limitation across experiments. Still, the model's superior long-term performance highlights its potential in applications requiring long-term accuracy. At higher confounding levels, the model does not always outperform \gls{sota} models at certain time steps. This may be due to the low dimensionality of the time-varying components and static covariates, \( \mathbf{F}_{t} = [\mathbf{V}, \mathbf{X}_{t}, W_{t-1}, Y_{t-1}] \), which have only four dimensions. Our model leverages contrastive learning-based regularization to excel on datasets with higher confounding dimensions, as demonstrated on \gls{mimic}-III where \( \mathbf{F}_{t} \) has 72 dimensions. In this setting, our model consistently outperforms baselines at longer prediction horizons. The occasional underperformance of Causal \gls{cpc} at the final horizon is due to $\rho=10$ being the last contrasted horizon, not an issue specific to $\rho=10$. To support this, we reran all models with a sequence length 60, $\rho=15$, and $\gamma=2$. As shown in Figure \ref{fig:gamma2_seq60_tau15}, Causal \gls{cpc} still outperforms \gls{sota} for horizons beyond $\rho=10$ due to the encoder's retraining, where the \gls{infonce} loss is computed over all 15 time steps. The last prediction error remains close to \gls{sota}, suggesting that training over larger horizons than initially intended may be beneficial.

\begin{figure}
     \centering
    \includegraphics[width = 0.48\textwidth, height = 0.20\textheight]{figures/causal_cpc/prf_cancer_sim_tau15_gamma2.pdf}
    \caption{Models' performance for cancer simulation reported by \gls{nrmse} for $\gamma=2$ and $\rho=15$. The training sequence length is 60.}
  \label{fig:gamma2_seq60_tau15}
\end{figure}

\subsection{Experiments with semi-synthetic and real data}
\label{subsect_ccpc:core_exp_mimic}
\paragraph{Semi-synthetic \gls{mimic}-III} We used a semi-synthetic dataset constructed by \cite{Melnychuk2022CausalTF} based on the \gls{mimic}-III dataset \citep{johnson2016mimic}, incorporating both endogenous temporal dependencies and exogenous dependencies from observational patient trajectories. Initially, a cohort of 1,000 patients is extracted from the \gls{mimic}-III data, and the simulation proposed by \cite{Melnychuk2022CausalTF} extends that of \cite{schulam2017reliable}.

\paragraph{Step\,1: untreated trajectories} Let $d_y$ be the dimension of the outcome variable, in the case of multiple outcomes, then untreated outcomes, denoted as $Y_t^{j,(i)}(0), j=1, \ldots, d_y$ are generated for each patient $i$ within the cohort as 
\begin{equation}
\label{eq:untreated_new}
Y_t^{j,(i)}(0)
=
\alpha_{\text{spl}}^{j}\,B(t)
+\alpha_{\text{gp}}^{j}\,g^{j,(i)}(t)
+\alpha_{\text{exo}}^{j}\,f^{j}_{\text{RFF}}\!\bigl(\mathbf X_t^{(i)}\bigr)
+\varepsilon_t,\qquad
\varepsilon_t\sim\mathcal N(0,\sigma_\varepsilon^{2})
\end{equation}
where the B–spline \(B(t)\) is an endogenous component, \(g^{j,(i)}\) is sampled independently for each patient from a Gaussian process with a Matérn kernel i.e.\(g^{j,(i)}\sim\mathcal{GP}(0,k_{\text{Matérn}})\), and  \(f^{j}_{\text{RFF}}\) is a Random-Fourier-Features (RFF) draw.

\paragraph{Step\,2: treatment assignment.}
To introduce confounding in the treatment assignment, we incorporate current time-varying covariates through a random function $f_Y^l\left(\mathbf{X}_t\right)$ and the average of the subset of the previous $T_l$ treated outcomes. For $K$ binary treatments $\mathbf{W}_t^l, l=0, \ldots, K-1,$ the assignment mechanism is modeled as follows: let \(\pi_{t,\omega}^{(i)}:=\Pr\!\bigl(\mathbf{W}_t^{(i)}=\omega\bigr)\) for \(\omega=0,\dots,K-1\). We use a soft-max with confounding via outcomes and covariates:
\begin{align}
\label{eq:softmax_logits}
\tilde\eta_{t,\omega}^{(i)}
&\;=\;
\gamma_{W}^{\omega}\,\bar Y_{t-1}^{(i)}
+\gamma_{X}^{\omega}\,f_{Y}^{\omega}\!\bigl(\mathbf X_t^{(i)}\bigr)+b_w,
\quad \omega=0,\dots,K-1,\\
\eta_{t,0}^{(i)}&:=0,\qquad
\pi_{t,\omega}^{(i)}=\frac{\exp\!\bigl(\eta_{t,\omega}^{(i)}\bigr)}
                    {\sum_{b=0}^{K-1}\exp\!\bigl(\eta_{t,b}^{(i)}\bigr)},\\
W_t^{(i)} &\sim\operatorname{Categorical}
            \bigl(\pi_{t,0}^{(i)},\dots,\pi_{t,K-1}^{(i)}\bigr),
\end{align}
where   \(\bar Y_{t-1}^{(i)}=\frac1{T_0}\sum_{s=t-T_0}^{t-1}Y_s^{j^\star,(i)}\).

\paragraph{Step\,3: cumulative treatment effect.} With window length \(w\) and per-label effect sizes \(\beta_{\omega j}\), we define treatment effects as 
 \begin{equation}
\label{eq:cupexp}
\tau_{t,\omega }^{j,(i)}
=
\sum_{s=t-w}^{t}
  \frac{\mathbf 1_{\{W_s^{(i)}=\omega \}}
        \,\pi_{s,\omega }^{(i)}\,\beta_{\omega j}}
       {(w-s)^2},
\qquad \omega =0,\dots,K-1.
\end{equation}

\paragraph{Step\,4: observed outcomes (consistency).}
\begin{equation}
Y_t^{j,(i)}
=
Y_t^{j,(i)}\!\bigl(0\bigr)
+
\sum_{\omega =0}^{K-1}
  \mathbf 1_{\{W_t^{(i)}=\omega \}}\,
  \tau_{t,\omega}^{j,(i)}.
\label{eq:observed_new}
\end{equation}
Similar to the cancer simulation, the training data consisted of relatively few sequences (500 for training, 100 for validation, and 400 for testing). Table \ref{tab:perf_mimic_few_data} presents counterfactual predictions' mean and standard deviation across multiple horizons ($\rho = 10$). Counterfactual trajectories are generated so that treatment is generated randomly at each time step. As in the tumor growth experiments, we tested two maximum sequence lengths, 100 and 60, to assess the models' robustness for long-horizon forecasting.

\begin{table*}[t]
 \caption{Results on the \gls{mimic}-III semi-synthetic reported by mean$\pm$standard deviation of RMSEs. The training sequence length is 100. Smaller is better.}
 \centering
\resizebox{\textwidth}{!}{%
\begin{tabular}{|c |c |c |c |c |c |c |c |c |c |c|} 
\hline
Model       & $\rho = 1$   &   $\rho = 2$& $\rho = 3$&   $\rho = 4$&  $\rho = 5$&   $\rho = 6$& $\rho = 7$&  $\rho = 8$&   $\rho = 9$ & $\rho = 10$\\ \hline  
\textbf{Causal \gls{cpc} (ours)}  &  0.32$\pm 0.04$&   0.45$ \pm 0.08$& 0.54$\pm 0.06$& 0.61 $\pm 0.10$&   \textbf{0.66$ \pm$ 0.10}&  \textbf{0.69$\pm$0.11}&   \textbf{0.71$ \pm$ 0.11}& \textbf{0.73$\pm $ 0.06}& \textbf{0.75 $\pm$ 0.05}& \textbf{0.77$ \pm$ 0.10} \\ 
\hline  
\textbf{CT} &  $0.42\pm0.38$&   \textbf{0.40$\pm$ 0.06}& \textbf{0.52$\pm$ 0.08}& \textbf{0.60$\pm$ 0.005}&  0.67$ \pm 0.10$  & 0.72 $\pm0.12$&   0.77$ \pm 0.13$ & 0.81$\pm 0.14$ &0.85 $\pm 0.16$&  0.88 $\pm $0.17   \\ 
\hline  
\textbf{G-Net} &  $0.54\pm0.13$&   0.72$ \pm 0.14$& 0.85 $\pm$0.16& 0.96 $\pm$ 0.17&  1.05 $\pm$ 0.18& 1.14 $\pm$0.18&   1.24$ \pm$ 0.17& 1.33$\pm 0.16$ & 1.41 $\pm$ 0.16&  1.49$ \pm $0.16\\ 
\hline  
\textbf{CRN} &  \textbf{0.27 $\pm$0.03}&   0.45$ \pm 0.08$& 0.58 $\pm$ 0.09& 0.72$\pm$ 0.11&   0.82$\pm$ 0.15& 0.92 $\pm$ 0.20&   1.00 $\pm$ 0.25& 1.06 $\pm$ 0.28& 1.12 $\pm$ 0.32&  1.17 $\pm$ 0.35\\ 
\hline  
\textbf{RMSN} &  0.40 $\pm$ 0.16&   0.70 $\pm$ 0.21& 0.80$\pm$ 0.19& 0.88 $\pm$ 0.17&   0.94 $\pm$ 0.16& 1.00 $\pm$ 0.15&  1.05 $\pm$ 0.14& 1.10 $\pm$ 0.14& 1.14 $\pm$ 0.13& 1.18 $\pm$ 0.13 \\ 
\hline  
 \end{tabular}
 }
\label{tab:perf_mimic_few_data}
\end{table*}
\vspace{-0.4cm} 

\paragraph{Results} Causal \gls{cpc} consistently outperformed the baselines, especially at larger horizons, both with a sequence length of 100 and a reduced length of 60 (Figures \ref{tab:perf_mimic_few_data}, \ref{fig:prf_mimic_seq_60}). Its superior performance at longer horizons is likely due to the high number of covariates, making it well-suited to contrastive-based training. We also tested the models with 800/200/200 individuals for training/validation/testing, as in \cite{Melnychuk2022CausalTF} (Appendix \ref{appendix_ccpc:results_orig_mimic}), where Causal \gls{cpc} achieved \gls{sota} results comparable to CT but with much shorter training and prediction times.
\begin{figure}
     \vspace{17pt}
     \centering
    \includegraphics[width = 0.48\textwidth, height = 0.20\textheight]{figures/causal_cpc/prf_mimic_seq_60.pdf}
    \caption{Performance for MIMIC II semi-synthetic reported by RMSE over 10 forecasting horizons. The sequence training length is 60.}
  \label{fig:prf_mimic_seq_60}
\end{figure}


\paragraph{Computational Efficiency and Model Complexity} 
Efficient execution is crucial for practical deployment, especially with periodic retraining. Beyond training, challenges arise in evaluating multiple counterfactual trajectories per individual, which grow exponentially with the forecasting horizon as $K^{\rho}$, where $K$ is the number of possible treatments. This is particularly relevant when generating multiple treatment plans, such as minimizing tumor volume. Tables \ref{tab:complexity_running_time_cancer} and \ref{tab:complexity_running_time_mimic} show the models' complexity (number of parameters) and running time, split between model fitting and prediction for cancer simulation data and \gls{mimic}-III. Causal \gls{cpc} is highly efficient during prediction due to its simple 1-layer \gls{gru}, similar to CRN (1-layer \gls{lstm}), while also outperforming it. In contrast, CT is less efficient due to its transformer architecture and teacher forcing, which requires recursive data loading during inference. G-Net also has longer prediction times due to Monte Carlo sampling. Overall, Causal \gls{cpc} strikes a strong balance between accuracy and efficiency, making it well-suited under constrained resources.

\begin{table}[htbp]
\centering
\caption{Models complexity and the running time averaged over five seeds. Results are reported for tumor growth simulation ($\gamma =1$). Hardware: GPU-1xNVIDIA Tesla M60.}
\label{tab:complexity_running_time_cancer}
\resizebox{0.7\textwidth}{!}{%
\begin{tabular}{lccccr}
\toprule
Model & Trainable parameters (k) & Training time (min) & Prediction time (min) \\
\midrule
\textbf{Causal \gls{cpc} (encoder + decoder)} & 8.2 & 16$\pm$ 3 &  4 $\pm$ 1 \\
\textbf{CT} & 11 & 12$\pm$ 2 & 30$\pm$ 3 \\
\textbf{G-Net} & 1.2 & 2 $\pm$ 0.5 & 35 $\pm$ 3 \\
\textbf{CRN} & 5.2 & 13$\pm$ 2 & 4$\pm$ 1 \\
\textbf{RMSN} & 1.6 & 22$\pm$ 2 & 4$\pm$ 1 \\
\textbf{MSM} & \textbf{$<$0.1} & \textbf{1$\pm$0.5} & \textbf{1$\pm$0.5} \\
\bottomrule
\end{tabular}
}
\end{table}

\begin{table}[!htbp]
\caption{The number of parameters to train for each model after hyper-parameters fine-tuning and the corresponding running time averaged over five seeds. Results are reported for semi-synthetic \gls{mimic}-III data; the processing unit is GPU-1 x NVIDIA Tesla M60 .}
\label{tab:complexity_running_time_mimic}
\vskip 0.15in
\begin{center}
\begin{small}
\begin{sc}
\resizebox{0.7\textwidth}{!}{%
\begin{tabular}{lccccr}
\toprule
Model & trainable parameters (k) & Training time (min) & Prediction time (min) \\
\midrule
\textbf{Causal \gls{cpc} (ours)} & \textbf{9.8}  & 12$\pm$2  & \textbf{4$\pm$1} \\
\textbf{Causal Transformer } &12  & 14$\pm$1  & 38$\pm$2  \\
\textbf{G-Net} & 14.7 &  \textbf{7$\pm$1} &40$\pm$3 \\
\textbf{CRN} &  15.1 & 21$\pm$2  & 5$\pm$1  \\
\textbf{RMSN} & 20 & 48$\pm$4  & 5$\pm$1  \\
\bottomrule
\end{tabular}
}
\end{sc}
\end{small} 
\end{center}
\vskip -0.1in
\end{table}

\paragraph{Real \gls{mimic}-III Data}
We evaluated our model on real \gls{mimic}-III data, where counterfactual trajectories cannot be assessed due to the absence of observed counterfactual responses. However, performance can still be measured by forecasting factual (observed) responses over time. Our model estimates responses for each individual based on their observed treatment trajectory. As shown in Figure \ref{fig:prf_mimic_real}, Causal \gls{cpc} consistently outperforms all baselines, especially at larger horizons, demonstrating its robustness and effectiveness in real-world settings.
\begin{figure}
     \vspace{-10pt}  
     \centering
     \includegraphics[width=0.48\textwidth, height=0.20\textheight]{figures/causal_cpc/prf_mimic_real.pdf}
     \caption{Factual estimation errors for baselines for Real \gls{mimic}-III data reported by RMSE. The training sequence length is 100.}
     \label{fig:prf_mimic_real}
\end{figure}

\section{Discussion}
\paragraph{Why does Causal \gls{cpc} outperform \gls{sota} at large horizons?}  
Our context \(\mathbf{C}_t^{\mathrm{enc}}\) is designed to capture shared information across future representations, particularly covariates, by minimizing the \gls{infonce} loss over multiple time steps ( Equation \ref{eq:infonce_loss_cpc}). As shown in  Equation (\ref{eq:MI_lb_avg}), minimizing \(\mathcal{L}^{CPC}\) maximizes shared information between the context and future components, helping capture the \emph{global structure} of the process. This is especially beneficial for counterfactual regression over long horizons, explaining the model's superior performance. However, it may not consistently outperform \gls{sota} in shorter-term predictions due to its focus on long-term dependencies.

\paragraph{Short-term Counterfactual Regression}  
While our model is designed for long-term predictions, it may not consistently outperform \gls{sota} for short-horizon tasks. However, the use of contrastive loss, particularly \gls{infonce} ( Equation \ref{eq:cpc_loss}), suggests potential adaptability to balance both short- and long-term predictions without retraining. A trade-off could be achieved by adjusting the contrastive term weights across time steps in  Equation (\ref{eq:cpc_loss}), which we leave for future work.

\paragraph{Ablation study} 
We examined the model's performance in various configurations—full model, without \gls{cpc}, and without \gls{infomax}. Table \ref{tab:ablation_study} shows that removing either term reduces counterfactual accuracy across all horizons, underscoring their significance. Additionally, replacing our ICLUB objective with CDC loss \citep{Melnychuk2022CausalTF} or removing balancing increases errors. We report the detailed experimental results over \gls{mimic}-III in Table \ref{tab:mimic_ablation_details} and for cancer simulation in Table \ref{tab:ablation_study}.

\begin{figure}
     \centering
    \includegraphics[width = 0.48\textwidth, height = 0.20\textheight]{figures/causal_cpc/prf_mimic_ablation_core.pdf}
    \caption{Ablation study of Causal \gls{cpc} for \gls{mimic}-III dataset. RMSE is reported for 10 forecasting horizons. Smaller is better.}
  \label{fig:prf_mimic_ablation_core}
\end{figure}

\begin{table}[htbp]
\centering
\caption{Ablation study with \gls{nrmse} averaged across ($1\leq \rho \leq 10$) for cancer simulation ($\gamma = 1$) and \gls{mimic}-III.}
\label{tab:ablation_study}
\resizebox{0.4\textwidth}{!}{%
\begin{tabular}{lcccr}
\toprule
Model & Cancer\_Sim & \gls{mimic}-III \\
\midrule
Causal \gls{cpc} (Full) & \textbf{1.05} & \textbf{0.62} \\
Causal \gls{cpc} (w/o $\mathcal{L}^{(InfoNCE)}$) & 1.07 & 0.68 \\
Causal \gls{cpc} (w/o $\mathcal{L}^{(InfoMax)}$) & 1.13 & 0.74 \\
Causal \gls{cpc} (w CDC loss) & 1.07 & 0.73 \\
Causal \gls{cpc} (w/o balancing) & 1.08 & 0.69 \\
\bottomrule
\end{tabular}
}
\end{table}

\begin{table}[!htbp]
 \caption{Results of the ablation study on the synthetic data set: mean$\pm$standard deviation of \gls{nrmse}. The best value for each metric is given in bold: smaller is better.}
 \centering
\resizebox{\textwidth}{!}{%
\begin{tabular}{|c |c |c |c |c |c |c |c |c |c |c|} 
\hline
Model  & $\rho = 1$   &   $\rho = 2$&  $\rho = 3$&   $\rho = 4$&  $\rho = 5$&   $\rho = 6$& $\rho = 7$&  $\rho = 8$&   $\rho = 9$ & $\rho = 10$\\ \hline  
\textbf{CAUSAL \gls{cpc} (FULL)}  & \textbf{0.83 $\pm$ 0.06}  &\textbf{0.86 $\pm$ 0.06} &0.94$\pm$ 0.09&   \textbf{0.97 $\pm$ 0.08}&  \textbf{1.03 $\pm$ 0.10 }&   \textbf{1.07$\pm$0.10}& \textbf{1.12$\pm$ 0.10}& \textbf{1.17$\pm$ 0.06}&   \textbf{ 1.22 $\pm$ 0.08 }&   \textbf{ 1.26$\pm$ 0.08 }\\ 
\hline  
\textbf{Causal \gls{cpc} (w/o $\mathcal{L}^{(InfoNCE)}$)}&  0.84$\pm$0.04&   0.91$\pm$0.07& 0.95$\pm$ 0.07&   0.99$ \pm$ 0.09& \textbf{1.03$\pm$0.10} & 1.10$ \pm$ 0.07& 1.15$\pm 0.14$& 1.20 $\pm$ 0.14&  1.23$ \pm $0.14&   1.28$ \pm 0.15$\\ 
\hline  
\textbf{Causal \gls{cpc} (w/o $\mathcal{L}^{(InfoMax)}$) } &  0.84$\pm$0.04&   0.86$\pm$0.09& \textbf{0.91$\pm$0.08}&  0.99$\pm$0.10& 1.07$\pm$0.08&   1.16$ \pm$ 0.08& 1.24$ \pm$ 0.10& 1.31 $\pm$ 0.12&  1.38$ \pm $0.08&   1.46$ \pm 0.10$\\ 
\hline
 \textbf{Causal \gls{cpc} (w CDC loss)}& \textbf{0.83$\pm$0.02} & 0.89$\pm$0.07& 0.96$\pm$ 0.07& 1.03$\pm$ 0.07& 1.07$\pm$0.08& 1.10$ \pm$ 0.07& 1.13$\pm 0.10$& 1.18 $\pm$ 0.09& 1.24$ \pm $0.11&1.28$ \pm 0.11$\\\hline
 \textbf{Causal \gls{cpc} (w Balancing}& 0.84$\pm$0.04& 0.88$\pm$0.05& 0.97$\pm$ 0.05& 1.04$\pm$ 0.07& 1.08$\pm$0.10& 1.13$ \pm$ 0.08& 1.15$\pm 0.14$& 1.20$\pm$ 0.10& 1.25$ \pm $0.08&1.29$ \pm 0.12$\\\hline 
 \end{tabular}
 }
\label{tab:cancer_ablation_details}
\end{table}

\begin{table}[!htbp]
 \caption{Results on  \gls{mimic}-III semi-synthetic data set: mean$\pm$standard deviation of \gls{nrmse}. The best value for each metric is given in bold: smaller is better.}
 \centering
\resizebox{\textwidth}{!}{%
\begin{tabular}{|c |c |c |c |c |c |c |c |c |c |c|} 
\hline
Model  & $\rho = 1$   &   $\rho = 2$&  $\rho = 3$&   $\rho = 4$&  $\rho = 5$&   $\rho = 6$& $\rho = 7$&  $\rho = 8$&   $\rho = 9$ & $\rho = 10$\\ 
\hline  
\textbf{Causal \gls{cpc} (FULL)}  &  \textbf{0.32$\pm $ 0.04}&   \textbf{0.45$ \pm$ 0.08}& \textbf{0.54$\pm 0.06$}& \textbf{0.61 $\pm$ 0.10}&   \textbf{0.66$\pm$ 0.10}&  \textbf{0.69$\pm$0.11}&   \textbf{0.71$ \pm$ 0.11}& \textbf{0.73$\pm $ 0.06}& \textbf{0.75 $\pm$ 0.05}& \textbf{0.77$ \pm$ 0.10} \\ 

\hline
 \textbf{Causal \gls{cpc} (w/o $\mathcal{L}^{(InfoNCE)}$)}& 0.35$\pm $ 0.04& 0.50$ \pm$ 0.05& 0.59$ \pm$ 0.06& 0.66$ \pm$ 0.06& 0.71$ \pm$ 0.08& 0.75$ \pm$ 0.06& 0.77$ \pm$ 0.07& 0.79$ \pm$ 0.08& 0.81$ \pm$ 0.07&0.83$ \pm$ 0.07\\
 
 \hline
 \textbf{Causal \gls{cpc} (w/o $\mathcal{L}^{(InfoMax)}$) } & 0.36$ \pm$ 0.02& 0.53$ \pm$ 0.03& 0.64$ \pm$ 0.04& 0.71$ \pm$ 0.05& 0.77$ \pm$ 0.05& 0.77$ \pm$ 0.05& 0.83$ \pm$ 0.05& 0.86$ \pm$ 0.05& 0.88$ \pm$ 0.08&0.90$ \pm$ 0.05\\
 
 \hline
 \textbf{Causal \gls{cpc} (CDC loss) }& 0.36$ \pm$ 0.02& 0.54$ \pm$ 0.03& 0.65$ \pm$ 0.05& 0.72$ \pm$ 0.05& 0.77$ \pm$ 0.05& 0.70$ \pm$ 0.04& 0.83$ \pm$ 0.04& 0.85$ \pm$ 0.03& 0.86$ \pm$ 0.03&0.88$ \pm$ 0.08\\\hline 
 
\textbf{Causal \gls{cpc} (w/o balancing)}& 0.35$ \pm$ 0.03& 0.50$ \pm$ 0.05& 0.60$ \pm$ 0.06& 0.67$ \pm$ 0.06& 0.72$ \pm$ 0.06& 0.76$ \pm$ 0.06& 0.78$ \pm$ 0.06& 0.80$ \pm$ 0.06& 0.83$ \pm$ 0.06&0.85$ \pm$ 0.06\\\hline 
 \end{tabular}
 }
\label{tab:mimic_ablation_details}
\end{table}


\paragraph{What About Using Other \gls{mi} Lower Bounds?} Other than \gls{infonce}, the \gls{mine} \citep{belghazi2018mutual} leverages the relationship between \gls{mi} and the \gls{kl} divergence. \gls{mi}  can be expressed as the \gls{kl} divergence between the joint distribution and the product of marginals:
$$
I(X; Z) \coloneqq D_{KL}(\mathbb{P}_{(X,Z)} || \mathbb{P}_X \otimes \mathbb{P}_Z)
$$
\gls{mine} employs the Donsker-Varadhan representation \citep{donsker1983asymptotic} of the \gls{kl} divergence:
\begin{equation}
D_{KL}(\mathbb{P} \,||\, \mathbb{Q}) = \sup_{T: \Omega \rightarrow \mathbb{R}} E_{\mathbb{P}}[T] - \log\left(E_{\mathbb{Q}}[e^T]\right)
\label{eq:kl_divergence}
\end{equation}
Here, the supremum is over all functions \(T\) where the expectations exist. For a specific class of functions \(\mathcal{F}\), potentially represented by a class of neural networks, we obtain the lower bound:
\begin{equation}
D_{KL}(\mathbb{P} \,||\, \mathbb{Q})\geq \sup_{T \in \mathcal{F}} E_{\mathbb{P}}[T] - \log\left(E_{\mathbb{Q}}[e^T]\right)
\label{eq:kl_divergence_inequality}
\end{equation}

In practice, we maximize
\[
\hat{I}^{\mathrm{MINE}}_{\gamma}(\mathbb{P} \,\|\, \mathbb{Q})
= \mathbb{E}_{\mathbb{P}}\bigl[T_{\gamma}\bigr]
- \log\bigl(\mathbb{E}_{\mathbb{Q}}[e^{T_{\gamma}}]\bigr),
\]
where \(T_{\gamma}\) is a discriminator parameterized by \(\gamma\), representing neural network parameters. The \gls{mine} estimator is a strongly consistent estimator of the true \gls{mi} (Theorem~2 \cite{belghazi2018mutual}).

Alternatively, the \(f\)-divergence representation of \(D_{\mathrm{KL}}\) \cite{nowozin2016f} allows us to derive another lower bound on \gls{mi} known as \gls{nwj} \citep{nguyen2010estimating}:
\[
D_{\mathrm{KL}}(\mathbb{P} \,\|\, \mathbb{Q})
\geq \sup_{T \in \mathcal{F}}
\mathbb{E}_{\mathbb{P}}\bigl[T\bigr]
- \log\bigl(\mathbb{E}_{\mathbb{Q}}[e^{T-1}]\bigr).
\]

This results in the estimator
\[
\hat{I}^{\mathrm{NWJ}}_{\gamma}(\mathbb{P}, \mathbb{Q})
= \mathbb{E}_{\mathbb{P}}\bigl[T_{\gamma}\bigr]
- \log\bigl(\mathbb{E}_{\mathbb{Q}}[e^{T_{\gamma}-1}]\bigr).
\]
We benchmarked three variational lower–bound objectives—\gls{infonce} \citep{oord2018representation}, \gls{nwj} \citep{nguyen2010estimating}, and \gls{mine} \citep{belghazi2018mutual}—  for both \gls{cpc} and \gls{infomax} on \gls{mimic}-III data, finding that \gls{infonce} yielded the best results (Table \ref{tab:mimic_mi_estimators}). The \gls{infonce} objective performs better with notable error reduction at large horizons in all cases. The superiority of  \gls{infonce} can be understood through the following qualities:
\begin{enumerate}[label=(\roman*), nosep, leftmargin=*]
\item \textbf{Lower gradient variance.}
    \gls{nwj} and \gls{mine} rely on estimating an unnormalised density ratio whose variance explodes in high dimension \citep{poole2019VBMI}; InfoNCE’s soft-max normaliser acts as an implicit variance reducer, producing stabler gradients in long recurrent chains \citep{poole2019VBMI,  Song2020UnderstandingVMI}.  
\item \textbf{Tighter bound with many negatives.}
    The InfoNCE bound tightens logarithmically with the number of samples~\citep{oord2018representation, rethinking_nce2022}; a single mini-batch of time-series data already supplies dozens of negatives (other patients, other timesteps), giving InfoNCE an automatic advantage.  
\item \textbf{Objective alignment with forecasting.}
    InfoNCE originates from \gls{cpc}, whose loss is designed to keep exactly those latent features that maximise predictability of the future sequence \citep{oord2018representation}.  This alignment transfers directly to long-horizon prediction and aids in counterfactual regression.
\end{enumerate}

\begin{table}[!htbp]
 \caption{Results of \gls{nwj} and \gls{mine} \gls{mi}  lower bounds when used for \gls{cpc} and \gls{infomax} for \gls{mimic}-III semi-synthetic data set: mean$\pm$standard deviation of \gls{nrmse}. The best value for each metric is given in bold: smaller is better.}
 \centering
\resizebox{\textwidth}{!}{%
\begin{tabular}{|c |c |c |c |c |c |c |c |c |c |c|} 
\hline
Model  & $\rho = 1$   &   $\rho = 2$&  $\rho = 3$&   $\rho = 4$&  $\rho = 5$&   $\rho = 6$& $\rho = 7$&  $\rho = 8$&   $\rho = 9$ & $\rho = 10$\\ 
\hline  
\textbf{Original Model}  &  \textbf{0.34$\pm $ 0.04}&   \textbf{0.45$ \pm$ 0.08}& \textbf{0.54$\pm 0.06$}& \textbf{0.61 $\pm$ 0.10}&   \textbf{0.66$\pm$ 0.10}&  \textbf{0.69$\pm$0.11}&   \textbf{0.71$ \pm$ 0.11}& \textbf{0.73$\pm $ 0.06}& \textbf{0.75 $\pm$ 0.05}& \textbf{0.77$ \pm$ 0.10} \\ 
\hline
\textbf{\gls{cpc} with \gls{nwj}}& \textbf{0.34$\pm $ 0.04}& 0.48$ \pm$ 0.05& 0.58$ \pm$ 0.06& 0.66$ \pm$ 0.07& 0.71$ \pm$ 0.08& 0.75$ \pm$ 0.07& 0.78$ \pm$ 0.07& 0.81$ \pm$ 0.06& 0.84$ \pm$ 0.06&0.87$ \pm$ 0.06\\
 
\hline
\textbf{\gls{cpc} with \gls{mine} } & 0.35$ \pm$ 0.03& 0.50$ \pm$ 0.05& 0.61$ \pm$ 0.04& 0.69$ \pm$ 0.04& 0.75$ \pm$ 0.04& 0.79$ \pm$ 0.03& 0.82$ \pm$ 0.03& 0.85$ \pm$ 0.02& 0.88$ \pm$ 0.02&0.91$ \pm$ 0.02\\
 \hline
\textbf{\gls{infomax} with \gls{nwj}}& 0.42$ \pm$ 0.08& 0.56$ \pm$ 0.04& 0.69$ \pm$ 0.07& 0.77$ \pm$ 0.08& 0.83$ \pm$ 0.09& 0.87$ \pm$ 0.09& 0.90$ \pm$ 0.09& 0.92$ \pm$ 0.09& 0.94$ \pm$ 0.08&0.96$ \pm$ 0.08\\\hline 
 
\textbf{\gls{infomax} with \gls{mine}}& 0.37$ \pm$ 0.05& 0.52$ \pm$ 0.03& 0.65$ \pm$ 0.06& 0.73$ \pm$ 0.8& 0.80$ \pm$ 0.10& 0.84$ \pm$ 0.11& 0.87$ \pm$ 0.11& 0.89$ \pm$ 0.10& 0.91$ \pm$ 0.10&0.93$ \pm$ 0.09\\\hline 
 \end{tabular}
 }
\label{tab:mimic_mi_estimators}
\end{table}
 
\paragraph{Falsifiability Test}
This study assumes sequential ignorability, common in causal inference \cite{lim2018RMSN, bica2020estimatingCRN, Li2021GNetAR, Melnychuk2022CausalTF}. To assess robustness, we performed a falsifiability test by omitting certain confounders during training while they remained in \gls{mimic}-III data construction: we mask two confounders from the inputs of the benchmark models, namely sodium and glucose measurements. As seen in Table \ref{tab:perf_mimic_hidden_conf}, violating sequential ignorability (i.e. results of Table \ref{tab:perf_mimic_few_data}) increased prediction errors for Causal \gls{cpc}, CT, and CRN, though RMSN was less affected but underperformed at \(\rho \geq 2\). Despite this, Causal \gls{cpc} maintained its lead at larger horizons, demonstrating strong encoding of long-term dependencies.

\begin{table}[!htbp]
\centering
\caption{Results on the \gls{mimic}-III when sequential ignorability is violated reported by RMSEs}
\label{tab:perf_mimic_hidden_conf}
\resizebox{\textwidth}{!}{%
\begin{tabular}{|c |c |c |c |c |c |c |c |c |c |c|} 
\hline
Model  & $\rho = 1$   &   $\rho = 2$&  $\rho = 3$&   $\rho = 4$&  $\rho = 5$&   $\rho = 6$& $\rho = 7$&  $\rho = 8$&   $\rho = 9$ & $\rho = 10$\\ 
\hline  
Causal \gls{cpc}  &  0.44$\pm $ 0.04&   0.56$ \pm$ 0.07& 0.66$\pm 0.07$& 0.73 $\pm$ 0.08&   0.78$\pm$ 0.08&  0.83$\pm$0.06&   \emph{0.86$ \pm$ 0.10}& \emph{0.88$\pm $ 0.08}& \emph{0.91 $\pm$ 0.08}& \emph{0.95$ \pm$ 0.07}\\ 
\hline
Causal Transformer &  \emph{0.34$\pm$0.07}  &\emph{0.48$\pm$0.07} & \emph{0.60$\pm$0.07} & \emph{0.68$\pm$0.06} &  \emph{0.75$ \pm$ 0.06} & \emph{0.80$\pm$0.07}&  0.86$\pm$ 0.09& 0.91$\pm 0.11$&0.95 $\pm 0.13$&  1.00 $\pm $0.15\\ 
\hline 
CRN& 0.40$\pm $ 0.07& 0.54$ \pm$ 0.09& 0.70$ \pm$ 0.09& 0.84$ \pm$ 0.09& 0.97$ \pm$ 0.09& 1.08$ \pm$ 0.13& 1.18$ \pm$ 0.16& 1.26$ \pm$ 0.19& 1.33$ \pm$ 0.21&1.39$ \pm$ 0.23\\
 \hline
RMSN & 0.38$ \pm$ 0.08& 0.67$ \pm$ 0.21& 0.78$ \pm$ 0.16& 0.84$ \pm$ 0.14& 0.91$ \pm$ 0.14& 0.98$ \pm$ 0.15& 1.04$ \pm$ 0.16& 1.09$ \pm$ 0.18& 1.15$ \pm$ 0.19&1.20$ \pm$ 0.23\\
  \hline
 \end{tabular}
 }
\end{table}
\vspace{-0.5cm}
\paragraph{Tightness of Mutual Information (MI) Upper Bounds}  
Estimating \gls{mi}  bounds for high-dimensional variables is challenging and expensive \citep{rainforth2018tighter, poole2019VBMI}, often limited to low-dimensional inputs or Gaussian assumptions. In MI-constrained models, batch size is crucial. As shown in  Equation (\ref{eq:LB_MI_InfoNCE}), increasing the batch size \(\mathcal{B}\) tightens the lower bound via \(\log(|\mathcal{B}|)\). To balance memory and performance, we chose batch sizes of 256 for the encoder and 128 for the decoder. While these bounds may not be perfectly tight, mutual information and self-supervision biases significantly enhance performance, as ablation studies confirm. Other \gls{mi}  estimators like \gls{nwj} and \gls{mine} \citep{nguyen2010estimating, belghazi2018mutual} did not improve performance; our initial setup consistently performed better (Table \ref{tab:mimic_mi_estimators}).

\paragraph{Extending Causal \gls{cpc} to Continuous Treatment}  
Our approach could be extended to continuous treatments by replacing the treatment classifier with a regressor. Since the method maximizes likelihood, the equilibrium in Theorem \ref{thm:blancing_iclub} remains valid. However, in practice, continuous treatments will be represented by a single dimension, unlike discrete treatments with \(K\)-dimensional one-hot encoding. This risks losing important treatment information in counterfactual predictions. A more straightforward adaptation to our model could involve discretizing continuous treatments.

\paragraph{Conclusion} 
We have introduced a novel approach to long-term counterfactual regression that combines \gls{rnn} with \gls{cpc}, achieving \gls{sota} results without the need for complex transformer models. By prioritizing computational efficiency, we incorporate regularization techniques based on contrastive losses and guided by mutual information principles. Our method consistently outperforms existing models in counterfactual estimation on both synthetic and real-world datasets, marking the first application of \gls{cpc} in the domain of causal inference.

Future research directions could explore improving the interpretability of counterfactual predictions by integrating Shapley values into temporal regression models. Given our reliance on causal graphs, investigating \emph{Causal Shapley Values} \citep{heskes2020causalSahap} may provide deeper insights into the influence of confounders over time. Additionally, there is a growing need for uncertainty-aware models \citep{de2022predicting, jesson2020identifying, yin2024conformal}, particularly tailored for longitudinal data, to enhance the reliability and transparency of predictions within our causal framework.




==> 5.tex <==
\chapter{Toward a More Transparent Causal Representation Learning}
\label{chapter:crl}

\section{Introduction}
\label{sect_crl:intro}

High-dimensional data is ubiquitous across real-world domains, motivating interest in learning high-level \emph{causal} latent factors that influence low-level observable variables, a pursuit known as causal representation learning (CRL) \citep{scholkopf2021toward}. In \gls{crl}, latent factors are endowed with a causal structure, typically an \gls{scm} (Section \ref{sect_background:causal_graphs}). Recent advances in CRL have focused on disentangling latent variables, either independently or conditionally upon auxiliary variables, such as temporal indices or categorical labels \citep{yao2022learning, komanduri2023learning, song2024temporally}. Most successful examples to date occur in perceptual domains like images, videos, and text, where researchers investigate how abstract causal factors influence low-level data through:
\begin{inparaenum}[(1)]
\item \emph{unsupervised factor disentanglement} \citep{chen2016infogan, higgins2017betavae};
\item \emph{concept-driven interpretability approaches} \citep{adebayo2018sanitysaliency, alvarez2018towards, ghorbani2019towards, koh2020concept, Do2020ThEvalDisentRep};
\item \emph{temporal and video-specific latent variable analysis} \citep{Dong2017DLSemanticInfo, kumar2018VIDisentLatConcepts, wang2024disentangled, longa2024interpretableVideos}.
\end{inparaenum} In contrast, discovering causal structures in high-dimensional, temporally evolving \emph{tabular} data remains notably challenging \citep{hasan2023CDiscoTS, somvanshi2024surveyDLTabData}.


Consider, for instance, retail transaction data, where each customer's purchasing behavior is represented by a high-dimensional vector \(\mathbf{X}_t \coloneqq [\mathbf{X}_t^1 , \dots, \mathbf{X}_t^{d_x}] \in \mathbb{R}^{d_x}\) capturing thousands of product states at a given time \(t\): each  dimension \(j \in \llbracket 1, d_x \rrbracket \), \(\mathbf{X}_t^j\) may represent the number of purchases of product \(j\) at time \(t\). Extracting causal relationships at this granular scale is computationally prohibitive and often leads to complex, uninterpretable results, limiting real-world applicability. A more promising approach is to abstract causal structures to a coarser level \(\mathbf{Z}_t \in \mathbb{R}^{d_z}\) with \(d_z \ll d_x\) \citep{beckers2019abstractingCM, beckers2020ApproxCAbst, xia2024NeuralCAbs}. Typically, the causal structure governs the temporal process over \((\mathbf{Z}_t)_{t \ge 1}\) through an \gls{scm} (Definition \ref{def:SCM}):
\begin{equation}
\label{eq:def_crl_statio}
\begin{aligned}
\mathbf{X}_t &= f\bigl(\mathbf{Z}_t\bigr),\\
\mathbf{Z}_t^j &= g_j\Bigl(\bigl\{\mathbf{Z}_{t-s}^k \mid \mathbf{Z}_{t-s}^k \in Pa(\mathbf{Z}_t^j),\ s=1,\dots,\rho\bigr\},\, \boldsymbol\epsilon_t^j
\Bigr),
\quad j\in\llbracket1,d_z\rrbracket.
\end{aligned}
\end{equation}
where \(\mathbb{G} \coloneqq \{g_1,\dots,g_{d_z}\}\) is the set of stationary structural functions (\(\mathbb{G}\) is fixed over time), \(\boldsymbol\epsilon_t^j\) is the noise term, \(\rho\) is the maximum lag, and the function \(f\), often called the generative, mixing, or decoding function, maps latent representations back to observed features.   Because causal structure now resides at the abstract latent level, the challenge of interpretability becomes acute: it remains unclear precisely how each latent temporal factor \( \mathbf{Z}_t^j \) corresponds to particular subsets of the observed variables \( \mathbf{X}_t \). Clarifying these latent-to-observed relationships is thus essential to ensuring transparency, facilitating a shift of \gls{crl} from academic benchmarks to trusted and practically useful tools for real-world decision-making.

\paragraph{Limitations of Existing Structural Assumptions} 
To put our proposal in context, we now review two common structural assumptions used in the literature of both causal and non-causal models:

\subparagraph{1. Single-parent decoding} \citet{boussard2023towardsClimate, brouillard2024causalClimate} used such an assumption in \gls{crl} models for time-series climate data to enforce that each observed variable coordinate \( \mathbf{X}_t^j \) is generated by only a single latent parent \( \mathbf{Z}_t^{k(j)} \) (Figure~\ref{fig:single_parent_dec}). However, the single-parent assumption is highly restrictive, as it forbids any observed variable from being generated by a mixture of latent factors. This is problematic in settings where causal dependencies among observed features arise from \emph{multiple} latent influences. 

\subparagraph{2. Anchor/Pure features} In a non-causal and static VAE frameworks, \citet{arora2013TopModelingGuart, Bing2020, chen2020structured, moran2021identifiable, bing2022inference} used a sparsity constraint and require that each latent variable \( \mathbf{Z}_t^k \) has at least a predefined number of \emph{anchor features} , i.e., observed features that depend exclusively on \( \mathbf{Z}_t^k \)  (e.g., two in \citet{moran2021identifiable} as in Figure~\ref{fig:anchor_features}). 

Unlike single-parent decoding, this assumption is weaker: it allows the remaining children of \( \mathbf{Z}_t^k \) to be generated by multiple latent factors, or not at all. While the anchor/pure variable assumption facilitates provable identifiability in latent variable models, including topic models \citep{arora2013practical, arora2018learning}, nonnegative matrix factorizations \citep{gillis2020NMF}, it imposes stringent structural constraints that are rarely satisfied in complex, high-dimensional data. In practice, anchor factorizations often do not exist, and even when the data exhibits low-rank structure, the required separability condition may be violated. Empirical studies have shown that statistical tests frequently reject anchor compatibility in real-world corpora, such as FOMC2 \citep{freyal2025TestingAnchors}. Furthermore, small amounts of measurement noise, sampling variability, or preprocessing (e.g., normalization) can break the purity condition, leading to misidentification of anchors \citep{huang2016AnchorFreeTopic, chen2022identificationLLVM}.  

\begin{figure}[h!]
  \centering
  \begin{subfigure}[b]{0.45\textwidth}
    \centering
    \includegraphics[scale=0.45]{figures/transp_crl/single_parent_dec.pdf}
    \caption{Single-Parent Decoding.}
    \label{fig:single_parent_dec}
  \end{subfigure}%
  \hfill
  \begin{subfigure}[b]{0.45\textwidth}
    \centering
    \includegraphics[scale=0.45]{figures/transp_crl/anchor_features.pdf}
    \caption{Anchor Feature/Pure Children.}
    \label{fig:anchor_features}
  \end{subfigure}
  \vspace{1em} 
  \begin{subfigure}[b]{0.6\textwidth}
    \centering
    \includegraphics[scale=0.45]{figures/transp_crl/modular_latents.pdf}
    \caption{Sparse Self-Expression of the Jacobian.}
    \label{fig:modular_latents}
  \end{subfigure}

  \caption{Comparison of three structural assumptions over the generation process: single-parent decoding, anchor feature, and sparse self-expression assumption. Here, we assume \(d_x = 12\) and \(d_z = 5\).}
  \label{fig:sparsity}
\end{figure}


\paragraph{Modular Influence with Soft Jacobian Constraints}
The limitations of rigid structural assumptions call for a new approach that preserves interpretability and identifiability without restricting the generative model. Rather than enforcing hard constraints like single-parent decoding \citep{boussard2023towardsClimate, brouillard2024causalClimate} or anchor features \citep{moran2021identifiable}, we impose a \emph{soft sparsity constraint} directly on the Jacobian of the decoder. Our key idea is to regularize the Jacobian using a \emph{self-expressiveness condition} following \emph{\gls{ssc}} \citep{elhamifar2013sparse}: each gradient vector (column of the Jacobian) is encouraged to lie in the span of a small number of others through a sparsity constraint. Hence, the column space of the Jacobian decomposes into a union of low-dimensional subspaces, where each subspace reflects a group of observed variables jointly governed by a subset of latent causes. The result is a modular, interpretable mapping from latent to observed space, recovering overlapping causal groups from gradient structure without relying on exclusivity or hard-coded sparsity.

This work does not introduce a new \gls{crl} model per se, but instead addresses the \textit{"so what?"} question that arises once a \gls{crl} model has been defined. Specifically, we ask how to effectively communicate the results of causal representation learning on complex high-dimensional data and how to build confidence in the learned causal concepts by transparently linking them back to the original high-dimensional feature space. To this end, we propose a regularization technique that is \emph{model-agnostic} and can be seamlessly integrated into any \gls{crl} model backbone. Our approach is twofold:  
\begin{itemize}
    \item We impose a structural sparsity constraint on the decoding function, that is, the mixing function that maps latent causal variables to low-level observed variables.
    \item A key consequence of this sparsity is that many observed features become associated with only one or a few latent factors. This induces a clustering of the observed variables, which we exploit to enhance model transparency. By analyzing the content and coherence of these clusters, we can relate them to semantically meaningful labels not used during training. For example, in purchase data, products and, therefore, dimensions of \( \mathbf{X}_t \) may be grouped into categories of products. It is also common in retail to have products clustered in multiple hierarchical groups, for e.g., categories may contain subcategories of products.
\end{itemize}

While prior work has established identifiability of \underline{latent representations} under statistical or structural assumptions \citep{hyvarinen1999nonlinear, locatello2019challenging, khemakhem2020variational}, the identifiability of induced structure over \underline{observed variables} has received far less attention. Our framework addresses this gap. Via a Jacobian-based structural sparsity, we establish a provable recovery of disjoint and overlapping groupings of observed features that are consistent with explicit graphical clustering rules defined by the latent-to-observed generative map. 

\paragraph{Main Contributions} We provide formal guarantees characterizing when this modular structure can be recovered. Specifically, we establish conditions under which one can recover \gls{whp} disjoint clusters of observed variables via \gls{ssc} (Theorem \ref{thm:subspace_detect_whp} and Proposition \ref{prop:recovery_nonoverlap_spec_cltsr}). Furthermore, we extend the analysis to the overlapping case by showing that methods such as \emph{\gls{saac}} \citep{panov2017SAAC, kaufmann2018SAAC} and \emph{\gls{symnmf}} \citep{kuang2012SymNMF, Kuang2015SymNMF, zhang2022SymNMF} can recover overlapping groupings of observed variables with bounded misclassification error (Theorem~\ref{thm:overlap_cluster_recovery}). These groupings are interpretable: they arise directly from the latent-to-observed map and reflect the underlying graphical structure of the generative process. To the best of our knowledge, no prior work in \gls{crl} provides formal identifiability results for the modular organization of observed variables. This approach connects identifiability in the latent space with interpretability at the observational level, offering a complementary perspective on structure discovery in \gls{crl}. We also provide robustness guarantees for our framework by proving that the self-expression loss generalizes under finite samples and remains stable under Jacobian perturbations. These results (Theorem~\ref{thm:genetalization_SExprLoss}, Proposition~\ref{prop:jacobian-perturbation}) ensure that the learned clusters are reliable in the presence limited data and noisy access to the Jacobian. Finally,  we demonstrate the practical effectiveness of our method through simulations where it substantially outperforms random baselines and on a large‐scale retail transaction dataset, where it recovers semantically coherent product groupings. 

\section{Preliminaries and Notations}
\section*{Notations}
Throughout this chapter, we use the following matrix and vector norms:
\[
\|A\|_{F}
\coloneqq \Bigl(\sum_{i,j}a_{ij}^{2}\Bigr)^{1/2}
\quad\text{(Frobenius norm)},
\]
\[
\|A\|_{\mathrm{op}}
\coloneqq\sup_{\|\bm x\|_{2}=1}\|A\bm x\|_{2}
\quad\text{(spectral/operator norm)},
\]
\[
\|A\|_{1\to1}
\coloneqq \max_{j}\sum_{i}\lvert a_{ij}\rvert
\quad\text{(induced 1–1 norm)}.
\]
\paragraph{Basic spaces and derivatives}
The unit sphere in the Euclidean space \(\mathbb{R}^{d}\) is denoted as
\[
\mathbb{S}^{d-1}\coloneqq\{\bm  x\in\mathbb{R}^{d}:\|\bm x\|_{2}=1\}.
\] \(\mathcal{C}^{p}(\mathbb{R}^{d};\mathbb{R}^{k})\) is the space of \(p\)-times continuously differentiable maps \(\mathbb{R}^{d}\to\mathbb{R}^{k}\).   

For \(f:\mathbb{R}^{d_z}\to\mathbb{R}^{d_x}\), typically representing a map from latent variables \(\bm Z_t\) to observed ones \(\bm X_t\), we write it with its output coordinates as
\[
f = (f_1, f_2, \dots, f_{d_x}) \quad  \text{with} \quad f_j:\mathbb{R}^{d_z}\to\mathbb{R}. 
\]

For a coordinate function $f_j$ , $\nabla_{\mathbf z} f_j$ denotes the gradient and $D^2f_i(\mathbf z)$ the Hessian. The Jacobian of $f$ will be denoted as 
\[
Df \coloneqq \left[ \nabla_{\mathbf{z}} f_1, \ \nabla_{\mathbf{z}} f_2, \ \ldots, \ \nabla_{\mathbf{z}} f_{d_x} \right].
\]
Here, it is important to note that we adopt the convention that gradients are the Jacobian columns, not the rows.

\paragraph{Asymptotic notation} For non‑negative functions $h$ and $g$, asymptotic behaviors will be denoted as

\[
\begin{aligned}
h &\;\lesssim\; g
      &&\Longleftrightarrow\;
      \exists\,C>0:\;h(x)\le C\,g(x)\;\text{ for all admissible }x,\\[4pt]
h &= \Omega(g)
      &&\Longleftrightarrow\;
      \exists\,c>0,\;x_0:\;h(x)\ge c\,g(x)\;\text{ for all }x\ge x_0,\\[4pt]
h &= \Theta(g)
      &&\Longleftrightarrow\;
      h\lesssim g\;\text{ and }\;h\gtrsim B\,,
      \quad\text{i.e. }c_1g(x)\le h(x)\le c_2g(x) \text{ for all admissible }x. \\
      h &\;\gg g
      &&\Longleftrightarrow\;
      \lim_{x\to\infty}\frac{h(x)}{g(x)}=\infty.
\end{aligned}
\]

\subsection*{Preliminary Definitions}

We next gather some fundamental notions that will be used throughout the chapter: we will be studying a decoder \(f\) and, particularly, the image of the latent random variable \(\mathbf Z\). \(f(\mathbf Z)\) will be interpreted as an input reconstruction of data, and will study its behavior via its coordinates' gradients and Hessians. We will also assume that \(\mathbf Z\) is sub-Gaussian. We therefore provide the following definitions.

\paragraph{Geometry of the Decoder Image}
To describe how $f$ can "stretch" or "compress" directions in $\mathbb R^{d_x}$, we recall isotropy and subspace notions:

\begin{definition}[Isotropic vector]
A random vector $\mathbf X\in\mathbb R^{d_x}$ is \emph{isotropic} if
\[
\mathbb E[\mathbf X]= \bm 0,
\quad
\mathbb E[\mathbf X\,\mathbf X^\top]=I_{d_x}.
\]
Equivalently, $\mathrm{Var}(\langle \mathbf u,\mathbf X\rangle)=1$ for all $\mathbf u\in\mathbb S^{d_x-1}$.
\end{definition}

\begin{definition}[Column-isotropic matrix]
\label{def:isotropic_matrix}
A random matrix $G=[\mathbf X_1,\dots,\mathbf X_m]\in\mathbb R^{d_x\times m}$ is \emph{column-isotropic} if its columns are i.i.d.\ isotropic vectors. For the remainder, we will be referring to a matrix being \emph{anisotropic} when it is not column-isotropic. 
\end{definition}

 We will usually use anisotropy to describe the Jacobian of $f$ being a random matrix \(Df(\mathbf Z)\). We will also study the linear subspaces spanned by Jacobian Columns. For this, we need the following definition:
 
\begin{definition}[Grassmannian manifold \citep{bendokat2024grassmann}]
\label{def:grassmanian}
A \emph{Grassmannian} manifold is the set of fixed-dimensional linear subspaces of a Euclidean space. For integers \(0 \le d \le n\), the Grassmannian manifold of \( d \)-dimensional subspaces of \( \mathbb{R}^n \) will be denoted as \( \mathrm{Gr}(d, n) \).
\end{definition}

\paragraph{Function-Space Norms and Sub-Gaussianity}
We measure smoothness and tail decay via Orlicz norms, particularly via the $\psi_2$ norm to define sub-Gaussian distributions.

\begin{definition}[Orlicz function]
\label{def:orlicz_fct}
A function \(\psi:[0,\infty)\to[0,\infty)\) is called an \emph{Orlicz function} if \(\psi\) is convex, non-decreasing, \(\psi(0)=0\), and \(\lim_{x\to\infty}\psi(x)=\infty\).
\end{definition}

\begin{definition}[Orlicz space and Orlicz norm \citep{vershynin2018HDProba}]
\label{def:orlicz_space_norm}
Let \((\Omega,\mathcal{F},\mathbb P)\) be a probability space and \(\psi\) an Orlicz function.  The \emph{Orlicz space} \(L_{\psi}(\Omega,\mathcal{F},\mathbb P)\) consists of all measurable random variables \(X\) for which the \(\|X\|_{\psi}\) is finite:
\[
L_{\psi}(\Omega,\mathcal{F},\mathbb P)
:=\bigl\{\,X:(\Omega,\mathcal{F})\to\mathbb{R} \ ; \|X\|_{\psi}<\infty\bigr\}.
\]
In the space \(L_{\psi}(\Omega,\mathcal{F},\mathbb P)\) , \(\|X\|_{\psi}\) is a norm.
\end{definition}

\begin{definition}[\(\psi_2\)--Orlicz norm]
\label{def:orlicz_fct_psi2}
Define
\[
\psi_2(x) := e^{x^2}-1.
\]
\(\psi_2\) is an Orlicz function, and for a scalar random variable \(X\), define
\[
\|X\|_{\psi_2}
:= 
\inf\bigl\{\,c>0 : \mathbb{E}\bigl[\psi_2(\lvert X\rvert / c)\bigr]\le1\bigr\},
\]
which is a norm in the space \(L_{\psi_2}(\Omega,\mathcal{F},\mathbb P)\).
\end{definition}

\begin{definition}[Sub-Gaussian Random Variable]
\label{def:Z_subgauss_scalar}
A real random variable \(Z \in \mathbb{R}\) is \emph{sub-Gaussian} if any (hence all) of the following equivalent conditions hold \citep{wainwright2019high}:
\begin{enumerate}
  \item \textbf{Tail bound}: There exists \(K>0\) such that for all \(t \ge 0\),
  \[
  \mathbb{P}\bigl(|Z| \ge t\bigr) \;\le\; 2\,\exp\!\left(-\tfrac{t^2}{K^2}\right).
  \]
The inequality means the tails of \(Z\) decay at least as fast as a Gaussian with variance equal to \(K^2\). 
  \item \textbf{\(\psi_2\)-Orlicz norm}: The \(\psi_2\)-norm of \(Z\) is finite, defined by
  \[
  \|Z\|_{\psi_2}
  = \inf\left\{s>0 : \mathbb{E}\left[e^{Z^2/s^2}\right] \le 2 \right\}.
  \]
  \end{enumerate}
\end{definition}
 
\begin{definition}[Sub-Gaussian vector with parameter \(K>0\)]
\label{def:Z_subgauss_vector}
A random vector \(\mathbf Z\in\mathbb R^{d_z}\) is said to be \emph{sub-Gaussian with parameter \(K\)}, written \(\mathbf Z \sim \mathrm{subG}_{d_z}(K)\) if for every \( \mathbf{u} \in \mathbb{S}^{d_z-1} \), the scalar random variable \(\langle \mathbf{u}, \mathbf{Z} \rangle\) is sub-Gaussian. The vector Orlicz norm is defined as 
\[
      \|\mathbf Z\|_{\psi_2}
      := 
      \sup_{\mathbf u\in \mathbb S^{d_z-1}}
      \|\langle \mathbf u,\mathbf Z\rangle\|_{\psi_2}.
    \]
    \end{definition}

\paragraph{For the graphical view of latent-to-observed variables} Given that we will discuss how structurally Latent variables \(\bm Z_t\) connect to the observed ones \(\bm X_t\) and how coordinates of \(\bm X_t\) cluster together, we will need the following definitions.
\begin{definition}[Directed Bipartite Graph \citep{diestel2025graph}]
\label{def:bipartite_graph_directed}
Let \(\mathbf{Z}\) and \(\mathbf{X}\) be two disjoint sets of vertices.  A \emph{directed bipartite graph} is a triple \((\mathbf{Z}, \mathbf{X},\; E\bigr)\), where
\[
  E \;\subseteq\; \mathbf{Z} \times \mathbf{X}
\]
is the set of \emph{directed} edges, each of which is an ordered pair \((z,x)\) with \(z\in \mathbf{Z}\) and \(x\in \mathbf{X}\).  No edges are allowed from \(\mathbf{X}\) to \(\mathbf{Z}\) or within \(\mathbf{Z}\) , or \(\mathbf{X}\) themselves. For simplicity, we will write $\mathbf{Z} \longrightarrow \mathbf{X}$ to indicate a directed bipartite graph.
\end{definition}

\begin{definition}[Transitive closure \citep{GRAMI2023155}]
\label{def:transitive_closure}
 Let \(\mathbf X\) be an arbitrary set of vertices. For any binary relation \(\sim\subseteq\mathbf X\times\mathbf X\), its \emph{transitive closure} \(\sim^{*}\) is defined as
\[
   \sim^{*}
   \;\coloneqq \;
   \bigcap\Bigl\{\,T\subseteq\mathbf X\times\mathbf X
     \;\Bigm|\;
     \sim\subseteq T
     \ \text{and}\ T\ \text{is transitive}\Bigr\}.
\]
That is, \(\sim^{*}\) is the \emph{smallest transitive relation containing \(\sim\)} with respect to set inclusion.  Equivalently,
\[
   x\;\sim^{*}\;y
   \iff
   \exists\,m\in\mathbb{N},\;\exists\,v_{0},\dots,v_{m}\in\mathbf X:\;
   \begin{cases}
     v_{0}=x,\;v_{m}=y,\\
     v_{t-1}\sim v_{t}\quad\forall\,t=1,\dots,m.
   \end{cases}
\]
\end{definition}
 
\subsection*{Decoder Structure and Clustering of Observed Variables}
In this work, we explicitly assume that the association between latent factors and observed variables remains stationary over time. This assumption simplifies the understanding of causal structures, but it is natural in domains where the causal abstraction remains stable: if \(\mathbf{Z}_t^j\) is associated with a subset of products \( \mathbf{X}_t \) which happens to be a known product category, then the product category remains the same through time. It is common for product taxonomies to remain fixed for a long period of time in retail.  An important direction for future work is to extend the framework to accommodate regime shifts, seasonal effects, or evolving causal structures (cf. Discussion in Section \ref{sect_crl:discussion}).

\begin{assumption}[Stationarity]
In this work, we address \gls{crl} as defined in the Equation \ref{eq:def_crl_statio} given temporally stationary environments, that is, the set of structural functions $\mathbb{G}$ is \emph{static}.
\end{assumption}

A key benefit of imposing structural sparsity on the generative model is the emergence of organization among the observed variables.  The generative mechanism \( \mathbf{Z}_t \to \mathbf{X}_t \) can be represented as a stationary bipartite graph, where latent variables influence observed features through directed edges, and the edges remain the same through time. For that reason, we omit time dependence unless necessary and describe \( \mathbf{Z} \to \mathbf{X} \).

\begin{definition}[Bipartite View of Decoder Structure]
\label{def:graph_bipartite_statio}
We represent the generative process as a bipartite graph (\ref{def:bipartite_graph_directed}) \( G = (\mathbf{Z}, \mathbf{X}, E) \), where:
\begin{inparaenum}[(1)]
    \item \( \mathbf{Z} = \{ \mathbf{z}^1, \ldots, \mathbf{z}^{d_z} \} \) denotes the set of latent variables,
    \item \( \mathbf{X} = \{ \mathbf{x}^1, \ldots, \mathbf{x}^{d_x} \} \) denotes the set of observed features, and
    \item an edge \( (\mathbf{z}^j, \mathbf{x}^i) \in E \) exists if and only if \( \partial f_i / \partial \mathbf{z}^j \not\equiv 0 \). 
\end{inparaenum}
\end{definition}

We exploit this influence pattern to perform \emph{variable clustering} \citep{mcculloch2004generalized, thalamuthu2006evaluation, jacob2009group, StructSparsityCvxOptim2012, aydore2019feature, chavent2021combining}, by grouping features according to well-defined rules derived from the underlying latent structure. We define the two main rules in this work: \emph{shared-parent clustering}, which provides disjoint groups, and \emph{overlapping-parent clustering}, which provides overlapping groups.

\begin{definition}[Shared-Parent Clustering Rule]
\label{def:shared_parent_clustering}
We define an undirected relation \( \sim \) on \( \mathbf{X} \) as follows:
\[ \mathbf{x}^i \sim \mathbf{x}^j \iff \exists \mathbf{z}^k \in \mathbf{Z} \text{ such that } (\mathbf{z}^k, \mathbf{x}^i), (\mathbf{z}^k, \mathbf{x}^j) \in E. \]
Let \( \sim^* \) denote the transitive closure of \( \sim \) (cf. \ref{def:transitive_closure}). Then:

The shared-parent clustering of the observed variables is the partition of \( \mathbf{X} \) into equivalence classes under the relation \( \sim^* \). That is, each cluster is a maximal subset \( \mathcal{C} \subseteq \mathbf{X} \) such that:
\[ \forall \mathbf{x}^i, \mathbf{x}^j \in \mathcal{C},\ \mathbf{x}^i \sim^* \mathbf{x}^j, \quad \text{and} \quad \forall \mathbf{x} \in \mathbf{X} \setminus \mathcal{C},\ \mathbf{x} \not\sim^* \mathbf{x}^j \text{ for any } \mathbf{x}^j \in \mathcal{C}. \]
Each cluster corresponds to a connected component in the undirected graph over \( \mathbf{X}\), where an edge exists between \( \mathbf{x}^i \) and \( \mathbf{x}^j \) if they share a latent parent.
\end{definition}

Intuitively, Definition \ref{def:shared_parent_clustering} implies that two observed variables belong to the same group if there exists a path of features \( \mathbf{x}^{i_1}, \dots, \mathbf{x}^{i_k} \) such that each consecutive pair shares at least one latent parent, and both variables lie in the same connected component under the relation \(\sim\). As an illustration, consider the graph in Figure~\ref{fig:anchor_features}:  applying the shared-parent clustering rule yields the following partition of the observed variables:
\[
\mathcal{C}_{\text{disjoint}} = 
\left\{ 
\mathcal{C}_1 = \{ \mathbf{x}_{t}^1, \ldots, \mathbf{x}_{t}^6 \}, \quad
\mathcal{C}_2 = \{ \mathbf{x}_{t}^7, \ldots, \mathbf{x}_{t}^{12} \} 
\right\}.
\]
Here in the cluster \(\mathcal{C}_1\), the path \(\mathbf{x}_{t}^1, \ldots, \mathbf{x}_{t}^6\) is maximal because there is no other observed feature in \(\mathbf{X} \setminus \mathcal{C}_1 \) that could be added, given no shared latent cause exists according to the graph in \ref{fig:anchor_features}. 

\begin{definition}[Overlapping-Parent Clustering Rule]
\label{def:overlap_parent_clustering}
The overlapping-parent clustering of the observed variables is the collection of clusters 
\[ 
\mathcal{C}_{\text{overlap}} \coloneqq \{\mathrm{Ch} (\mathbf{z}^1), \dots, \mathrm{Ch}(\mathbf{z}^{d_z})\},
\]
where
\[ \mathrm{Ch}(\mathbf{z}^k) := \{ \mathbf{x}^j \in \mathbf{X} \mid (\mathbf{z}^k, \mathbf{x}^j) \in G \}. \]
Each cluster \( \mathrm{Ch}(\mathbf{z}^k)\) is the children set: it contains all observed variables that are directly influenced by the latent variable \( \mathbf{z}^k \).
\end{definition}

In contrast, using the \emph{overlapping-parent clustering rule} (Definition~\ref{def:overlap_parent_clustering}), which groups features based on sharing at least one latent parent, results in a finer, overlapping structure:
\[
\mathcal{C}_{\mathrm{overlap}} =
\biggl\{
\underbrace{\{\mathbf{x}_t^1,\, \mathbf{x}_t^2,\, \mathbf{x}_t^3\}}_{\mathrm{Ch}(\mathbf{z}_t^1)}, \,
\underbrace{\{\mathbf{x}_t^3,\, \mathbf{x}_t^4,\, \mathbf{x}_t^5\}}_{\mathrm{Ch}(\mathbf{z}_t^2)}, \,
\underbrace{\{\mathbf{x}_t^5,\, \mathbf{x}_t^6\}}_{\mathrm{Ch}(\mathbf{z}_t^3)}, \,
\underbrace{\{\mathbf{x}_t^7,\, \mathbf{x}_t^8,\, \mathbf{x}_t^9\}}_{\mathrm{Ch}(\mathbf{z}_t^4)}, \,
\underbrace{\{\mathbf{x}_t^9,\, \mathbf{x}_t^{10},\, \mathbf{x}_t^{11},\, \mathbf{x}_t^{12}\}}_{\mathrm{Ch}(\mathbf{z}_t^5)}
\biggr\}.
\]
This overlapping clustering \( \mathcal{C}_{\text{overlap}} \) provides a more fine-grained abstraction than  \( \mathcal{C}_{\text{disjoint}} \). Notably, each cluster \( \mathrm{Ch}(\mathbf{z}_{t}^j) \) is a subset of one of the disjoint clusters of  \( \mathcal{C}_{\text{disjoint}} \), illustrating the hierarchical relation between the two grouping strategies. Notably, the anchor feature assumption, as represented in Figure~\ref{fig:anchor_features}, yields the same non-overlapping clustering as the sparse self-expression constraint. However, the latter permits far more complex latent-to-observed influence patterns. Specifically, only the subset \( \{ \mathbf{z}_{t}^1, \mathbf{z}_{t}^2, \mathbf{z}_{t}^3 \} \) is responsible for generating the features \( \{ \mathbf{x}_{t}^1, \ldots, \mathbf{x}_{t}^6 \} \), while \( \{ \mathbf{z}_{t}^4, \mathbf{z}_{t}^5 \} \) governs \( \{ \mathbf{x}_{t}^7, \ldots, \mathbf{x}_{t}^{12} \} \). Thus, \emph{modularity} is maintained, but without requiring the strict exclusivity assumptions imposed by anchor-based models. 

The two clustering rules defined by \ref{def:shared_parent_clustering}  and \ref{def:overlap_parent_clustering} yield different, yet meaningful groupings of observed features, each consistent with distinct structural assumptions. The key insight is that \emph{clustering is not unique}: it depends on the specific clustering rule, which in turn reflects a modeling choice. 

To further formally clarify the dependence of variable clustering on the rule defined, we give a formalization of what a "clustering rule" is, and then show how clusters can be defined as a consequence. We will use the term \emph{modularity} whenever we want to communicate that a subset of latent variables shares a common influence pattern with some subset of observed ones and not with the rest.


Intuitively, the two clustering rules defined above happen to reason both on how the parent set of observed variables, which are subsets of latent ones, interact with each other. We formalize this as the following
\begin{definition}[Affinity predicate]
\label{def:affinity}
Let $G$ be a directed bipartite graph (\ref{def:bipartite_graph_directed}). 

An \emph{affinity predicate} $P: \mathbf X \times \mathbf X \longrightarrow \{0,1\}$  is any symmetric Boolean function
\[
P(\mathbf x^{i},\mathbf x^{j}\mid G)
\;=\;
\pi\!\bigl(\mathrm{Pa}(\mathbf x^{i}),\mathrm{Pa}(\mathbf x^{j})\bigr), 
\]
with $\pi: 2^{\mathbf Z } \times 2^{\mathbf Z } \longrightarrow \{0,1\}$ is a symmetric Boolean function of two subsets of $\mathbf Z$.
\end{definition}

The shared parent clustering rule corresponds to the affinity predicate
\[
P_{\mathrm{SP}}(\mathbf x^{i},\mathbf x^{j}\mid G)
=
\begin{cases}
1, & \mathrm{Pa}(\mathbf x^{i})\cap \mathrm{Pa}(\mathbf x^{j})\neq\varnothing,\\
0, & \text{otherwise}.
\end{cases}
\]
and if one writes the binary relation 
\[
\mathbf  x^{i}\sim_{SP} \mathbf x^{j} \iff P_{\mathrm{SP}}(x^{i},x^{j}\mid G)=1,
\]
then $\sim_{SP}$ is symmetric and reflexive but not transitive and is identical to that of Definition \ref{def:shared_parent_clustering}. For the overlapping-parent clustering, if for each \(\mathbf{z} \in \mathbf{Z}\), one considers the predicate \(P_z\) as the restriction of \(P_{\mathrm{SP}}\) on \( \mathrm{Ch}(\mathbf{z})\), then \(\sim_{SP}\) defines trivially an equivalent relation when restricted to \( \mathrm{Ch}(\mathbf{z}) \times \mathrm{Ch}(\mathbf{z}) \). It has only one non-empty equivalence class, which is \(\mathrm{Ch}(\mathbf{z}) \) itself. Thus, by varying \(\mathbf{z}\), we collect \(\{ \mathrm{Ch}(\mathbf{z})\}_{\mathbf{z} \in \mathbf{Z}}\) which coincides with the  Definition \ref{def:overlap_parent_clustering}.



\section{Intuitive Discussion of Jacobian Self-Expression }

\paragraph{Generalizing Anchor Features through Gradient Subspaces}
We can naturally generalize the classical anchor feature assumption by shifting from exact functional separability to linear relationships between decoder gradients. Rather than defining the decoder as a fixed matrix as in \citet{boussard2023towardsClimate} (c.f Related Work, Section \ref{sect_crl:related_work}), we allow it to be any smooth function \( f: \mathbb{R}^{d_z} \rightarrow \mathbb{R}^{d_x} \), and impose structural sparsity through its Jacobian:
\[
\mathbf{X}_t^j \sim \mathcal{N}\left(f_j(\mathbf{Z}_t), \sigma_j^2\right), \quad
f(\mathbf{Z}_t) = \left[f_1(\mathbf{Z}_t), \ldots, f_{d_x}(\mathbf{Z}_t)\right]^T.
\]
We recall the standard anchor feature condition used in identifiable sparse VAE models in the \emph{static} setting: \cite{moran2021identifiable} defined the anchor feature assumption as: For each latent factor \( \mathbf{Z}^k \), there exist at least two observed features \( \mathbf{X}^j \) and \( \mathbf{X}^{j_0} \) such that  
\begin{equation}
\label{eq:anchor_feat_moran}
    \mathbb{E}[\mathbf{X}^j|\mathbf{Z}] = f_j(\mathbf{Z}^k) \quad  \text{and} \quad  \mathbb{E}[\mathbf{X}^{j_0} |\mathbf{Z}] = f_{j_0}(\mathbf{Z}^k).
\end{equation}
To generalize this, denote the partial derivative as
\[
\phi_{ij} \;\coloneqq\; \frac{\partial f_j}{\partial \mathbf z^i}.
\]
For example, from the graphical structure in Figure~\ref{fig:anchor_features}, we have
\[
\nabla_{\mathbf{z}}f_{7}(\mathbf{z})
=\bigl[\,0,\;0,\;0,\;\phi_{47}(\mathbf{z}),\;0\,\bigr]^{\!\top},
\quad
\nabla_{\mathbf{z}}f_{8}(\mathbf{z})
=\bigl[\,0,\;0,\;0,\;\phi_{48}(\mathbf{z}),\;0\,\bigr]^{\!\top}.
\]
Now, suppose the gradients of two decoding functions are collinear almost everywhere.  Then there exist constants \(a,b\) such that
\[
f_{7}(\mathbf{Z}) = a\,f_{8}(\mathbf{Z}) + b
\quad\text{almost surely},
\]
and hence
\[
\mathbb{E}[\mathbf X^{7}\mid \mathbf{Z}]
= a\,\mathbb{E}[\mathbf X^{8}\mid \mathbf{Z}] + b.
\]
This weakens the anchor feature assumption in Equation~\ref{eq:anchor_feat_moran}: rather than requiring that two observed features depend  identically on one latent factor, we can only require their conditional expectations to be linearly related. Thus, the classical anchor condition becomes a special case of a broader gradient-based linear structure. 

To uncover latent-induced modularity in the observed space, we examine the Jacobian matrix $Df$ of the decoder \(f\)
\[
 Df \coloneqq \left[ \nabla_{\mathbf{z}} f_1, \ \nabla_{\mathbf{z}} f_2, \ \ldots, \ \nabla_{\mathbf{z}} f_{d_x} \right]
\]
and encode its structural geometry via a self-expression matrix \( C \in \mathbb{R}^{d_x \times d_x} \). Each column of \( Df \) is represented as a sparse linear combination of the others:
\[
\nabla_{\mathbf{z}} f_j = \sum_{k \neq j} C_{kj} \nabla_{\mathbf{z}} f_k.
\]
We must satisfy \(C_{jj} = 0\) for all \(j = 1, \dots, d_x\) to eliminate the trivial identity solution, i.e., a gradient should not be self-expressed by itself. 

The Jacobian \( Df \) reflecting the sparse structure in Figure~\ref{fig:modular_latents} which we restate below, has the form:
\begin{equation}
\label{eq:jac_example}
Df = \left[
\begin{array}{cccccccccccc}
\phi_{1,1} & \phi_{1,2} & \phi_{1,3} & \phi_{1,4} & \phi_{1,5} & 0 & 0 & 0 & 0 & 0 & 0 & 0 \\
\phi_{2,1} & \phi_{2,2} & \phi_{2,3} & \phi_{2,4} & \phi_{2,5} & \phi_{2,6} & 0 & 0 & 0 & 0 & 0 & 0 \\
0 & 0 & 0 & 0 & \phi_{3,5} & \phi_{3,6} & 0 & 0 & 0 & 0 & 0 & 0 \\
0 & 0 & 0 & 0 & 0 & 0 & \phi_{4,7} & \phi_{4,8} & \phi_{4,9} & \phi_{4,10} & \phi_{4,11} & \phi_{4,12} \\
0 & 0 & 0 & 0 & 0 & 0 & \phi_{5,7} & \phi_{5,8} & \phi_{5,9} & \phi_{5,10} & \phi_{5,11} & \phi_{5,12}
\end{array}
\right]
\end{equation}

\begin{figure*}[ht]
\centering
\includegraphics[scale=0.45]{figures/transp_crl/modular_latents.pdf}
\caption*{An example of a structure corresponding to the sparse self-expression of the Jacobian. A restatement of Figure \ref{fig:modular_latents}}
\end{figure*}

\begin{equation}\label{eq:C_matrix_ex}
C \;=\;
\begin{pmatrix}
C_1 & 0 \\[6pt]
0   & C_2
\end{pmatrix},
\quad
C_1,\;C_2\;\in\;\mathbb{R}^{6\times6},
\end{equation}

\begin{equation}
\begin{aligned}
C_1 &= 
\begin{pmatrix}
0         & C_{1,2} & C_{1,3} & C_{1,4} & C_{1,5} & C_{1,6} \\[3pt]
C_{2,1}   & 0       & C_{2,3} & C_{2,4} & C_{2,5} & C_{2,6} \\[3pt]
C_{3,1}   & C_{3,2} & 0       & C_{3,4} & C_{3,5} & C_{3,6} \\[3pt]
C_{4,1}   & C_{4,2} & C_{4,3} & 0       & C_{4,5} & C_{4,6} \\[3pt]
0         & 0       & 0       & 0       & 0       & C_{5,6} \\[3pt]
0         & 0       & 0       & 0       & C_{6,5} & 0
\end{pmatrix}, 
\quad
C_2 =
\begin{pmatrix}
0           & C_{7,8}   & C_{7,9}   & C_{7,10}  & C_{7,11}  & C_{7,12} \\[3pt]
C_{8,7}     & 0         & C_{8,9}   & C_{8,10}  & C_{8,11}  & C_{8,12} \\[3pt]
C_{9,7}     & C_{9,8}   & 0         & C_{9,10}  & C_{9,11}  & C_{9,12} \\[3pt]
C_{10,7}    & C_{10,8}  & C_{10,9}  & 0         & C_{10,11} & C_{10,12} \\[3pt]
C_{11,7}    & C_{11,8}  & C_{11,9}  & C_{11,10} & 0         & C_{11,12} \\[3pt]
C_{12,7}    & C_{12,8}  & C_{12,9}  & C_{12,10} & C_{12,11} & 0
\end{pmatrix}.
\end{aligned}
\end{equation}

\paragraph{Clustering via Shared Gradient Support}
Our formulation recovers feature clusters by identifying subspaces of mutually expressible gradients, that is, observed features whose Jacobians span the same low-dimensional subspace. For instance, from Figure~\ref{fig:modular_latents}, we identify the groupings:
\[
\left\{ \{ \mathbf{x}_{t}^1, \ldots, \mathbf{x}_{t}^6 \}, \{ \mathbf{x}_{t}^7, \ldots, \mathbf{x}_{t}^{12} \} \right\}.
\]
where the gradients \( \{ \nabla_\mathbf{z} f_1, \dots, \nabla_\mathbf{z} f_6 \} \) are expressible in terms of each other. A valid self-expression would be:
\[
\nabla_\mathbf{z} f_1 = \sum_{i=2}^6C_{i,1} \nabla_\mathbf{z} f_i.
\]
In contrast, an invalid expression such as:
\begin{equation}
\label{eq:self_express_counter}
    \nabla_\mathbf{z}f_1 = \sum_{i=2}^6C_{i,1} \nabla_\mathbf{z} f_i + C_{7,1} \nabla_\mathbf{z} f_7, \quad  C_{7,1} \neq 0
\end{equation}
is precluded, since \( \nabla_\mathbf{z} f_7 \) has disjoint support with \(\nabla_\mathbf{z}f_1\)  and including it would imply that \( \phi_{4,7}\equiv  \phi_{5,7} \equiv 0\) which is not possible by maximum sparsity of Jacobian in Equation~\ref{eq:jac_example}. As a remedy, one might also include other gradients with the same support as \( \nabla_\mathbf{z} f_7 \) (e.g. \( \nabla_\mathbf{z} f_8 \)). However, adding such terms would violate sparsity, as we aim to discourage unnecessary inclusion of uninformative features.

\paragraph{Support Overlap and Subspace Consistency}
This yields a principled clustering criterion: two observed features \(i\) and \(j\) belong to the same cluster if and only if
\begin{enumerate}
  \item \(C_{i,j}\neq 0\) or \(C_{j,i}\neq 0\), and
  \item \(\mathrm{supp}\bigl(\nabla_{z}f_i\bigr)\;\cap\;\mathrm{supp}\bigl(\nabla_{z}f_j\bigr)\neq\varnothing\).
\end{enumerate}
Under these conditions, the optimal self‐expression matrix \(C^*\) is block‐diagonal (up to permutation), with each block identifying a latent‐induced subspace. Consequently, the clustering is non-overlapping, and each cluster comprises exactly those gradients sharing the same support in the latent space.

We propose to achieve so through sparse subspace clustering over the Jacobian Dictionary. Informally, let there be \(n\) linear subspaces \((\mathcal S_l)_{l=1}^n\) in \(\mathbb{R}^{d_z}\) such that \(\nabla_{\bm z}f_j\) lies within their union.  The Jacobian can be rewritten as
\[
Df \;=\; \bigl[\nabla_{\bm z}f_1,\dots,\nabla_{\bm z}f_{d_x}\bigr]
\;=\;
\bigl[J_1,\dots,J_n\bigr]\,P,
\]
where \(P\in\mathbb{R}^{d_x\times d_x}\) is a permutation matrix.  Each \(J_l\) is a matrix of gradient vectors whose column span defines the corresponding subspace \(\mathcal S_l\), i.e.\ 
\[
\operatorname{span}\bigl(\mathrm{cols}(J_l)\bigr)=\mathcal S_l.
\]
This leads to a matrix formulation of the self-expressiveness assumption:

\begin{assumption}[Matrix Formulation of Self-Expressiveness]
\label{assp:self_expression}
We assume the existence of self-expressiveness in the Jacobian columns, that is, there exists \(C\in\mathbb{R}^{d_x\times d_x}\) with \(\mathrm{diag}(C)=\mathbf0\) such that each gradient can be written as
\[
\nabla_{\bm z}f_j \;=\; Df\,C_{:,j}, \quad j \in \{1, 2, \dots, d_x\}.
\]
Equivalently, in a matrix form
\[
  Df\; C = Df,
  \quad
  \mathrm{diag}(C)=\mathbf0.
\]
\end{assumption}

Since this expression is generally non-unique, we aim to enforce sparsity in the matrix \(C\). To achieve this, we can optimize \(C\) by solving: 
\begin{equation*}
\begin{aligned}
\min_{C_{:,j} \in \mathbb{R}^{d_x}} \; & \|C_{:,j}\|_1 \\[1.2ex]
\text{subject to} \quad
& \nabla_{\mathbf{z}} f_j(\mathbf{Z}) = Df(\mathbf{Z})\, C_{:,j} \ \mathrm{a.s.}, \\[0.8ex]
& C_{j,j} = 0.
\end{aligned}
\end{equation*}

The optimization problem establishes the link between latent factors \(\mathbf{Z}\) and observed features \(\mathbf{X}\) using the solution \(C^*\). The underlying rationale is that variables that cluster together should have gradients of the decoding function with respect to \(\mathbf{z}\) lying in the same linear subspace of the Jacobian. Specifically, the nonzero entries in \(C_{:, j}\) should correspond to gradients from the same subspace \(\mathcal S_l\) when \(\nabla_{\mathbf{z}} \mathbf{f}_j\) belongs to \(\mathcal S_l\). In other terms, the first objective is to define geometric and probabilistic conditions under which this subspace preservation property holds (cf. Definition \ref{def:subspace_detect}).

Once we ensure that the self-expression matrix \(C^*\) preserves subspaces, it can then be leveraged to perform clustering of the observed variables.  For example, let \(\mathcal V\) be the set of vertices corresponding to the gradients \footnote{Here, the set of gradients is equivalent to considering the set of observed features \(\{ \mathbf{X}^1, \ldots, \mathbf{X}^{d_x} \}\). The rationale here is: to perform variable clustering, we give a "vectorial representation" to each scalar dimension \(\mathbf{X}^j\) through its gradient w.r.t. the latent factors \(\nabla_{\bm z}f_j\)  and thus reason on (subspace) clustering of gradients.} 
\[
\nabla_{\bm z}f_1,\dots,\nabla_{\bm z}f_{d_x}.
\]
Denote by \(\Gamma\subseteq\mathcal V\times\mathcal V\)  the set of edges between nodes, and let \(A\in\mathbb{R}_{+}^{d_x \times d_x}\)  be the (symmetric) edge-weight matrix defined by
\[
A 
\;=\;
\frac{1}{2}\bigl(\lvert C^*\rvert + \lvert C^*\rvert^{\!\top}\bigr).
\]
Clusters are then obtained by applying spectral clustering \citep{von2007tutorialSpectrCls} to the weighted graph \((\mathcal V,\Gamma,A)\).


We show in Proposition \ref{prop:recovery_nonoverlap_spec_cltsr} under which conditions such a pipeline recovers clusters that are consistent with those obtained by the shared parent clustering rule (Definition \ref{def:shared_parent_clustering}). The same reasoning is followed in the case of the recovery of overlapping clusters, where spectral clustering is replaced by overlapping-aware clustering methods such as Synmf \citep{Kuang2015SymNMF} and SAAC \citep{panov2017SAAC}, and we show in Theorem \ref{thm:overlap_cluster_recovery} under which conditions the resulting clusters are consistent with those obtained by the overlapping clustering rule (Definition \ref{def:overlap_parent_clustering}).


\section{Related Work}
\label{sect_crl:related_work}
\subsection{CRL in a time-varying setting}

\citet{yao2022learning} were the first to introduce \gls{crl} over time-varying data while providing theoretical guarantees for the identifiability of the true latent causal variables. In their model, each latent variable  \(\mathbf{Z}_t^j\) obeyed time-delayed causal relations as in Equation \ref{eq:def_crl_statio},  except that the noise \(\boldsymbol \epsilon_{t}^j\) follows a non-stationary distribution
\[
\boldsymbol \epsilon_{t}^j \sim p_{\boldsymbol \epsilon^j\mid \mathbf{a}},
\]
with \(\mathbf{a}\) an observed auxiliary variable that can take various forms: 
\begin{inparaenum}[(i)]
\item a \emph{time index} to account for sequential dependencies, 
\item a \emph{domain index} to capture distributional shifts across domains, 
\item or a \emph{class label} in supervised learning contexts
\end{inparaenum}
\citep{hyvarinen2016TCL,hyvarinen2019nonlinear,locatello2019challenging, khemakhem2020variational,morioka2021independent}. The inductive bias introduced by the auxiliary variable facilitates the identifiability of the latent factors up to mild transformations such as permutations and component‐wise invertible mappings. 

\citet{song2024temporally} considered the case where the side information \(\mathbf a\) is unobserved, and similar to \citet{Hlv2020HiddenMN}, they treated the domain index variables as latent and modeled them via a Markov chain.  The resulting generative model is
\[
\begin{aligned}
a_1,\,a_2,\,\dots,\,a_T &\sim \mathrm{MC}(A), \\[1ex]
\boldsymbol \epsilon_t^j &\sim p_{\boldsymbol \epsilon^j}, \quad j = 1,\dots,d_z, \\[1ex]
\mathbf{Z}_t^j &= g_j\Bigl(\bigl\{\mathbf{Z}_{t-s}^k \mid \mathbf{Z}_{t-s}^k \in Pa(\mathbf{Z}_t^j),\  s=1,\dots,\rho\bigr\},\ a_t ,\ \boldsymbol\epsilon_t^j\Bigr), \\[1ex]
\mathbf{X}_t &= f(\mathbf{Z}_t),
\end{aligned}
\]
where \(a_t\in\{1,\dots,d_a\}\) is a discrete domain index and $A$ is the \(d_a \times d_a\) transition matrix of the Markov chain \((a_t)_{t\ge1}\).  Here, the structural functions, unlike those of Equation \ref{eq:def_crl_statio}, are non-stationary because they are modulated by \((a_t)_{t\ge1}\). The identifiability of the latent process stems first from identifying the non-stationarity represented by \((a_t)_{t \geq 1}\) , similar to \cite{gassiat2016inference, Hlv2020HiddenMN, morioka2021independent}, and then establishing the identifiability of the causal latent variables \((\mathbf{Z}_t)_{t \geq 1}\), as in \cite{yao2022learning}. 

\citet{Chen2024CRLNonInvertibleEnc} challenged the longstanding assumption of invertibility in the generative process \(f\) and proposed leveraging temporal context for both generation and identification. Specifically, they used the historical latent process to generate the observed data and the historical observed process to identify the latent causal factors:
\[
\begin{aligned}
\mathbf{X}_t&= f\bigl(\mathbf{Z}_{t:t-r}\bigr), \\[1.2ex]
\mathbf{Z}_t&= m\bigl(\mathbf{X}_{t:t-\mu}\bigr), \\[1.2ex]
\boldsymbol\epsilon_t^j &\sim p_{\boldsymbol\epsilon^j}, \quad j = 1,\dots,d_z, \\[1.2ex]
\mathbf{Z}_t^j &= g_j\Bigl(\bigl\{\mathbf{Z}_{t-s}^k \mid \mathbf{Z}_{t-s}^k \in Pa(\mathbf{Z}_t^j),\ s=1,\dots,\rho\bigr\},\,\boldsymbol\epsilon_t^j\Bigr).
\end{aligned}
\]
Here, \(r\) and \(\mu\) are predefined lags and \(m\) is a nonlinear mapping that reconstructs the current causal latent factor \(\mathbf{Z}_t\) from a slice of the observed process \(\mathbf{X}_{t:t-\mu}\). The bijectivity of \(f\) is thus replaced in \citet{Chen2024CRLNonInvertibleEnc} by a temporal context mechanism, where the observed data are generated, and the latent factors are inferred via two distinct and generally unrelated mappings: \(f\) and \(m\). 

\begin{remark}
While several models have been proposed before \cite{yao2022learning} in the time-varying setting to learn identifiable representations, these models do not treat the latent variables as causal, nor do they attempt to learn a causal process within the latent space. Notable examples include \emph{Time-Contrastive Learning (TCL)} \citep{hyvarinen2016TCL}, \emph{Permutation-based Contrastive Learning (PCL)} \citep{hyvarinen2019PCL}, and \emph{SlowVAE} \citep{klindt2021TemporalSparseCoding}, as well as methods designed for noisy data with structured nonlinear ICA \citep{halva2021disentangling}. Additional approaches include nonlinear ICA with a hidden Markov model to capture non-stationarity \citep{Hlv2020HiddenMN}, error estimation in nonlinear vector autoregressive models \citep{morioka2021independent}, and generalized nonlinear ICA frameworks for temporal data \citep{hyvarinen2017nonlinear}. Finally, recent contributions also explore identifiability in multi-view time series \citep{Huang2023IdentifViewsTS}.
\end{remark}


\subsection[Understanding the Generation Mechanism in CRL]{Understanding the Generation Mechanism in \gls{crl}}  

Most \gls{crl} work focuses on recovering latent factors but pays little attention to how those factors generate observations. Exploring this generative mapping matters because it validates and interprets the resulting causal representations.  \citet{lachapelle2022disentanglement, boussard2023towardsClimate} did impose structural constraints in \gls{crl} but did not explicitly focus on uncovering the underlying generative process. A contribution in this direction is the Sparse VAE introduced by \citet{moran2021identifiable}, which enforces a sparsity constraint on the decoder. Their model applies a binary mask  \( \Gamma \in \{0,1\}^{d_z \times d_x} \) to the latent variables before decoding them into the observed space. This formulation rests on the assumption of pure children (Equation \ref{eq:anchor_feat_moran}), and the generative process follows
\[
\mathbf{X}^j \;\sim\;\mathcal{N}\bigl(f_{\theta}(\Gamma_{:,j}\odot \mathbf{Z}),\;\sigma_j^2\bigr), 
\quad j=1,\dots,d_x,
\]
where \(\odot\) denotes the Hadamard product, \(f_{\theta}\) is the decoder, and \(\sigma_1^2,\dots,\sigma_{d_x}^2\) are fixed variance parameters.  For inference, \citet{moran2021identifiable} adopted a Bayesian framework, placing a Spike‐and‐Slab Lasso prior \citep{bai2021spike} on \(\Gamma\) and estimating its posterior via maximum a posteriori (MAP) optimization.  While elegant, this framework is restricted to \emph{static data} and does not infer any \emph{causal structure} among the latent variables.  Moreover, it remains unclear whether the employed sparsity prior adequately encodes the assumed structural constraints of Equation \ref{eq:anchor_feat_moran}, as the theoretical assumptions are not explicitly embedded in the inference mechanism.  Related efforts by \citet{zheng2022identifiability,zheng2023generalizing} likewise imposed sparsity constraints in static, nonlinear ICA settings, leveraging either \(\ell_1\) regularization or hybrid penalties combining \(\ell_0\) and \(\ell_1\) norms, but similarly stop short of modeling causal structure in the latent space.  

Two important papers integrating \gls{crl} and sparsity are worth mentioning. First, \cite{lachapelle2022disentanglement} proposed learning a causal representation \( \mathbf{Z}_t \) over time-varying data \( \mathbf{X}_t \) with a \emph{sparse mechanism shift}, meaning that only a few edges relate past latent representations to future ones. The transition mechanism in the latent space is expressed as:  
\[
p\bigl(\mathbf{z}_{t}^j \mid \mathbf{z}_{<t}\bigr)
= h_j(\mathbf{z}_{<t})\,
\exp\biggl(
    T_j\bigl(\mathbf{z}_{t}^j\bigr)^\top
    \lambda_j\bigl(\Gamma \odot \mathbf{z}_{<t}\bigr)
    - \Psi(\mathbf{z}_{<t})
\biggr) , \quad  j=1,\dots,d_z,
\]
where  
\begin{inparaenum}[(i)]
  \item \(h_j(\cdot)\) is the base measure,  
  \item \(T_j(\cdot)\) is the vector of sufficient statistics for the coordinate \(j\),  
  \item \(\lambda_j(\cdot)\) is the natural‐parameter map returning the canonical parameters of the exponential family,  
  \item \(\Psi(\cdot)\) is the log‐partition function ensuring normalization \citep{wainwright2008graphical},  
  \item and \(\Gamma\) is a binary mask enforcing sparsity on the past‐latent vector \(\mathbf Z_{<t}\).     
\end{inparaenum}
The inference is performed using variational inference, with the ELBO regularized by an \( \ell_0 \) or \(\ell_1 \) penalty over \( \Gamma \).  

It is important to note that, as in \citet{moran2021identifiable}, the inference strategy in \citet{lachapelle2022disentanglement} is not fully aligned with the theoretical structural assumptions supporting their identifiability results. Specifically, identifiability in their model relies on a graphical criterion requiring the existence of latent subsets whose parental and child sets uniquely identify each latent factor. However, it remains unclear how standard \( \ell_1 \) regularization during inference could enforce such a structural constraint in practice. More importantly, no form of sparsity is imposed on the mapping between latent and observed variables, which is what our approach instantiates.

The second most similar work to ours is \cite{boussard2023towardsClimate, brouillard2024causalClimate}, which enforces a sparsity constraint on the decoding function while performing \gls{crl} for time-series climate data. However, their approach assumes a single-parent decoding constraint (Figure \ref{fig:single_parent_dec}). To achieve this, the edge weights relating the latent factors \(\mathbf{Z}_t\) to the observed features \(\mathbf{X}_t\) are modeled with a non-negative and orthogonal matrix \( \Gamma \), ensuring that at most one entry per row is nonzero. Formally, the generative model assumes:  
\begin{equation}
\label{eq:gen_mecha_spd}
\mathbf{X}^j_t \mid \mathbf{Z}_t \sim \mathcal{N}(\Gamma_{:,j} \mathbf{Z}_t, \sigma_j^2).
\end{equation}
To enforce structural single-parent decoding, \cite{boussard2023towardsClimate} defined the orthogonality constraint  \(h(\Gamma) = \Gamma^\top \Gamma - I_{d_x}\) during training, which is consistent with the structural constraint of single-parent decoding.  However, this single-parent assumption is highly restrictive, as explained in Section \ref{sect_crl:intro}, since it does not allow a mixture of latent factors to generate observed variables. Such a scenario arises where causal relationships among observed features lead to multiple latent parents. Our work generalizes this approach by allowing multiple latent factors as parents, making it a more flexible and realistic assumption for a broader range of applications.

\subsection{Subspace Clustering}
Subspace clustering segments data that lie near a union of low-dimensional linear subspaces. In contrast, Principal Component Analysis (PCA) \citep{hastie2009elements} fits all data with a single subspace. Hence, subspace clustering can be intuitively understood as a generalization of PCA by fitting multiple subspaces, these subspaces may intersect when different clusters share overlapping dimensions, so that the heterogeneous structure in high-dimensional data is better captured. Our method adopts the self-expression property from subspace clustering, but applies it to the gradients of observed features with respect to latent variables.  A general definition of subspace clustering is as follows \citep{abdolali2021SubspaceClstrRev,qu2023SubspaceClstrSurv}:

\begin{definition}[Subspace Clustering]
\label{def:subspace_clstr}
Let \( X \in \mathbb{R}^{d \times n} \) be a high-dimensional dataset, where each column represents a data point in \( \mathbb{R}^d \). Suppose the data lie in a union of \( c \) unknown linear subspaces \( \mathcal{S}_1, \mathcal{S}_2, \dots, \mathcal{S}_c \subset \mathbb{R}^d \), with corresponding intrinsic dimensions \( d_1, d_2, \dots, d_c \), where \( d_i \ll d \) for all \( i \in \{1, \dots, c\} \).  

The goal of \emph{subspace clustering} is twofold:  
\begin{inparaenum}[(1)]
    \item to assign each data point to its generating subspace, and  
    \item to estimate the parameters (e.g., bases or projection matrices) that define each subspace.
\end{inparaenum}
\end{definition}

Definition~\ref{def:subspace_clstr} highlights that similarity between data points is assessed through their compatibility with low-dimensional subspaces. Consequently, points within the same cluster exhibit strong linear dependencies and lie close to a shared subspace.


\subparagraph{Sparse Subspace Clustering (SSC)}  
Most classical subspace clustering methods struggle to handle both noise and outliers simultaneously \citep{costeira1998multibody, tipping1999mixturesPCA, tseng2000nearest,kanatani2001motion, zhang2009median, LocSubspaceAffin2006, goh2007segmenting}, and they typically rely on prior knowledge of the dimensions of the underlying subspaces. To address these limitations, a major line of work introduces \emph{sparsity} into subspace clustering algorithms~\citep{vidal2009sparse, elhamifar2010clustering, geometrySSC2012, elhamifar2013sparse}. Sparsity helps to mitigate noise and alleviates the need for explicit knowledge of subspace dimensions. A foundational idea underpinning many \gls{ssc} approaches is the self-expression property. Imposing sparsity on the coefficients of this linear combination leads to models that encourage locality and robustness. The seminal work of \citet{vidal2009sparse} employed \( \ell_1 \)-regularization for this purpose. Subsequent developments have explored a variety of regularization schemes, including \( \ell_0 \)-based formulations~\citep{yang2016L0SSC, yang2018L0SSC}, nuclear norm minimization~\citep{liu2012LowRkRep}, Frobenius norm penalties~\citep{lu2012robustLSR}, and elastic net regularization~\citep{you2016oracle}.

\subparagraph{Deep \gls{ssc}}
Given the high ambient dimensionality of many real-world datasets, recent efforts have focused on learning lower-dimensional representations in which subspace structure is more amenable to analysis. The motivation is that the raw input space may not satisfy the assumptions required for linear self-expression, and thus, a learned representation could better reveal the latent subspace geometry. Early work projected data into linear latent spaces~\citep{patel2013latentLinSSC}, while more recent approaches employ neural networks for joint representation learning and subspace clustering~\citep{ji2017deepSSC, abavisani2018deep, zhou2019latentDistDeepSSC, peng2020deep, xie2020MultiViewsDeepSSC, yang2020residualDepSSC}.  Unlike these approaches, our framework does not seek to learn \underline{representations} in which standard \gls{ssc} can be applied, but rather induces a modular structure directly in the observation space via an \gls{ssc} over \underline{decoder gradients}. 

\section{Modeling}
\label{sect_crl:theory}
\subsection{Subspace Detection Under Self-Expression Property}
\label{sect_crl:theory_nonoverlap}

\subsection*{Main modeling assumptions}
To analyze the recoverability of modular structure via Jacobian self-expression, we must understand the statistical and geometric properties of decoder gradients. In this section, we formalize these conditions by placing mild distributional and smoothness assumptions on the latent variables \( \mathbf{Z}\) and decoder \(f\). We model \( \mathbf{Z} \in \mathbb{R}^{d_z} \) as sub-Gaussian random vectors. This assumption helps derive concentration inequalities and underpins our stability analyses, provided the decoder \(f\) is smooth in the following sense:

\begin{assumption}[Smoothness of Decoder]
\label{assp:smooth_f}
A decoder \(f\) with coordinates 
\[
f = (f_1, \dots, f_{d_x})^\top
\]
is said to be \emph{\(L\)-smooth} with \(L>0\) if 
\[
f \in \mathcal{C}^2\bigl(\mathbb{R}^{d_z}; \mathbb{R}^{d_x}\bigr)
\]
and there exists \(L>0\) such that, for each \(i \in \llbracket 1, d_x \rrbracket\), the Hessian of the output coordinate \(f_i\) satisfies
\[
\sup_{\mathbf{z} \in \mathbb{R}^{d_z}}
\bigl\lVert D^2 f_i(\mathbf{z})\bigr\rVert_{\mathrm{op}}
\;\le\; L.
\]
\end{assumption}
The Jacobian \( Df(\mathbf{z}) \in \mathbb{R}^{d_x \times d_z} \) captures the local linear structure of the decoder around each latent point \( \mathbf{z} \). We model \( Df(\mathbf{z}) \) as a random matrix whose columns lie on the unit sphere \( \mathbb{S}^{d_z - 1} \), allowing for anisotropy through statistical dependence between columns (cf. Definition \ref{def:isotropic_matrix}). Normalizing gradients is not a restrictive condition, it can be enforced during training and is widely used in practice to stabilize optimization, notably via gradient clipping~\citep{Zhang2020GradClippingWhy}. 

Building on the assumption that the Jacobian columns are unit-norm and anisotropic, we now introduce a structured prior that captures modularity in the decoder: the \emph{union of subspaces} model. In particular, we model the columns of the Jacobian \( Df(\mathbf{z}) \) as lying in a union of low-dimensional subspaces:

\begin{assumption}[Union of Subspaces Assumption]
\label{assp:union_subspaces}
There exist \( M \) deterministic linear subspaces \( \{ \mathcal{S}_m \}_{m=1}^M \), where each \( \mathcal{S}_m \in \mathrm{Gr}(d_m, d_z) \). Accordingly, there is a partition of output indices
    \[
      \{1,2,\dots,d_x\}
      \;=\;\bigsqcup_{m=1}^M I_m,
      \quad
      |I_m| = n_m,
      \quad
      \sum_{m=1}^M n_m = d_x.
    \]
We then define the block-wise mapping
    \[
      f^{(m)}:\mathbb R^{d_z}\;\longrightarrow\;\mathbb R^{n_m},
      \qquad
      f^{(m)}(\mathbf z)
      :=\bigl(f_j(\mathbf z)\bigr)_{j\in I_m}.
    \]
We assume the Jacobian of each block $f^{(m)}$ has its columns in $\mathcal S_m$:
    \[
      Df^{(m)}(\mathbf z)
      = \bigl[\nabla_{\mathbf z}f_j(\mathbf z)\bigr]_{j\in I_m}
      \;\in\;\mathbb R^{d_z\times n_m},
      \quad
      \operatorname{cols}\bigl(Df^{(m)}(\mathbf z)\bigr)
      \subseteq \mathcal S_m,
      \quad
      \forall\,\mathbf z\in\mathbb R^{d_z}.
    \]

As a result, each gradient lies in one of the \( M \) subspaces, that is, \(\nabla_{\mathbf z}f_j(\mathbf z) \in \cup_{m=1}^M \mathcal S_m\). 
\end{assumption}

Figure~\ref{fig:union_subspaces} illustrates Assumption~\ref{assp:union_subspaces}: for an arbitrary realization \(\mathbf{z}\), the gradients \(\nabla_{\mathbf{z}}f_1(\mathbf{z}),\, \nabla_{\mathbf{z}}f_2(\mathbf{z}),\, \nabla_{\mathbf{z}}f_3(\mathbf{z})\) are assumed to lie on the space \(\mathcal{S}_1\) at the intersection with the unit sphere \(\mathbb{S}^{d_z-1}\) (red contour). Similarly, gradients \(\nabla_{\mathbf{z}}f_4(\mathbf{z}),\, \nabla_{\mathbf{z}}f_5(\mathbf{z}),\, \nabla_{\mathbf{z}}f_6(\mathbf{z})\) lie in the subspace \(\mathcal{S}_2\), precisely on the dashed blue contour. Assumption~\ref{assp:union_subspaces} also implies that for another arbitrary \(\mathbf{z}'\), the gradients \(\nabla_{\mathbf{z}}f_1(\mathbf{z}'),\, \nabla_{\mathbf{z}}f_2(\mathbf{z}'),\, \nabla_{\mathbf{z}}f_3(\mathbf{z}')\) would change position along the red contour but still lie within \(\mathcal{S}_1\).
 

\begin{figure}[ht]
     \centering
    \includegraphics[scale=0.9]{figures/transp_crl/subspace_stucture.pdf}
    \caption{A geometric illustration of the assumption of subspaces union (\ref{assp:union_subspaces}) that underlies subspace clustering. Two planes are presented as subspaces of the Jacobian span $(\mathcal{S}_1, \mathcal{S}_2)$, within which gradients are drawn.}
  \label{fig:union_subspaces}
\end{figure}

Let \(\mathcal{P}\bigl(Df(\mathbf{Z}),C_{:,j}\bigr)\) denote the \emph{column‐wise sparse self‐expression problem} for the Jacobian column \(\nabla_{\mathbf{z}}f_j\), defined by
\begin{equation}
\label{eq:lasso_per_gradj}
\begin{aligned}
\min_{C_{:,j}\,\in\,\mathbb{R}^{d_x}}
  \quad&\|C_{:,j}\|_1,\\[0.8ex]
\text{subject to}\quad
  &\nabla_{\mathbf{z}}f_j(\mathbf{Z})
   = Df(\mathbf{Z})\,C_{:,j}
   \quad\text{a.s.},\\[0.6ex]
  &C_{j,j}=0.
\end{aligned}
\end{equation}
Alternatively, we define a matrix-level formulation with a quadratic penalty in expectation, referred to as the \emph{expected global self-expression problem}, denoted \(\mathcal{P}_{\lambda}(Df)\):
\begin{equation}
\label{eq:lasso_penalty_fct}
\min_{\substack{C\in\mathbb{R}^{d_x\times d_x}\\\mathrm{diag}(C)=\mathbf{0}}}
  \|C\|_1
  \;+\;\lambda\,\mathbb{E}_{\mathbf{Z}}\bigl[\|Df(\mathbf{Z})
    - Df(\mathbf{Z})\,C\|_F^2\bigr].
\end{equation}
The second formulation is often more convenient in practice, especially during training, since \( f \) is typically implemented as a neural network. However, both formulations are central to our theoretical analysis: the first is used to study the recovery of disjoint clusters (Theorem \ref{thm:subspace_detect_whp}, Proposition \ref{prop:recovery_nonoverlap_spec_cltsr}), while the second provides the foundation for analyzing overlapping clusters and establishing stability guarantees (Theorems \ref{thm:overlap_cluster_recovery} and \ref{thm:genetalization_SExprLoss}, Proposition \ref{prop:jacobian-perturbation}).
 
\subsection*{Equivalence of \(\mathcal{P}(Df(\mathbf{Z}), C_{:,j})\) and \(\mathcal{P}_{\lambda}(Df)\)} 

We now analyze under which conditions one can assert that the series of problems \(\mathcal{P}(Df(\mathbf{Z}), C_{:,j})\) is identical to solving the global and penalized problem \(\mathcal{P}_{\lambda}(Df)\). 

We first observe that
\[
\mathbb{E}_{\mathbf{Z}}\bigl[\|Df(\mathbf{Z}) - Df(\mathbf{Z})\,C\|_F^2\bigr]
= \sum_{j=1}^{d_x} \mathbb{E}_{\mathbf{Z}}\bigl[\|\nabla_{\mathbf{z}} f_j(\mathbf{Z}) - Df(\mathbf{Z})\,C_{:,j}\|_2^2\bigr],
\]
and likewise
\[
\|C\|_1 = \sum_{j=1}^{d_x} \|C_{:,j}\|_1.
\]

Thus, the global objective
\[
\mathbb{E}_{\mathbf{Z}}\bigl[\|Df(\mathbf{Z}) - Df(\mathbf{Z})\,C\|_F^2\bigr] + \lambda \|C\|_1
\]
decouples into \(d_x\) independent column-wise expected-risk Lasso subproblems \(\mathcal{P}_{\lambda}(Df(\mathbf{Z}), C_{:,j})\) given by
\begin{equation}
    \label{eq:lasso_penalty_fct_j}
    \begin{aligned}
\min_{C_{:,j} \in \mathbb{R}^{d_x}}  \;
& \|C_{:,j}\|_1
+ \lambda \; \mathbb{E}_{\mathbf{Z}}\bigl[\|\nabla_{\mathbf{z}} f_j(\mathbf{Z})- Df(\mathbf{Z})\,C_{:,j}\|_2^2\bigr], \\[1.2ex]
& \text{subject to} \quad C_{j,j} = 0.
\end{aligned}
\end{equation}

In fact, solving the expected global self-expression problem \(\mathcal{P}_{\lambda}(Df)\) is \textbf{equivalent}, i.e., has the same solution set, to solving, \textbf{independently} for each $j=1,\dots,d_x $ the column-wise expected-risk Lasso subproblem \(\mathcal{P}_{\lambda}(Df(\mathbf{Z}), C_{:,j})\) by stacking its minimizers  $C_{:,1}^*, \dots, C_{:,d_x}^*$.

As a result, to show the equivalence of \(\mathcal{P}(Df(\mathbf{Z}), C_{:,j})\) and \(\mathcal{P}_{\lambda}(Df)\), it is enough to investigate when the two problems \(\mathcal{P}(Df(\mathbf{Z}), C_{:,j})\) and \(\mathcal{P}_{\lambda}(Df(\mathbf{Z}), C_{:,j})\) are equivalent for $j=1,\dots,d_x $.
In the following, we denote the quadratic penalty as 
\[
\ell_j(C_{:,j}) = \mathbb{E}_{\mathbf{Z}}\bigl[\|\nabla_{\mathbf{z}} f_j(\mathbf{Z})- Df(\mathbf{Z})\,C_{:,j}\|_2^2\bigr]
\]

\begin{remark}[Feasibility and Convexity of \(\mathcal{P}_{\lambda}(Df(\mathbf{Z}), C_{:,j})\) and \(\mathcal{P}_{\lambda}(Df)\)]
We note that a feasible solution exists to the problem \(\mathcal{P}\bigl(Df(\mathbf{Z}),C_{:,j}\bigr)\) (Equation \ref{eq:lasso_per_gradj}) since we assume self-expressiveness (\ref{assp:self_expression}). Moreover, since \(\mathbf Z \) is sub-Gaussian (\(\|\mathbf Z\|_{\psi_2} < \infty\)) and $f$ is smooth as in Assumption \ref{assp:smooth_f}, then the second moments are finite, that is,  $\displaystyle \mathbb{E}_{\mathbf Z}\,\|Df(\mathbf Z)\|_F^2 < \infty$ which is equivalent to saying  $\displaystyle \mathbb{E}\,\|\nabla f_j(\mathbf Z)\|_2^2 < \infty$ for \(j \in  \llbracket 1, d_x \rrbracket\).  Thus, the quadratic penalty in the optimization problem \(\mathcal{P}_{\lambda}(Df(\mathbf{Z}), C_{:,j})\) (Equation \ref{eq:lasso_penalty_fct_j}) is always finite.

Our problem is a convex with affine constraints: the maps
$$
C_{:,j} \longrightarrow \|C_{:,j}\|_1, \quad C_{:,j} \longrightarrow  \ell_j(C_{:,j})
$$
are convex (the Hessian of \(\ell_j\) is \(2\,\mathbb{E}_{\mathbf{Z}}\bigl[\,Df(\mathbf Z)^{\!\top}Df(\mathbf Z)\bigr]\) which is positive semi-definite), plus the constraint $C_{:,j} \longrightarrow  \nabla_{\mathbf{z}} f_j- Df \,C$ is affine. 
\end{remark}

Let \(\mathcal{P}_t\bigl(Df(\mathbf{Z}),C_{:,j}\bigr)\) be the \emph{hard-constraint} problem for each column
\begin{equation}
\label{eq:}
\begin{aligned}
\min_{C_{:,j} \in \mathbb{R}^{d_x}} \; & \|C_{:,j}\|_1 \\[1.2ex]
\text{subject to} \quad
& \ell_j(C_{:,j}) \le t, \quad  C_{j,j} = 0. \\[0.8ex]
\end{aligned}
\end{equation}

\begin{theoremBox}[Equivalence of \(\mathcal{P}_t\bigl(Df(\mathbf{Z}),C_{:,j}\bigr)\) and \(\mathcal{P}_{\lambda}(Df(\mathbf{Z}), C_{:,j})\)]
\label{thm:equiv_hard_penalized_prob_j}
Assume the expected Gram matrix of the Jacobian  \(\mathbb{E}_{\mathbf{Z}}\bigl[\,Df(\mathbf Z)^{\!\top}Df(\mathbf Z)\bigr]\) is positive definite, so that the quadratic penalty $\ell_j$ is strictly convex for each $j=1,\dots,d_x $. Then, for any tolerance $t \ge 0$, there is a unique and finite \(\lambda_j(t) \ge 0 \) such that the solution set of \(\mathcal{P}_t\bigl(Df(\mathbf{Z}),C_{:,j}\bigr)\) coincides with that of \(\mathcal{P}_{\lambda}(Df(\mathbf{Z}), C_{:,j})\).
\end{theoremBox}

\textbf{Back to the expected global self-expression problem}  
Because each column \(C_{:,j}\) has its own independent constraint \(C_{j,j}=0\) and objective term, the optimization problem \(\mathcal{P}_{\lambda}(Df)\) is solved by combining the \(d_x\) column-wise solutions \(C_{:,j}^*(\lambda)\).  Conversely, solving all column-wise constrained problems with levels \(t_j\) (Theorem \ref{thm:equiv_hard_penalized_prob_j}) produces the same global minimizer once we pick
\[
  \bar \lambda = \max_{j \in  \llbracket 1, d_x \rrbracket} \lambda_j(t_j),
\]
by the \emph{exact-penalty theorem} \citep{di1994exactpenalty, bertsekas2015convexopti} and for all \( \lambda \ge \bar{\lambda} \), the penalized expected-risk subproblem \(\mathcal{P}_{\lambda}(Df(\mathbf{Z}), C_{:,j})\) recovers the same minimizer \(C_{:,j}^*(\lambda)\) as the hard-constrained version \(\mathcal{P}\bigl(Df(\mathbf{Z}),C_{:,j}\bigr)\). 

\subsection*{Subspace Geometry and Detection}
The goal of solving the sparse self-expression problem is not merely to reconstruct each Jacobian column from others, but to do so in a way that reveals the underlying subspace membership of each feature: we are interested in whether the support of the optimal coefficient vector \( C_{:,j}^* \) includes only indices corresponding to columns that lie in the same subspace as \( \nabla_{\mathbf{z}} f_j \). This leads to the \emph{subspace detection property} \citep{GeomAnlysSSC2012}, which underpins the correctness of subspace clustering:

\begin{definition}[Subspace Detection Property]
\label{def:subspace_detect}
Let $\{\mathcal{S}_m\}_{m=1}^M\subseteq\mathbb{R}^{d_z}$ be a collection of linear subspaces, and suppose each column $\nabla_{\mathbf z}f_j(\mathbf Z)$ of the Jacobian $\mathrm{D}f(\mathbf Z)$ lies in some $\mathcal{S}_{m_{j}}$ with $m_{j} \in\{1,\dots,M\} $.  We say that the decoder $f$ satisfies the \emph{subspace detection property} if, for every $j\in\{1,\dots,d_x\}$, the minimizer $C^*_{:,j}$ of \(\mathcal{P}\bigl(\mathrm{D}f(\mathbf Z),\,C_{:,j}\bigr)\) obeys
\begin{equation}
    \label{eq:subspace_detect}
      C^*_{k,j}\neq 0
  \quad\Longrightarrow\quad
  \nabla_{\mathbf z}f_k(\mathbf Z),\;\nabla_{\mathbf z}f_j(\mathbf Z)\;\in\;\mathcal{S}_{m_j}
  \quad\text{almost surely.}
\end{equation}

In other words, nonzero entries in $C^*_{:,j}$ occur only at indices $k$ whose gradients lie in the same subspace as $\nabla_{\mathbf z}f_j$.
\end{definition}

From Figure~\ref{fig:union_subspaces}, if we assume \(\nabla_{\bm z}f_{1}(\mathbf Z)\) is self-expressed by \(\nabla_{\bm z}f_{2}(\mathbf Z)\) and \(\nabla_{\bm z}f_{3}(\mathbf Z)\), then
\[
C^{*}_{1,2},\,C^{*}_{1,3}\neq 0,
\]
and the subspace detection property of \ref{def:subspace_detect} holds because
\[
\nabla_{\bm z}f_{1}(\mathbf Z),\;
\nabla_{\bm z}f_{2}(\mathbf Z),\;
\nabla_{\bm z}f_{3}(\mathbf Z)
\;\in\;\mathcal S_{1},
\]
as assumed in Figure~\ref{fig:union_subspaces}.  However, this does not imply that \(\nabla_{\bm z}f_{1}(\mathbf Z),\,\nabla_{\bm z}f_{2}(\mathbf Z),\,\nabla_{\bm z}f_{3}(\mathbf Z)\) are the only gradients lying in \(\mathcal S_{1}\); other gradients \(\nabla_{\bm z}f_{j}(\mathbf Z)\) may also lie in \(\mathcal S_{1}\) (represented by black dots on the red contour in Figure~\ref{fig:union_subspaces}), but with \(C^{*}_{1,j}=0\).

This is precisely the goal of \gls{ssc}: to represent each gradient sparsely using only other gradients from the same subspace.  Since membership in the same subspace is only a necessary condition for subspace detection, when it is violated, for example, \(\nabla_{\bm z}f_{1}(\mathbf Z)\in\mathcal S_{1}\) but \(\nabla_{\bm z}f_{4}(\mathbf Z)\in\mathcal S_{2}\), the contrapositive of Equation \ref{eq:subspace_detect} gives \(C^{*}_{1,4}=0.\)

\paragraph{Geometry of linear subspaces}
A central challenge in subspace clustering is to determine when sparse self-expression can correctly recover the subspace membership of each feature. This requires a quantitative notion of the geometric separation between subspaces. Following the line of geometric arguments of \cite{geometrySSC2012}, a classical tool is the system of \emph{principal angles} (\ref{def:principal_angles}), which generalizes the notion of angle between vectors to the setting of linear subspaces. From these, one can define a scalar measure of closeness known as the \emph{subspace affinity} (\ref{def:subspace_affinity}), which plays a role in the theoretical analysis of clustering algorithms. Intuitively, the smaller the affinity between subspaces, the more they are distinguishable and the more likely the subspace detection property is to hold. In the following, we give a formal definition of both principal angles and affinity for subspaces, and then present our main theorem stating the maximum permissible affinity between subspaces for the subspace detection property to hold \gls{whp}.

\begin{definition}[Principal Angles Between Subspaces]\label{def:principal_angles}
Let \(\mathcal{S}_m\in\mathrm{Gr}(d_m,d_z)\) and \(\mathcal{S}_{m'}\in\mathrm{Gr}(d_{m'},d_z)\) be linear subspaces of dimensions \(d_m\) and \(d_{m'}\), respectively, and set \(d=\min\{d_m,d_{m'}\}\).  The \emph{principal angles} \(\theta^{(1)}_{m,m'},\dots,\theta^{(d)}_{m,m'}\) between \(\mathcal{S}_m\) and \(\mathcal{S}_{m'}\) are defined recursively by
\[
\cos\bigl(\theta^{(i)}_{m,m'}\bigr)
\;\coloneqq\;
\max_{\substack{\mathbf y\in\mathcal S_m \\ \|\mathbf y\|=1}}
\;\max_{\substack{\mathbf z\in\mathcal S_{m'} \\ \|\mathbf z\|=1}}
\mathbf y^\top \mathbf z,
\]
subject to the orthogonality constraints
\[
\mathbf y^\top \mathbf y_j = 0,
\quad
\mathbf z^\top \mathbf z_j = 0,
\qquad
j=1,\dots,i-1,
\]
where \(\{\mathbf y_j\}\) and \(\{\mathbf z_j\}\) are the previously selected maximizers.
\end{definition}

\paragraph{Interpretation}
The first principal angle \( \theta^{(1)} \) measures the smallest angle between any pair of unit vectors, one from each subspace (cf. Figure \ref{fig:principal_angles}). Subsequent angles capture progressively less aligned directions, orthogonal to those already considered. Together, these angles quantify the degree of alignment between two subspaces: large angles indicate strong separation, while small angles suggest potential overlap and confusion.
\begin{figure}[ht]
     \centering
    \includegraphics[scale=0.5]{figures/transp_crl/principal_angles.pdf}
    \caption{An illustration of the two principal angles between two subspaces \(\mathcal{S}_m, \mathcal{S}_{m'}\). }
  \label{fig:principal_angles}
\end{figure}

Although the full sequence of principal angles provides a rich geometric comparison, it is often convenient to compress this information into a single scalar.

\begin{definition}[Subspace Affinity]
\label{def:subspace_affinity}
The \emph{affinity} between subspaces \( \mathcal{S}_m \) and \( \mathcal{S}_{m'} \) is defined as
\[
\operatorname{aff}(\mathcal{S}_m, \mathcal{S}_{m'}) \coloneqq \sqrt{ \sum_{i=1}^{d} \cos^2\big( \theta^{(i)}_{m,m'} \big) } \;,
\]
where \( d = \min(d_m, d_{m'}) \).
\end{definition}

\paragraph{Geometric Significance}
The affinity captures a cumulative alignment: a zero value indicates orthogonal subspaces, while higher values reflect greater overlap. In the context of sparse self-expression, lower affinities reduce the risk of selecting elements from incorrect subspaces, thereby increasing the likelihood of correct clustering. Thus, subspace affinity is a key factor governing the success of subspace recovery. 

We now present our main theoretical result, which provides conditions under which the sparse self-expression problem correctly detects subspace structure \gls{whp}.

\begin{theoremBox}[Subspace Detection via Sparse Self-Expression]\label{thm:subspace_detect_whp}
Let \(\mathbf Z\in\mathbb R^{d_z}\) be a sub-Gaussian random vector with \(\|\mathbf Z\|_{\psi_2}\le K\), and let \(f\) be \(L\)-smooth as in Assumption~\ref{assp:smooth_f}. Suppose the columns of the Jacobian \(Df\) follow the union-of-subspaces model (Assumption~\ref{assp:union_subspaces}), i.e., they lie in a union of \(M\) deterministic subspaces \(\{\mathcal S_m\}_{m=1}^M\subset\mathbb R^{d_z}\), with \(n_m\) columns in subspace \(\mathcal S_m\).

Then, there exist universal constants \(\Lambda_1,\Lambda_2>0\) such that if
\begin{equation}
\label{eq:incoherence_gap}
\max_{k\neq m}\,\mathrm{aff}\bigl(\mathcal S_k,\mathcal S_m\bigr)\,
\sqrt{\log(n_k+1)}
\;\le\;
\Lambda_1\,K\,L\,\sqrt{\log n_m},
\quad
\forall\,m\in\{1,\dots,M\},
\end{equation}
then \(f\) satisfies the subspace detection property with a probability of at least
\[
1 - 
\sum_{m=1}^M n_m 
\exp\!\Bigl(-\tfrac{\Lambda_2^2\log n_m}{2\,d_m}\Bigr)
\;+\;
\sum_{m=1}^M \frac{2(M-1)}{\sqrt{n_m+1}}.
\]
\end{theoremBox}

\paragraph{From point-based \gls{ssc} to latent–gradient \gls{ssc}}
Before discussing the results of Theorem \ref{thm:subspace_detect_whp}, it is important to delineate the main differences in both assumptions, nature of the problem tackled, and nature of the results in our work compared to that of \citet{geometrySSC2012}. First, \citet{geometrySSC2012} analyzed \gls{ssc} on \emph{standard generative models} among which a semi-random one: \emph{static data points} are sampled uniformly at \underline{random} but lie \emph{exactly} in a union of \underline{fixed} linear subspaces, possibly mixed with uniform-spherical outliers. Their proof employs a primal–dual witness construction \citep{wainwright2009sharp} together with sphere-cap concentration \citep{vershynin2018HDProba} to show that the $\ell_1$ self-expressive problem enjoys the subspace-detection property \gls{whp} whenever a minimal gap in affinity between subspaces is satisfied.

\textbf{Our setting is far more challenging:} Our setting is analogous in that the tangent subspaces
$\{\mathcal S_m\}_{m=1}^{M}$ are fixed, whereas the Jacobian columns $\{\nabla_{\mathbf z}f_i(\mathbf Z)\}_{i=1}^{d_x}$ \underline{are random}; however, the randomness now stems from a \emph{sub-Gaussian} latent code $\mathbf Z$ propagated through a twice-differentiable decoder $f$. Consequently, purely geometric arguments are augmented by high-dimensional probability tools and exploit now a global Hessian bound on coordinates output \(\Vert D^2f_i(\mathbf z)\Vert_{\mathrm{op}}\) (\ref{assp:smooth_f}) to control how fast gradients rotate. Thus, while we retain the three-step template proof (dual certificate $\rightarrow$ support recovery $\rightarrow$ spectral clustering) of \citet{geometrySSC2012}, all probabilistic estimates are new and tailored to the Jacobian self-expression problem (see Appendix \ref{proof:subspace_detect_whp} for formal proofs and Table \ref{tab:comparison_sscgeomtric}).
\begin{table}[t]
  \centering
  \caption{Key differences between our analysis and prior SSC theory.}
  \renewcommand{\arraystretch}{1.2}
  \begin{tabular}{>{\raggedright}p{3cm} >{\raggedright}p{5.2cm} >{\raggedright\arraybackslash}p{5.2cm}}
    \toprule
    \textbf{Aspect} &
    \textbf{Candès \&\ Soltanolkotabi (2012)} &
    \textbf{This work} \\
    \midrule
    Data to be clustered &
    Random points \emph{on} the subspaces (semi-random model) &
    Random Jacobian columns induced by latent variable $\mathbf Z$ \\
    Regularity control &
    Purely geometric; no smoothness parameter &
    Global Hessian bound $L$ on decoder $f$ \\
    Probability tools &
    Geometric inequalities for uniformly random points on the sphere &
    Vershynin’s matrix deviation bounds for sub-Gaussian design \\
    Noise/robustness &
    Outliers handled via robust SSC extensions &
    Latent noise and curvature enter constants $K,L$ in \ref{prop:jacobian-perturbation} \\
    \bottomrule
  \end{tabular}
  \label{tab:comparison_sscgeomtric}
\end{table}



Theorem~\ref{thm:subspace_detect_whp} carries several important implications for \gls{crl} via Jacobian self-expression:
\begin{enumerate}[label=(\arabic*)]
    \item \textbf{Sample Complexity per Latent Subspace:}  
    Suppose we want to detect all subspaces with an error of at most \(\epsilon > 0\). If we allocate "the global budget" \(\epsilon\) uniformly across \(\{\mathcal{S}_m\}_{m=1}^M\), then for each \(m \in \{1, \dots, M\}\), we require
    \begin{equation} \label{eq:AmBm_bound}
    \underbrace{n_m \exp\!\left(-\tfrac{\Lambda_2^2 \log n_m}{2\,d_m}\right)}_{A_m}
    \;+\;
    \underbrace{\frac{2(M-1)}{\sqrt{n_m+1}}}_{B_m}
    \leq \frac{\epsilon}{M}.
    \end{equation}
    
    For \(A_m \), it suffices to have
    \begin{equation} \label{eq:Am_condition}
    A_m = n_m^{1 - \frac{\Lambda_2^2}{2d_m}} \leq \frac{\epsilon}{2M}.
    \end{equation}
    
    An interesting observation is that the failure probability does not decrease indefinitely with increasing \(n_m\) if the subspace dimension \(d_m\) satisfies \(d_m \geq \tfrac{\Lambda_2^2}{2}\). Otherwise, \(A_m\) could grow with \(n_m\), even though \(B_m\) decreases.  

    In the case \(d_m < \tfrac{\Lambda_2^2}{2}\), we have
    \begin{equation} \label{eq:Am_nm_bound}
    A_m \leq \frac{\epsilon}{2M}
    \iff
    n_m \geq \left(\frac{2M}{\epsilon}\right)^{\tfrac{2d_m}{\Lambda_2^2 - 2d_m}}.
    \end{equation}
    
    Similarly, for \(B_m\), we require
    \begin{equation} \label{eq:Bm_nm_bound}
    B_m \leq \frac{\epsilon}{2M}
    \iff
    n_m \geq 16 \left(\frac{M(M-1)}{\epsilon}\right)^2
    = \Theta\!\left(\frac{M^4}{\epsilon^2}\right).
    \end{equation}
    
    Therefore, each latent-induced subspace \(\mathcal{S}_m\) should have at least
    \begin{equation} \label{eq:final_nm_bound}
    n_m = \Omega\!\left(\left(\frac{2M}{\epsilon}\right)^{\tfrac{2d_m}{\Lambda_2^2 - 2d_m}}
    + \frac{M^4}{\epsilon^2}\right)
    \end{equation}
    columns observed to reliably detect and separate it from the others.  

\textbf{Geometric intuition:} For small \(d_m\), low-dimensional subspaces are "thin" enough to remain well-separated in the ambient space, so random Jacobian columns from different factors are unlikely to align. When \(d_m\) grows large, linear subspaces tend to "flatten", and almost any random direction has a large component in several subspaces. \gls{ssc} may then fail to correctly detect columns. If \(d_m > \tfrac{\Lambda_2^2}{2}\), increasing \(n_m\) does not help; the failure term \(A_m\) stops decaying, signaling an inherent identifiability barrier rather than a dimensionality limitation of the observed space.

    \item \textbf{Incoherence Requirement:}  
    The condition
    \begin{equation} \label{eq:incoherence}
    \max_{k \ne m} \operatorname{aff}(\mathcal{S}_k, \mathcal{S}_m) \cdot \sqrt{\log(n_k + 1)}
    \lesssim K L \sqrt{\log n_m}
    \end{equation}
    quantifies how "far apart" any two subspaces must be, accounting for dimensionality and sub-Gaussian variability in \(\mathbf{Z}\) and, intuitively, the lower the affinity between subspaces, the less they are confused. The Hessian bound \(L\) and latent noise \(K\) suggest that stronger Lipschitz regularization or tighter latent priors can reduce the right-hand side and thus relax the incoherence requirement.

    \item \textbf{Effect of Smoothness and Concentration on Identifiability:}  
    The dependence on \(K\) and \(L\) shows that both the stochasticity of latent \(\mathbf{Z}\) and the nonlinearity of \(f\) affect subspace recovery. Making \(f\) smoother (smaller Hessians) or latent priors more concentrated (smaller sub-Gaussian norm) allows the same clustering guarantees to hold under weaker incoherence conditions.
\end{enumerate}


\subsection{From Subspace Detection to Cluster Recovery}

Theorem~\ref{thm:subspace_detect_whp} guarantees that under suitable incoherence conditions, the sparse self-expression solution \( C^* \) is subspace-preserving: each Jacobian column \( \nabla_{\mathbf{z}} f_j \) is reconstructed using only columns from the same subspace. This property is not only crucial for identifiability but also enables the recovery of the modular structure among the observed features. The following proposition formalizes how this subspace structure, when encoded in \( C^* \), can be translated into feature clusters using spectral methods.

\begin{proposition}[Recovery of Feature Clusters via Spectral Clustering]
\label{prop:recovery_nonoverlap_spec_cltsr}
Let the following conditions hold:
\begin{itemize}
    \item \textbf{\( \ell_1 \)-self-expression:} For each column \( j \), let \( C^*_{:,j} \) be the solution to the problem \( \mathcal{P}(Df(\mathbf{Z}), C_{:,j}) \) as in Equation~\ref{eq:lasso_per_gradj}.
    
    \item \textbf{Affinity matrix:} Assemble \( C^* \in \mathbb{R}^{d_x \times d_x} \), and define the symmetric matrix
    \begin{equation}
    \label{eq:affinity_mat}
    A^* \coloneqq \frac{1}{2} \left( |C^*| + |C^*|^\top \right).
    \end{equation}
\end{itemize}

\noindent Suppose the subspace incoherence condition of Equation \ref{eq:incoherence_gap} is satisfied. Then, with the same high probability as in Theorem~\ref{thm:subspace_detect_whp}, the following holds:
\begin{enumerate}
    \item \textbf{Block-diagonal structure:} Up to a column-wise permutation, \( A^* \) is block-diagonal, with block sizes \( \{ n_m \}_{1 \le m \le M} \) corresponding to the subspace decomposition.
    
    \item \textbf{Correct clustering:} Unnormalized spectral clustering applied to \( A^* \) recovers the ground-truth feature clusters.
\end{enumerate}
\end{proposition}

\paragraph{Constructing the Feature Graph}
To operationalize the result of \ref{prop:recovery_nonoverlap_spec_cltsr}, we interpret the absolute entries of \( C^* \) as encoding similarity between decoder gradients:
\[
(i, j) \in E \quad \Leftrightarrow \quad C^*_{ij} \ne 0 \quad \text{or} \quad C^*_{ji} \ne 0 \Leftrightarrow A_{i,j}^* \ne 0.
\]
The resulting graph has vertex set \( \mathcal{V} = \{ \nabla_{\mathbf{z}} f_1, \dots, \nabla_{\mathbf{z}} f_{d_x} \} \), and the affinity matrix \( A^* \) defines edge weights. Its block-diagonal structure reflects the disjointness of subspaces: gradients in different subspaces exhibit no mutual support under sparse coding (Figure \ref{fig:modular_latents}).

\paragraph{Feature-Level Interpretation}
The affinity structure in \( A^* \) mirrors latent support overlap among features. This motivates the following graph-theoretic abstraction:

\begin{definition}[Feature Graph via Self-Expression]
Let each observed feature \( \mathbf{x}_i \) have latent parent set \( \mathrm{Pa}(i) \subseteq \llbracket 1, d_z \rrbracket \). Define the \emph{feature graph} \( G_F = (\llbracket 1, d_x \rrbracket, E) \), where
\[
(i, j) \in E \quad \Leftrightarrow \quad A_{i,j}^*  \ne \emptyset.
\]
\end{definition}

Under the union‐of‐subspaces model \eqref{assp:union_subspaces}, the feature‐graph \(G_F\) is naturally block‐structured.  Proposition~\ref{prop:recovery_nonoverlap_spec_cltsr} shows that this combinatorial structure is recoverable via optimization and spectral decomposition, completing the link from geometric identifiability to discrete modular recovery (Figure~\ref{fig:feature_graph}).  In practice, one chooses the number of clusters \(\hat M\) in spectral clustering by inspecting the eigenvalue spectrum of the graph Laplacian of \(G_F\),

\begin{equation}\label{eq:laplacian}
\operatorname{Laplacian}(G_F)
:=
D - A^*,
\end{equation}

where \(D=\mathrm{diag}(d_1,\dots,d_{d_x})\in\mathbb{R}^{d_x\times d_x}\) is the \emph{degree matrix} with
\[
d_i \;:=\;\sum_{j=1}^{d_x}A^*_{ij}.
\]
We then apply the so‐called \emph{eigengap heuristic} \citep{von2007tutorialSpectrCls}: let
\[
\lambda_1 \le \lambda_2 \le \cdots \le \lambda_{d_x}
\]
be the eigenvalues of \(\operatorname{Laplacian}(G_F)\) in non-decreasing order, and set

\[
\hat M
\;=\;
\arg\max_{1 \le i \le d_x - 1}
\bigl(\lambda_{i+1} - \lambda_i\bigr),
\]

i.e.\ the index at which the consecutive eigenvalue gap is largest.




\begin{figure}[ht]
     \centering
    \includegraphics[scale=0.8]{figures/transp_crl/feature_graph_v2.pdf}
   \caption{Illustration of the modular latent structure from Proposition~\ref{prop:recovery_nonoverlap_spec_cltsr}. Solving the sparse self-expression problem yields an adjacency matrix $A^*$ (cf. Equation\ref{eq:C_matrix_ex}), whose nonzero entries define connected components in the feature graph $G_F$. We recover these components via spectral clustering.}
  \label{fig:feature_graph}
\end{figure}
\subsubsection{Towards Recovery of Overlapping Feature Clusters}

The spectral clustering result established in Proposition~\ref{prop:recovery_nonoverlap_spec_cltsr} relies on a hard partitioning of observed variables into disjoint subspaces following the shared-parent clustering rule of Definition \ref{def:shared_parent_clustering}. We now focus on the overlapping-parent clustering rule of Definition \ref{def:overlap_parent_clustering}: the children set \( \mathrm{Ch}(\mathbf{z}^j)  \) of each latent variable \( \mathbf{z}^j \). The resulting clustering structure is naturally overlapping: an observed feature \( \mathbf{x}^i \) may have multiple latent parents. The next result provides sufficient conditions under which such overlapping groupings can be recovered from the self-expression matrix \( C^* \). Importantly, our analysis does not assume disjointness or even separability of the influence of latents over observable features as in the anchor feature (Section\ref{sect_crl:intro}). Instead, we work under a set of relaxed structural assumptions on the decoder (Assumption~\ref{assp:latent_feature_model}). These assumptions ensure that the self-expression affinity matrix \(A^*\) encodes latent parent structure in its edge weights, and that overlapping clustering algorithms, such as \gls{saac} \citep{panov2017SAAC, kaufmann2018SAAC} or \gls{symnmf} \citep{Kuang2015SymNMF, zhang2022SymNMF}, can recover \gls{whp} the true groups with bounded misclassification error.

\begin{assumption}[Structured Latent–Feature Model]
\label{assp:latent_feature_model}
Let \(\mathbf Z\in\mathbb R^{d_z}\) be a sub-Gaussian random vector with \(\|\mathbf Z\|_{\psi_2}\le K\), and let \(f\) be \(L\)-smooth as in Assumption~\ref{assp:smooth_f}.  Recall the parental and children sets
\[
\mathrm{Pa}(i)
=\{\,j:\partial f_i/\partial z^j\not\equiv0\}, 
\quad
\mathrm{Ch}(j)
=\{\,i:j\in\mathrm{Pa}(i)\}.
\]
Assume:
\begin{enumerate}[label=(A\arabic*)]
  \item \textbf{Sparsity:} \label{assp:sparsity} Each coordinate \(f_i\) depends on at most \(s\ll d_z\) latents, i.e.
    \[
      \max_{1\le i\le d_x}\lvert\mathrm{Pa}(i)\rvert\;\le\;s.
    \]
    
  
  \item \textbf{Incoherence:} \label{assp:incoherence_grad} For each \(j\in\llbracket1,d_z\rrbracket\), let
    \[
      \partial_j f(\mathbf Z)
      :=\bigl[\tfrac{\partial f_1}{\partial z_j},\dots,\tfrac{\partial f_{d_x}}{\partial z_j}\bigr](\mathbf Z),
    \]
    and define
    \[
      m_j := \mathbb E_{\mathbf Z}\|\partial_j f(\mathbf Z)\|^2,
      \quad
      \Sigma_{jk} := \mathbb E_{\mathbf Z}\langle\partial_j f(\mathbf Z),\,\partial_k f(\mathbf Z)\rangle.
    \]
    We assume that \(\lvert\Sigma_{jk}\rvert\le\mu\sqrt{m_jm_k}\) for all \(j\neq k\), with \(\mu<1\).    

  \item \textbf{Dominance:}  \label{assp:dominance_partial}  For each \(i\), there exists \(j_i\in\mathrm{Pa}(i)\) such that
    \[
      \mathbb E_{\mathbf Z}\bigl[\lvert\partial f_i/\partial z_{j_i}\rvert\bigr]
      \;\ge\;
      (1-\delta)\,\sqrt{\mathbb E_{\mathbf Z}\|\nabla_z f_i(\mathbf Z)\|^2},
      \quad \delta\ll1.
    \]
   
  \item \textbf{Group Size:} \label{assp:grp_size} There exists \(\gamma=\Omega(\log d_x)\) such that
    \[
      \min_{1\le j\le d_z}\lvert\mathrm{Ch}(j)\rvert\;\ge\;\gamma.
    \]
    

  \item \textbf{Restricted Eigenvalue:} \label{assp:restrict_eigenval} There exists \(\kappa>0\) such that for all \(\mathbf v\in\mathbb R^{d_z}\) with \(\|\mathbf v\|_0\le s\),
    \[
      \mathbf v^\top\mathbb E_{\mathbf Z}\bigl[Df(\mathbf Z)\,Df(\mathbf Z)^\top\bigr]\mathbf v
      \;\ge\;
      \kappa\,\|\mathbf v\|_2^2.
    \]
\end{enumerate}
\end{assumption}

\paragraph{Intuition} We explain the role of each assumption in clustering recovery: 
\begin{itemize}
    \item \ref{assp:sparsity}: Restricting \( |\mathrm{Pa}(i)| \le s \) ensures each feature \( f_i \) depends only on \( s \) latent coordinates, preventing overparameterization in the Lasso regression; 
    \item \ref{assp:incoherence_grad}: Mutual incoherence \( |\Sigma_{jk}| \le \mu \sqrt{m_j m_k} \)  with \(\mu < 1\) controls correlations between gradient directions. It is in principle analogous to the \emph{irrepresentable condition} for Lasso support recovery \citep{zhao2006model, wainwright2009sharp, MeinshausenLassoRecovery2009}: it guarantees no unused latent direction can enter as a linear combination of the true ones. In our case, the conditions bear the following geometric intuition: if we associate to each latent dimension a stochastic direction vector \( \partial_j f(\mathbf Z)\) in the observational ambient space \(\mathbb R^{d_x}\), then the condition implies that the expected correlation coefficient between two different direction vectors \( \partial_j f(\mathbf Z), \partial_k f(\mathbf Z)\) is bounded by \(\mu\). Thus, if one considers the one-dimensional subspaces spanned respectively by \( \partial_j f(\mathbf Z)\) and \(\partial_k f(\mathbf Z)\), then the principal angle \(\theta_{jk}\) (\ref{def:principal_angles}) between them verifies in expectation \(\theta_{jk} \ge \arccos{\mu}\). We therefore prevent "near-parallelism" in Jacobian rows, which is important in cluster recovery because it helps bound between-cluster affinities;
    \item \ref{assp:dominance_partial}: Requiring that a partial derivative \( \frac{\partial f_1}{\partial \mathbf{z}_j} \) dominates guarantees that each output coordinate \( i \) is most strongly coupled to a latent variable without being decoded with only one latent as in the single-parent decoding assumption and without requiring having exact "pure children" as in the anchor features assumption; 
    \item \ref{assp:grp_size}: Having \( |Ch(j)| \ge \gamma = \Omega(\log d_x) \) ensures sufficient "samples" (here observed feature) for concentration inequalities to hold; and 
    \item \ref{assp:restrict_eigenval}: Strong convexity (Restricted Eigenvalue condition) is essential for the uniqueness of the Lasso minimizer and for support recovery proofs.
\end{itemize}


\begin{theoremBox}[Self‐Expression and Overlapping Cluster Recovery]
\label{thm:overlap_cluster_recovery}
Assume assumptions \ref{assp:latent_feature_model} hold. Let \(C^*\) be the unique solution to the population‐level self‐expression problem \(\mathcal P_{\lambda}(Df)\) (Equation \ref{eq:lasso_penalty_fct}), and let \(A^*\) be the resulting symmetric affinity matrix. Choose
\[
\lambda \;\ge\; c_1\,\mu \;+\; c_2\,K\,L\;\sqrt{d_x\log\!\bigl(d_x^2/\varepsilon\bigr)},
\]
for constants \(c_1>1\), \(c_2\ge2\), and confidence parameter \(\varepsilon\in(0,1)\). Then, with probability at least \(1-\varepsilon\), for each latent group \(\mathrm{Ch}(j)\) the following hold:

\begin{itemize}
  \item {\bf Intra‑cluster affinities:}  For all \(i,i'\in\mathrm{Ch}(j)\),
  \[
    A^*_{ii'}
    \;\ge\;
    \bigl(1 - \delta - \mu\bigr)\,m_j
    \;-\;
    C_3\,K\,L\,\;\sqrt{d_x\log\!\bigl(d_x^2/\varepsilon\bigr)}.
  \]
  
  \item {\bf Inter‑cluster affinities:}  For all \(i\in\mathrm{Ch}(j)\), \(i'\in\mathrm{Ch}(k)\), \(k\neq j\),
  \[
    A^*_{ii'}
    \;\le\;
    \mu\,\sqrt{m_j\,m_k}
    \;+\;
    C_3\,K\,L\;\sqrt{d_x\log\!\bigl(d_x^2/\varepsilon\bigr)},
  \]
\end{itemize}

where \(C_3=2\,c_2\).  Moreover, if
\[
\min_{1\le j\le d_z}\,m_j \;-\;\mu\max_{k\neq j}\sqrt{m_jm_k}
\;\gg\;
K\,L\,\;\sqrt{d_x\log\!\bigl(d_x^2/\varepsilon\bigr)},
\]
then overlap‑aware clustering methods such as SAAC \citep{panov2017SAAC,kaufmann2018SAAC} or SymNMF \citep{Kuang2015SymNMF,zhang2022SymNMF} recover clusters \(\widehat G_j\) satisfying
\begin{equation}
\label{eq:misclassif_overlap_clstr}
\min_{1\le j\le d_z}\frac{|\widehat G_j\triangle\mathrm{Ch}(j)|}{|\mathrm{Ch}(j)|}
\;=\;
\mathcal O\!\Bigl(\delta + \tfrac{\mu}{\gamma} + \tfrac{K\,L\,\;\sqrt{d_x\log(d_x^2/\varepsilon)}}{\min\limits_{ 1 \leq j \leq d_z} m_j}\Bigr).
\end{equation}
\end{theoremBox}

\paragraph{Interpretation}
At a high level, both \gls{saac} and \gls{symnmf} succeed because they first convert the overlapping‑community problem into a geometric grouping task in a low‑dimensional spectral embedding, then recover the clusters.  The misclassification bound in Equation~\ref{eq:misclassif_overlap_clstr} splits into three intuitive contributions:
\begin{inparaenum}
  \item \emph{Dominance error} \(\delta\), reflecting that each feature’s strongest latent parent only \emph{almost} dominates its gradient (Assumption \ref{assp:dominance_partial}).
  \item \emph{Incoherence–rounding error} \(\mu/\gamma\), arising because residual cross‑group correlations of size \(\mu\) must be averaged out over clusters of minimum size \(\gamma\).
  \item \emph{Embedding‑noise error}
  \[
    \frac{K\,L\,\sqrt{d_x\log(d_x^2/\varepsilon)}}{\min_{1\le j\le d_z}m_j}\,,
  \]
  which quantifies how sub‑Gaussian fluctuations (\(K\)), Hessian smoothness (\(L\)), Frobenius norm over the Jacobian (\(\sqrt{d_x}\)) degrade the ideal block affinities. Again similar to discussion of Theorem \ref{thm:subspace_detect_whp}, tighter latent priors (smaller $K$), smoother decoder (smaller $L$) tighten the embedding noise term, improving overlap‑clustering accuracy. Dependence on $d_x$ highlights the intuition that the more the input space is higher dimensional, the more an overlapping variables clustering is prone to error.
\end{inparaenum}

\subsection{Generalization and Stability of the Self-Expression Objective}

We now address the gap between theory and practice in modeling the self-expression loss. The previous results guarantee identifiability under idealized assumptions about the decoder and its Jacobian structure. However, practical training operates on finite data and noisy gradients, often approximated via samples from the latent posterior. This raises three key questions:
\begin{inparaenum}
    \item \textbf{Bias:} \emph{How much does the mismatch between the prior and the aggregated posterior distort the self-expression loss?}
    \item \textbf{Generalization:} \emph{Given a known decoder, how well does the empirical self-expression loss approximate its population counterpart?}
    \item \textbf{Stability:} \emph{How sensitive is the self-expression loss to perturbations or noise in the Jacobian?}
\end{inparaenum}


\paragraph{Bias from Aggregated Posterior}
In practice, variational autoencoders sample latent variables \(\mathbf z\) not from the prior \(p(\mathbf z)\) but from the approximate posterior \(q_{\phi}(\mathbf z\mid\mathbf x)\).  Consequently, expectations such as those over the self‐expression loss
\[
\ell(C,\mathbf z)
\;=\;
\bigl\lVert Df(\mathbf z) - Df(\mathbf z)\,C \bigr\rVert_{F}^{2}
\]
are taken under the \emph{aggregated posterior}
\[
q_{\phi}(\mathbf z)
\;:=\;
\mathbb{E}_{\mathbf X\sim p_{\mathrm{data}}}\bigl[q_{\phi}(\mathbf z\mid\mathbf X)\bigr],
\]
rather than the prior.  This distributional mismatch introduces an \emph{aggregation bias}, which can be quantified in terms of the Kullback–Leibler divergence \(D_{\mathrm{KL}}(q_{\phi}\,\|\,p)\), exactly the term that appears as the ELBO gap in VAE training.  The argument relies on bounding the expectation gap via total variation distance:
\[
 \|q - p\|_{\mathrm{TV}} \coloneqq \frac{1}{2} \int |q(\mathbf{z}) - p(\mathbf{z})|\,d\mathbf{z}.
\]

\begin{lemma}[Bias via Total Variation]
\label{lemma:penalty_bias_tv}
Let \( q \) and \( p \) be probability densities on \( \mathbb{R}^{d_z} \), and let \( \ell : \mathbb{R}^{d_z} \to \mathbb{R} \) be measurable with \( \|\ell\|_\infty < \infty \). Then
\[
\left| \mathbb{E}_{\mathbf{Z} \sim q}[\ell(C, \mathbf{Z})] - \mathbb{E}_{\mathbf{Z} \sim p}[\ell(C, \mathbf{Z})] \right| \le \|\ell\|_\infty \cdot \|q - p\|_{\mathrm{TV}}.
\]
\end{lemma}

\begin{lemma}[Pinsker’s Inequality {\citep{AlisonIPM2002}}]
\label{lemma:pinsker}
For any distributions \( q \), \( p \),
\[
\|q - p\|_{\mathrm{TV}} \le \sqrt{ \tfrac{1}{2} D_{\mathrm{KL}}(q \,\|\, p) }.
\]
\end{lemma}

Combining Lemmas \ref{lemma:penalty_bias_tv} and \ref{lemma:pinsker}, and assuming unit-norm gardients, we obtain:
\begin{proposition}[Bias Bound via ELBO Gap]
\label{prop:aggregation_bias_bound}
\[
\left| \mathbb{E}_{\mathbf{Z} \sim q_\phi}[\ell(C, \mathbf{Z})] - \mathbb{E}_{\mathbf{Z} \sim p}[\ell(C, \mathbf{Z})] \right|
\le \sqrt{d_x} (1 + \|C\|_{\mathrm{op}}) \cdot \sqrt{ \tfrac{1}{2} D_{\mathrm{KL}}(q_\phi \,\|\, p) }.
\]
\end{proposition}

This bound reveals a trade-off between model structure and posterior mismatch. The larger the spectral norm \( \|C\|_{\mathrm{op}} \), the more sensitive the loss becomes to deviations from the prior. Thus, better variational approximations not only improve reconstruction, but also yield more faithful estimates of latent-space geometry.

\paragraph{Generalization from Finite Data}

We now consider generalization from empirical estimates to population risk. Let \( \bar{J}_f(\mathbf{x}; q_\phi) \coloneqq \mathbb{E}_{\mathbf{Z} \sim q_\phi(\cdot \mid \mathbf{x})}[Df(\mathbf{Z})] \) denote the expected Jacobian under the posterior. Define the self-expression loss:
\[
\bar{\ell}(C, f; \mathbf{x}) \coloneqq \| \bar{J}_f(\mathbf{x}; q_\phi) - C \bar{J}_f(\mathbf{x}; q_\phi) \|_F^2,
\]
and consider the hypothesis class \(\mathcal{C}_\lambda \coloneqq \left\{ C \in \mathbb{R}^{d_x \times d_x} : \|C\|_1 \le \lambda,\ \operatorname{diag}(C) = \mathbf 0 \right\}.\)

\begin{theoremBox}[Generalization of Self-Expression Loss]
\label{thm:genetalization_SExprLoss}
Let \( M_\phi \coloneqq \sup_{\mathbf{x}} \| \bar{J}_f(\mathbf{x}; q_\phi) \|_F \). Then with probability at least \( 1 - \delta \) over \( N \) i.i.d. samples \( \{ \mathbf{X}_i \}_{i=1}^N \), we have:
\[
\sup_{C \in \mathcal{C}_\lambda} \left| \mathbb{E}_{\mathbf{X} \sim p_{data}}[\bar{\ell}(C, f; \mathbf{X})] - \frac{1}{N} \sum_{i=1}^N \bar{\ell}(C, f; \mathbf{X}_i) \right|
\le 8 \lambda M_\phi^2 \sqrt{ \frac{2 d_z \log d_x}{N} } + \frac{M_\phi^2}{2} \sqrt{ \frac{\log(1/\delta)}{N} }.
\]
\end{theoremBox}

Since gradients are unit-norm by assumption, Jensen’s inequality implies \( M_\phi^2 \le d_x \). Thus, empirical minimization of the self-expression loss generalizes well under mild conditions on the decoder and sparsity constraint \( \lambda \). The logarithmic dependence on \( d_x \) ensures scalability in high-dimensional regimes.

\paragraph{Stability under Jacobian Perturbation}

Finally, we analyze the stability of the self-expression loss under stochastic perturbations of the Jacobian, which may arise from encoder sampling or numerical noise.

\begin{proposition}[Stability of Self-Expression Loss under Jacobian Noise]
\label{prop:jacobian-perturbation}
Suppose
\[
Df(\mathbf{Z}) = \widetilde{Df}(\mathbf{Z}) + E(\mathbf{Z}),
\]
where \( \widetilde{Df}(\mathbf{Z}) \in \mathbb{R}^{d_x \times d_z} \) is the true Jacobian and each column of \( E \) is an independent, zero-mean sub-Gaussian vector: \( E_{:,j}(\mathbf{Z}) \in \mathrm{subG}_{d_x}(\varepsilon) \). Let \( C^* \in \mathbb{R}^{d_x \times d_x} \) satisfy \( \operatorname{diag}(C^*) = \mathbf 0 \). 
Define the self-expression loss deviation as 
\[
\Delta(\mathbf{Z}) \coloneqq \|Df(\mathbf{Z}) - Df(\mathbf{Z}) C^* \|_F^2 - \| \widetilde{Df}(\mathbf{Z}) - \widetilde{Df}(\mathbf{Z}) C^* \|_F^2.
\]
Then, for any \( \delta \in (0,1) \), with probability at least \( 1 - \delta \),
\[
\left| \Delta(\mathbf{Z})\right|
\le (1 + \|C^*\|_{\mathrm{op}}) \left( 2 d_x B(\delta) \varepsilon + (1 + \|C^*\|_{\mathrm{op}}) B(\delta)^2 \varepsilon^2 \right),
\]
where
\[
B(\delta) \coloneqq \Lambda \sqrt{d_z d_x} + \sqrt{2 d_z \log(2 d_x / \delta)},
\]
and \( \Lambda > 0 \) is a universal constant.
\end{proposition}

\paragraph{Interpretation}
A key implication of Proposition \ref{prop:jacobian-perturbation} is a stability bound that establishes a principled connection between sparsity, low-rank structure, and robustness of the self-expression loss under perturbations: 

\begin{itemize}
\item \textbf{Perturbation Scaling and Deviation Bound:}
Proposition~\ref{prop:jacobian-perturbation} shows that when the true Jacobian \(\widetilde{Df}\) is corrupted by sub-Gaussian noise of magnitude \(\varepsilon\), the self-expression loss deviation \(\Delta(\mathbf{Z})\) is controlled by two terms scaling as \(\mathcal{O}\bigl(d_x\,B(\delta)\,\varepsilon\bigr)\) and \(\mathcal{O}\bigl(d_x\,B(\delta)^2\,\varepsilon^2\bigr)\). 
The leading absolute deviation is
\begin{equation}
    \label{eq:deviation_Delta_simple}
    \left|\Delta(\mathbf{Z})\right| =
\mathcal{O}\bigl((1+\|C^*\|_{\mathrm{op}})\,d_x\,B(\delta)\,\varepsilon\bigr),
\end{equation}
and remains small whenever
\[
2\,d_x\,B(\delta)\,\varepsilon \,\ll\, \frac{1}{1+\|C^*\|_{\mathrm{op}}}.
\]
\item \textbf{Role of sparsity:}
Sparsity improves stability since
\[
\|C^*\|_{\mathrm{op}} \le \|C^*\|_{1 \to 1}, \quad \text{where} \quad
\|C^*\|_{1 \to 1} \coloneqq \max_{1 \le j \le d_x} \sum_{i=1}^{d_x} \big|C^*_{ij}\big|,
\]
and thus sparser coefficients imply lower operator norms and better robustness by Equation~\ref{eq:deviation_Delta_simple}.
\item \textbf{Influence of Low Rank:} For fixed Frobenius norm, lower-rank solutions are more stable because the lower the rank of \(C^*\), the smaller the spectral norm, as justified by the matrix-norm inequality \citep{horn2012MatrixAnalysis}:
\[
\|C^*\|_{\mathrm{op}}
\;\le\;
\sqrt{\operatorname{rank}(C^*)}\,\|C^*\|_F,
\]
highlighting the beneficial trade-off between sparsity, rank, and noise sensitivity in subspace modeling.
\end{itemize}


\subsection{Computational efficiency: Calculating the Penalty \(\bar{\ell}(C, f; \mathbf{x})\)} 

Suppose we wish to compute the penalty \(\bar{\ell}(C, f; \mathbf{x})\) by first forming the \emph{full} expected Jacobian \(\bar{J}_f(\mathbf{x}; q_\phi) \in \mathbb{R}^{d_z \times d_x}\). This poses a computational challenge: in practice, \(\bar{J}_f(\mathbf{x}; q_\phi)\) is approximated using samples \(\mathbf{z}_1, \dots, \mathbf{z}_{S'} \sim q_\phi(\cdot \mid \mathbf{x})\),
\[
\bar{J}_f(\mathbf{x}; q_\phi)
\approx \frac{1}{S'} \sum_{j=1}^{S'} Df(\mathbf{z}_j).
\]

By "backpropagating" once per input dimension, obtaining every row vector \(\nabla_{\mathbf{z}}f_i(\mathbf{z}_j)\) requires one backward pass per output, for a total of \(\mathcal{O}(d_x)\) gradient evaluations, each itself requiring \(\mathcal{O}(T_f)\), the cost of one forward+backward through the network. Hence, explicitly assembling \(\bar{J}_f(\mathbf{x}; q_\phi) \in \mathbb{R}^{d_z \times d_x}\) takes
\[
\mathcal{O}\bigl(S'\,d_x\,T_f\bigr),
\]
which grows linearly with \(d_x\) and is thus computationally demanding. The following theorem provides a better computation strategy.

\begin{theoremBox}[Efficient Approximation of the Self-Expression Penalty]
\label{thm:penalty-efficient-approx}
The self-expressiveness penalty
\[
\bar{\ell}(C, f; \mathbf{x}) = \left\| \bar{J}_f(\mathbf{x}; q_\phi) - C \bar{J}_f(\mathbf{x}; q_\phi) \right\|_F^2
\]
can be efficiently approximated via Hutchinson-style trace estimation \citep{hutchinson1989stochastic}:
\[
\bar{\ell}(C, f; \mathbf{x}) \approx \sum_{i=1}^S \left\| \eta(\epsilon_i, f; \mathbf{x}) \right\|_2^2,
\]
where \( \epsilon_1, \dots, \epsilon_S \sim \mathcal{N}(0, I_{d_x}) \) are independent Gaussian probe vectors, and
\[
\begin{aligned}
\eta(\epsilon, f; \mathbf{x})
&= \bar{J}_f(\mathbf{x}; q_\phi)\left(
    \epsilon - \sum_{j=1}^{d_x}
    \bigl\langle \epsilon, C_{:,j} \bigr\rangle\, \mathbf{e}_j
\right) \\[1.2ex]
&= \bar{J}_f(\mathbf{x}; q_\phi)\bigl(\epsilon - C^\top\epsilon\bigr).
\end{aligned}
\]
where \(C_{:,j} \) is the \( j \)-th column of \( C \). In practice, \( \bar{J}_f(\mathbf{x}; q_\phi) \) is approximated using samples \( \mathbf{z}_1, \dots, \mathbf{z}_{S'} \sim q_\phi(\cdot \mid \mathbf{x}) \):
\[
\bar{J}_f(\mathbf{x}; q_\phi) \approx \frac{1}{S'} \sum_{j=1}^{S'} Df(\mathbf{z}_j),
\]
so the full approximation becomes:
\[
\bar{\ell}(C, f; \mathbf{x}) \approx \sum_{i=1}^S \left\| \left( \frac{1}{S'} \sum_{j=1}^{S'} Df(\mathbf{z}_j) \right) \left( \epsilon_i - C^\top \epsilon_i \right) \right\|_2^2.
\]
\end{theoremBox}

Theorem~\ref{thm:penalty-efficient-approx} leverages Hutchinson’s trace estimator, which states that:
\[
\operatorname{tr}(AA^T) = \mathbb{E}_{\epsilon \sim \mathcal{N}(0, I_{d_x})} \left[ ||\epsilon^T A||_2^2 \right]
\]
to approximate the self‐expressiveness penalty in \(\mathcal{O}((S+S')\times T_f)\) Jacobian–vector products, rather than the \(\mathcal O\bigl(S' \times d_x\times T_f\bigr)\) full Jacobian computation required by naive methods. By sampling \(S \ll d_x\) Gaussian probes, one obtains an unbiased estimate of the Frobenius‐norm residual with constant per-sample complexity. This reduces both computation by a factor of \(\frac{S'}{S+S'}d_x\), enabling the incorporation of the self‐expression penalty into training loops in PyTorch with only a few extra backpropagations per batch. In experiments, \(S'=1, S=4\) and for purchase data \(d_x = 2521\), so the speed factor is \(\frac{d_x}{5} \approx 504\) compared to using the standard PyTorch’s "\verb|autograd.functional.jacobian|" \citep{Paszke2019PyTorchAI}.



\subsection[{Applying Static Self-Expression Theory in a CRL in Time-Series Setting} ]{Applying Static Self-Expression Theory in a \gls{crl} in Time-Series Setting}  
In our temporal model  
\[
\mathbf X_t = f(\mathbf Z_t), 
\]
the decoder \(f:\mathbb R^{d_z}\to\mathbb R^{d_x}\) in Equation \ref{eq:def_crl_statio} is \emph{memoryless}: it depends only on the current latent \(\mathbf z_t\), which evolves by a fixed structural law, but we assume that it remains marginally \(\mathrm{subG}_{d_z}(K)\) at each \(t\).  Consequently,  under the smoothness over \(f\) (\ref{assp:smooth_f}), the exact same concentration and subspace‐detection guarantees developed in Section~\ref{sect_crl:theory_nonoverlap} (e.g., Theorem~\ref{thm:subspace_detect_whp} and Proposition~\ref{prop:jacobian-perturbation}) apply verbatim to each time slice \(\mathbf z_t\).  In particular:
\begin{itemize}[nosep,leftmargin=*]
  \item For every \(t\), \(\mathbf z_t\sim\mathrm{subG}_{d_z}(K)\) and \(f\) is $L$-smooth, so all static‐Jacobian concentration bounds hold at time \(t\).  
  \item Solving 
    \(\displaystyle \min_{C}\;\mathbb E_{\mathbf Z_t}\bigl\|Df(\mathbf Z_t)-Df(\mathbf Z_t)\,C\bigr\|_F^2+\lambda\|C\|_1\)
    and clustering via \((|C|+|C|^\top)/2\) recovers feature groups exactly as in the static case.  
  \item No "augmented" input or multi-lag decoder is required: since \(f\) never sees \(\mathbf z_{t-\rho}\) for \(\rho>0\), our proofs carry over unchanged.  
\end{itemize}
Thus, under the stationarity assumption on the latent process, one can import our entire static \gls{crl} framework into a time-series context without modification. 


\section{Experiments}
\paragraph{Evaluation}  
We conceptually associate each scalar observed feature \(\mathbf{x}_t^i\) with a vector given by its gradient \(\nabla_{\mathbf{z}}f_i\). Clustering the nodes represented by these gradients leads to a \emph{stationary} grouping of features in the observed space. Evaluating such clustering is challenging because internal validation techniques (e.g, Silhouette score, Davies-Bouldin index \citep{Schubert2023stop}) are not easily applicable, the data points being clustered are scalar and vary over time. Instead, we rely on \emph{external validation}, assuming the existence of labels that define semantically coherent and temporally stable groups of variables. For instance, in purchase data, \(\mathbf{x}_t^i\) may represent the quantity of product \(i\) purchased at time \(t\), but it is well established that products are typically organized into stable categories and subcategories. We, therefore, assess the coherence of our clusters with respect to these predefined labels. Some datasets, like purchase logs, contain multiple layers of labeling (e.g., subcategories and categories), forming a nested structure where subcategories are embedded within broader categories. This hierarchy allows for a more rigorous evaluation of our inferred groupings by measuring their alignment with known label structures.

\paragraph{Metrics} As an external validation, we adopt the standard suite proposed in \citep{rosenberg2007VMeasure}:
\begin{inparaenum}
    \item \emph{Homogeneity (H)}: A clustering is homogeneous if each cluster contains only data points from a single class.
    \item \emph{Completeness (C)}: A clustering is complete if all members of a class are assigned to the same cluster.
    \item \emph{Normalized Mutual Information (NMI)}: Also known as the \emph{V-measure}, it balances homogeneity and completeness to quantify clustering quality.
\end{inparaenum}


\paragraph{Benchmark} We compare the \gls{crl} model Leap \citep{yao2022learning} to a baseline that consists of "pseudo"-random generation of labels, where labels are randomly assigned to each feature while following the true categorical distribution of labels across observed features. If multiple labels are available for each feature, then the "pseudo"-random approach will be evaluated for labeling. H, C, and \gls{nmi} are reported for each configuration.



\subsection{Synthetic data}

\paragraph{Synthetic Data Generation}
In our experiments, we generate synthetic data by simulating three main components: 
\begin{inparaenum}
    \item the causal process in the latent space, 
    \item the decoding function mapping latent variables to observed features, and 
    \item the sparsity structure of the decoding process.
\end{inparaenum}


We define a latent process \(\{\mathbf{z}_t \in \mathbb{R}^{d_z}\}_{t=1}^{T}\) governed by a structured non-linear and non-Gaussian autoregressive process of lag order \(L\). Specifically, the latent dynamics incorporate nonlinear transformations of lagged components modulated through a set of transition matrices \(\{B^{(\ell)}\}_{\ell=1}^L\). The latent update equation is
\[
\mathbf{z}_t
= \mathrm{LeakyReLU}\left(
    \sum_{\ell=1}^{L} \sin\bigl(\mathbf{z}_{t-\ell} B^{(\ell)}\bigr)
    + \epsilon_t
\right),
\quad \epsilon_t \sim \mathrm{Laplace}(0,1).
\]
\paragraph{Decoder Network and Observed Data Generation}
Each latent vector \(\mathbf{z}_t\) is decoded to generate an observed vector \(\mathbf{x}_t \in \mathbb{R}^{d_x}\) using a sparse linear transformation followed by a nonlinear probabilistic decoder. First, a sparse adjacency matrix \(A \in \{0,1\}^{d_x \times d_z}\) is generated using Algorithm~\ref{alg:crl_adjcency_matrix}, encoding which latent factors influence which observed features.

A weight matrix \(W\) is formed by element-wise multiplication \(W = A \odot B\), where \(B\) contains continuous values sampled from a uniform distribution \([0.1, 1]\). Then, for each time step \(t\), the observed data is generated as follows (see Algorithm~\ref{alg:crl_sim_algo}):
\[
\begin{aligned}
\mathbf{u}_t &= \mathbf{z}_t W^\top, \\[0.8ex]
\boldsymbol{\mu}_t &= \mu_\theta(\mathbf{u}_t), \\[0.8ex]
\boldsymbol{\sigma}_t &= \sigma_\theta(\mathbf{u}_t), \\[0.8ex]
\mathbf{x}_t &\sim \mathcal{N}\bigl(\boldsymbol{\mu}_t,\, \operatorname{diag}(\boldsymbol{\sigma}_t^2)\bigr).
\end{aligned}
\]
The decoder networks \(\mu_\theta\) and \(\sigma_\theta\) are randomly initialized 2-layer fully connected networks with LeakyReLU activations and Softplus at the output of \(\sigma_\theta\) to ensure positivity.

\begin{algorithm}[ht]
\caption{Nonlinear Non-Gaussian Data Generation}
\begin{algorithmic}[1]
\REQUIRE Lag order \( H \), Layers \( K \), Sequence length \( T \), Negative slope \( \alpha \), Latent dimension \( d_z \), Observed dimension \( d_x \), Batch size \( N \), Noise scale \( \sigma \), Structural matrix \( \Gamma \in \{0,1\}^{d_x \times d_z} \), Transition matrices \( \{B_h\}_{h=1}^H \), Decoder functions \( f_\mu \), \( f_\sigma \)
\ENSURE Observed data \( \mathbf{X} \in \mathbb{R}^{N \times (H+T) \times d_x} \), Latent data \( \mathbf{Z} \in \mathbb{R}^{N \times (H+T) \times d_z} \)

\STATE \textbf{Initialize} \( \mathbf{Z}_{\text{lags}} \sim \mathcal{N}(0, 1) \) of shape \( (N, H, d_z) \)
\STATE Normalize \( \mathbf{Z}_{\text{lags}} \) along the batch axis
\STATE Initialize empty sequences: \( \mathbf{Z} \gets [\,] \), \( \mathbf{X} \gets [\,] \)
\FOR{\(i = 1\) \TO \(H\)}
    \STATE Append \( \mathbf{Z}_{\text{lags}}[:, i, :] \) to \( \mathbf{Z} \)
\ENDFOR
\STATE \( \mathbf{M} \gets \mathbf{Z}_{\text{lags}} \)
\STATE \( \mathbf{D} \gets \mathbf{M} \cdot \Gamma \)
\STATE \( \boldsymbol{\mu} \gets f_\mu(\mathbf{D}) \), \quad \( \boldsymbol{\sigma} \gets f_\sigma(\mathbf{D}) \)
\STATE \( \mathbf{M}' \sim \mathcal{N}(\boldsymbol{\mu}, \boldsymbol{\sigma}) \)
\STATE \( \mathbf{X}_{\text{lags}} \gets \mathbf{M}' \)
\FOR{\(i = 1\) \TO \(H\)}
    \STATE Append \( \mathbf{X}_{\text{lags}}[:, i, :] \) to \( \mathbf{X} \)
\ENDFOR

\FOR{\(t = 1\) \TO \(T\)}
    \STATE Sample \( \mathbf{z}_t \sim \text{Laplace}(0, \sigma) \) of shape \( (N, d_z) \)
    \FOR{\(h = 1\) \TO \(H\)}
        \STATE \( \mathbf{z}_t \gets \mathbf{z}_t + \sin(\mathbf{Z}_{\text{lags}}[:, h, :] \cdot B_h) \)
    \ENDFOR
    \STATE \( \mathbf{z}_t \gets \text{LeakyReLU}(\mathbf{z}_t, \alpha) \)
    \STATE Append \( \mathbf{z}_t \) to \( \mathbf{Z} \)
    \STATE \( \mathbf{D} \gets \mathbf{z}_t \cdot \Gamma \)
    \STATE \( \boldsymbol{\mu} \gets f_\mu(\mathbf{D}) \), \quad \( \boldsymbol{\sigma} \gets f_\sigma(\mathbf{D}) \)
    \STATE \( \mathbf{x}_t \sim \mathcal{N}(\boldsymbol{\mu}, \boldsymbol{\sigma}) \)
    \STATE Append \( \mathbf{x}_t \) to \( \mathbf{X} \)
    \STATE Update \( \mathbf{Z}_{\text{lags}} \): append \( \mathbf{z}_t \), remove oldest lag
\ENDFOR

\STATE Stack \( \mathbf{Z} \) and \( \mathbf{X} \) along the time axis to shape \( (N, H+T, d_z) \) and \( (N, H+T, d_x) \)
\RETURN \( \mathbf{X}, \mathbf{Z}, \Gamma \)
\end{algorithmic}
\label{alg:crl_sim_algo}
\end{algorithm}


\begin{algorithm}[ht]
\caption{Generate Sparse Structural Matrix \(\Gamma \in \{0,1\}^{d_x \times d_z}\)}
\begin{algorithmic}[1]
\REQUIRE Number of observed features \(d_x\), number of latent subspaces \(M\), random seed \(s\)
\ENSURE Structural matrix \(\Gamma \in \{0,1\}^{d_x \times d_z}\), subspace sizes \(\mathbf{n} \in \mathbb{N}^M\)

\STATE Set \(\text{min\_per\_subspace} \gets 2\)
\STATE Set \(\text{leftover} \gets d_x - M \times \text{min\_per\_subspace}\)
\STATE Initialize random number generator with seed \(s\)
\STATE Draw \(\text{raw} \sim \text{Dirichlet}(\mathbf{1}_M)\)
\STATE \(\mathbf{n} \gets \lfloor \text{raw} \times \text{leftover} \rfloor\) \COMMENT{Initial subspace sizes}
\STATE \(\text{diff} \gets \text{leftover} - \sum_{j=1}^M n_j\)
\FOR{\(i = 1\) to \(\text{diff}\)}
    \STATE \(n_{(i \bmod M) + 1} \gets n_{(i \bmod M) + 1} + 1\)
\ENDFOR
\FOR{\(j = 1\) to \(M\)}
    \STATE \(n_j \gets n_j + \text{min\_per\_subspace}\)
\ENDFOR
\STATE Initialize \(\Gamma \gets 0_{d_x \times d_z}\)
\STATE \(i \gets 0\)
\FOR{\(m = 1\) to \(M\)}
    \FOR{\(k = 1\) to \(n_m\)}
        \STATE \(\Gamma[i, m] \gets 1\)
        \STATE \(i \gets i + 1\)
    \ENDFOR
\ENDFOR
\STATE Draw a random permutation \(\pi\) of \(\{0, 1, \ldots, d_x - 1\}\)
\STATE Permute the rows of \(\Gamma\) according to \(\pi\)
\RETURN \(\Gamma\), \(\mathbf{n}\)
\end{algorithmic}
\label{alg:crl_adjcency_matrix}
\end{algorithm}

\paragraph{Experimental results: Non-Overlapping clusters} From Table \ref{tab:perf_sim_nonoverlap}, Leap achieves \(H \approx 0.85\), \(C \approx 0.84\), and \(NMI \approx 0.84\) on average, compared to \(H \approx 0.25\), \(C \approx 0.28\), and \(NMI \approx 0.26\) for random labeling. This gap demonstrates that our inferred clusters capture fine-grained product groupings with more than three times better homogeneity and completeness than chance. Notably, high homogeneity indicates that clusters seldom mix subcategories, while strong completeness shows that most items within a given subcategory are clustered together.

\begin{table}[h!]
    \centering    
    \caption{Clustering coherence on simulated data, true labels are simulated.}
    \label{tab:perf_sim_nonoverlap}
    \resizebox{8cm}{!}{%
    \begin{tabular}{|c|c|c|c|} \hline 
        Model & H & C & \gls{nmi} \\ \hline 
        \textbf{Leap + SSC} & \textbf{0.85$\pm$0.02} & \textbf{0.84$\pm$0.04} & \textbf{0.84$\pm$0.03} \\ \hline 
        \textbf{Random clustering} &  0.25$\pm$0.08 & 0.28$\pm$0.07 & 0.26$\pm$0.07 \\ \hline 
    \end{tabular}}
\end{table}%


\paragraph{Experimental results: Overlapping clusters}

We evaluate two overlapping‐community algorithms, \gls{symnmf} and \gls{saac}, on features grouping generated by simulation data (Algorithms \ref{alg:crl_adjcency_matrix} and \ref{alg:crl_sim_algo}), and varying Dirichlet concentration \(\alpha \in \{0.2, 0.5, 1.0\}\) to control overlap. We assess recovery quality using three standard metrics:

\begin{enumerate}
  \item \textbf{Overlapping Normalized Mutual Information (oNMI)}, which generalizes \gls{nmi} to soft or overlapping labels \citep{mcdaid2011normalized}.
  \item \textbf{F1-score}, averaged over true and estimated memberships, measuring the harmonic mean of precision and recall for node‐community assignments \citep{lancichinetti2009detecting}.
  \item \textbf{Omega Index}, a chance-corrected measure of agreement for overlapping partitions \citep{collins1988mega}.
\end{enumerate}

We report performances in Table \ref{tab:perfs_overap_sim}. Both methods substantially outperform a random‐assignment baseline, demonstrating overlap recovery. As overlap increases (\(\alpha \uparrow\)), performance degrades slowly, e.g., \gls{symnmf} ’s oNMI drops from 0.72 to 0.58, reflecting higher ambiguity in dense overlaps.
\begin{table}
\centering
\caption{Performance metrics under overlapping features for synthetic data with varying overlap levels \(\alpha\).}
\resizebox{0.6\textwidth}{!}{
\begin{tabular}{|c|l|c|c|c|} \hline 
\(\alpha\) & Method & oNMI & F1-score & Omega \\
\hline
0.2 & \textbf{\gls{symnmf}}  & \(\mathbf{0.72 \pm 0.04}\) & \(\mathbf{0.75 \pm 0.03}\) & \(\mathbf{0.68 \pm 0.05}\) \\  
    & \textbf{\gls{saac}}  & \(0.68 \pm 0.05\) & \(0.70 \pm 0.04\) & \(0.64 \pm 0.06\) \\  
    & \textbf{Random clustering} & \(0.12 \pm 0.03\) & \(0.11 \pm 0.04\) & \(0.01 \pm 0.06\) \\ \hline 
0.5 & \textbf{\gls{symnmf}}   & \(\mathbf{0.65 \pm 0.03}\) & \(\mathbf{0.67 \pm 0.04}\) & \(\mathbf{0.60 \pm 0.05}\) \\  
    & \textbf{\gls{saac}}  & \(0.62 \pm 0.04\) & \(0.64 \pm 0.05\) & \(0.57 \pm 0.06\) \\  
    & \textbf{Random clustering}  & \(0.13 \pm 0.04\) & \(0.12 \pm 0.04\) & \(0.01 \pm 0.03\) \\ \hline
1.0 & \textbf{\gls{symnmf}}   & \(\mathbf{0.58 \pm 0.05}\) & \(\mathbf{0.60 \pm 0.06}\) & \(\mathbf{0.52 \pm 0.07}\) \\  
    & \textbf{\gls{saac}}  & \(0.55 \pm 0.06\) & \(0.57 \pm 0.07\) & \(0.49 \pm 0.08\) \\
    & \textbf{Random clustering}  & \(0.14 \pm 0.04\) & \(0.14 \pm 0.03\) & \(0.01 \pm 0.05\) \\
\hline
\end{tabular}}
\label{tab:perfs_overap_sim}
\end{table}

\subsection{Real data}

\paragraph{Saint-Gobain Transaction Data}

This dataset contains transaction histories, where each client is uniquely identified. Transactions are timestamped and associated with products that can be grouped into bundles or categories. Sequential purchases, such as buying plasterboards, followed by screws and glue for a renovation project, suggest underlying causal structures. Yet, inferring these structures is difficult, especially when many products are similar. For example, two distinct items might simply be plasterboards that differ only in size or brand. In such cases, it is more meaningful to examine whether causal representation learning can be transparently aligned with coherent product groupings in the observational space. Products can be represented at varying levels of granularity (Figure~\ref{fig:categ_abstractions_saintgob}). The purchase vector might encode the quantity bought per product, per subcategory, or according to broader groupings such as product families or specialties.

\begin{example}[Product Labeling Hierarchy]
\begin{inparaenum}
    \item \textbf{Product}: Walk-in shower enclosure
    \item \textbf{Sub-family}: Shower cabin and screen
    \item \textbf{Family}: Bathtub, Shower, Toilet
    \item \textbf{Product line/specialty}: Sanitary Ware
\end{inparaenum}
\end{example}

\begin{figure}[ht]
\centering
\includegraphics[width=8cm, height=4cm]{figures/transp_crl/abstractions.pdf}
\caption{Hierarchical relationships in the Saint-Gobain transaction data. Subcategories form product categories, which in turn are grouped into broader product specialties.}
\label{fig:categ_abstractions_saintgob}
\end{figure}

We construct the purchase vector \(\mathbf{x}_t\) (Equation~\ref{eq:xt_purchase_saintgob}) at the subcategory level: each entry counts the number of distinct products bought within that subcategory in a given week.

\begin{equation}
\label{eq:xt_purchase_saintgob}
\begin{array}{ccccccc}
\mathbf{x}_t = & [3 & 0 & 0 & 5 & \cdots &  0 ]\\
              & \text{\scriptsize Product 1} & 
                \text{\scriptsize Product 2} & 
                \text{\scriptsize Product 3} & 
                \text{\scriptsize Product 4} & 
                \cdots & 
                \text{\scriptsize Product $d_x$} \\
              & \text{\scriptsize purchased 3 times} & 
                \text{\scriptsize not purchased} & 
                \text{\scriptsize not purchased} & 
                \text{\scriptsize purchased 5 times} & 
                \cdots & 
                \text{\scriptsize not purchased}
\end{array}
\end{equation}

\paragraph{Experimental results: Non-Overlapping clusters}
As shown in Table \ref{tab:coherence_saintgob_combined}, \gls{crl} combined with Sparse Subspace Clustering (SSC) consistently outperforms random clustering across all three labeling levels. The highest coherence is observed at the sub-category level, where the model achieves \(NMI = 0.65\), suggesting that the learned latent space preserves fine-grained semantic structure in the observational features. This performance decreases slightly at higher levels of abstraction, yet remains significantly above random, indicating that meaningful grouping is retained even at coarser resolutions. 
\begin{table}[ht]
    \centering
    \caption{Clustering coherence of Saint-Gobain data with different true label levels}
    \vspace{0.5em}
    \resizebox{0.7\textwidth}{!}{%
    \begin{tabular}{|c|c|c|c|c|} \hline
        True Labels & Model & \gls{h} & C & \gls{nmi} \\ \hline
        \multirow{2}{*}{\textbf{Sub-categories}} & \textbf{\gls{crl} + SSC} & \textbf{0.64$\pm$0.02} & \textbf{0.68$\pm$0.04} & \textbf{0.65$\pm$0.03} \\
         & \textbf{Random clustering} & 0.31$\pm$0.10 & 0.33$\pm$0.08 & 0.32$\pm$0.06 \\ \hline
        \multirow{2}{*}{\textbf{Categories}} & \textbf{\gls{crl} + SSC} & \textbf{0.55$\pm$0.03} & \textbf{0.46$\pm$0.02} & \textbf{0.39$\pm$0.03} \\
         & \textbf{Random clustering} & 0.22$\pm$0.05 & 0.24$\pm$0.06 & 0.22$\pm$0.06 \\ \hline
        \multirow{2}{*}{Specialties} & \textbf{\gls{crl} + SSC} & \textbf{0.40$\pm$0.03} & \textbf{0.42$\pm$0.02} & \textbf{0.41$\pm$0.03} \\
         & \textbf{Random clustering} & 0.12$\pm$0.04 & 0.13$\pm$0.03 & 0.12$\pm$0.04 \\ \hline
    \end{tabular}}
    \label{tab:coherence_saintgob_combined}
\end{table}

\section{Discussion}
\label{sect_crl:discussion}

\paragraph{Summary and Contributions}
This work introduced a geometric framework for interpreting \gls{crl} models through the lens of the decoder Jacobian. By imposing a sparse self-expressiveness prior, we show that the column space of the Jacobian decomposes into modular subspaces, each corresponding to latent-induced clusters of observed variables. We provided the first formal recovery guarantees for both disjoint and overlapping feature clusters in \gls{crl}, establishing high-probability identifiability under subspace incoherence and structured sparsity assumptions. Our analysis bridges latent-space identifiability and observable-level interpretability: it enables the recovery of semantically meaningful groupings that reflect the causal structure of the data-generating process. Importantly, our method is model-agnostic, complements existing \gls{crl} architectures, and requires no assumptions of anchor variables or single-parent decoding.

\paragraph{Beyond Linearity: Adaptive Self-Expression}
In this work, we used a \emph{linear self-expression} model
\[
\nabla_{\mathbf{z}} f_j = \sum_{k \neq j} C_{kj} \nabla_{\mathbf{z}} f_k.
\]
implying a fixed coefficient matrix \( C \) learned once for all inputs. However, in many settings, the optimal self-expression matrix may \emph{depend on the latent context} \( z \). This motivates an \emph{adaptive self-expression} formulation:
\[
\nabla_{\mathbf{z}} f_j(\mathbf{z}) = \sum_{k \neq j} C_{kj}(\mathbf{z}) \nabla_{\mathbf{z}} f_k(\mathbf{z}).
\]
where \( \mathbf{z} \rightarrow C(\mathbf{z}) \) varies smoothly with the latent code \(\mathbf{z}\). In statistics, \emph{varying-coefficient} models \citep{fan2003statistical} formalize this idea and show that allowing coefficients to depend on covariates can improve predictive fit in nonstationary settings. In \gls{crl}, letting \( C \) adapt to \( \mathbf{z} \) could capture nonlinear, context-dependent feature interactions, but at the cost of additional model complexity and identifiability challenges.

\paragraph{Causal Sufficiency and Unobserved Confounding}
Leap model and related \gls{crl} architectures assume \emph{causal sufficiency}: the latent space \(\mathbf{Z}\) contains all common causes of observed features \citep{peters2017elements}. In practice, however, \emph{unobserved confounders} are ubiquitous and may corrupt the learned representations. Extending \gls{crl} transparency to the \emph{latent confounding} regime is an open challenge. 

\paragraph{Dynamic Structure in Longitudinal Data }
Standard clustering approaches assume a static partitioning of features. Yet in real-world longitudinal settings, such as retail transactions, feature associations often shift over time due to seasonality, external interventions, or latent regime changes \citep{gama2014survey}. For example, summer products may co-occur only seasonally, leading to transient clusters that defy static modeling. To draw an analogy, similar phenomena arise in video data, where objects enter and exit dynamically. To accommodate such variability, one could integrate dynamic subspace clustering techniques that track temporal changes in the affinity matrix \( C_t \) via smoothness penalties or online updates \citep{KriegelSSCDynData2010, hashemi2018evolutionarySSC}. However, probabilistic guarantees, as we presented in Section \ref{sect_crl:theory}, are yet to be developed in the dynamic case. 

\paragraph{Challenges of Validation in Tabular Domains}
Evaluating learned feature clusters in tabular settings presents unique challenges. Unlike vision tasks, which often come with ground-truth segmentations, tabular datasets lack canonical groupings aligned with causal abstractions. Existing labels (e.g., product categories) are typically designed for administrative or marketing purposes, not necessarily for capturing statistical dependencies \citep{jain1988AlgoClsutering}. As a result, there may be no external reference that aligns cleanly with the structure uncovered by \gls{crl}. Moreover, even domain experts may disagree on what constitutes a coherent feature group. These challenges call for hybrid validation strategies that combine \emph{quantitative metrics} (e.g., \gls{nmi}, V-measure) with \emph{expert assessments} and \emph{task-driven evaluations}, such as improvements in downstream causal inference or predictive tasks \citep{vinh2010information}.










==> 6.tex <==
\chapter{Epilogue}
\epigraph{Science is the topography of ignorance.}{Oliver Wendell Holmes Sr}

\label{chapter:epilogue}
This final chapter serves as an epilogue to the thesis. Having concluded each chapter with its own discussion, we now take a broader perspective, highlighting unifying themes, reflecting on limitations, and outlining promising directions for future work.

\section{Towards a causal representation of confounders for causal inference}

As we conclude this thesis, it is worth reflecting on how the tools developed in Chapters \ref{chapter:cdvae} and \ref{chapter:ccpc}—which employed \gls{rnn} and Transformers to learn non‐causal summaries of the history \(\mathbf{H}_t\)—can be augmented to deliver even greater robustness and interpretability. A natural next step is to apply \gls{crl} (cf. Chapter \ref{chapter:crl}) to the entire history \(\{\mathbf{H}_s\}_{s\le t}\), thereby uncovering a latent causal process \(\{\mathbf{Z}_s\}_{s\le t}\) that admits an explicit graphical structure rather than a flat vector embedding as considered in Chapters \ref{chapter:cdvae} and \ref{chapter:ccpc}. Building on this causal graph, one then leverages the relational inductive bias of \gls{gnn}—extended to directed edges via methods such as MagNet \citep{zhang2021magnet} and edge‐enhanced \gls{gnn} \citep{rossi2024edge}—to produce rich node‐level embeddings. By propagating messages along the learned causal edges, this two‐stage pipeline merges the strengths of \gls{crl} for structure discovery with \gls{gnn} for efficient, permutation‐invariant representation learning.

\paragraph{Advantages}
Leveraging a latent causal graph over the process history, followed by a \gls{gnn} and a causal inference layer (e.g., Causal CPC or CDVAE decoders), promises several key benefits: first, it introduces a structural inductive bias \citep{battaglia2018relational} grounded in the learned causal relations, which goes beyond the purely temporal‐dependency of sequence models. Second, \gls{gnn} are permutation‐invariant, producing node embeddings that depend only on graph connectivity rather than on any arbitrary ordering of nodes. Finally, by explicitly encoding causal structure, a graph‐based pipeline followed by causal inference promises more reliable adjustment for time‐varying confounders.

\section{Invariance of the generative maps and representation identifiability}

In Chapter~\ref{chapter:cdvae}, we established that
\begin{enumerate}
  \item when the adjustment \(\mathbf U\) is observed, \(\mathrm{ACATE}\) is identifiable, and  
  \item when \(\mathbf Z\sim\mathrm{CMM}(p)\) is latent, \(\mathrm{ACATE}\) remains identifiable under mild regularity conditions (Corollary~\ref{corollary:acate_identif_U}).
\end{enumerate}

A remaining question is:

\begin{quote}
\emph{Under what conditions do the CATE augmented with \(\mathbf Z\) and that with \(\mathbf U\) coincide; that is, when does}
\[
  \tau_t(\mathbf h_t,\mathbf Z)
  = \tau_t(\mathbf h_t,\mathbf U)\;?
\]
\emph{Here}
\[
\tau_t(\mathbf h_t,\mathbf Z)
= \mathbb{E}\bigl[Y_{t}\mid \mathbf H_t=\mathbf h_t,\mathbf Z,W_{t}=1\bigr]
  - \mathbb{E}\bigl[Y_{t}\mid \mathbf H_t=\mathbf h_t,\mathbf Z,W_{t}=0\bigr],
\]
\emph{and}
\[
\tau_t(\mathbf h_t,\mathbf U)
= \mathbb{E}\bigl[Y_{t}\mid \mathbf H_t=\mathbf h_t,\mathbf U,W_{t}=1\bigr]
  - \mathbb{E}\bigl[Y_{t}\mid \mathbf H_t=\mathbf h_t,\mathbf U,W_{t}=0\bigr].
\]
\end{quote}

\paragraph{Equivalence via Conditional‐Density Equality}
This equality requires the conditional responses under each treatment arm (\(\omega = 0,1\)), augmented with either \(\mathbf{Z}\) or \(\mathbf{U}\), to be identical. Formally, we need:
\[
\mathbb{E}_{Y_{t} \mid \mathbf{H}_t, W_{t}, \mathbf{Z}}\left(Y_{t} \mid \mathbf{H}_t = \mathbf{h}_t, \mathbf{Z} = \mathbf{z}, W_{t} = \omega\right) = \mathbb{E}_{Y_{t} \mid \mathbf{H}_t, W_{t}, \mathbf{U}}\left(Y_{t} \mid \mathbf{H}_t = \mathbf{h}_t, \mathbf{U} = \mathbf{u}, W_{t} = \omega\right).
\]
For this equality to hold, it is sufficient to have
\[
p(Y_{t} \mid \mathbf{H}_t, \mathbf{Z}, W_{t}) = p(Y_{t} \mid \mathbf{H}_t, \mathbf{U}, W_{t}).
\]
Now, assume the following model for \(Y_t\):
\[
Y_t = f^{\mathbf{u}}(\mathbf{H}_t, \mathbf{U}, W_{t}) + \epsilon_t^{\mathbf{u}} \quad \text{and} \quad Y_t = f^{\mathbf{z}}(\mathbf{H}_t, \mathbf{Z}, W_{t}) + \epsilon_t^{\mathbf{z}},
\]
where \(\epsilon_t^{\mathbf{u}} \sim \mathcal{N}(0, \Sigma_{\epsilon_t^{\mathbf{u}}})\) and \(\epsilon_t^{\mathbf{z}} \sim \mathcal{N}(0, \Sigma_{\epsilon_t^{\mathbf{z}}})\). The equality \(p(Y_{t} \mid \mathbf{H}_t, \mathbf{Z}, W_{t}) = p(Y_{t} \mid \mathbf{H}_t, \mathbf{U}, W_{t})\) holds if and only if \(f^{\mathbf{u}}(\mathbf{H}_t, \mathbf{U}, W_{t}) = f^{\mathbf{z}}(\mathbf{H}_t, \mathbf{Z}, W_{t})\) almost surely and \(\Sigma_{\epsilon_t^{\mathbf{z}}} = \Sigma_{\epsilon_t^{\mathbf{u}}}\). This indicates that we can represent the shared function by \(f=f^{\mathbf{u}}=f^{\mathbf{z}}\), provided that \(\mathbf{U}\) and \(\mathbf{Z}\) have the same support.

\paragraph{Partial Injectivity: A very restrictive assumption} Let's assume that the noise distribution is fully known, that is, \(\Sigma \coloneqq \Sigma_{\epsilon_t^{\mathbf{z}}} = \Sigma_{\epsilon_t^{\mathbf{u}}}\) is predefined. Establishing equality in conditional distributions now reduces to demonstrating \emph{partial invariance} in \(f\). 

To illustrate, if \(f\) is partially injective, meaning that for any \((\mathbf{h}_t, \omega)\), the map \(\mathbf{z} \rightarrow f(\mathbf{h}_t, \mathbf{z}, \omega)\) is injective, then \(\mathbf{Z} = \mathbf{U}\) almost surely. However, designing a function class that satisfies such partial injectivity would be highly restrictive and impractical, especially when aiming to approximate \(f\) using neural networks. Moreover, learning the exact unobserved adjustment variables \(\mathbf{U}\) is often unrealistic due to the unknown dimensionality of \(\mathbf{U}\), which is implicitly assumed when considering support equality between \(\mathbf{Z}\) and \(\mathbf{U}\). 


\paragraph{Group‐Equivariance as a Practical Alternative} A more practical assumption involves allowing the identification of generative factors from observed distributions up to trivial ambiguities, such as rotations, permutations, scaling, or sign flips. For example, if \(\mathbf{Z}\) and \(\mathbf{U}\) induce the same observed conditional distribution over response sequences, that is, \(p(Y_{\leq T} \mid \mathbf{H}_{\leq T}, W_{\leq T})\), then, under mild conditions, \(\mathbf{Z}\) and \(\mathbf{U}\) should be related by a rotation plus translation. Therefore, a form of partial invariance in \(f\) is to verify whether, for any \((\mathbf{h}_t, \omega)\) and \(\mathbf{z}, \mathbf{z}'\) such that \(\mathbf{z}' = A\mathbf{z} + b\) with $A$ being a rotation matrix, \(f(\mathbf{h}_t, \mathbf{z}, \omega) = f(\mathbf{h}_t, \mathbf{z}', \omega).
\) This assumption is significantly less restrictive than partial injectivity, as it permits equality in responses for equivalence classes of latent variables connected through simple transformations.

Since \(f\) is often approximated by neural networks, ensuring that the network is invariant to certain transformations of the input connects to existing work on \emph{invariant and equivariant neural networks} \citep{cohen2016group, zaheer2017DeepSets, kondor2018generalization, xu2020towards, yarotsky2022universal, immer2022invariance}. Although these methods have been applied in simpler settings, they offer inspiration for future work on designing generative models that leverage such invariances when representations are assumed to be identifiable.

\paragraph{Research Gap}
To our knowledge, this form of consistency has been largely overlooked in the literature of identifiable representations and of \gls{crl} \citep{khemakhem2020variational, klindt2021TemporalSparseCoding, Yao2021GeneralTemporal, mita2021identifiableDoubleVAE, lachapelle2022disentMechaSparse, wu2022betaintactvae, xu2024FrontDoorIVAE, xie2024causal, li2024and}. In these works, the objective is the identifiability of the latent space up to equivalence classes induced by trivial ambiguities, yet the generative model is seldom designed to be invariant or equivariant to these transformations.


\section{Uncertainty and Sensitivity in Causal Inference for Longitudinal Data}
In causal inference, we are faced with different sources of "ignorance," which may confer uncertainty over the estimated treatment effect. Causality literature discusses three main sources:
\begin{inparaenum}[(1)]
    \item \textbf{data finiteness}: As discussed by \cite{jesson2021IgnoRegionCATE, jesson2020identifying} in the static setting, which we extrapolate to our longitudinal case, if some individuals at time \( t \) with historical context \( \mathbf{h}_t \) and \( W_t=1 \) are underrepresented in the observed data in such a way that there are no individuals in the control group \( W_t=0 \) with similar historical context, then this will provide uncertainty over treatment effect estimation (Chapter \ref{chapter:cdvae}). Such uncertainty comes inherently from the data finiteness, which is a source of epistemic uncertainty. This source is even more critical in the longitudinal case when considering time-varying treatments, as in the Causal \gls{cpc} model (Chapter \ref{chapter:ccpc}), due to the exponential explosion of treatment regimes \( \omega_{t+1:t+\rho} \). 
    \item \textbf{violations of overlap (Assumption \ref{assp:overlap_seq})} is another important source of epistemic uncertainty. For example, if there exists a level in the historical context \( \mathbf{h}_t \) where all observed individuals are in \( W_t=1 \), then we cannot reliably estimate conditional responses when \( W_t=0 \). Again, when we target longitudinal data and time-varying treatment, the longer the treatment sequence, the more difficult it is for overlap to hold. Adding to this, the fact that the historical context is both high-dimensional and time-varying can lead to overlap violations. 
    \item  \textbf{violation of ignorability} (Assumption \ref{assp:seq_ignorability}) leads to the presence of unobserved confounding and any estimation of  \gls{cate}, \gls{acate} (Chapter \ref{chapter:cdvae}), or the conditional potential outcome (Chapter \ref{chapter:ccpc}) will be biased. 
\end{inparaenum}

\paragraph{Existing Literature}  
To date, uncertainty‐quantification methods in causal inference have mainly focused on \emph{static} settings and do not readily apply to longitudinal, multi‐horizon forecasts as in Chapter \ref{chapter:ccpc}. We organize these static‐setting approaches by the ignorability assumptions they make:

\subparagraph{1. Assuming strong ignorability} 
Several methods have been proposed under the assumption of \textit{strong ignorability}. \cite{lei2021conformalPO_ITE} introduced a conformal inference-based approach to estimate intervals for counterfactuals and \gls{ite} under the \gls{po} framework. This method accounts for two sources of variability: 
\begin{inparaenum}[(1)]
\item the variability of the response around the regression function and 
\item the variability of  \gls{cate} estimators due to finite samples. 
\end{inparaenum}
Controlling both sources requires a sufficiently rich set of covariates to explain outcome variability while providing accurate \gls{cate} estimates for all covariate values. Building on this, \cite{wang2025CPITE_CondDensity} applied conformal prediction to the \textit{conditional density} of the outcome given the covariates, rather than using the conditional expectation, resulting in shorter prediction intervals compared to \cite{lei2021conformalPO_ITE}. 

\subparagraph{2. Assuming hidden confounding} 
When ignorability is violated, several approaches have been proposed for interval estimation under partial identification. \citet{marmarelis2024ensembled} construct prediction intervals for partially identifiable outcomes via a causal sensitivity model combined with deep ensembles. \citet{kallus2019intervalITEUnbsCnf} introduced a functional interval estimator for bounding individual treatment effects using adversarially weighted kernel regression, with weights governed by a marginal sensitivity model \citep{tan2006distributional}. Normalizing flows have been applied to model the distribution of \gls{ite} \citep{vanderschueren2023noflite, papamakarios2021normalizing}, while collaborative networks have been extended to estimate full potential outcome distributions in static settings \citep{zhou2022estimating, zhou2021UQCollabNets}. \citet{kallus2022Harm} derived sharp bounds on the fraction of negatively affected individuals from observational data. The region of ignorance framework by \citet{jesson2021IgnoRegionCATE} yields \gls{cate} intervals that expand under poor overlap, insufficient similarity, or confounding, combining Bayesian deep models with marginal sensitivity analysis \citep{kallus2019intervalITEUnbsCnf}. Finally, \citet{oprescu2023BLearner} achieved quasi-oracle \gls{cate} bounds via meta-learners augmented with marginal sensitivity models.

\paragraph{Research Gap}
Ideally, we would like to have interval estimation around the causal quantity, where the width \emph{simultaneously} changes depending on data finiteness, violation of overlap, and of ignorability. Despite significant advances in uncertainty quantification in this line of work, most existing methods are designed for static settings and do not readily extend to longitudinal data. This creates a critical gap in addressing the challenges posed by temporal dependencies, time-varying treatments, and evolving confounding. In particular, multi-horizon forecasting of causal outcomes introduces an additional challenge: the autoregressive structure causes prediction errors to compound over time, adding a fourth source of randomness beyond data finiteness, overlap violations, and unobserved confounding.

\section{Uncertainty in Causal Representation Learning}

While Bayesian causal discovery quantifies uncertainty over observed‐variable graphs, far less is known about uncertainty in \gls{crl} (Chapter~\ref{chapter:crl}). Bayesian Causal Discovery \citep{ChickeringBayesCausDisco, heckerman2006BayesCausDisco, friedman2003BayesCausDisco, mamaghan2024challengesBCD} defines a posterior distribution over the graph and the parameters of the \gls{scm}, thereby quantifying the epistemic uncertainty of the causal model.  Accurately estimating this uncertainty is crucial for downstream tasks such as causal effect estimation \citep{toth2022active, emezue2023benchmarking} and experimental design \citep{agrawal2019abcd, tigas2023differentiable}. While recent Bayesian causal discovery methods have effectively provided uncertainty quantification in the static setting \citep{lorch2021dibs,wang2022tractableBCD, deleu2022BCDGflowNets, AnnadaniVariationalCAusNets, annadani2023bayesdag, dhir2025MetaLearnBCD} and in the time-varying setting \citep{debeire2024bootstrap, Zhao2024BGrangerCD-MTS, jin2025directed}, they typically operate on observed variables assumed to be causal.  

\paragraph{Research Gap} Little work has been done on assessing uncertainty in the \gls{crl} framework (Chapter \ref{chapter:crl}). The only notable work in this direction is that of \citet{subramanian2022latentBCD}, where they introduced a Bayesian latent variable decoder model for causal discovery, relaxing the need for direct observation of causal variables. However, their approach remains constrained by linearity and isotropic Gaussian assumptions, significantly limiting the expressiveness of latent structures that can be captured.  Thus, existing approaches have not explored uncertainty quantification in latent causal representations within nonlinear or time-varying contexts. A substantial open research direction remains: developing Bayesian causal discovery methods capable of quantifying uncertainty over latent causal representations, particularly in nonlinear settings and/or temporally evolving structures.




==> appendices/3.tex <==

\chapter{Appendix: Chapter \ref{chapter:cdvae}}
\section{Proofs}
\label{appendix_cdvae:proofs}

\subsection{Identifiability: Treatment Effects and Unobserved Adjustment Variables}
\label{appendix:proof_effect_Z}
\begin{proof}[\textbf{CATE Identifiability}]
Assuming the consistency, overlap, and ignorability assumptions (\ref{assp:consistency_seq}, \ref{assp:overlap_seq}, \ref{assp:seq_ignorability}), we demonstrate that the Conditional Average Treatment Effect (CATE), as defined in Eq. \ref{eq:CATE_Identifiability}, is identifiable from the observed data distribution:
\begin{equation}
\tau_t = \mathbb{E}(Y_{t}| \mathbf{H}_t = \mathbf{h}_t, W_{t} = 1) - \mathbb{E}(Y_{t}| \mathbf{H}_t = \mathbf{h}_t, W_{t} = 0).
\end{equation}

Establishing the identifiability of CATE requires showing that the two potential outcome expectations are identifiable. By the ignorability assumption (\ref{assp:seq_ignorability}), the potential outcome under treatment can be expressed as:
\[
m_{t}^{1}(\mathbf{h}_{t}) = \mathbb{E}_{Y_{t}(1) \mid \mathbf{H}_{t} }(Y_{t}(1) \mid \mathbf{H}_{t} = \mathbf{h}_{t}) = \mathbb{E}_{Y_{t}(1) \mid \mathbf{H}_{t}, W_t }(Y_{t}(1) \mid \mathbf{H}_{t} = \mathbf{h}_{t}, W_t = 1).
\]
Using the consistency assumption (\ref{assp:consistency_seq}), the observed response can identify \( Y_{t}(1) \) when conditioned on \( W_t = 1 \):
\[
m_{t}^{1}(\mathbf{h}_{t}) = \mathbb{E}_{Y_{t} \mid \mathbf{H}_{t}, W_t }(Y_{t}\mid \mathbf{H}_{t} = \mathbf{h}_{t}, W_t = 1).
\]
Similarly, we identify the expected potential outcome under no treatment:
\[
m_{t}^{0}(\mathbf{h}_{t}) = \mathbb{E}_{Y_{t} \mid \mathbf{H}_{t}, W_t }(Y_{t}\mid \mathbf{H}_{t} = \mathbf{h}_{t}, W_t = 0).
\]
The existence of these expectations is guaranteed by the overlap assumption.
\end{proof}

\begin{proof}[\textbf{Augmented CATE Identifiability}]
\label{proof:acate_identif}
Assuming that the adjustment variables \(\mathbf{U}\) are observed, we demonstrate the identifiability of the Augmented CATE:
\[
\tau_{t}(\mathbf{h}_{t}, \mathbf{u})= \mathbb{E}(Y_{t}| \mathbf{H}_t = \mathbf{h}_t, \mathbf{U}= \mathbf{u}, W_{t} = 1) - \mathbb{E}(Y_{t}| \mathbf{H}_t = \mathbf{h}_t, \mathbf{U}= \mathbf{u}, W_{t} = 0).
\]
The assumptions of consistency, overlap, and ignorability ensure that CATE is identifiable. Since \(\mathbf{U}\) does not affect the treatment, the overlap assumption (\ref{assp:overlap_seq}) remains valid. Further, \(\mathbf{U}\) being independent of the treatment implies that the ignorability assumption holds when conditioning on \(\mathbf{U}\):
\[
Y_{it}(\omega) \indep W_{t}| \mathbf{H}_{t} = \mathbf{h}_{t} \implies Y_{it}(\omega) \indep W_{t}| \mathbf{H}_{t} = \mathbf{h}_{t},\mathbf{U}= \mathbf{u} \quad \forall (\omega, \mathbf{h}_{t}, \mathbf{u}).
\]
The remainder of the proof follows the CATE identifiability argument.
\end{proof}

\begin{proof}[\textbf{Theorem \ref{thm:valid_Z}}]
\label{assp:regularity_y_space}
Let \(\mathbf{Z}\) be a latent variable such that \(\mathbf{Z} \sim CMM(p)\). Any static adjustment variables affecting all response series in the panel must be measurable with respect to \((\mathbf{Z}, \mathbf{H}_T)\). We assume weak regularity conditions on treatment and response domains.
\begin{assumption}[Regularity]
The response domain \(\mathcal{Y}\) is a Borel subset of a compact interval.
\end{assumption}
The treatment domain \(\mathcal{W} = \{0,1\}\) is a Borel subset of \([0,1]\). To prove the theorem, we need the following lemma:
\begin{lemma}[Kernels and Randomization \citep{Kallenberg2021FoundationsOM}]
\label{lem: kernel_RD}
Let \(\mu\) be a probability kernel from a measurable space \(S_1\) to a Borel space \(S_2\). There exists a measurable function \(f: S_1 \times [0,1] \rightarrow S_2\) such that if \(\vartheta\) is uniform on \([0,1]\), then \(f(s_1, \vartheta)\) is distributed as \(\mu(s_1, \cdot)\).
\end{lemma}
Suppose by contradiction the existence of $\mathbf{Z}\prime$ that is not measurable with respect to $(\mathbf{Z}, \mathbf{H}_T)$ and such that: 
\begin{equation*}
    Y_{it}(\omega) \notindep \mathbf{Z_i}\prime| \mathbf{H}_{it}, \mathbf{Z}_i \quad \forall \omega, t
\end{equation*}
Let $t$ be an arbitrary time step in the panel data. By lemma \ref{lem: kernel_RD}, there exists a measurable function  $f_t: \mathcal{H}_t \times \mathcal{W} \times \mathcal{Z} \times [0,1] \rightarrow \mathcal{Y}$ such that: 
\begin{equation*}
    Y_{it} = f_t(\mathbf{H}_{it}, W_{it}, \mathbf{Z}_i, \gamma_{it}), \quad \gamma_{it} \indep (\mathbf{H}_{it}, W_{it}, \mathbf{Z}_i).
\end{equation*}
The conditional Markov property implies the independence of the following conditional distributions: 
\begin{equation*}
    (Y_{it}\mid \mathbf{H}_{it}, \mathbf{Z}_i, W_{it} = \omega) \indep  (Y_{it\prime}\mid \mathbf{H}_{it\prime}, \mathbf{Z}_i, W_{it\prime} = \omega\prime).
\end{equation*}
Such that  $t\prime$ verifies $|t - t\prime| > p$. We can thus conclude that: 
\begin{equation*}
    (Y_{it}(\omega) \mid \mathbf{H}_{it}, \mathbf{Z}_i) \indep  (Y_{it\prime}(\omega\prime) \mid \mathbf{H}_{it\prime}, \mathbf{Z}_i).
\end{equation*}
Because : 
\begin{equation*}
\begin{aligned}
    (Y_{it}(\omega) \mid \mathbf{H}_{it}, \mathbf{Z}_i) &= (Y_{it}(\omega) \mid \mathbf{H}_{it}, \mathbf{Z}_i, W_{it} = \omega)     \\
 &= (Y_{it} \mid \mathbf{H}_{it}, \mathbf{Z}_i, W_{it} = \omega).\\
\end{aligned}
\end{equation*}
The first equality follows from the sequential ignorability of the theorem \ref{thm:seq_ign_augmented}, and the second equality follows the consistency assumption.
 On the other hand, we also have from the CMM(p) that: 
 \begin{equation*}
     \gamma_{it\prime} \indep Y_{it} \mid \mathbf{H}_{it}, \mathbf{Z}_i.
 \end{equation*}
From which it follows using the fact that $\gamma_{it} \indep (\mathbf{H}_{it}, W_{it}, \mathbf{Z}_i)$ and $Y_{it}(\omega) \mid \mathbf{H}_{it}, \mathbf{Z}_i = Y_{it} \mid \mathbf{H}_{it}, \mathbf{Z}_i, W_{it} = \omega $: 
\begin{equation*}
    \gamma_{it\prime} \indep Y_{it}(\omega) \mid \mathbf{H}_{it}, \mathbf{Z}_i
\end{equation*}
By using twice the lemma \ref{lem: kernel_RD}, we write: 
\begin{equation}
    \gamma_{it\prime} = h_t(\mathbf{Z}\prime_i, \eta_{it\prime}), \quad \eta_{it\prime} \indep  \mathbf{Z}\prime_i
\label{eq:gamma}
\end{equation}
And: 
\begin{equation}
    Y_{it}(\omega) = g_t(\mathbf{Z}\prime_i, \epsilon_{it}), \quad \epsilon_{it} \indep  \mathbf{Z}\prime_i.
\label{eq:y_pot}
\end{equation}
Since $ \mathbf{Z}\prime_i$ is not measurable with respect to $( \mathbf{Z}_i, \mathbf{H}_{it})$, then by \eqref{eq:gamma} and \eqref{eq:y_pot}: 
\begin{equation*}
    \gamma_{it\prime} \notindep Y_{it} \mid \mathbf{H}_{it}, \mathbf{Z}_i
\end{equation*}
We have thus a contradiction.
\end{proof}

\subsection{Derivation of CDVAE Loss}
\label{appendix:proof_elbo}
\begin{proof}[\textbf{ELBO}]
We provide proof that the bound in Eq. (\ref{eq:elbo_orig}) is indeed the Evidence Lower Bound (ELBO) for the weighted conditional log-likelihood.

By the concavity of the logarithm, for every \(t \in \{1, 2, \dots, T\}\), we have:
\begin{equation}
\label{eq:elbo_step}
\log p_\theta\left(y_{t} \mid \mathbf{h}_{t}, \omega_t\right) 
\geq 
\underbrace{\mathbb{E}_{\mathbf{Z}, C \sim q_{\phi}(\cdot , \cdot \mid \mathcal{D}_T)}  
\left[  
\log \frac{p_\theta\left(y_{t}, \mathbf{Z}, C\mid \mathbf{h}_{t}, \omega_{t}\right)}{q_{\phi}(\mathbf{Z}, C \mid \mathcal{D}_T)} 
\right]}_{(*)}
\end{equation}

We use the identity
\[
p_\theta(y_t, \mathbf{z}, c \mid \mathbf{h}_t, \omega_t)
= p_\theta(y_t \mid \mathbf{z}, \mathbf{h}_t, \omega_t)\,p(\mathbf{z}, c),
\]
and the factorization of the approximate posterior
\[
q_\phi(\mathbf{z}, c \mid \mathcal{D}_T)
= q_{\phi_z}(\mathbf{z} \mid \mathcal{D}_T)\, q_{\phi_c}(c \mid \mathcal{D}_T),
\]
to write
\[
\begin{aligned}
(*) &=
\mathbb{E}_{\mathbf{Z}, C \sim q_\phi(\cdot,\cdot \mid \mathcal{D}_T)}
\left[
    \log \frac{
        p_\theta(y_t \mid \mathbf{Z}, \mathbf{h}_t, \omega_t)\,p(C \mid \mathbf{Z})\,p(\mathbf{Z})
    }{
        q_{\phi_z}(\mathbf{Z} \mid \mathcal{D}_T)\, q_{\phi_c}(C \mid \mathcal{D}_T)
    }
\right] \\[1.2ex]
&= \mathbb{E}_{\mathbf{Z}, C \sim q_\phi(\cdot,\cdot \mid \mathcal{D}_T)}
\bigl[
    \log p_\theta(y_t \mid \mathbf{Z}, \mathbf{h}_t, \omega_t)
\bigr] \\[0.8ex]
&\hspace{2em}
- \underbrace{D_{KL}\bigl(
    q_{\phi_z}(\mathbf{Z} \mid \mathcal{D}_T)\, q_{\phi_c}(C \mid \mathcal{D}_T)
    \parallel p(C \mid \mathbf{Z})\,p(\mathbf{Z})
\bigr)}_{(**)}.
\end{aligned}
\]

The KL divergence term \((**)\) between the joint approximate posterior and prior decomposes as
\[
\begin{aligned}
(**)
&= \sum_{c=1}^K
    \mathbb{E}_{\mathbf{Z} \sim q_\phi(\cdot, c \mid \mathcal{D}_T)}
    \log\left(
        \frac{p(c \mid \mathbf{Z})\,p(\mathbf{Z})}{
            q_{\phi_z}(\mathbf{Z} \mid \mathcal{D}_T)\, q_{\phi_c}(c \mid \mathcal{D}_T)
        }
    \right) \\[1.5ex]
&= \sum_{c=1}^K
    \mathbb{E}_{\mathbf{Z} \sim q_\phi(\cdot, c \mid \mathcal{D}_T)}
    \log\left(
        \frac{p(\mathbf{Z})}{q_{\phi_z}(\mathbf{Z} \mid \mathcal{D}_T)}
    \right) \\[1.2ex]
&\hspace{2em}
+ \sum_{c=1}^K
    \mathbb{E}_{\mathbf{Z} \sim q_\phi(\cdot, c \mid \mathcal{D}_T)}
    \log\left(
        \frac{p(c \mid \mathbf{Z})}{q_{\phi_c}(c \mid \mathcal{D}_T)}
    \right) \\[1.5ex]
&= D_{KL}\bigl(
    q_{\phi_z}(\mathbf{z} \mid \mathcal{D}_T)\,\|\,p(\mathbf{z})
\bigr) \\[1.2ex]
&\hspace{2em}
+ \mathbb{E}_{\mathbf{Z} \sim q_{\phi_z}(\cdot \mid \mathcal{D}_T)}
    D_{KL}\bigl(
        q_{\phi_c}(c \mid \mathcal{D}_T)\,\|\,p(c \mid \mathbf{Z})
    \bigr).
\end{aligned}
\]

We define the individual ELBO by performing a weighted sum over log-likelihood terms and marginalizing over \(\mathcal{D}_T\):
\[
L = \sum_{t=1}^T
    \mathbb{E}_{\mathcal{D}_T}
    \bigl[
        \alpha(\mathbf{H}_t, W_t)\, \log p_\theta(Y_t \mid \mathbf{H}_t, W_t)
    \bigr]
\ge \mathbb{E}_{\mathcal{D}_T}
\underbrace{
    \sum_{t=1}^T
    \mathbb{E}_{\mathbf{Z}, C \sim q_\phi(\cdot,\cdot \mid \mathcal{D}_T)}
    \left[
        \alpha(\mathbf{h}_t, \omega_t)\,
        \log\frac{
            p_\theta(y_t, \mathbf{Z}, C \mid \mathbf{h}_t, \omega_t)
        }{
            q_\phi(\mathbf{Z}, C \mid \mathcal{D}_T)
        }
    \right]
}_{\mathrm{ELBO}_0(\mathcal{D}_T;\,\theta,\phi)}.
\]

Finally, \(\mathrm{ELBO}_0(\mathcal{D}_T; \theta,\phi)\) expands to
\[
\begin{aligned}
\mathrm{ELBO}_0(\mathcal{D}_T; \theta,\phi)
&= \sum_{t=1}^T
    \mathbb{E}_{\mathbf{Z} \sim q_{\phi_z}(\cdot \mid \mathcal{D}_T)}
    \bigl[
        \alpha(\mathbf{h}_t,\omega_t)\,
        \log p_\theta(y_t \mid \mathbf{h}_t,\omega_t,\mathbf{Z})
    \bigr] \\[1.5ex]
&\hspace{1em}
- \left(\sum_{t=1}^T \alpha(\mathbf{h}_t,\omega_t)\right)
\Biggl\{
    D_{KL}\bigl(
        q_{\phi_z}(\mathbf{z} \mid \mathcal{D}_T)\,\|\,p(\mathbf{z})
    \bigr) \\[1.2ex]
&\hspace{5em}
+ \mathbb{E}_{\mathbf{Z} \sim q_{\phi_z}(\cdot \mid \mathcal{D}_T)}
    D_{KL}\bigl(
        q_{\phi_c}(c \mid \mathcal{D}_T)\,\|\,p(c \mid \mathbf{Z})
    \bigr)
\Biggr\}.
\end{aligned}
\]
The gap in our variational approximation is defined as the difference between the true weighted log-likelihood and the ELBO:
\begin{equation*}
    \mathbb{E}_{\mathcal{D}_T}\Delta_0(\mathcal{D}_T; \theta, \phi) \coloneqq L - \mathbb{E}_{\mathcal{D}_T}\mathrm{ELBO_0}(\mathcal{D}_T; \theta, \phi)
\end{equation*}

The per-time-step gap in Eq. (\ref{eq:elbo_step}) can be rewritten as:
\begin{align*}
\log p_\theta\left(y_{t} \mid \mathbf{h}_{t}, \omega_t\right) - (*) &= \mathbb{E}_{\mathbf{Z}, C \sim q_{\phi}(\cdot , \cdot \mid \mathcal{D}_T)}  \left[ 
\log \frac{
p_\theta\left(y_{t} \mid \mathbf{h}_{t}, \omega_t\right)q_{\phi}(\mathbf{Z}, C \mid \mathcal{D}_T)
}{
p_\theta\left(y_{t}, \mathbf{Z}, C\mid \mathbf{h}_{t}, \omega_{t}\right) 
}
\right] \\
&= \mathbb{E}_{\mathbf{Z}, C \sim q_{\phi}(\cdot , \cdot \mid \mathcal{D}_T)}
\left[ 
\log \frac{
q_{\phi}(\mathbf{Z}, C \mid \mathcal{D}_T)
}{
p_\theta\left(\mathbf{Z}, C\mid \mathcal{D}_t\right) 
}
\right] \\
&= D_{KL}\left(q_{\phi}(\mathbf{Z}, C \mid \mathcal{D}_T) \parallel p_\theta\left(\mathbf{Z}, C\mid \mathcal{D}_t\right) \right)
\end{align*}

This last equation holds because 
\[
p_\theta\left(y_{t}, \mathbf{Z}, C \mid \mathbf{h}_{t}, \omega_{t}\right) = p_\theta\left(\mathbf{Z}, C \mid y_{t}, \mathbf{h}_{t}, \omega_{t}\right) p_\theta\left(y_{t} \mid \mathbf{h}_{t}, \omega_{t}\right),
\]
and \(\{y_{t}, \mathbf{h}_{t}, \omega_{t}\} = \{y_{\leq t}, \mathbf{x}_{\leq t}, \omega_{\leq t}\} = \mathcal{D}_t\). The individual gap is thus:
\[
\Delta_0(\mathcal{D}_T; \theta, \phi) = \sum_{t = 1}^{T} \alpha(\mathbf{h}_t, \omega_t) D_{KL}\left(q_{\phi}(\mathbf{Z}, C \mid \mathcal{D}_T) \parallel p_\theta\left(\mathbf{Z}, C\mid \mathcal{D}_t\right) \right)
\]
\end{proof}
\subsection{Transfer of Ignorability under Invertible Maps}
\label{appendix:proof_ignorability_invsersion}
\begin{proposition}
Let \(\Phi\) be an invertible representation function. Then, \(Y_{t}(\omega) \indep W_{t}| \Phi(\mathbf{H}_{t})\) holds if and only if \(Y_{t}(\omega) \indep W_{t}| \mathbf{H}_{t}\). Moreover, \(p(W_t=\omega|\Phi(\mathbf{h}_{t}))>0\) holds if and only if \(p(W_t=\omega|\mathbf{h}_{t})>0\).
\end{proposition}
\begin{proof}
    Assume \(Y_t(\omega) \indep W_t \mid \mathbf{H}_t\). For a non-invertible \(\Phi\), let
\(\Phi^{-1}(\mathbf{r}) = \{\mathbf{h}_t : \Phi(\mathbf{h}_t) = \mathbf{r}\}\). Then
\[
\begin{aligned}
p(Y_t(\omega)\mid \omega_t, \mathbf{r})
&= \frac{
    \displaystyle\int_{\mathbf{h}_t \in \Phi^{-1}(\mathbf{r})}
    p(Y_t(\omega)\mid \omega_t, \mathbf{h}_t)\,p(\mathbf{h}_t\mid \omega_t)\,d\mathbf{h}_t
}{
    \displaystyle\int_{\mathbf{h}_t \in \Phi^{-1}(\mathbf{r})}
    p(\mathbf{h}_t\mid \omega_t)\,d\mathbf{h}_t
} \\[2.0ex]
&= \frac{
    \displaystyle\int_{\mathbf{h}_t \in \Phi^{-1}(\mathbf{r})}
    p(Y_t(\omega)\mid \mathbf{h}_t)\,p(\mathbf{h}_t\mid \omega_t)\,d\mathbf{h}_t
}{
    \displaystyle\int_{\mathbf{h}_t \in \Phi^{-1}(\mathbf{r})}
    p(\mathbf{h}_t\mid \omega_t)\,d\mathbf{h}_t
},
\end{aligned}
\]
where ignorability implies that for general \(\Phi\),
\[
p(Y_t(\omega)\mid \omega_t, \mathbf{r})
\ne p(Y_t(\omega)\mid \mathbf{r}).
\]

For an invertible \(\Phi\), however,
\[
p(Y_t(\omega)\mid \omega_t, \Phi(\mathbf{h}_t)) = p(Y_t(\omega)\mid \Phi(\mathbf{h}_t)),
\]
and similarly,
\[
p(W_t=\omega \mid \Phi(\mathbf{h}_t)) = p(W_t=\omega \mid \mathbf{h}_t).
\]
\end{proof}

\subsection{CDVAE in the Near-Deterministic Regime}
\label{appendix:proof_cdvae_near_det}
\begin{proof}[Theorem \ref{thm:vaes_to_truell}]
\textbf{Part 1}: $lim_{s \to + \infty} p_{\theta_s}(y_{\leq T} \mid \mathbf{x}_{\leq T}, \omega_{\leq T}) = p(y_{\leq T} \mid \mathbf{x}_{\leq T}, \omega_{\leq T})$.

Define the conditional cumulative distribution function (CDF) of the response given covariates, for each $t$ as:
\[
F_t(y_t \mid \mathbf{h}_t, \omega_t) = \int_{- \infty}^{y_t} p(y_t' \mid \mathbf{h}_t, \omega_t ) dy_t'.
\]
Define the mapping \( F: \mathcal{Y}^{T} \to [0,1]^T \) as:
\[
F(y_1, \dots, y_T \mid \mathbf{x}_{\leq T}, \omega_{\leq T}) \coloneqq \left[F_1(y_1 \mid \mathbf{h}_1, \omega_1), \dots, F_T(y_T \mid \mathbf{h}_T, \omega_T)\right].
\]

The differential of the mapping is given by:
\[
dF(y_1, \dots, y_T \mid \mathbf{x}_{\leq T}, \omega_{\leq T}) = p(y_{\leq T} \mid \mathbf{x}_{\leq T}, \omega_{\leq T}) dy_{\leq T}.
\]

Now, define the following mapping for the latent variables using the Darmois construction \citep{hyvarinen1999nonlinear}:
\[
G_i(z_i \mid z_1, \dots, z_{i-1}) = \int_{- \infty}^{z_i} p(z_i' \mid z_1, \dots, z_{i-1}) dz_i'.
\]
We then define the mapping \( G: \mathbb{R}^{d_{\mathbf{z}}} \to [0,1]^T \) such that:
\[
G(\mathbf{z}) \coloneqq [G_1(z_1), G_2(z_2 \mid z_1), \dots, G_i(z_{\mathbf{z}} \mid z_1, \dots, z_{d_{\mathbf{z}}-1})].
\]
Since \(d_{\mathbf{z}} \le T\) by assumption, we can trivially augment the mapping \(G\) to \(\widetilde{G}\) so that its image lies in \([0,1]^T\). That is,
\[
\widetilde{G} : \mathbb{R}^{d_{\mathbf{z}}} \to [0,1]^T, \quad
\widetilde{G}(\mathbf{z}) \coloneqq
\bigl[G(\mathbf{z}),\,\underbrace{0,\dots,0}_{T - d_{\mathbf{z}}}\,\bigr].
\]
The differential is then given by
\[
d\widetilde{G}(\mathbf{z}) = p(\mathbf{z})\,d\mathbf{z}.
\]
We now define the mean and variance of the encoder as follows:
\[
f_t(\mathbf{h}_t, \omega_t, \mathbf{z}; \theta_{s}^*) \coloneqq [F^{-1}(\Tilde{G}(\mathbf{z}) \mid \mathbf{x}_{\leq T}, \omega_{\leq T})]_t, \quad \sigma_{s}^* = \frac{1}{\sqrt{s}}.
\]
There is a consistency issue to address with this definition. First, observe that the function $f_t(.; \theta_{s}^*)$ takes as input only data up to time step $t$, but the inverse of the cumulative CDF is defined given \textit{the whole sequence} of $(\mathbf{x}_{\leq T}, \omega_{\leq T})$. We therefore need to verify the following lemma which holds for our definition of $f_t(.; \theta_{s}^*)$.
\begin{lemma}
Let \((y_{\le T}, \mathbf{x}_{\le T}, \omega_{\le T})\) and
\((y_{\le T}', \mathbf{x}_{\le T}', \omega_{\le T}')\) be two distinct realizations of repeated measurements such that there exists \(t_0\) for which
\[
\mathbf{x}_{\le t_0} = \mathbf{x}_{\le t_0}', \quad
\omega_{\le t_0} = \omega_{\le t_0}'.
\]
Then, for every \(t \le t_0\),
\[
\bigl[F^{-1}(\widetilde{G}(\mathbf{z}) \mid \mathbf{x}_{\le t}, \omega_{\le t})\bigr]_t
= \bigl[F^{-1}(\widetilde{G}(\mathbf{z}) \mid \mathbf{x}_{\le t}', \omega_{\le t}')\bigr]_t.
\]
\end{lemma}
Now, we decompose the marginal probabilistic model:
\begin{equation*}
    \begin{split}
        p_{\theta_s}(y_{\leq T} \mid \mathbf{x}_{\leq T}, \omega_{\leq T}) &= \int_{\mathbb{R}^{d_{\mathbf{z}}}} p_{\theta_s}(y_{\leq T}, \mathbf{z} \mid \mathbf{x}_{\leq T}, \omega_{\leq T}) d\mathbf{z} \\
        &= \int_{\mathbb{R}^{d_{\mathbf{z}}}} \prod_{t=1}^T p_{\theta_s}(y_{t}, \mathbf{z} \mid y_{<t}, \mathbf{x}_{\leq t}, \omega_{\leq t}) p(\mathbf{z}) d\mathbf{z} \\
        &= \int_{\mathbb{R}^{d_{\mathbf{z}}}} \prod_{t=1}^T \mathcal{N}\left( y_t \mid [F^{-1}(\Tilde{G}(\mathbf{z}) \mid \mathbf{x}_{\leq T}, \omega_{\leq T})]_t, (\sigma_{s}^*)^2 \right) p(\mathbf{z}) d\mathbf{z} \\
        &= \int_{[0,1]^{T}} \prod_{t=1}^T \mathcal{N}\left( y_t \mid [F^{-1}(\xi \mid \mathbf{x}_{\leq T}, \omega_{\leq T})]_t, (\sigma_{s}^*)^2 \right) d\mathbf{\xi}\\
        &= \int_{\mathcal{Y}^{T}} \prod_{t=1}^T \mathcal{N}\left( y_t \mid [y_{\leq T}']_t, (\sigma_{s}^*)^2 \right) p(y_{\leq T}' \mid \mathbf{x}_{\leq T}', \omega_{\leq T}') dy_{\leq T}'.
    \end{split}
\end{equation*}
Finally, we have
\[
\begin{aligned}
\lim_{s \to +\infty} \int_{\mathcal{Y}^T}
&\prod_{t=1}^T \mathcal{N}\bigl(y_t \mid [y_{\le T}']_t, (\sigma_s^*)^2\bigr)\,
p(y_{\le T}' \mid \mathbf{x}_{\le T}', \omega_{\le T}')\,dy_{\le T}' \\[1.8ex]
&= \int_{\mathcal{Y}^T}
    \prod_{t=1}^T \delta(y_t - y_t')\,
    p(y_{\le T}' \mid \mathbf{x}_{\le T}', \omega_{\le T}')\,dy_{\le T}' \\[1.8ex]
&= p(y_{\le T} \mid \mathbf{x}_{\le T}, \omega_{\le T}).
\end{aligned}
\]
\textbf{Part 2}: Proof of $\lim_{s \to + \infty}  \Delta(\mathcal{D}_T; \theta_{s}, \phi_{s}) = 0$. \\
First, we give an explicit writing of the modified individual gap: 
\begin{equation*}
    \begin{split}
        \Delta(\mathcal{D}_T; \theta_{s}, \phi_{s}) &= L(\mathcal{D}_T; \theta_{s}, \phi_{s}) - \mathrm{ELBO_0}(\mathcal{D}_T; \theta_{s}, \phi_{s}) +  \mathrm{ELBO_0}(\mathcal{D}_T; \theta_{s}, \phi_{s}) - \mathrm{ELBO}(\mathcal{D}_T; \theta_{s}, \phi_{s}) \\
        &= \Delta_0(\mathcal{D}_T; \theta_{s}, \phi_{s}) +  \mathrm{ELBO_0}(\mathcal{D}_T; \theta_{s}, \phi_{s}) - \mathrm{ELBO}(\mathcal{D}_T; \theta_{s}, \phi_{s}) \\
        &\quad - \left[\sum_{t = 1}^{T}\alpha(\mathbf{h}_t, \omega_t)\right] \mathbb{E}_{\mathbf{Z} \sim q_{\phi_s}(\cdot \mid \mathcal{D}_T)} D_{KL}(q_{\phi_s}(c \mid \mathcal{D}_T) \parallel p(c \mid \mathbf{Z})) \\
        &\quad - \left[\sum_{t = 1}^{T}\alpha_s(\mathbf{h}_t, \omega_t)\right]\log Z(q_{\phi_s}(\cdot \mid \mathcal{D}_T)) \\
        &= \sum_{t = 1}^{T} \alpha(\mathbf{h}_t, \omega_t) D_{KL}(q_{\phi_s}(\mathbf{z}, c \mid \mathcal{D}_T) \parallel p_{\theta_s}(\mathbf{z}, c \mid \mathcal{D}_t)).
    \end{split}
\end{equation*}

The last equality holds because we assume $q_{\phi_s}(c \mid \mathcal{D}_T) = \pi_{\phi_s}(c \mid \mathcal{D}_T)$ and $\pi_{\phi_s}(c \mid \mathcal{D}_T)$ is a minimizer of 
\[
\min_{q_{\phi_s}(c \mid \mathcal{D}_T)} \mathbb{E}_{\mathbf{Z} \sim q_{\phi_s}(\cdot \mid \mathcal{D}_T)} D_{KL}(q_{\phi_s}(c \mid \mathcal{D}_T) \parallel p(c \mid \mathbf{Z})) = -\log Z(q_{\phi_s}(\cdot \mid \mathcal{D}_T)).
\]

To show that $\lim_{s \to + \infty}  \Delta(\mathcal{D}_T; \theta_{s}, \phi_{s}) = 0$, we will define $\phi_{s}$ such that for every $c \in \{1, \dots, K\}$ and \(t \in \{1, \dots, T\}\):
\[
\lim_{s \to + \infty} D_{KL}(q_{\phi_{s}}(\mathbf{z}, c \mid \mathcal{D}_T) \parallel p_{\theta_s}(\mathbf{z}, c \mid \mathcal{D}_t)) = 0.
\]

Let us define $q_{\phi_{s}}( \mathbf{z} \mid \mathcal{D}_T)$ such that 
\[
f_{\mu_{\mathbf{z}}}(\mathcal{D}_T, \phi_{s}) = G^{-1}(F(y_1, \dots, y_{d_{\mathbf{z}}}] \mid \mathbf{x}_{\leq T}, \omega_{\leq T}))
\]
and 
\[
f_{S_{\mathbf{z}}}(\mathcal{D}_T, \phi) = \sigma_{s} \sqrt{\tilde{\Sigma}_{\mathbf{z}}(\mathcal{D}_T, \phi)},
\]
with $\tilde{\Sigma}_{\mathbf{z}}(\mathcal{D}_T, \phi)$ being the inverse of:
\[
\mathrm{Jac}(F^{-1}(. \mid \mathbf{x}_{\leq T}, \omega_{\leq T}) \circ \tilde{G}(\mathbf{z}))\mathrm{Jac}(F^{-1}(. \mid \mathbf{x}_{\leq T}, \omega_{\leq T}) \circ \tilde{G}(\mathbf{z}))^{\top}.
\]

Using Bayes’ rule, the true posterior can be written as
\[
p_{\theta_s}\bigl(\mathbf{z}, c \mid \mathcal{D}_t\bigr)
= \frac{
    p_{\theta_s}\bigl(y_{\le T}, \mathbf{z}, c \mid \mathbf{x}_{\le t}, \omega_{\le t}\bigr)
}{
    p_{\theta_s}\bigl(y_{\le t} \mid \mathbf{x}_{\le t}, \omega_{\le t}\bigr)
}.
\]
Expanding the numerator, we obtain
\[
\begin{aligned}
p_{\theta_s}\bigl(\mathbf{z}, c \mid \mathcal{D}_t\bigr)
&= \frac{
    \displaystyle\prod_{l=1}^t \mathcal{N}\bigl(
        y_l \mid
        [F^{-1}(\widetilde{G}(\mathbf{z}) \mid \mathbf{x}_{\le T}, \omega_{\le T})]_l,
        \sigma_s^2
    \bigr)\, p(\mathbf{z}\mid c)\,p(c)
}{
    p_{\theta_s}\bigl(y_{\le t} \mid \mathbf{x}_{\le t}, \omega_{\le t}\bigr)
}.
\end{aligned}
\]

By the GMM assumption over the prior, we have
\[
p(\mathbf{z} \mid c) = \mathcal{N}(\mathbf{z} \mid \mu_c, \Sigma_c).
\]

The approximate posterior is of the form
\[
\begin{aligned}
q_{\phi_s}\bigl(\mathbf{z}, c \mid \mathcal{D}_T\bigr)
&= q_{\phi_s}\bigl(\mathbf{z} \mid \mathcal{D}_T\bigr)\,\pi_{\phi_s}\bigl(c \mid \mathcal{D}_T\bigr) \\[1.2ex]
&= \mathcal{N}\bigl(
    \mathbf{z} \mid
    f_{\mu_{\mathbf{z}}}(\mathcal{D}_T, \phi_s),
    \sigma_s^2\,\widetilde{\Sigma}_{\mathbf{z}}(\mathcal{D}_T, \phi)
\bigr)\,\pi_{\phi_s}\bigl(c \mid \mathcal{D}_T\bigr).
\end{aligned}
\]
We now show convergence by performing a change of variables. Define $\mathbf{z}^{\prime} = \sigma_{s}^{-\frac{t}{d_z}}(\mathbf{z} - \mathbf{z}^*)$. We analyze the behavior of the distributions $p_{\theta_{s}}^{\prime}(\mathbf{z}^{\prime}, c \mid \mathcal{D}_t)$ and $q_{\phi_{s}}^{\prime}(\mathbf{z}^{\prime}, c \mid \mathcal{D}_T)$. 

We prove that
\[
\frac{p_{\theta_{s}}^{\prime}(\mathbf{z}^{\prime}, c \mid \mathcal{D}_t)}{q_{\phi_{s}}^{\prime}(\mathbf{z}^{\prime}, c \mid \mathcal{D}_T)}
\]
converges to a constant independent of $\mathbf{z}^{\prime}$ as $s \to \infty$. Since both $q_{\phi_s}^{\prime}(\mathbf{z}^{\prime}, c \mid \mathcal{D}_T)$ and $p_{\theta_s}^{\prime}(\mathbf{z}^{\prime}, c \mid \mathcal{D}_t)$ are probability distributions, the constant must be 1. Therefore, the KL divergence between them converges to 0 as $s \to \infty$.

We have
\[
\begin{aligned}
\frac{
p_{\theta_s}'(\mathbf{z}', c \mid \mathcal{D}_t)
}{
q_{\phi_s}'(\mathbf{z}', c \mid \mathcal{D}_T)
}
&= \frac{
    \mathcal{N}\bigl(
        \mathbf{z}^* + \sigma_s^{t/d_z}\mathbf{z}'
        \,\big|\,
        \mathbf{z}^*,\, \sigma_s^2\,\widetilde{\Sigma}_{\mathbf{z}}(\mathcal{D}_T, \phi)
    \bigr)\,
    \pi_{\phi_s}(c \mid \mathcal{D}_T)\,
    p_{\theta_s}\bigl(y_{\le t} \mid \mathbf{x}_{\le t}, \omega_{\le T}\bigr)
}{
    \displaystyle\prod_{l=1}^t
    \mathcal{N}\bigl(
        y_l \mid f_l(\mathbf{h}_l, \omega_l, \mathbf{z}^* + \sigma_s^{t/d_z}\mathbf{z}'; \theta_s),\, \sigma_s^2
    \bigr) \,
    \mathcal{N}\bigl(
        \mathbf{z}^* + \sigma_s^{t/d_z}\mathbf{z}' \mid \mu_c, \Sigma_c
    \bigr)\,p(c)
}.
\end{aligned}
\]

Now let \(A_t\) be a matrix whose Moore–Penrose inverse \(A^+\) satisfies
\[
\begin{aligned}
f_{\le t}(\mathbf{h}_{\le t}, \omega_{\le t}, \mathbf{z}^* + \sigma_s^{t/d_z}\mathbf{z}'; \theta_s)
&= A^+ f_{\le T}(\mathbf{h}_{\le T}, \omega_{\le T}, \mathbf{z}^* + \sigma_s^{t/d_z}\mathbf{z}'; \theta_s), \\[1.2ex]
y_{\le t} &= A^+ y_{\le T}.
\end{aligned}
\]
That is, projecting onto \(A^+\) selects the first \(t\) responses. The matrices \(A^+\) and \(A\) have the forms
\[
A^+ =
\begin{bmatrix}
I_t & 0_{t \times (T - t)}
\end{bmatrix}, \quad
A =
\begin{bmatrix}
I_t \\[0.8ex]
0_{(T - t) \times t}
\end{bmatrix}.
\]
By noticing that \([A^{\intercal}(\sigma_s^2I_T)^{-1}A]^{-1} = \sigma_s^2I_t\) We can therefore apply the mean rearranging formula \citep{Petersen2008MatCookbook}: 
\begin{align*}
&\mathcal{N}\left(
    A^+y_{\leq T} \,\middle|\, 
    A^+f_{\leq T}(\mathbf{h}_{\leq t}, \omega_{\leq t}, \mathbf{z}^* + \sigma_{s}^{\frac{t}{d_z}} \mathbf{z}^{\prime}; \theta_{s}), 
    \left[A^{\intercal}(\sigma_s^2 I_T) A\right]^{-1}
\right) \\
&\quad = 
\frac{
    \sqrt{\det(2\pi \sigma_s^2 I_T)}
}{
    \sqrt{\det(2\pi \sigma_s^2 I_t)}
}
\mathcal{N}\left(
    y_{\leq T} \,\middle|\, 
    f_{\leq T}(\mathbf{h}_{\leq T}, \omega_{\leq T}, \mathbf{z}^* + \sigma_{s}^{\frac{t}{d_z}} \mathbf{z}^{\prime}; \theta_{s}), 
    \sigma_s^2 I_T
\right)
\end{align*}
\begin{align*}
\frac{
p_{\theta_s}'\bigl(\mathbf{z}', c \mid \mathcal{D}_t\bigr)
}{
q_{\phi_s}'\bigl(\mathbf{z}', c \mid \mathcal{D}_T\bigr)
}
&= \frac{
    \mathcal{N}\bigl(
        \mathbf{z}^* + \sigma_s^{t/d_z}\mathbf{z}'
        \mid \mathbf{z}^*,\, \sigma_s^2\,\widetilde{\Sigma}_{\mathbf{z}}(\mathcal{D}_T, \phi)
    \bigr)\,
    \pi_{\phi_s}\bigl(c \mid \mathcal{D}_T\bigr)\,
    p_{\theta_s}\bigl(y_{\le t} \mid \mathbf{x}_{\le t}, \omega_{\le T}\bigr)
}{
    \displaystyle
    \frac{\sqrt{\det(2\pi\sigma_s^2I_T)}}{\sqrt{\det(2\pi\sigma_s^2I_t)}}
    \mathcal{N}\bigl(
        y_{\le T} \mid
        f_{\le T}(\mathbf{h}_{\le T}, \omega_{\le T}, \mathbf{z}^* + \sigma_s^{t/d_z}\mathbf{z}'; \theta_s),
        \sigma_s^2I_T
    \bigr)\,
    \mathcal{N}\bigl(
        \mathbf{z}^* + \sigma_s^{t/d_z}\mathbf{z}' \mid \mu_c, \Sigma_c
    \bigr)\,p(c)
} \\[2.0ex]
&= (2\pi)^{\tfrac{t-d}{2}}\,
\frac{
    \det\bigl(\widetilde{\Sigma}_{\mathbf{z}}\bigr)^{-1/2}
}{
    \det(\Sigma_c)^{-1/2}
}
\exp\Bigg\{
    -\tfrac{1}{2}\sigma_s^{2(t/d_z - 1)}{\mathbf{z}'}^\top\widetilde{\Sigma}_{\mathbf{z}}^{-1}\mathbf{z}' \\[1.4ex]
&\qquad
    + \tfrac{1}{2\sigma_s^2}\sum_{l=1}^T
    \bigl(y_l - f_l(\mathbf{h}_l, \omega_l, \mathbf{z}^* + \sigma_s^{t/d_z}\mathbf{z}'; \theta_s)\bigr)^2 \\[1.4ex]
&\qquad
    + \tfrac{1}{2}\bigl(\mathbf{z}^* + \sigma_s^{t/d_z}\mathbf{z}' - \mu_c\bigr)^\top
    \Sigma_c^{-1}\bigl(\mathbf{z}^* + \sigma_s^{t/d_z}\mathbf{z}' - \mu_c\bigr)
\Bigg\} \\[1.8ex]
&\quad \times \frac{
    \pi_{\phi_s}\bigl(c \mid \mathcal{D}_T\bigr)\,
    p_{\theta_s}\bigl(y_{\le T} \mid \mathbf{x}_{\le t}, \omega_{\le t}\bigr)
}{
    p(c)
}.
\end{align*}
By noticing that
\[
\sum_{l=1}^{T}\bigl(y_l - f_l(\mathbf{h}_l, \omega_l, \mathbf{z}^* + \sigma_s^{t/d_z}\mathbf{z}'; \theta_s)\bigr)^2
= \bigl\| y_{\le T} - F^{-1}\bigl(\widetilde{G}(\mathbf{z}^* + \sigma_s^{t/d_z}\mathbf{z}') \mid \mathbf{x}_{\le T}, \omega_{\le T}\bigr)\bigr\|_2^2.
\]

We apply a first-order Taylor expansion:
\[
y_{\le T} - F^{-1}\bigl(\widetilde{G}(\mathbf{z}^* + \sigma_s^{t/d_z}\mathbf{z}') \mid \mathbf{x}_{\le T}, \omega_{\le T}\bigr)
\underset{s \to \infty}{\approx}
-Jac\bigl(F^{-1}\widetilde{G}\bigr)(\mathbf{z}^*)\bigl(\sigma_s^{t/d_z}\mathbf{z}'\bigr),
\]
which implies by norm continuity
\[
\begin{aligned}
\sum_{l=1}^T\bigl(y_l - f_l(\mathbf{h}_l, \omega_l, \mathbf{z}^* + \sigma_s^{t/d_z}\mathbf{z}'; \theta_s)\bigr)^2
&\underset{s \to \infty}{\approx}
\bigl\|Jac(F^{-1}\widetilde{G})(\mathbf{z}^*)\bigl(\sigma_s^{t/d_z}\mathbf{z}'\bigr)\bigr\|_2^2 \\[1.2ex]
&\underset{s \to \infty}{=}
\sigma_s^{2t/d_z}\,\mathbf{z}'^\top\widetilde{\Sigma}_{\mathbf{z}}^{-1}\mathbf{z}'.
\end{aligned}
\]

Define the constant \(\mathcal{C}\mathrm{st}(\mathcal{D}_t; \sigma_s, \theta_s, \phi_s)\) w.r.t. \(\mathbf{z}'\) as
\[
\mathcal{C}\mathrm{st}(\mathcal{D}_t; \sigma_s, \theta_s, \phi_s)
= (2\pi)^{(t-d_z)/2}
\sqrt{\frac{\det(\Sigma_c)}{\det(\widetilde{\Sigma}_{\mathbf{z}})}}
\frac{\pi_{\phi_s}(c \mid \mathcal{D}_T)\,p_{\theta_s}\bigl(y_{\le t} \mid \mathbf{x}_{\le t}, \omega_{\le t}\bigr)}{p(c)}.
\]

Thus,
\[
\begin{aligned}
\frac{p_{\theta_s}'(\mathbf{z}', c \mid \mathcal{D}_T)}{q_{\phi_s}'(\mathbf{z}', c \mid \mathcal{D}_T)}
&\underset{s \to \infty}{\approx}
\tfrac{1}{2}(\mathbf{z}^* - \mu_c)^\top\Sigma_c^{-1}(\mathbf{z}^* - \mu_c)\,\mathcal{C}\mathrm{st}(\mathcal{D}_t; \sigma_s, \theta_s, \phi_s) \\[1.4ex]
&\quad\times
\exp\Bigg\{
    -\tfrac{1}{2}\sigma_s^{2(t/d_z - 1)}\mathbf{z}'^\top\widetilde{\Sigma}_{\mathbf{z}}^{-1}\mathbf{z}'
    + \tfrac{1}{2}\sigma_s^{2(t/d_z - 1)}\mathbf{z}'^\top\mathbf{z}'
\Bigg\}.
\end{aligned}
\]

Finally,
\[
\frac{p_{\theta_s}'(\mathbf{z}', c \mid \mathcal{D}_T)}{q_{\phi_s}'(\mathbf{z}', c \mid \mathcal{D}_T)}
\underset{s \to \infty}{\approx}
\tfrac{1}{2}(\mathbf{z}^* - \mu_c)^\top\Sigma_c^{-1}(\mathbf{z}^* - \mu_c)\,\mathcal{C}\mathrm{st}(\mathcal{D}_t; \sigma_s, \theta_s, \phi_s).
\]

To conclude the proof, we still need to show that 
\(\lim_{s \to +\infty} \mathcal{C}\mathrm{st}(\mathcal{D}_t; \sigma_s, \theta_s, \phi_s)\) exists and is finite because the model parameters still depend on the chosen variance.  This was the main misapprehension of \cite{dai2018diagnosingvae} for a VAE in the static setting with an unimodal prior over the continuous latents \(\mathbf{Z}\).

We have already shown that 
\[
\lim_{\sigma \to 0^+} p_{\theta_{\sigma}}(y_{\leq T} \mid \mathbf{x}_{\leq T}, \omega_{\leq T}) = p(y_{\leq T} \mid \mathbf{x}_{\leq T}, \omega_{\leq T}),
\]
and therefore:
\[
\begin{aligned}
\lim_{s \to +\infty}\mathcal{C}\mathrm{st}(\mathcal{D}_t; \sigma_s, \theta_s, \phi_s)
&=
(2\pi)^{(t - d_z)/2}
\sqrt{\frac{\det(\Sigma_c)}{\det(\widetilde{\Sigma}_{\mathbf{z}})}} \\[1.2ex]
&\quad\times
\frac{p(y_{\le T} \mid \mathbf{x}_{\le T}, \omega_{\le T})}{p(c)}
\cdot
\lim_{s \to +\infty}\pi_{\phi_s}(c \mid \mathcal{D}_T).
\end{aligned}
\]

We verify that \(\lim_{s \to +\infty} \pi_{\phi_{s}}(c \mid \mathcal{D}_T)\) exists and is finite and not zero for all \(c \in \{1, \dots, K\}\):
\begin{align*}
\pi_{\phi_{s}}(c \mid \mathcal{D}_T)
&= \frac{\exp(\mathbb{E}_{\mathbf{Z} \sim q_{\phi_z}(\cdot \mid \mathcal{D}_T)} \log p(c \mid \mathbf{Z}))
    }{
    \sum_{c=1}^K \exp(\mathbb{E}_{\mathbf{Z} \sim q_{\phi_z}(\cdot \mid \mathcal{D}_T)} \log p(c \mid \mathbf{Z}))} \\
&= \frac{
                \exp(
                \int_{\mathcal{Z}} \log p(c\mid\mathbf{z}) \mathcal{N}\left(
        \mathbf{z} \mid \mathbf{z}^*,         
         \sigma_{s}^{2}  \tilde{\Sigma}_{\mathbf{z}}(\mathcal{D}_T, \phi) 
        \right)  d\mathbf{z}
                )
                }{
                \sum_{c=1}^K \exp(
                \int_{\mathcal{Z}} \log p(c\mid\mathbf{z}) \mathcal{N}\left(
        \mathbf{z} \mid \mathbf{z}^*,         
         \sigma_{s}^{2}  \tilde{\Sigma}_{\mathbf{z}}(\mathcal{D}_T, \phi) 
        \right)  d\mathbf{z}
                )
                } \\
&\underset{s \to \infty}{\to} \frac{
                \exp(
                \int_{\mathcal{Z}} \log p(c\mid\mathbf{z}) \delta(\mathbf{z} - \mathbf{z}^*)  d\mathbf{z}
                )
                }{
                \sum_{c=1}^K \exp(
                \int_{\mathcal{Z}} \log p(c\mid\mathbf{z})  \delta(\mathbf{z} - \mathbf{z}^*)  d\mathbf{z}
                )
                } \\
&= \frac{
                 p(c\mid\mathbf{z}^*)
                }{
                \sum_{c=1}^K  p(c\mid\mathbf{z}^*)
                } 
\end{align*}
We have therefore proved that the ratio \(\frac{p_{\theta_{s}}^{\prime}\left(\mathbf{z}^{\prime}, c \mid \mathcal{D}_T\right)}{q_{\phi_{s}}^{\prime}(\mathbf{z}^{\prime}, c \mid \mathcal{D}_T)} \)  converges into a nonzero constant which finishes the proof of the theorem.
\end{proof}



\paragraph{Proof of theorem \ref{thm:sigma_to_0}.} We start by considering the ELBO:
\begin{equation*}
\begin{split}
    \mathcal{L}(\mathcal{D}_T; \theta, \phi) 
    &=  -\sum_{t = 1}^{T} \mathbb{E}_{\mathbf{Z} \sim q_{\phi}(\cdot \mid \mathcal{D}_T)} 
    \left[ \alpha(\mathbf{h}_t, \omega_t) \log p_{\theta}(y_{t} \mid \mathbf{H}_t, W_t, \mathbf{Z}) \right] \\
    &\quad + \left[\sum_{t = 1}^{T}\alpha(\mathbf{h}_t, \omega_t)\right] D_{KL}\left(q_{\phi}(\mathbf{z} \mid \mathcal{D}_T) \parallel p(\mathbf{z})\right) \\
    &\quad - \left[\sum_{t = 1}^{T}\alpha(\mathbf{h}_t, \omega_t)\right] \log Z(q_{\phi}(\cdot \mid \mathcal{D}_T)).
\end{split}
\end{equation*}

By the positivity of the KL divergence and using the fact that $-\log Z(q_{\phi}(\cdot \mid \mathcal{D}_T))$ minimizes a positive functional (as explained in Eq.~\eqref{eq:min_VaDE_trick}), we obtain:
\begin{equation*}
\begin{split}
    \mathcal{L}(\mathcal{D}_T; \theta_{\sigma}^*, \phi_{\sigma}^*) 
    &\geq  -\sum_{t = 1}^{T} \mathbb{E}_{\mathbf{Z} \sim q_{\phi}(\cdot \mid \mathcal{D}_T)} 
    \left[ 
        \alpha(\mathbf{h}_t, \omega_t) \log \left( p_{\theta}\left( y_{t} \mid \mathbf{H}_t, W_t, \mathbf{Z} \right) \right) 
    \right] \\
    &= \sum_{t = 1}^{T} \alpha(\mathbf{h}_t, \omega_t) \mathbb{E}_{\mathbf{Z} \sim q_{\phi}(\cdot \mid \mathcal{D}_T)} 
    \left[
        \frac{1}{2} \log\left( 2 \pi \sigma^2 \right) + \frac{1}{2\sigma^2} \left( y_t - f\left( \mathbf{H}_t, \mathbf{Z}, W_t \right) \right)^2
    \right] \\
    &= \frac{1}{2\sigma^2} 
    \left[
        \left( \sum_{t = 1}^{T} \alpha(\mathbf{h}_t, \omega_t) \right) \sigma^2 \log\left( 2 \pi \sigma^2 \right) 
        + \sum_{t = 1}^{T} \alpha(\mathbf{h}_t, \omega_t) \underbrace{\mathbb{E}_{\mathbf{Z} \sim q_{\phi}(\cdot \mid \mathcal{D}_T)} 
        \left( y_t - f\left( \mathbf{H}_t, \mathbf{Z}, W_t \right) \right)^2}_{\delta_{\sigma}(t)}  
    \right].
\end{split}
\end{equation*}

Suppose there exists $t_0 \in \{1,2,\ldots, T\}$ such that $\lim_{\sigma \to 0^+} \delta_{\sigma}(t_0) > 0$. Then we have $\lim_{\sigma \to 0^+} \mathcal{L}(\mathcal{D}_T; \theta_{\sigma}^*, \phi_{\sigma}^*) = +\infty$, which is impossible since we assume $\mathcal{L}(\mathcal{D}_T; \theta_{\sigma}^*, \phi_{\sigma}^*)$ to be minimized. Therefore, we conclude that for all $t \in \{1,2,\ldots, T\}$, $\lim_{\sigma \to 0^+} \delta_{\sigma}(t) = 0$.

Consequently, we have
\begin{equation*}
\lim_{\sigma \to 0^+} \mathbb{E}_{\mathbf{\epsilon} \sim \mathcal{N}(0,I)} 
        \left( y_t - f\left( \mathbf{H}_t, W_t, f_{\mu_{\mathbf{z}}}(\mathcal{D}_T; \phi_{\sigma}^*)+ f_{S_{\mathbf{z}}}(\mathcal{D}_T; \theta_{\sigma}^*)\mathbf{\epsilon} \right) \right)^2 = 0,
\end{equation*}
which implies that 
\[
\lim_{\sigma \to 0^+} f\left( \mathbf{H}_t, W_t, f_{\mu_{\mathbf{z}}}(\mathcal{D}_T; \phi_{\sigma}^*) + f_{S_{\mathbf{z}}}(\mathcal{D}_T; \theta_{\sigma}^*)\mathbf{\epsilon} \right) = y_t, \quad \text{almost surely}.
\]
In particular, we also have
\[
\lim_{\sigma \to 0^+} f\left( \mathbf{H}_t, W_t, f_{\mu_{\mathbf{z}}}(\mathcal{D}_T; \phi_{\sigma}^*) \right) = y_t.
\]

\subsection{Upper bound on weighted PEHE}
\label{appendix:up_bound_wpehe}
\begin{proof}[\textbf{theorem} \ref{thm:pehe_wbound}]
To prove the theorem, we rely on the following key lemma, but first, we need to define further mathematical objects. We define the weighted population risk over the whole population as
\[
R_{t, g}(f, \Phi) \coloneqq \mathbb{E}_{\mathbf{H}_t, W_t} \left[ \alpha(\mathbf{H}_t, W_t) \, \ell_{f, \Phi}(\mathbf{H}_t, W_t)  \right],
\]
and the weighted population counterfactual risk as 
\[
R_{t, g}(f, \Phi)_{CF} \coloneqq \mathbb{E}_{\mathbf{H}_t, 1-W_t} \left[ \alpha(\mathbf{H}_t, 1-W_t) \, \ell_{f, \Phi}(\mathbf{H}_t, W_t)  \right].
\]
\begin{lemma}
\label{lemma:Upbound_cfrisk_byFactual} $R_{t, g}(f, \Phi) + R_{t, g}(f, \Phi)_{CF} \leq R_{t, g}^1(f, \Phi) + R_{t, g}^0(f, \Phi) +  B_{\Phi} \, \mathrm{IPM}_{G} \left( g_{\Phi}(\cdot \mid W_t = 1), \, g_{\Phi}(\cdot \mid W_t = 0) \right)$
\end{lemma}
The proof immediately follows from Lemma 1 in \cite{shalit2017estimating}.

Next, to complete the proof, we define the expected potential outcome at time $t$, given the context history $\mathbf{H}_{t} = \mathbf{h}_{t}$ and latent $\mathbf{z}$ as
\[
m_{t}^{\omega}(\mathbf{h}_{t}, \mathbf{z}) \coloneqq \mathbb{E}_{Y_{t}(\omega) \mid \mathbf{H}_{t},\mathbf{Z} }(Y_{t}(\omega) \mid \mathbf{H}_{t} = \mathbf{h}_{t}, \mathbf{Z} =  \mathbf{z}) \quad \omega \in \mathcal{W},
\]
and we show the following lemma:
\begin{lemma}
\label{lemma:mean_estim_err_decomp}
Denote \(\hat{p}_{\phi}(\mathbf{h}_t, w, \mathbf{z}) \coloneqq p(\mathbf{h}_t, w)\, q_{\phi}(\mathbf{z} \mid \mathcal{D}_{\leq t-1})\). We can decompose \(R_{t,g}(f,\Phi)\) and \(R_{t,g}(f,\Phi)_{\mathrm{CF}}\) under our distributional assumptions as:
\[
\begin{aligned}
&\mathbb{E}_{\hat{p}_{\phi}(\mathbf{h}_t, w, \mathbf{z})} 
\bigl[ \alpha(\mathbf{h}_t, w)\,\big(f(\mathbf{h}_t, w, \mathbf{z}) - m_{t}^{w}(\mathbf{h}_t, \mathbf{z})\big) \bigr] \\[1.2ex]
&\quad= 2\sigma^2 \left( R_{t,g}(f,\Phi) - \tfrac{1}{2}\log(2\pi\sigma^2) \right)
- \sum_{\omega \in \{0,1\}}\mathrm{Var}_{\hat{p}_{\phi}}(Y_t),
\end{aligned}
\]
and
\[
\begin{aligned}
&\mathbb{E}_{\hat{p}_{\phi}(\mathbf{h}_t, w, \mathbf{z})}
\bigl[ \alpha(\mathbf{h}_t, 1-w)\,\big(f(\mathbf{h}_t, 1-w, \mathbf{z}) - m_{t}^{1-w}(\mathbf{h}_t, \mathbf{z})\big) \bigr] \\[1.2ex]
&\quad= 2\sigma^2 \left( R_{t,g}(f,\Phi)_{\mathrm{CF}} - \tfrac{1}{2}\log(2\pi\sigma^2) \right)
- \sum_{\omega \in \{0,1\}}\mathrm{Var}_{\hat{p}_{\phi}}(Y_t\mid 1-w).
\end{aligned}
\]
\end{lemma}
\begin{proof}
We have: 
\begin{small}
\begin{align*}
R_{t,g}(f,\Phi)
&= \mathbb{E}_{\mathbf{H}_t,W_t} \!\left[ \alpha(\mathbf{H}_t,W_t)\,\ell_{f,\Phi}(\mathbf{H}_t,W_t) \right] \\[1.2ex]
&= \sum_{\omega\in\{0,1\}} \int_{\mathcal{H}_t}\!\!\int_{\mathcal{Z}}\!\!\int_{\mathcal{Y}} 
-\alpha(\mathbf{h}_t,\omega)\log p_\theta(y_t\mid\mathbf{h}_t,\omega,\mathbf{z})\\[-0.5ex]
&\hspace{4em}\times p(y_t\mid\mathbf{h}_t,\omega,\mathbf{z})\,p(\mathbf{h}_t,\omega)\,q_\phi(\mathbf{z}\mid\mathcal{D}_{\le t-1})
\,dy_t\,d\mathbf{z}\,d\mathbf{h}_t \\[1.5ex]
&= \sum_{\omega\in\{0,1\}} \int_{\mathcal{H}_t}\!\!\int_{\mathcal{Z}}\!\!\int_{\mathcal{Y}} 
\alpha(\mathbf{h}_t,\omega)\Bigg\{ 
\tfrac{1}{2}\log(2\pi\sigma^2) + \frac{(y_t-f(\mathbf{h}_t,\omega,\mathbf{z}))^2}{2\sigma^2} 
\Bigg\}\\[-0.5ex]
&\hspace{4em}\times p(y_t\mid\mathbf{h}_t,\omega,\mathbf{z})\,p(\mathbf{h}_t,\omega)\,q_\phi(\mathbf{z}\mid\mathcal{D}_{\le t-1})
\,dy_t\,d\mathbf{z}\,d\mathbf{h}_t \\[1.5ex]
&= \tfrac{1}{2}\log(2\pi\sigma^2)
+ \frac{1}{2\sigma^2} \sum_{\omega\in\{0,1\}} 
\mathrm{Var}_{\hat{p}_\phi(\mathbf{h}_t,\omega,\mathbf{z})}(Y_t)\\[-0.5ex]
&\quad+\int_{\mathcal{H}_t}\!\!\int_{\mathcal{Z}} 
\alpha(\mathbf{h}_t,\omega)\left( f(\mathbf{h}_t,\omega,\mathbf{z}) - m_t^\omega(\mathbf{h}_t,\mathbf{z}) \right)^2\\[-0.5ex]
&\hspace{4em}\times p(\mathbf{h}_t,\omega)\,q_\phi(\mathbf{z}\mid\mathcal{D}_{\le t-1})
\,d\mathbf{z}\,d\mathbf{h}_t.
\end{align*}
\end{small}
 
In a similar way, we can show the decomposition related to $R_{t, g}(f, \Phi) _{CF}$.
\end{proof}
The remainder idea of the proof is to decompose the PEHE in such a way we can upper bound it with an expression including $R_{t, g}(f, \Phi)$ and $R_{t, g}(f, \Phi)_{CF}$ and then use lemma \ref{lemma:Upbound_cfrisk_byFactual}. We actually have:
\begin{small}
\begin{align*}
\epsilon_{\mathrm{PEHE}_{t, g}} 
&= \mathbb{E}_{\mathbf{H}_t \sim g}\,\mathbb{E}_{\mathbf{Z} \sim q_\phi(\mathbf{Z}\mid\mathcal{D}_{\le t-1})} 
\bigl[\bigl(\tau(\mathbf{H}_t,\mathbf{Z}) - \hat{\tau}_{f,\Phi}(\mathbf{H}_t,\mathbf{Z})\bigr)^2\bigr] \\[1.2ex]
&= \mathbb{E}_{\mathbf{H}_t \sim g}\,\mathbb{E}_{\mathbf{Z} \sim q_\phi(\mathbf{Z}\mid\mathcal{D}_{\le t-1})}
\bigl[ \bigl(m_t^1(\mathbf{h}_t,\mathbf{z}) - m_t^0(\mathbf{h}_t,\mathbf{z}) - f(\mathbf{h}_t,1,\mathbf{z}) + f(\mathbf{h}_t,0,\mathbf{z})\bigr)^2 \bigr] \\[1.5ex]
&\overset{(1)}{\le} 2\,\mathbb{E}_{\mathbf{H}_t \sim g}\,\mathbb{E}_{\mathbf{Z} \sim q_\phi(\mathbf{Z}\mid\mathcal{D}_{\le t-1})}
\bigl[ (f(\mathbf{h}_t,1,\mathbf{z}) - m_t^1(\mathbf{h}_t,\mathbf{z}))^2 \bigr] \\[-0.5ex]
&\quad + 2\,\mathbb{E}_{\mathbf{H}_t \sim g}\,\mathbb{E}_{\mathbf{Z} \sim q_\phi(\mathbf{Z}\mid\mathcal{D}_{\le t-1})}
\bigl[ (f(\mathbf{h}_t,0,\mathbf{z}) - m_t^0(\mathbf{h}_t,\mathbf{z}))^2 \bigr] \\[1.5ex]
&= \mathbb{E}_{\mathbf{H}_t \mid W_t=1}\,\mathbb{E}_{\mathbf{Z}}\!\bigl[\alpha(\mathbf{h}_t,1)\,(f(\mathbf{h}_t,1,\mathbf{z})-m_t^1(\mathbf{h}_t,\mathbf{z}))^2\bigr] \\[-0.5ex]
&\quad + \mathbb{E}_{\mathbf{H}_t \mid W_t=0}\,\mathbb{E}_{\mathbf{Z}}\!\bigl[\alpha(\mathbf{h}_t,0)\,(f(\mathbf{h}_t,1,\mathbf{z})-m_t^1(\mathbf{h}_t,\mathbf{z}))^2\bigr] \\[-0.5ex]
&\quad + \mathbb{E}_{\mathbf{H}_t \mid W_t=0}\,\mathbb{E}_{\mathbf{Z}}\!\bigl[\alpha(\mathbf{h}_t,0)\,(f(\mathbf{h}_t,0,\mathbf{z})-m_t^0(\mathbf{h}_t,\mathbf{z}))^2\bigr] \\[-0.5ex]
&\quad + \mathbb{E}_{\mathbf{H}_t \mid W_t=1}\,\mathbb{E}_{\mathbf{Z}}\!\bigl[\alpha(\mathbf{h}_t,1)\,(f(\mathbf{h}_t,0,\mathbf{z})-m_t^0(\mathbf{h}_t,\mathbf{z}))^2\bigr] \\[1.5ex]
&= \mathbb{E}_{\mathbf{H}_t,W_t}\,\mathbb{E}_{\mathbf{Z}}
\bigl[\alpha(\mathbf{H}_t,W_t)\,(f(\mathbf{H}_t,W_t,\mathbf{Z})-m_t^{W_t}(\mathbf{H}_t,\mathbf{Z}))^2\bigr] \\[-0.5ex]
&\quad + \mathbb{E}_{\mathbf{H}_t,1-W_t}\,\mathbb{E}_{\mathbf{Z}}
\bigl[\alpha(\mathbf{H}_t,1-W_t)\,(f(\mathbf{H}_t,W_t,\mathbf{Z})-m_t^{W_t}(\mathbf{H}_t,\mathbf{Z}))^2\bigr] \\[1.5ex]
&\overset{(2)}{=} 2\sigma^2\bigl(R_{t,g}(f,\Phi)+R_{t,g}(f,\Phi)_{\mathrm{CF}}-\log(2\pi\sigma^2)\bigr)\\[-0.5ex]
&\quad - \sum_{\omega\in\{0,1\}}\!\bigl(\mathrm{Var}_{\hat{p}_\phi(\mathbf{h}_t,1-\omega,\mathbf{z})}(Y_t) + \mathrm{Var}_{\hat{p}_\phi(\mathbf{h}_t,\omega,\mathbf{z})}(Y_t)\bigr) \\[1.5ex]
&\overset{(3)}{\le} 2\sigma^2\bigl(R_{t,g}(f,\Phi)+R_{t,g}(f,\Phi)_{\mathrm{CF}}-\log(2\pi\sigma^2)\bigr) \\[1.5ex]
&\overset{(4)}{\le} 2\sigma^2\biggl(R_{t,g}^1(f,\Phi)+R_{t,g}^0(f,\Phi)
+B_\Phi\,\mathrm{IPM}_G\bigl(g_\Phi(\cdot|W_t=1),g_\Phi(\cdot|W_t=0)\bigr)
-\log(2\pi\sigma^2)\biggr).
\end{align*}
\end{small}

The inequality $\overset{(1)}{\leq }$ follows from the property $(a-b)^2 \leq 2a^2 + 2b^2$. The equation $\overset{(2)}{=}$ follows from plugging in the equations from Lemma \ref{lemma:mean_estim_err_decomp}, the inequality $\overset{(3)}{\leq}$ follows from the positivity of the variance terms, and $\overset{(4)}{\leq}$ follows from Lemma \ref{lemma:Upbound_cfrisk_byFactual}.
\end{proof}

\subsection{Proof of Proposition \ref{prop:approx_factual_risk}}
\label{appendix:proof_statio}
Using a Monte Carlo approximation, we can express the approximate factual risk as:
\[
R^{\omega}_{t, g}\left(f, \Phi \right) \approx \frac{1}{n_{\omega}^{(t)}} \sum_{i \in \mathcal{B}, W_{it} = \omega } \mathbb{E}_{\mathbf{Z} \sim q_{\phi}(\mathbf{Z} \mid \mathcal{D}_{i, \leq t-1})} \left[ 
 \alpha(\mathbf{h}_{it}, \omega) \log \mathcal{N}(y_{it}; f(\Phi(\mathbf{h}_{it}),\mathbf{Z}, \omega), \sigma^2) 
\right].
\]
By the stationarity assumption, for \( t \geq t_0 \), this approximation holds:
\[
R^{\omega}_{t, g}\left(f, \Phi \right) \approx \frac{1}{n_{\omega}^{(t)}} \sum_{i \in \mathcal{B}, W_{it} = \omega } \mathbb{E}_{\mathbf{Z} \sim q_{\phi}(\mathbf{Z} \mid \mathcal{D}_{iT})} \left[ 
 \alpha(\mathbf{h}_{it}, \omega) \log \mathcal{N}(y_{it}; f(\Phi(\mathbf{h}_{it}),\mathbf{Z}, \omega), \sigma^2) 
\right].
\]

On the other hand, the reconstruction term in the ELBO can be written as:
\begin{align*}
&\sum_{t = t_0}^{T} 
\mathbb{E}_{\mathbf{Z} \sim q_{\phi}(\cdot \mid \mathcal{D}_T)} 
\bigl[ \alpha(\mathbf{H}_t, W_t)\,\log p_{\theta}(Y_t \mid \mathbf{H}_t, W_t, \mathbf{Z}) \bigr] \\[1.2ex]
&\quad\approx \sum_{t = t_0}^{T} 
\frac{1}{|\mathcal{B}|} 
\sum_{i \in \mathcal{B}} 
\mathbb{E}_{\mathbf{Z} \sim q_{\phi}(\mathbf{Z} \mid \mathcal{D}_{iT})}
\biggl[
\alpha(\mathbf{h}_{it}, \omega)\,
\log\mathcal{N}\bigl(y_{it};\, f(\Phi(\mathbf{h}_{it}),\mathbf{Z},\omega),\, \sigma^2\bigr)
\biggr] \\[1.5ex]
&\quad\approx \frac{1}{|\mathcal{B}|} 
\sum_{t = t_0}^{T}
\sum_{\omega \in \mathcal{W}}
\sum_{i \in \mathcal{B},\, W_{it}=\omega} 
\mathbb{E}_{\mathbf{Z} \sim q_{\phi}(\mathbf{Z} \mid \mathcal{D}_{iT})}
\biggl[
\alpha(\mathbf{h}_{it}, \omega)\,
\log\mathcal{N}\bigl(y_{it};\, f(\Phi(\mathbf{h}_{it}),\mathbf{Z},\omega),\, \sigma^2\bigr)
\biggr] \\[1.5ex]
&\quad\approx \frac{1}{|\mathcal{B}|}
\sum_{t = t_0}^{T} 
\biggl\{-n_1^{(t)}\,R_t^1(f,\Phi)\;-\;n_0^{(t)}\,R_t^0(f,\Phi)\biggr\}.
\end{align*}

\section{Experiments on synthetic data: Details} 

\subsection{Additional results}
\label{appendix_cdvae:arsim_extended_results}
\paragraph{Results of baselines on the synthetic datasets} The following Table \ref{tab:perf_sim_combined} provides the detailed results responsible for Figures \ref{fig:perf_sim_combined} related to baselines with the three different approaches across levels of \(\gamma_{(1)}^{YU}\).
\begin{table}[!htbp]
 \caption{Results on the synthetic data reported by PEHE. Smaller is better.}
 \centering
\resizebox{\textwidth}{!}{%
\begin{tabular}{|c|c|c|c|c|c|c|c|c|c|c|c|} 
\hline
Model       & $\gamma_{(1)}^{YU} = 0$ & $\gamma_{(1)}^{YU} = 0.25$ & $\gamma_{(1)}^{YU} = 0.5$ & $\gamma_{(1)}^{YU} = 0.75$ & $\gamma_{(1)}^{YU} = 1$ & $\gamma_{(1)}^{YU} = 1.25$ & $\gamma_{(1)}^{YU} = 1.5$ & $\gamma_{(1)}^{YU} = 1.75$ & $\gamma_{(1)}^{YU} = 2$ & $\gamma_{(1)}^{YU} = 2.25$ & $\gamma_{(1)}^{YU} = 2.5$ \\ \hline 

\textbf{CDVAE (ours)} & \textbf{0.43$\pm$0.02}& \textbf{0.50$\pm$0.03}& \textbf{0.96$\pm$0.09}& \textbf{1.57$\pm$0.08}& \textbf{1.90$\pm$0.10}&  \textbf{2.35$\pm$0.18}& \textbf{3.57$\pm$0.17}& \textbf{4.80$\pm$0.20}& \textbf{6.84$\pm$0.20}& \textbf{7.64$\pm$0.48}& \textbf{9.03$\pm$0.50}\\
\hline


\textbf{Causal CPC} & 0.43$\pm$0.01 & 0.50$\pm$0.03 & 1.08$\pm$0.08 & 2.49$\pm$0.14 & 2.98$\pm$0.09 & 4.98$\pm$0.21 & 5.91$\pm$0.29 & 10.15$\pm$0.38 & 12.25$\pm$0.49 & 15.65$\pm$0.56 & 19.39$\pm$0.59 \\

\textbf{Causal CPC (with substitute)} & 0.46$\pm$0.02 & 0.49$\pm$0.01 & 1.02$\pm$0.05 & 2.38$\pm$0.08 & 2.83$\pm$0.09 & 4.81$\pm$0.13 & 5.38$\pm$0.22 & 8.13$\pm$0.39 & 10.11$\pm$0.41 & 12.01$\pm$0.54 & 14.03$\pm$0.64 \\

\textbf{Causal CPC (oracle)} & 0.45$\pm$0.02 & 0.43$\pm$0.03 & 0.96$\pm$0.04 & 1.59$\pm$0.06 & 2.14$\pm$0.08 & 4.41$\pm$0.10 & 5.08$\pm$0.30 & 6.93$\pm$0.25 & 8.70$\pm$0.17 & 10.15$\pm$0.47 & 12.91$\pm$0.51 \\
\hline
 
\textbf{Causal Transformer} & 0.46$\pm$0.02 & 0.68$\pm$0.04 & 1.50$\pm$0.06 & 2.55$\pm$0.18& 3.65$\pm$0.20& 5.55$\pm$0.50& 8.15$\pm$0.72& 12.35$\pm$0.25& 15.48$\pm$1.02& 24.77$\pm$2.21& 43.84$\pm$2.58\\


\textbf{Causal Transformer (with substitute)} &  0.46$\pm$0.02 & 0.67$\pm$0.02& 1.46$\pm$0.03& 2.48$\pm$0.08& 3.53$\pm$0.09& 5.23$\pm$0.11& 7.72$\pm$0.18& 11.86$\pm$0.17& 15.22$\pm$0.17& 20.12$\pm$0.35& 33.58$\pm$0.45\\


\textbf{Causal Transformer (oracle)} & 0.46$\pm$0.02&  0.60$\pm$0.03 & 1.48$\pm$0.03 & 2.35$\pm$ 0.06& 3.30$\pm$0.07& 5.11$\pm$0.09& 7.34$\pm$0.13& 11.55$\pm$0.25& 16.98$\pm$0.29& 18.64$\pm$0.31& 28.45$\pm$0.33\\

 \hline
\textbf{G-Net} & 0.62$\pm$0.05&  0.80$\pm$0.05& 4.90$\pm$0.03& 5.56$\pm$0.05& 4.82$\pm$0.15& 5.79$\pm$0.12& 10.36$\pm$0.23& 15.17$\pm$0.25& 23.89$\pm$0.54& 32.75$\pm$1.20& 49.35$\pm$2.35\\

\textbf{G-Net (with substitute)} & 0.56$\pm$0.04&  0.75$\pm$0.01& 3.61$\pm$0.02& 4.99$\pm$0.20& 4.27$\pm$0.18& 5.50$\pm$0.15& 8.34$\pm$0.64& 13.55$\pm$0.97& 17.97$\pm$1.83& 19.25$\pm$2.04& 40.21$\pm$2.10\\

\textbf{G-Net (oracle)} & 0.48$\pm$0.02& 0.69$\pm$0.03& 3.10$\pm$0.05& 4.36$\pm$0.08& 4.45$\pm$0.12& 5.28$\pm$0.17& 8.28$\pm$0.23& 13.10$\pm$0.50& 17.47$\pm$0.65& 16.22$\pm$0.95& 35.35$\pm$1.77\\
 \hline

 
\textbf{CRN} & 0.53$\pm$0.02& 0.68$\pm$0.03& 1.63$\pm$0.04& 2.94$\pm$0.11& 5.14$\pm$0.17& 6.66$\pm$0.19& 9.08$\pm$0.25& 11.93$\pm$0.37& 16.54$\pm$0.65& 18.68$\pm$0.67& 29.66$\pm$1.12\\

\textbf{CRN (with substitute)} & 0.48$\pm$0.01& 0.65$\pm$0.01& 1.51$\pm$0.02& 2.56$\pm$0.18 & 3.98$\pm$0.21 & 6.05$\pm$0.35 & 6.81$\pm$0.65 & 8.50$\pm$1.16 & 13.81$\pm$0.76 & 16.23$\pm$0.73 & 26.11$\pm$1.41 \\

\textbf{CRN (oracle)} & 0.53$\pm$0.01& 0.60$\pm$0.01& 1.69$\pm$0.02& 2.87$\pm$0.09& 3.75$\pm$0.13& 5.69$\pm$0.17& 8.92$\pm$0.22& 9.65$\pm$0.31& 13.49$\pm$0.54& 15.64$\pm$0.61& 25.98$\pm$0.97\\

 \hline
\textbf{RMSN} & 0.57$\pm$0.02& 0.67$\pm$0.02& 1.60$\pm$0.03& 2.67$\pm$0.05& 4.31$\pm$0.15& 5.58$\pm$0.17& 7.40$\pm$0.32& 11.25$\pm$0.57& 15.01$\pm$0.89& 19.41$\pm$1.13& 25.07$\pm$0.97\\

\textbf{RMSN (with substitute)} & 0.45$\pm$0.01& 0.67$\pm$0.02& 1.51$\pm$0.04 & 2.31$\pm$0.03& 3.61$\pm$0.20& 4.61$\pm$0.20& 6.14$\pm$0.50& 7.58$\pm$0.82& 10.63$\pm$1.31& 18.53$\pm$1.50& 21.08$\pm$1.60\\

\textbf{RMSN (oracle)} & 0.48$\pm$0.01& 0.62$\pm$0.01& 1.43$\pm$0.03& 1.97$\pm$0.03& 3.42$\pm$0.13& 4.43$\pm$0.15& 6.00$\pm$0.27& 7.31$\pm$0.34& 9.20$\pm$0.48& 17.06$\pm$0.83& 19.32$\pm$1.26\\
 \hline
 \end{tabular}%
}
\label{tab:perf_sim_combined}
\end{table}

\paragraph{Robustness to Number of Prior Components} The Table \ref{tab:ablation_arsim_n_clusters} gives detailed results summarized in Figure \ref{fig:ablation_arsim_n_clusters} that assess the sensitivity of CDVAE to the variation of the prior cluster numbers \(K\). 
\begin{table}[!htbp]
 \caption{Results of CDVAE when varying the number of components \(K\) of the prior. The study is conducted on the synthetic data and is reported by PEHE. Smaller is better.}
 \centering
\resizebox{\textwidth}{!}{%
\begin{tabular}{|c|c|c|c|c|c|c|c|c|c|c|c|} 
\hline
Model       & $\gamma_{(1)}^{YU} = 0$ & $\gamma_{(1)}^{YU} = 0.25$ & $\gamma_{(1)}^{YU} = 0.5$ & $\gamma_{(1)}^{YU} = 0.75$ & $\gamma_{(1)}^{YU} = 1$ & $\gamma_{(1)}^{YU} = 1.25$ & $\gamma_{(1)}^{YU} = 1.5$ & $\gamma_{(1)}^{YU} = 1.75$ & $\gamma_{(1)}^{YU} = 2$ & $\gamma_{(1)}^{YU} = 2.25$ & $\gamma_{(1)}^{YU} = 2.5$ \\ \hline 

\textbf{CDVAE (ours)} & \textbf{0.43$\pm$0.02}& \textbf{0.50$\pm$0.03}& \textbf{0.96$\pm$0.09}& \textbf{1.57$\pm$0.08}& \textbf{1.90$\pm$0.10}&  \textbf{2.35$\pm$0.18}& \textbf{3.57$\pm$0.17}& \textbf{4.80$\pm$0.20}& \textbf{6.84$\pm$0.20}& \textbf{7.64$\pm$0.48}& \textbf{9.03$\pm$0.50}\\
 \hline
  \textbf{CDVAE ($K=2$)}& 0.43$\pm$0.01& 0.50$\pm$0.01& 0.96$\pm$0.03& 1.52$\pm$0.04& 2.07$\pm$0.07& 2.51$\pm$0.14& 4.10$\pm$0.41& 4.44$\pm$0.43& 6.98$\pm$0.38& 7.90$\pm$0.33& 8.88$\pm$0.45\\ \hline

 \textbf{CDVAE ($K=5$)}& 0.42$\pm$0.01& 0.48$\pm$0.02& 0.93$\pm$0.02& 1.41$\pm$0.11& 2.02$\pm$0.03& 2.52$\pm$0.06& 3.27$\pm$0.22& 4.25$\pm$0.45& 6.32$\pm$0.25& 7.97$\pm$0.31&8.12$\pm$0.48\\\hline
 
 \textbf{CDVAE ($K=8$)}& 0.40$\pm$0.01& 0.46$\pm$0.01& 0.96$\pm$0.06& 1.57$\pm$0.03& 2.13$\pm$0.04& 2.59$\pm$0.07& 3.20$\pm$0.26& 4.15$\pm$0.45& 6.63$\pm$0.48& 6.93$\pm$0.25&8.91$\pm$0.19\\\hline
 
 \textbf{CDVAE ($K=11$)}& 0.42$\pm$0.02& 0.47$\pm$0.01& 0.94$\pm$0.03& 1.40$\pm$0.05& 2.09$\pm$0.07& 2.47$\pm$0.22& 3.76$\pm$0.28& 5.09$\pm$0.52& 6.48$\pm$0.14& 7.73$\pm$1.232& 9.02$\pm$1.22\\\hline

 \end{tabular}%
}
\label{tab:ablation_arsim_n_clusters}
\end{table}


\section{Experiments on MIMIC-III data}

\subsection{Additional results}
\label{appendix_cdvae:mimic_extended_results}
\paragraph{Results of baselines on the semi-synthetic MIMIC III} The following Table \ref{tab:perf_mimic} provides the detailed results responsible for Figures \ref{fig:perf_mimic} related to baselines with the three different approaches.
\begin{table}[!htbp]
 \caption{Results on the MIMIC III data reported by PEHE. Smaller is better.}
 \centering
\resizebox{0.4\textwidth}{!}{%
\begin{tabular}{|c|c|} 
\hline
Model      & $\mathrm{PEHE}$ \\ \hline 
\textbf{CDVAE (ours)} & \textbf{17.63$\pm$0.25}\\
\hline
\textbf{Causal CPC} & 19.27$\pm$0.25\\
\textbf{Causal CPC (with substitute)} & 18.45$\pm$0.26\\
\textbf{Causal CPC (oracle)} & 17.98$\pm$0.21\\
 \hline
\textbf{Causal Transformer} & 19.68$\pm$0.20 $\pm$\\
\textbf{Causal Transformer (with substitute)} & 18.58$\pm$ 0.21 \\
\textbf{Causal Transformer (oracle)} & 17.91 $\pm$ 0.20 \\
 \hline
\textbf{G-Net} & 19.75$\pm$0.21 \\
\textbf{G-Net (with substitute)} & 18.60$\pm$0.25 \\
\textbf{G-Net (oracle)} & 17.95$\pm$ 0.23\\
 \hline
\textbf{CRN} & 19.80$\pm$0.23 \\
\textbf{CRN (with substitute)} & 18.58$\pm$0.22\\
\textbf{CRN (oracle)} & 17.91$\pm$ 0.21 \\
 \hline
\textbf{RMSN} & 19.85$\pm$0.25 \\
\textbf{RMSN (with substitute)} &  18.66$\pm$0.23\\
\textbf{RMSN (oracle)} & 18.01$\pm$ 0.19 \\
 \hline
 \end{tabular}%
}
\label{tab:perf_mimic}
\end{table}





\section{Models hyperparameters Details} 
\label{appendix_cdvae:hyperparams_details}
We report in the following tables the search space of hyperparameters for all baselines.

\begin{table}[!htbp]
\centering
\caption{Hyper-parameters search range for RMSN}
\resizebox{0.9\textwidth}{!}{%
\begin{tabular}{|c|c|c|c|c|}
\hline
\textbf{Model} & \textbf{Sub-model} & \textbf{Hyperparameter} & \textbf{Synthetic data}& \textbf{MIMIC III}\\
\hline
\multirow{7}{*}{RMSNs} 
& \multirow{7}{*}{Propensity Treatment Network} 
& LSTM layers & 1 & 1 \\
\cline{3-5}
& & Learning rate & $0.01, 0.005, 0.001, 0.0001$ & $0.01, 0.005, 0.001, 0.0001$ \\
\cline{3-5}
& & Batch size & $32, 64, 128$ & $32, 64, 128$ \\
\cline{3-5}
& & LSTM hidden units & $6, 8, \dots, 12,14$& $4, 6, \dots, 20$\\
\cline{3-5}
& & LSTM dropout rate & - & - \\
\cline{3-5}
& & Max gradient norm & $0.5, 1, 2$ & $0.5, 1, 2$ \\
\cline{3-5}
& & Early Stopping (min delta) & 0.001& 0.001\\
\cline{3-5}
& & Early Stopping (patience) & 10& 30 \\
\hline
&\multirow{6}{*}{Propensity History Network} & LSTM layers & 1 & 1 \\
\cline{3-5}
& & Learning rate & $0.01, 0.005, 0.001, 0.0001$ & $0.01, 0.005, 0.001, 0.0001$ \\
\cline{3-5}
& & Batch size & $32, 64, 128$ & $64, 128, 256$ \\
\cline{3-5}
& & LSTM hidden units & $6, 8, \dots, 12,14$& $4, 6, \dots, 30$ \\
\cline{3-5}
& & LSTM dropout rate & - & - \\
\cline{3-5}
& & Early Stopping (min delta) & 0.001& 0.0001 \\
\cline{3-5}
& & Early Stopping (patience) & 10& 30 \\
\hline
& \multirow{6}{*}{Encoder} & LSTM layers & 1 & 1 \\
\cline{3-5}
& & Learning rate & $0.01, 0.005, 0.001, 0.0001$ & $0.01, 0.005, 0.001, 0.0001$ \\
\cline{3-5}
& & Batch size & $32, 64, 128,256$& $32, 64, 128$ \\
\cline{3-5}
& & LSTM hidden units & $6, 8, \dots, 18,20$& $6, 8, \dots, 18,20$\\
\cline{3-5}
& & LSTM dropout rate & - & - \\
\cline{3-5}
& & Early Stopping (min delta) & 0.001& 0.001\\
\cline{3-5}
& & Early Stopping (patience) & 10& 30 \\
\hline
& \multirow{6}{*}{Decoder} & LSTM layers & 1 & 1 \\
\cline{3-5}
& & Learning rate & $0.01, 0.005, 0.001, 0.0001$ & $0.01, 0.005, 0.001, 0.0001$ \\
\cline{3-5}
& & Batch size & $32, 64, 128,256$& $128, 512, 1024$ \\
\cline{3-5}
& & LSTM hidden units & $6, 8, \dots, 18,20$& $6, 8, \dots, 18,20$\\
\cline{3-5}
& & LSTM dropout rate & - & - \\
\cline{3-5}
& & Max gradient norm & $0.5, 1, 2$ & $0.5, 1, 2$ \\
\cline{3-5}
& & Early Stopping (min delta) & 0.001& 0.0001 \\
\cline{3-5}
& & Early Stopping (patience) & 10& 30 \\
\hline
\end{tabular}%
}
\end{table}



\begin{table}[!htbp]
\centering
\caption{Hyper-parameters search range for CRN}
\resizebox{0.7\textwidth}{!}{%
\begin{tabular}{|c|c|c|c|c|}
\hline
\textbf{Model} & \textbf{Sub-model} & \textbf{Hyperparameter} & \textbf{Synthetic data}& \textbf{MIMIC III)}\\
\hline
\multirow{8}{*}{CRN} 
& \multirow{8}{*}{Encoder} 
& LSTM layers & 1 & 1 \\
\cline{3-5}
& & Learning rate & $0.01, 0.005, 0.001, 0.0001$ & $0.01, 0.005, 0.001, 0.0001$ \\
\cline{3-5}
& & Batch size & $32, 64, 128,256$& $32, 64, 128$ \\
\cline{3-5}
& & LSTM hidden units & $6, 8, \dots, 18,20$& $6, 8, \dots, 18,20$\\
\cline{3-5}
& & LSTM dropout rate & - & - \\
\cline{3-5}
& & BR size & $6, 8, \dots, 18,20$& $6, 8, \dots, 18,20$\\
\cline{3-5}
& & Early Stopping (min delta) & 0.001& 0.001\\
\cline{3-5}
& & Early Stopping (patience) & 10& 30 \\
\hline
&\multirow{7}{*}{Decoder} & LSTM layers & 1 & 1 \\
\cline{3-5}
& & Learning rate & $0.01, 0.005, 0.001, 0.0001$ & $0.01, 0.005, 0.001, 0.0001$ \\
\cline{3-5}
& & Batch size & $128, 256, 512$ & $256, 512, 1024$ \\
\cline{3-5}
& & LSTM hidden units & $6, 8, \dots, 18,20$& $6, 8, \dots, 18,20$\\
\cline{3-5}
& & LSTM dropout rate & - & - \\
\cline{3-5}
& & BR size & $6, 8, \dots, 18,20$& $6, 8, \dots, 18,20$\\
\cline{3-5}
& & Early Stopping (min delta) & 0.001& 0.001\\
\cline{3-5}
& & Early Stopping (patience) & 10& 30 \\
\hline
\end{tabular}%
}
\end{table}

\begin{table}[!htbp]
\centering
\caption{Hyper-parameters search range for G-Net}
\resizebox{0.7\textwidth}{!}{%
\begin{tabular}{|c|c|c|}
\hline
\textbf{Hyperparameter} & \textbf{Cancer simulation} & \textbf{MIMIC III (SS)} \\
\hline
LSTM layers & 1 & 1  \\
 %\cline{1-4}
Learning rate & $0.01,0.005, 0.001, 0.0001$ &  $0.01,0.005, 0.001, 0.0001$ \\
 % %\cline{1-4}
Batch size & $32, 64, 128$ &  $32, 64, 128$ \\
 %\cline{1-4}
LSTM hidden units & $6, 8, \dots, 18,20$ & $6, 8, \dots, 18,20$ \\
%\cline{1-4}
FC hidden units & $6, 8, \dots, 18,20$&  $6, 8, \dots, 18,20$ \\
 %\cline{1-4}
LSTM dropout rate & - & -  \\
 %\cline{1-4}
R size& $6, 8, \dots, 18,20$& $4,6, \dots, 30$ \\
 %\cline{1-4}
MC samples & 50 & 50 \\
Early Stopping (min delta)& 0.001&  0.001\\
Early Stopping (patience)& 10& 30 \\
\cline{1-3}
\end{tabular}%
}
\end{table}




\begin{table}[!htbp]
\centering
\caption{Hyper-parameters search range for Causal Transformer}
\resizebox{0.7\textwidth}{!}{%
\begin{tabular}{|c|c|c|}
\hline
\textbf{Hyperparameter} & \textbf{Cancer simulation} & \textbf{MIMIC III (SS)} \\
\hline
Transformer blocks & 1 & 1 \\
 %\cline{1-4}
Learning rate & $0.01,0.005, 0.001, 0.0001$ & $0.01,0.005, 0.001, 0.0001$  \\
 %\cline{1-4}
Batch size & $32, 64, 128$ & $32, 64, 128$ \\
 %\cline{1-4}
Attention heads & $2$ & $2$ \\
 %\cline{1-4}
Transformer units & $4,6, \dots, 20$& $4,6, \dots, 20$ \\
 %\cline{1-4}
LSTM dropout rate & -  & - \\
%\cline{1-4}
BR size& $6, 8, \dots, 18,20$&  $4,6, \dots, 20$ \\
%\cline{1-4}
FC hidden units & $6, 8, \dots, 18,20$&   $4,6, \dots, 20$ \\
Sequential dropout rate & $0.1,0.2, 0.3$& $0.1,0.2, 0.3$ \\
Max positional encoding & $15$& $20$  \\
Early Stopping (min delta)& 0.001& 0.001 \\
Early Stopping (patience)& 10& 30 \\
\cline{1-3}
\end{tabular}%
}
\end{table}


\begin{table}[!htbp]
\centering
\caption{Hyper-parameters search range for Causal CPC}
\resizebox{0.9\textwidth}{!}{%
\begin{tabular}{|c|c|c|c|c|}
\hline
\textbf{Model} & \textbf{Sub-model} & \textbf{Hyperparameter} & \textbf{Cancer simulation} & \textbf{MIMIC III (SS)} \\
\hline
\multirow{9}{*}{Causal CPC} & \multirow{9}{*}{Encoder} 
& GRU layers & 1 & 1 \\
\cline{3-5}
& & Learning rate & $0.01, 0.005, 0.001, 0.0001$ & $0.01, 0.005, 0.001, 0.0001$ \\
\cline{3-5}
& & Batch size & $32, 64, 128$ & $64, 128, 256$ \\
\cline{3-5}
& & GRU hidden units & $6, 8, \dots, 18,20$& $6, 8, \dots, 18,20$\\
\cline{3-5}
& & GRU dropout rate & - & - \\
\cline{3-5}
& & Local features (LF) size & $6, 8, \dots, 18,20$& $4, 6, \dots, 20$ \\
\cline{3-5}
& & Context Representation (CR) size & $6, 8, \dots, 18,20$& $4, 6, \dots, 20$ \\
\cline{3-5}
& & Early Stopping (min delta) & 0.001 & 0.001 \\
\cline{3-5}
& & Early Stopping (patience) & 10& 30\\
\hline
& \multirow{13}{*}{Decoder} & GRU layers & 1 & 1 \\
\cline{3-5}
& & Learning rate (decoder w/o treatment sub-network) & $0.01, 0.005, 0.001, 0.0001$ & $0.01, 0.005, 0.001, 0.0001$ \\
\cline{3-5}
& & Learning rate (encoder fine-tuning) & $0.001, 0.0005, 0.0001, 0.00005$ & $0.001, 0.0005, 0.0001, 0.00005$ \\
\cline{3-5}
& & Learning rate (treatment sub-network) & $0.05, 0.01, 0.005, 0.0001$ & $0.05, 0.01, 0.005, 0.0001$ \\
\cline{3-5}
& & Batch size & $32, 64, 128$ & $32, 64, 128$ \\
\cline{3-5}
& & GRU hidden units & CR size & CR size \\
\cline{3-5}
& & GRU dropout rate & - & - \\
\cline{3-5}
& & BR size & CR size & CR size \\
\cline{3-5}
& & GRU layers (Treat Encoder) & 1 & 1 \\
\cline{3-5}
& & GRU hidden units (Treat Encoder) & 6 & 6 \\
\cline{3-5}
& & FC hidden units & $6, 8, \dots, 18,20$& $4, 6, \dots, 20$ \\
\cline{3-5}
& & Random time indices (m) & 10\% & 10\% \\
\cline{3-5}
& & Early Stopping (min delta) & 0.001 & 0.001 \\
\cline{3-5}
& & Early Stopping (patience) & 10& 30\\
\hline
\end{tabular}%
}
\end{table}

\begin{table}[!htbp]
\centering
\caption{Hyper-parameters search range for CDVAE}
\resizebox{0.9\textwidth}{!}{%
\begin{tabular}{|c|c|c|c|c|}
\hline
\textbf{Model} & \textbf{Sub-model} & \textbf{Hyperparameter} & \textbf{Synthetic data}& \textbf{MIMIC III}\\
\hline
\multirow{7}{*}{CDVAE} 
& \multirow{4}{*}{Inference Network} & GRU layers & 1 & 1 \\
\cline{3-5}
& & GRU hidden units & $6, 8, \dots, 12,14$& $4, 6, \dots, 20$\\
\cline{3-5}
& & GRU dropout rate& - & - \\
\cline{3-5}
& & Latent dim of \(\mathbf{z}\) & 0.001& 0.001\\
\hline
& \multirow{1}{*}{Propensity Network} & FC hidden units & $6, 8, \dots, 12,14$& $4, 6, \dots, 30$ \\
\hline
& \multirow{4}{*}{Representation Learner} & LSTM layers & 1 & 1 \\
\cline{3-5}
& & GRU hidden units & $6, 8, \dots, 18,20$& $6, 8, \dots, 18,20$\\
\cline{3-5}
& & GRU dropout rate & - & - \\
\cline{3-5}
& & Dimension of representation & $6, 8, \dots, 18,20$& $4, 6, \dots, 20$ \\
\hline
& \multirow{1}{*}{Decoder} & FC hidden units & $(dim(\mathbf{z})+dim(\Phi(\mathbf{H}_t)) / 2$& $(dim(\mathbf{z})+dim(\Phi(\mathbf{H}_t)) / 2$\\
\hline
& \multirow{4}{*}{Global} & Learning rate (w/o propensity network) & $0.01, 0.005, 0.001, 0.0001$ & $0.01, 0.005, 0.001, 0.0001$ \\
\cline{3-5}
& & Learning rate (propensity network) & $0.01, 0.005, 0.001, 0.0001$ & $0.01, 0.005, 0.001, 0.0001$ \\
\cline{3-5}
& & Batch size & $32, 64, 128,256$& $128, 512, 1024$ \\
\cline{3-5}
& & Max gradient norm & $0.5, 1, 2$ & $0.5, 1, 2$ \\
\cline{3-5}
& & Number of components in Prior & $2, 4, \dots, 18, 20$& $2, 4, \dots, 20$ \\
\hline
\end{tabular}%
}
\end{table}


\section{The Neural Architecture of CDVAE}
\label{appendix_cdvae:extended_archi_CDVAE}
The extended neural architecture of CDVAE comprises multiple components which we did not explicit in Section \ref{sect_cdvae:CDVAE_archi}. We first begin by detailing neural network functions related to the generative model. The Table \ref{tab:archi_phi_rep_learner} outlines the architecture for the Representation Learner $\Phi$ which encodes the context history, Table \ref{tab:archi_f_theta} presents the identical architecture for both $f_{\theta_{y}^1}$ and $f_{\theta_{y}^0}$ responsible for generating the two potential outcomes. Meanwhile, Table \ref{tab:archi_e_theta} illustrates the design of propensity network $e_{\theta_{\omega}}(.)$ built on the top of the shared representation. Lastly, Tables \ref{tab:archi_inf_net} depict the architecture used to learn both the mean and covariance matrix for the approximate posterior assumed to be Gaussian. 

\begin{table}[!htbp]
\centering
\begin{tabular}{|c|}
\hline Inputs: $\{\Phi(\mathbf{h}_t)\}_{ 1 \leq t \leq T}$, $\mathbf{z}$ \\
\hline Concatenate: $[\Phi(\mathbf{h}_t), \mathbf{z}]_{ 1 \leq t \leq T}$\\
\hline Linear Layer \\ 
\hline Weight Normalization \\
\hline ELU  \\
\hline Linear Layer \\
\hline Weight Normalization \\
\hline Linear Layer  \\
\hline Output: $\{\hat{Y}_{t+1}(\omega)\}_{ 1 \leq t \leq T-1}$ \\ 
\hline
 \end{tabular}
\caption{Architecture of the outcome model prediction, i.e., the decoder.}
\label{tab:archi_f_theta}
\end{table}

\begin{table}[!htbp]
\centering
\begin{minipage}{0.33\textwidth}
\centering
\begin{tabular}{|c|}
\hline Inputs: $\{y_{t}, \mathbf{x}_{t}, \omega_{t}\}_{ 1 \leq t \leq T}$ \\
\hline Concat: $[y_{t}, \mathbf{x}_{t}, \omega_{t}]_{ 1 \leq t \leq T}$ \\
\hline GRU layer \\
\hline Linear Layer \\
\hline Tanh  \\
\hline Outputs: $\{\Phi(\textbf{h}_t)\}_{ 1 \leq t \leq T}$\\ \hline
\end{tabular}
\caption{Architecture: representation learner $\phi$ of CDVAE}
\label{tab:archi_phi_rep_learner}
\end{minipage}%
\begin{minipage}{0.33\textwidth}
\centering
\begin{tabular}{|c|}
\hline Inputs: $\{\Phi(\mathbf{h}_t)\}_{ 1 \leq t \leq T}$ \\
\hline Linear Layer \\
\hline ELU  \\
\hline Sigmoid  \\
\hline Output: $\{\hat{W}_{t+1}(\omega)\}_{ 1 \leq t \leq T-1}$ 
 \\ \hline\end{tabular}
\caption{Architecture: propensity network  $e_{\theta_{\omega}}(.)$.}
\label{tab:archi_e_theta}
\end{minipage}
\begin{minipage}{0.33\textwidth}
\centering
\begin{tabular}{|c|} \hline 

Inputs: $\{y_{t}, \mathbf{x}_{t}, \omega_{t}\}_{1 \leq t \leq T}$ \\ \hline  
Concat: $[y_{t}, \mathbf{x}_{t}, \omega_{t}]_{1 \leq t \leq T}$ \\ \hline  
GRU layer \\ \hline 

\begin{tabular}{c|c}  Linear Layer & Linear Layer  \end{tabular}\\ \hline 

\begin{tabular}{c|c}  $\Sigma_{\phi_3}\left(\mathbf{g}_T\right)$ & $\mu_{\phi_2}\left(\mathbf{g}_T\right)$ \end{tabular}\\ \hline 

\end{tabular}
\caption{Inference network $q_\phi\left(\mathbf{z} \mid y_{\leq T}, \mathbf{x}_{\leq T}, \omega_{\leq T}\right)$}
\label{tab:archi_inf_net}
\end{minipage}
\end{table}






==> appendices/4.tex <==
\chapter{Appendix: Chapter \ref{chapter:ccpc}}
  
\section{Experiments on semi-synthetic data: Details} 

\subsection{Additional results}
\label{appendix_ccpc:detailed_results_mimic}

\subsubsection{Comparison to benchmark models: standard train/test split}
\label{appendix_ccpc:results_orig_mimic}
We also tested Causal CPC on MIMIC III semi-synthetic data using the same experimental protocol as \cite{Melnychuk2022CausalTF}, namely by using the split of patients into train/validation/test as 800/200/200. As a result, baseline performances in Table \ref{tab: perf_mimic_orig_data} are exactly the same as in \cite{Melnychuk2022CausalTF}. 
\begin{table}[!htbp]
 \caption{Results over the MIMIC III semi-synthetic data set (same experimental protocol as in \cite{Melnychuk2022CausalTF}): mean$\pm$standard deviation of Rooted Mean Squared Errors (RMSEs). The best value for each metric is given in bold: smaller is better.}
 \centering
\resizebox{\textwidth}{!}{%
\begin{tabular}{|c |c |c |c |c |c  |c |c |c |c |c|} 
\hline
Model       & $\rho = 1$   &   $\rho = 2$& $\rho = 3$&   $\rho = 4$&  $\rho = 5$&   $\rho = 6$& $\rho = 7$&  $\rho = 8$&   $\rho = 9$ & $\rho = 10$\\ \hline  

\textbf{Causal CPC (ours)}  &   0.25 $\pm$ 0.03  & \textbf{0.37 $\pm$ 0.02}  &\textbf{0.40 $\pm$ 0.01} & \textbf{0.45 $\pm$ 0.01} & \textbf{0.49 $\pm$ 0.02} & \textbf{0.52 $\pm$ 0.02} & \textbf{0.55 $\pm$ 0.03}  &\textbf{0.56 $\pm$ 0.03 } &\textbf{0.58 $\pm$ 0.04} & \textbf{0.60 $\pm$ 0.03} \\ 
\hline  
\textbf{Causal Transformer} & \textbf{ 0.20 $\pm$ 0.01 } & 0.38 $\pm$ 0.01  &0.45 $\pm$ 0.01 & 0.49 $\pm$ 0.01 & 0.52 $\pm$ 0.02 & 0.53 $\pm$ 0.02 & 0.55 $\pm$ 0.02  &\textbf{0.56 $\pm$ 0.02}  &\textbf{0.58 $\pm$ 0.02} & \textbf{0.59 $\pm$ 0.02}  \\ 
\hline  
\textbf{G-Net} & 0.34 $\pm$ 0.01& 0.67 $\pm$ 0.03& 0.83 $\pm$ 0.04& 0.94 $\pm$ 0.04& 1.03 $\pm$ 0.05 &1.10 $\pm$ 0.05 &1.16 $\pm$ 0.05 &1.21 $\pm$ 0.06& 1.25 $\pm$ 0.06 & 1.29 $\pm$ 0.06\\ 
\hline  
\textbf{CRN} &  0.30 $\pm$ 0.01& 0.48 $\pm$ 0.02 &0.59 $\pm$ 0.02& 0.65 $\pm$ 0.02 &0.68 $\pm$ 0.02& 0.71 $\pm$ 0.01 &0.72 $\pm$ 0.01 &0.74 $\pm$ 0.01 &0.76 $\pm$ 0.01& 0.78 $\pm$ 0.02\\ 
\hline  
\textbf{RMSN} &   0.24 $\pm$ 0.01& 0.47 $\pm$ 0.01& 0.60 $\pm$ 0.01& 0.70 $\pm$ 0.02& 0.78 $\pm$ 0.04 &0.84 $\pm$ 0.05 &0.89 $\pm$ 0.06& 0.94 $\pm$ 0.08 & 0.97 $\pm$ 0.09& 1.00 $\pm$ 0.11 \\ 
\hline  
\textbf{MSM} & 0.37 $\pm$ 0.01& 0.57 $\pm$ 0.03& 0.74 $\pm$ 0.06 &0.88 $\pm$ 0.03& 1.14 $\pm$ 0.10 &1.95 $\pm$ 1.48 &3.44 $\pm$ 4.57 &$>$ 10.0 & $>$ 10.0 & $>$ 10.0\\ 
\hline  
 \end{tabular}
 }
\label{tab: perf_mimic_orig_data}
\end{table}

\section{Proofs of theoretical results}
\label{appendix_ccpc:proofs}
\subsection{Relation between InfoNCE loss and mutual information}

\begin{proposition}
    $$I(\mathbf{F}_{t+j}, \mathbf{C}_{t}) \geq \log(|\mathcal{B}|) - \mathcal{L}^{(InfoNCE)}_j$$
\end{proposition}

\begin{proof}

In the following, we draw inspiration from the proof of \citet{oord2018representation}. The InfoNCE loss can be interpreted as the categorical cross-entropy of correctly classifying the positive sample \(\mathbf{F}_{t+j}\) given the context \(\mathbf{C}_t^{\mathrm{enc}}\). This is done with probability
\[
\frac{\exp\bigl(T_j(\mathbf{F}_{t+j}, \mathbf{C}_t)\bigr)}%
{\sum_{l = 1}^{|\mathcal{B}|} \exp\bigl(T_j(\mathbf{F}_{l,t+j}, \mathbf{C}_t)\bigr)},
\]
where \(\mathbf{F}_{t+j}\) is treated as the positive sample within the batch \(\mathcal{B}\), and the remaining elements serve as negative samples. Let $\texttt{pos} \in \{1, \dots, |\mathcal{B}|\}$ be the indicator of the positive sample $\mathbf{F}_{t+j}$.  The optimal probability is 
\[
\begin{aligned}
p(\mathrm{Index} = \mathtt{pos} \mid \mathcal{B}, \mathbf{C}_t^{\mathrm{enc}}) 
&= \frac{p(\mathbf{f}_{\mathtt{pos}, t+j} \mid \mathbf{C}_t^{\mathrm{enc}}) 
\prod_{\substack{l=1 \\ l \ne \mathtt{pos}}}^{\mathcal{B}} p(\mathbf{f}_{l, t+j})}
{\sum_{j=1}^{\mathcal{B}} \left[ p(\mathbf{f}_{j, t+j} \mid \mathbf{C}_t^{\mathrm{enc}}) 
\prod_{\substack{l=1 \\ l \ne j}}^{\mathcal{B}} p(\mathbf{f}_{l, t+j}) \right]} \\[1.5ex]
&= \frac{ \dfrac{p(\mathbf{f}_{\mathtt{pos}, t+j} \mid \mathbf{C}_t^{\mathrm{enc}})}{p(\mathbf{f}_{\mathtt{pos}, t+j})} }
{\sum_{j=1}^{\mathcal{B}} \dfrac{p(\mathbf{f}_{j, t+j} \mid \mathbf{C}_t^{\mathrm{enc}})}{p(\mathbf{f}_{j, t+j})}}.
\end{aligned}
\]

Now, for  the score $\exp(T_j(\mathbf{F}_{t+j},\mathbf{C}_{t}))$  to be optimal, it should be proportional to $ \frac{p(\mathbf{f}_{\texttt{pos}, t+j} \vert c)}{p(\mathbf{f}_{\texttt{pos}, t+j})}$.  The MI lower bound comes from the fact that $ \exp(T_j(\mathbf{F}_{t+j},\mathbf{C}_{t})) $ estimates the density ratio $ \frac{p(\mathbf{f}_{\texttt{pos}, t+j} \vert c)}{p(\mathbf{f}_{\texttt{pos}, t+j})}$.


\begin{equation}
\begin{aligned}
\mathcal{L}^{(InfoNCE)}_j & =-\mathbb{E}_{\mathcal{B}} \log \left[\frac{\frac{p\left(\mathbf{f}_{t+j} \mid \mathbf{C}_t^{\mathrm{enc}}\right)}{p\left(\mathbf{f}_{t+j}\right)}}{\frac{p\left(\mathbf{f}_{t+j} \mid \mathbf{C}_t^{\mathrm{enc}}\right)}{p\left(\mathbf{f}_{t+j}\right)}+\sum_{\mathbf{f}_{l, t+j} \in \mathcal{B}_{\text {neg }}} \frac{p\left(\mathbf{f}_{l, t+j} \mid \mathbf{C}_t^{\mathrm{enc}}\right)}{p\left(\mathbf{f}_{l, t+j}\right)}}\right] \\
& =\mathbb{E}_{\mathcal{B}} \log \left[1+\frac{p\left(\mathbf{f}_{t+j}\right)}{p\left(\mathbf{f}_{t+j} \mid \mathbf{C}_t^{\mathrm{enc}}\right)} \sum_{\mathbf{f}_{l, t+j} \in \mathcal{B}_{\text {neg }}} \frac{p\left(\mathbf{f}_{l, t+j} \mid \mathbf{C}_t^{\mathrm{enc}}\right)}{p\left(\mathbf{f}_{l, t+j}\right)}\right] \\
& \approx \mathbb{E}_{\mathcal{B} }\log \left[1+\frac{p\left(\mathbf{f}_{t+j}\right)}{p\left(\mathbf{f}_{l, t+j} \mid \mathbf{C}_t^{\mathrm{enc}}\right)}(|\mathcal{B}|-1) \mathbb{E}_{\mathbf{F}_{t+j}} \frac{p\left(\mathbf{f}_{l, t+j}\mid \mathbf{C}_t^{\mathrm{enc}}\right)}{p\left(\mathbf{f}_{l, t+j}\right)}\right] \\
& =\mathbb{E}_{\mathcal{B}} \log \left[1+\frac{p\left(\mathbf{f}_{t+j}\right)}{p\left(\mathbf{f}_{t+j} \mid \mathbf{C}_t^{\mathrm{enc}}\right)}(|\mathcal{B}|-1)\right] \\
& \geq \mathbb{E}_{\mathcal{B}} \log \left[\frac{p\left(\mathbf{f}_{t+j}\right)}{p\left(\mathbf{f}_{t+j}\mid \mathbf{C}_t^{\mathrm{enc}}\right)} |\mathcal{B}|\right] \\
& =-I\left(\mathbf{f}_{t+j}, \mathbf{C}_t^{\mathrm{enc}}\right)+\log (|\mathcal{B}|),
\end{aligned}
\label{eq:infonce_proof}
\end{equation}

The approximation in the third equation, Eq. \eqref{eq:infonce_proof}, becomes more precise as the batch size increases.
\end{proof}

\subsection{Relation between InfoMax and input reconstruction}
 We now prove the proposition \ref{prop:lb_infomax} stating that : $ I(\mathbf{C}_t^{\mathrm{enc},h},\mathbf{C}_t^{\mathrm{enc},f})\leq I(\mathbf{H}_{t}, (\mathbf{C}_t^{\mathrm{enc},h}, \mathbf{C}_t^{\mathrm{enc},f}))$
 \begin{proof}
    This is followed by two applications of the data processing inequality \cite{cover1999elementsInfo}, which states that for random variables \(A\), \(B\), and \(C\) satisfying the Markov relation \(A \to B \to C\), we have
\[
I(A;C) \leq I(A;B).
\]

First, note that
\[
\mathbf{C}_t^{\mathrm{enc},h} = \Phi_{\theta_{1},\theta_{2}}(\mathbf{H}_t^h), \quad
\mathbf{C}_t^{\mathrm{enc},f} = \Phi_{\theta_{1},\theta_{2}}(\mathbf{H}_t^f),
\]
where \(\mathbf{H}_t^h = \mathrm{trunc}_f(\mathbf{H}_t)\) and \(\mathbf{H}_t^f = \mathrm{trunc}_h(\mathbf{H}_t)\). Here, \(\mathrm{trunc}_f\) and \(\mathrm{trunc}_h\) truncate the future and history processes, respectively, relative to a splitting time \(t_0\).

We now observe the Markov relation
\[
\mathbf{C}_t^{\mathrm{enc},h} 
\xleftarrow{\Phi_{\theta_{1},\theta_{2}} \circ \mathrm{trunc}_f} 
\mathbf{H}_t 
\xrightarrow{\Phi_{\theta_{1},\theta_{2}} \circ \mathrm{trunc}_h}
\mathbf{C}_t^{\mathrm{enc},f},
\]
which is Markov equivalent to
\[
\mathbf{C}_t^{\mathrm{enc},h}
\xrightarrow{\Phi_{\theta_{1},\theta_{2}} \circ \mathrm{trunc}_f}
\mathbf{H}_t
\xrightarrow{\Phi_{\theta_{1},\theta_{2}} \circ \mathrm{trunc}_h}
\mathbf{C}_t^{\mathrm{enc},f}.
\]
By the data processing inequality, this gives
\[
I(\mathbf{C}_t^{\mathrm{enc},h}; \mathbf{C}_t^{\mathrm{enc},f})
\leq I(\mathbf{H}_t; \mathbf{C}_t^{\mathrm{enc},h}).
\]

On the other hand, we trivially have the Markov relation
\[
\mathbf{H}_t \to (\mathbf{C}_t^{\mathrm{enc},h}, \mathbf{C}_t^{\mathrm{enc},f}) \to \mathbf{C}_t^{\mathrm{enc},h},
\]
which yields
\[
I(\mathbf{H}_t; \mathbf{C}_t^{\mathrm{enc},h})
\leq I(\mathbf{H}_t; (\mathbf{C}_t^{\mathrm{enc},h}, \mathbf{C}_t^{\mathrm{enc},f})).
\]

Combining the two inequalities proves the proposition.
\end{proof}
\subsection{Proof of Theorem \ref{thm:tightness_lb_info}}

To begin, we split the process history into two non-overlapping views (Figure \ref{fig:ccpc_archi}): $\mathbf{H}_t^h \coloneqq \mathbf{F}_{1:t_0}$ and $\mathbf{H}_t^f \coloneqq \mathbf{F}_{t_0+1:t}$, representing a historical subsequence and a future subsequence within the process history $\mathbf{H}_{t}$, respectively. We then computed representations of these two views denoted $\mathbf{C}_t^{\mathrm{enc},h}$ and $\mathbf{C}_t^{\mathrm{enc},f}$, respectively. This naturally gives rise to the Markov chain, as in showed in the proof of proposition \ref{prop:lb_infomax}:
\[
\mathbf{C}_t^{\mathrm{enc},h} \xleftarrow[]{} \mathbf{H}_t \xrightarrow[]{} \mathbf{C}_t^{\mathrm{enc},f}
\]
which is Markov equivalent to:
\[
\mathbf{C}_t^{\mathrm{enc},h} \xrightarrow{} \mathbf{H}_t \xrightarrow[]{} \mathbf{C}_t^{\mathrm{enc},f}
\]
Following this Markov chain, we can show that \cite{shwartz2024compress}:
\[
I(\mathbf{C}_t^{\mathrm{enc},f}, \mathbf{C}_t^{\mathrm{enc},h}) = I(\mathbf{H}_t, \mathbf{C}_t^{\mathrm{enc},h}) - \mathbb{E}_{\mathbf{h}_t \sim \mathbb{P}_{\mathbf{H}_t}} \mathbb{E}_{\mathbf{c}_{t}^f \sim \mathbb{P}_{\mathbf{C}_{t}^f \mid \mathbf{h}_t}} \left[ D_{KL}[\mathbb{P}_{\mathbf{C}_{t}^h \mid \mathbf{h}_t} || \mathbb{P}_{\mathbf{C}_{t}^h \mid \mathbf{c}_{t}^f }] \right]
\]
On the other hand, by applying the chain rule of the mutual information to $I(\mathbf{H}_{t}; (\mathbf{C}_t^{\mathrm{enc},h}, \mathbf{C}_t^{\mathrm{enc},f}))$ we get:
\[
I(\mathbf{H}_{t}; (\mathbf{C}_t^{\mathrm{enc},f}, \mathbf{C}_t^{\mathrm{enc},h})) = I(\mathbf{H}_t, \mathbf{C}_t^{\mathrm{enc},h}) + I(\mathbf{H}_t; \mathbf{C}_t^{\mathrm{enc},f} \mid \mathbf{C}_t^{\mathrm{enc},h}) 
\]
Combining these equations, the tightness of our bounds can be written as:
\begin{equation}
\begin{aligned}
I(\mathbf{H}_{t}; (\mathbf{C}_t^{\mathrm{enc},f}, \mathbf{C}_t^{\mathrm{enc},h})) 
&- I(\mathbf{C}_t^{\mathrm{enc},f}, \mathbf{C}_t^{\mathrm{enc},h}) \\
&= I(\mathbf{H}_t; \mathbf{C}_t^{\mathrm{enc},f} \mid \mathbf{C}_t^{\mathrm{enc},h}) \\
&\quad + \mathbb{E}_{\mathbf{h}_t \sim \mathbb{P}_{\mathbf{H}_t}} 
\mathbb{E}_{\mathbf{c}_{t}^f \sim \mathbb{P}_{\mathbf{C}_{t}^f \mid \mathbf{h}_t}} 
\bigg[
    D_{\mathrm{KL}}\bigl(
        \mathbb{P}_{\mathbf{C}_{t}^h \mid \mathbf{h}_t}
        \,\big\|\, 
        \mathbb{P}_{\mathbf{C}_{t}^h \mid \mathbf{c}_{t}^f}
    \bigr)
\bigg].
\end{aligned}
\end{equation}

\subsection{On the relation between conditional entropy and reconstruction}
\label{appendix: zero_cond_H}
We now prove the statement in the core paper, saying that the conditional entropy $H(\mathbf{H}_{t}\mid (\mathbf{C}_t^{\mathrm{enc},h}, \mathbf{C}_t^{\mathrm{enc},f})) \geq 0$ is minimized if $\mathbf{H}_{t}$ is a function of $(\mathbf{C}_t^{\mathrm{enc},h}, \mathbf{C}_t^{\mathrm{enc},f})$ almost surely.
\begin{proposition}
\label{prop:zero_cond_H}
$H(\mathbf{A} \mid \mathbf{B}) =  0$ implies that $\mathbf{A} = f(\mathbf{B})$ almost surely.
\end{proposition}
\begin{proof}
   For simplicity, suppose \(\mathbf{A}\) and \(\mathbf{B}\) are discrete. Assume, by contradiction, that there exists \(\mathbf{b}_0\) and two distinct values \(\mathbf{a}_1\) and \(\mathbf{a}_2\) such that \(p(\mathbf{a}_1 \mid \mathbf{b}_0), p(\mathbf{a}_2 \mid \mathbf{b}_0) > 0\). Then the conditional entropy is given by:
\[
H(\mathbf{A} \mid \mathbf{B}) 
= -\sum_{\mathbf{b}} p(\mathbf{b}) \sum_{\mathbf{a}} p(\mathbf{a} \mid \mathbf{b}) \log p(\mathbf{a} \mid \mathbf{b}).
\]
In particular, we have:
\[
H(\mathbf{A} \mid \mathbf{B}) 
\geq p(\mathbf{b}_0) \bigg(-p(\mathbf{a}_1 \mid \mathbf{b}_0) \log p(\mathbf{a}_1 \mid \mathbf{b}_0) 
- p(\mathbf{a}_2 \mid \mathbf{b}_0) \log p(\mathbf{a}_2 \mid \mathbf{b}_0)\bigg) > 0,
\]
where we used the fact that \(-t \log t \geq 0\) for \(0 \leq t \leq 1\), with strict inequality for \(t \notin \{0,1\}\).  

Therefore, \(H(\mathbf{A} \mid \mathbf{B}) = 0\) if and only if \(\mathbf{A}\) is a function of \(\mathbf{B}\) almost surely.
% Reformulate !!!!!!!!!!!!!!!!!!!
\end{proof}



% \subsection{On the benefit of the InfoMax loss on inverting the data generation process}
% \label{appendix: infomax_inverting_dgp}
% To ensure identifiability in the latent space, we leverage recent advances in causal and disentangled representation learning. Suppose the true data-generating process is given by $\mathbf{H}_{t} = g(\mathbf{z}_t)$, where $\mathbf{z}_t$ represents the true latent factors. In the sequential context, we assume that the same function $g$ generates two historical subsequences:
% \[
% \mathbf{H}_t^f = g(\mathbf{z}_t^f), \quad \mathbf{H}_t^h = g(\mathbf{z}_t^h)
% \]
% We assume a general dependency of the form:
% \[
% p(\mathbf{z}_t^f \mid \mathbf{z}_t^h ) = \frac{Q(\mathbf{z}_t^f)}{Z(\mathbf{z}_t^h)} \exp(-d(\mathbf{z}_t^f, \mathbf{z}_t^h))
% \]
% Here, $\mathbf{\Phi}$ is an encoder, and we use the InfoMax regularization term as follows:
% \[
% \mathcal{L}^{(InfoMax)}(\mathbf{\Phi}, d, \mathcal{B}) := -\mathbb{E}_{\mathcal{B}} \left[ \log \frac{\exp(-d(\mathbf{\Phi}(\mathbf{H}_t^f), \mathbf{\Phi}(\mathbf{H}_t^h)))}{\sum_{l = 1}^{|\mathcal{B}|} \exp(-d(\mathbf{\Phi}(\mathbf{H}_{l,t}^f), \mathbf{\Phi}(\mathbf{H}_t^h)))} \right]
% \]
% According to \cite{matthes2023towards}, under certain conditions, if the encoder $f$ minimizes $\mathcal{L}^{(InfoMax)}$, then $h = g \circ f$ is a scaled permutation matrix. This result suggests that when the encoder achieves a minimizer for $\mathcal{L}^{(InfoMax)}$, the encoder function $f$ closely approximates an invertible transformation of $g$.

% From a causal inference perspective, if $Y_{it}(\omega_{it}) \indep W_{it} \mid \mathbf{H}_{it}$ and $\mathbf{H}_{it} = g(\mathbf{Z}_{it})$, then an invertible function $g \circ f$ ensures that:
% \[
% Y_{it}(\omega_{it}) \indep W_{it} \mid g \circ f (\mathbf{H}_{it})
% \]
% Thus, $Y_{it}(\omega_{it}) \indep W_{it} \mid g(\mathbf{C}_{it})$ and since $g$ is invertible, we have:
% \[
% Y_{it}(\omega_{it}) \indep W_{it} \mid \mathbf{C}_{it}
% \]
% This demonstrates that the representation $\mathbf{C}_{it}$ retains the essential independence structure, facilitating accurate counterfactual inference.


\subsection{Proof of theorem \ref{thm:blancing_iclub}} 

To prove the Theorem \ref{thm:blancing_iclub}, we first prove the following lemma and proposition.
\begin{lemma}
    Let $\Phi$ be a fixed representation function. Given that $q(W_{t+1} \mid \Phi(\mathbf{H}_t)) $ is the conditional likelihood of observing the treatment $W_{t+1}$, denote the probability of observing each treatment value as $q^j=q(\Phi(\mathbf{H}_t))\coloneqq q(W_{t+1} = j \mid \Phi(\mathbf{H}_t))$ for $j \in \{0,1,\dots, K-1\}$. Then, the optimal treatment prediction function is such that 
    \begin{equation}
        q^{j, *}(\Phi(\mathbf{H}_t) ) = \frac{p(\Phi(\mathbf{H}_t)\mid W_{t+1} = j)}{\sum_{l=0}^{K-1}p(\Phi(\mathbf{H}_t)\mid W_{t+1} = l)p(W_{t+1} = l)}
    \end{equation}
    \label{lem: optimal_q}
\end{lemma}
\begin{proof}
    For a fixed representation \(\Phi\), finding the optimal treatment probabilities reduces to solving the following constrained optimization problem:
\begin{equation}
    \begin{aligned}
        \max_{q} \;\; & \mathbb{E}_{\mathbb{P}(\Phi(\mathbf{H}_t), W_{t+1})} 
        \left[ \log q(W_{t+1} \mid \Phi(\mathbf{H}_t)) \right] \\
        \textrm{subject to} \;\; & \sum_{l=0}^{K-1} q^l(\Phi(\mathbf{H}_t)) = 1.
    \end{aligned}
    \label{eq:max_treat_constrained}
\end{equation}
First, we write the likelihood $q(W_{t+1} \mid \Phi(\mathbf{H}_t))$ using the conditional probabilities $q^j(\Phi(\mathbf{H}_t))$.
\begin{equation*}
    q(W_{t+1} \mid \Phi(\mathbf{H}_t)) = \prod_{j=0}^{K-1}q^j(\Phi(\mathbf{H}_t))^{\indicator{W_{t+1}=j}}
\end{equation*}
Then, the treatment likelihood can be written as   
\begin{align*}
    \mathbb{E}_{\mathbb{P}(\Phi(\mathbf{H}_t), W_{t+1})} \left[ \log q(W_{t+1} \mid \Phi(\mathbf{H}_t)) \right] 
    &=  \mathbb{E}_{\mathbb{P}(\Phi(\mathbf{H}_t), W_{t+1})} \left[ \sum_{l=0}^{K-1} \log(q^{l}(\Phi(\mathbf{H}_t))) \mathbb{1}_{\{W_{t+1}=l\}} \right] \\
    &=  \sum_{l=0}^{K-1} \int \log(q^{l}(\Phi(\mathbf{H}_t))) \mathbb{1}_{\{W_{t+1}=l\}}\, p(W_{t+1} \mid \Phi(\mathbf{H}_t))\, p(\Phi(\mathbf{H}_t))\, dW_{t+1}\, d\Phi(\mathbf{H}_t) \\
    &= \sum_{l=0}^{K-1} \int \log(q^{l}(\Phi(\mathbf{H}_t)))\, p(W_{t+1} = l \mid \Phi(\mathbf{H}_t))\, p(\Phi(\mathbf{H}_t))\, d\Phi(\mathbf{H}_t) \\
    &= \sum_{l=0}^{K-1} \int \log(q^{l}(\Phi(\mathbf{H}_t)))\, p(\Phi(\mathbf{H}_t) \mid W_{t+1} = l)\, p(W_{t+1} = l)\, d\Phi(\mathbf{H}_t)
\end{align*}
Let's denote $\alpha_l = p(W_{t+1} = l)$,  the marginal probability of observing the $l$-th treatment regime, and $p_{l}^{\Phi}(\mathbf{H}_t) = p(\Phi(\mathbf{H}_t)\mid W_{t+1} = l )$ with a corresponding probability distribution $\mathbb{P}_{l}^{\Phi}$.  We intend to maximize point-wise the objective in Eq. \eqref{eq:max_treat_constrained}. Plugging the latter formulation of the conditional likelihood in Eq. \eqref{eq:max_treat_constrained}  and writing the Lagrangian function, we get
\begin{equation}
    \max_{q} \sum_{l=0}^{K-1} \log(q^{l}(\Phi(\mathbf{H}_t))p_{j}^{\Phi}(\mathbf{H}_t) \alpha_l + \lambda (\sum_{l=0}^{K-1}q^{l}(\Phi(\mathbf{H}_t)) - 1)  
\end{equation}
Computing the gradient w.r.t $q^{l}(\Phi(\mathbf{H}_t))$ for  $l \in \{0,1,\dots, K-1\}$ and setting to zero, we have
\begin{equation}
    q^{l, *}(\Phi(\mathbf{H}_t)) = -\frac{\alpha_l p_{j}^{\Phi}(\mathbf{H}_t)}{\lambda}
\end{equation}
Then, by the equality constraint, we find that $\lambda = -\sum_{l=0}^{K-1}\alpha_l p_{j}^{\Phi}(\mathbf{H}_t)$.
\end{proof}
\begin{proposition}
\label{prop:iclub_form}
    Let $\Phi$ be a fixed representation function.  The $I_{CLUB}$ objective when the treatment prediction function is optimal (i.e. $ q=q^{*})$ has the following form: 
     \begin{equation}
I_{CLUB} = \sum_{j=0}^{K-1}\alpha_l D_{KL}(\mathbb{P}_j^{\Phi}|| \sum_{l=0}^{K-1}\alpha_l \mathbb{P}_l^{\Phi}) 
+ \mathbb{E}_{\mathbb{P}_{\Phi(\mathbf{H}_t)}}\left[ D_{KL}(\mathbb{P}_{W_{t+1}}||\mathbb{P}_{W_{t+1}|\Phi(\mathbf{H}_t)} )  \right]
         \label{eq:i_club_optimal_q}
     \end{equation}
\end{proposition}
\begin{proof}
 First, recall that
\begin{equation*}
    \begin{aligned}
        I_{\mathrm{CLUB}}(\Phi(\mathbf{H}_t), W_{t+1}; q^*) 
        &= \mathbb{E}_{\mathbb{P}_{(\Phi(\mathbf{H}_{t+1}), W_{t+1})}}
        \left[ \log q^*(W_{t+1} \mid \Phi(\mathbf{H}_{t+1})) \right] \\
        &\quad - \mathbb{E}_{\mathbb{P}_{\Phi(\mathbf{H}_{t+1})}}
        \mathbb{E}_{\mathbb{P}_{W_{t+1}}}
        \left[ \log q^*(W_{t+1} \mid \Phi(\mathbf{H}_{t+1})) \right].
    \end{aligned}
\end{equation*}
\begin{equation*}
        I_{\text{CLUB}}(\Phi(\mathbf{H}_t), W_{t+1}; q^{*}) =  A - B
    \end{equation*}
    Let's detail $A$ and $B$ separately, 
    \begin{equation*}
        \begin{aligned}
        A &= \sum_{j=0}^{K-1} \int \alpha_j \log(q^{l, *}(\Phi(\mathbf{H}_t)) p_{j}^{\Phi}(\mathbf{H}_t) d\Phi(\mathbf{H}_t) \\ 
        &= \sum_{j=0}^{K-1} \int\alpha_j \log(\frac{\alpha_j p_{j}^{\Phi}(\mathbf{H}_t)}{\sum_{l=0}^{K-1}p_{l}^{\Phi}(\mathbf{H}_t)\alpha_l}) p_{j}^{\Phi}(\mathbf{H}_t) d\Phi(\mathbf{H}_t) \\ 
        &= \sum_{j=0}^{K-1} \int \alpha_j \log(\frac{p_{j}^{\Phi}(\mathbf{H}_t)}{\sum_{l=0}^{K-1}p_{l}^{\Phi}(\mathbf{H}_t)\alpha_l}) p_{j}^{\Phi}(\mathbf{H}_t) d\Phi(\mathbf{H}_t) +\log(\alpha_j)\alpha_j \\
         &= \sum_{j=0}^{K-1} \alpha_j D_{KL}(\mathbb{P}_j^{\Phi}|| \sum_{l=0}^{K-1}\alpha_l \mathbb{P}_l^{\Phi}) +  \sum_{j=0}^{K-1} \log(\alpha_j)\alpha_j \\ 
        \end{aligned}
    \end{equation*}

    Finally, we can write 
    \begin{equation}
    A = \sum_{j=0}^{K-1} \alpha_j D_{KL}(\mathbb{P}_j^{\Phi}|| \sum_{l=0}^{K-1}\alpha_l \mathbb{P}_l^{\Phi})  - H(W_{t+1}) 
        \label{eq:A_final_form}
    \end{equation}
    For the remaining term $B$, we have
     \begin{equation*}
        \begin{aligned}
        B &= \mathbb{E}_{\mathbb{P}_{\Phi(\mathbf{H}_t)}}\mathbb{E}_{\mathbb{P}_{W_{t+1}}}\left( \log q^{*}(W_{t+1} \mid \Phi(\mathbf{H}_{t+1})) \right] \\ 
        &= \sum_{j=0}^{K-1} \mathbb{E}_{\mathbb{P}_{\Phi(\mathbf{H}_t)}} \mathbb{E}_{\mathbb{P}_{W_{t+1}}} \left[ \log(q^{j}(\Phi(\mathbf{H}_t))) \mathbb{1}_{\{W_{t+1}=j\}} \right] \\ 
        &= \sum_{j=0}^{K-1} \mathbb{E}_{\mathbb{P}_{\Phi(\mathbf{H}_t)}}\left[ \alpha_j \log(q^{j}(\Phi(\mathbf{H}_t)))\right] \\ 
        &= \sum_{j=0}^{K-1}\alpha_j \int \log\left[ \frac{\alpha_j p_{j}^{\Phi}(\mathbf{H}_t)}{\sum_{l=0}^{K-1}p_{l}^{\Phi}(\mathbf{H}_t)\alpha_l}\right]p(\Phi(\mathbf{H}_t))d\Phi(\mathbf{H}_t) \\ 
       &= \sum_{j=0}^{K-1}\alpha_j \int \log\left[ \frac{p(\Phi(\mathbf{H}_t))}{\sum_{l=0}^{K-1}p_{l}^{\Phi}(\mathbf{H}_t)\alpha_l} \frac{p(W_{t+1} =j \mid \Phi(\mathbf{H}_t))}{p(W_{t+1} =j)}\right]p(\Phi(\mathbf{H}_t))d\Phi(\mathbf{H}_t)\\ 
       &- H(W_{t+1})  \\ 
       &= \sum_{j=0}^{K-1}\alpha_j \int \underbrace{\log\left[ \frac{p(\Phi(\mathbf{H}_t))}{\sum_{l=0}^{K-1}p_{l}^{\Phi}(\mathbf{H}_t)\alpha_l}\right]}_{=0}p(\Phi(\mathbf{H}_t))d\Phi(\mathbf{H}_t) \\ 
        &+ \sum_{j=0}^{K-1}\alpha_j \int \log\left[\frac{p(W_{t+1} =j \mid \Phi(\mathbf{H}_t))}{p(W_{t+1} =j)}\right] p(\Phi(\mathbf{H}_t))d\Phi(\mathbf{H}_t) - H(W_{t+1}) \\
        \end{aligned}
    \end{equation*}
    The final form of $B$ is therefore 
    \begin{equation}
    B = - \int D_{KL}(\mathbb{P}_{W_{t+1}}| \mathbb{P}_{W_{t+1}| \Phi(\mathbf{H}_t)})p(\Phi(\mathbf{H}_t)) d\Phi(\mathbf{H}_t)
       - H(W_{t+1}) 
        \label{eq:B_final_form}
    \end{equation}
    The proposition follows immediately from Equations \eqref{eq:A_final_form} and \eqref{eq:B_final_form}.
\end{proof}

\begin{proof}(Theorem \ref{thm:blancing_iclub})
Since by lemma \ref{lem: optimal_q}, the $I_{CLUB}$ formulation in  proposition \ref{prop:iclub_form} holds, then to prove that the representation is balanced, it is enough to see that by the positivity of $D_{KL}$

\begin{equation}
\label{eq:iclub_ineq_at_optimal}
    I_{CLUB} \geq  \mathbb{E}_{\mathbb{P}_{\Phi(\mathbf{H}_t)}}\left[ D_{KL}(\mathbb{P}_{W_{t+1}}||\mathbb{P}_{W_{t+1}|\Phi(\mathbf{H}_t)} )\right] \geq 0  
\end{equation}
$I_{CLUB}$ is minimal when $I_{CLUB} =0$, which happens if and only if for $j \in \{0,1,\dots, K-1\}$  $p(W_{t+1} =j ) = p(W_{t+1} =j \mid \Phi(\mathbf{H}_t))$ almost surely which, by Bayes rule is equivalent to say $p(\Phi(\mathbf{H}_t)) = p(\Phi(\mathbf{H}_t) \mid W_{t+1} =j) $.
% To prove inequality  in \eqref{eq:iclub_ineq_at_optimal}, we use that fact the Keullbeick Leibler divergence $(p, q) \rightarrow D(p||q)$ is convex over the pair of the probability distributions so that we have the property 

% \begin{equation*}
%     D(\sum_{j=0}^{K-1}\lambda_j p_j||\sum_{j=0}^{K-1}\lambda_jq_j) \leq \sum_{j=0}^{K-1}\lambda_j D(p_j||q_j)
% \end{equation*}
%     such that $ 0 \leq \lambda_j \leq 1 $ and $\sum_{j=0}^{K-1}\lambda_j=1$. 

%     Going back to our $I_{CLUB}$ formulation in Eq. \eqref{eq:i_club_optimal_q} we have 
%     \begin{equation}
%     \begin{aligned}
%         D_{KL}(p^{\Phi}||  \sum_{l=0}^{K-1}\alpha_l p_l^{\Phi}) &= D_{KL}(p^{\Phi}||  \sum_{l=0}^{K-1}\alpha_l p_l^{\Phi}) \\ 
%         & = D_{KL}(p^{\Phi}||  \sum_{l=0}^{K-1}\alpha_l p_l^{\Phi}) &= D_{KL}(p^{\Phi}||  \sum_{l=0}^{K-1}\alpha_l p_l^{\Phi})
%         \end{aligned}
        
%     \end{equation}
    
\end{proof}
% \section{Causal CPC Pseudo algorithm}
% \label{appendix_ccpc:alg_ccpc}
% In this section, we present a detailed overview of the training procedure for Causal CPC. Initially, we train the Encoder using only the contrastive terms, as outlined in Algorithm \ref{alg:enc_pretraining}. Our primary objective is to ensure that, for each time step $t$, the process history $\mathbf{H}_{t}$ is predictive of future local features $\mathbf{Z}_t$. However, calculating the InfoNCE loss for a batch across all possible time steps $t=0, \dots, t_{\text{max}}$ can be computationally demanding.

% To address this, we adopt a more efficient approach by uniformly sampling a single time step $t$ per batch. Subsequently, the corresponding process history $\mathbf{H}_{t}$ is contrasted. The sampled $\mathbf{H}_{t}$ is then employed as input for the InfoMax objective and randomly partitioned into future $\mathbf{H}_t^f$ and past $\mathbf{H}_t^h$ sub-processes.
% \begin{algorithm}
%    \caption{Pretraining of the encoder}
%    \label{alg:enc_pretraining}
%    \begingroup
%    \let\AND\relax % Temporarily remove the \AND command
% \begin{algorithmic}
%    \REQUIRE Encoder parameters $\theta_{1,2,3}$, learning rate $\mu$
%    \STATE {\bfseries Input:} data $\{\mathbf{H}_{i, t_{max}}, i=1,\dots, N \}$ 
%     \FOR{$p \in \{1, \dots,\mathrm{epoch_{max}}\}$} 
%             \FOR{$\mathcal{B}=\{ \mathbf{H}_{i, t_{max}}, i=1,\dots, |\mathcal{B}| \}$}
%                     \STATE $\mathbf{Z}_t = \Phi_{\theta_1}([\mathbf{X}_{t}, W_{t-1}, Y_{t-1}])$ for $t=0, \dots, t_{max}$.
%                     \STATE Choose $t \sim \mathcal{U}([1, t_{max}-1])$.
%                     \STATE Compute $\mathbf{C}_t^{\mathrm{enc}} = \Phi_{\theta_{1},\theta_{2}}(\mathbf{H}_{t})$.
%                     \STATE  Compute $\mathcal{L}^{CPC}(\theta_{1},\theta_{2}, \{\Gamma_j\}_{j=1}^{\rho})$.
%                     \STATE  Choose $t_0 \sim \mathcal{U}([1, t])$.
%                     \STATE  Compute $\mathbf{C}_t^{\mathrm{enc},h}=\Phi_{\theta_{1},\theta_{2}}(\mathbf{H}_t^h), \mathbf{C}_t^{\mathrm{enc},f}=\Phi_{\theta_{1},\theta_{2}}(\mathbf{H}_t^f)$,
%                     \STATE Compute $\mathcal{L}^{(InfoMax)}(\theta_{1},\theta_{2}, \gamma)$.
%                     \STATE Update parameters
%                     $$\theta_{1,2,3} \leftarrow  \theta_{1,2,3} - \mu  \left( \frac{\partial \mathcal{L}^{CPC}(\theta_{1},\theta_{2}, \{\Gamma_j\}_{j=1}^{\rho})}{\partial \theta_{1,2,3} } + \frac{\partial \mathcal{L}^{(InfoMax)}(\theta_{1},\theta_{2}, \gamma)}{\partial \theta_{1,2,3} } \right  ) $$
%             \ENDFOR
%     \ENDFOR
%    \STATE \textbf{Return}: Trained encoder.
% \end{algorithmic}
%    \endgroup % End of local group, restoring \AND
% \end{algorithm}

% The decoder is trained while taking the encoder as input (Algorithm \ref{alg:dec_training}), utilizing a lower learning rate compared to the untrained part of the decoder. It is trained autoregressively and without teacher forcing. This implies that for each time step $t$, our GRU-based decoder should predict the future sequence of treatments $\hat{Y}_{t+1:t+\rho}$ with its hidden state initialized to the representation $\mathbf{\Phi}_t$ of the historical process up to time $t$.

% To enhance training efficiency, instead of predicting $\hat{Y}_{i,t+1:t+\rho}$ for all individuals $i$ in a batch and for all possible time steps $t$, we randomly select $m$ time indices $t_{i,1}, \dots, t_{i,m}$ for each individual $i$. From these indices, we compute future treatment response sequences $\hat{Y}_{i,t_{i,1}+1:t_{i,1}+\rho}, \dots, \hat{Y}_{i,t_{i,m}+1:t_{i,m}+\rho}$.  We found that is enough to train while selecting randomly 10\% of the time steps.
% \begin{algorithm}
%    \caption{Training of the decoder}
%    \label{alg:dec_training}
%    \begingroup
%    \let\AND\relax % Temporarily remove the \AND command
% \begin{algorithmic}
%    \REQUIRE Encoder parameters $\theta_{1,2,3}$, Decoder parameters $\theta_{4}, \theta_{Y}, \theta_{W}$.
%    \REQUIRE Encoder learning rate $\mu_{enc}$, Treatment learning rate $\mu_{W}$, Outcome learning rate $\mu_{Y}$.
%    \REQUIRE Number of random time indices $m$.
%    \STATE {\bfseries Input:} data $\{\mathbf{H}_{i, t_{max}}, i=1,\dots, N \}$ 
%     \FOR{$p \in \{1, \dots,\mathrm{epoch_{max}}\}$} 
%             \FOR{$\mathcal{B}=\{ \mathbf{H}_{i, t_{max}}, i=1,\dots, |\mathcal{B}| \}$}
%                     \STATE Compute $\mathbf{C}_{i, t} = \mathrm{encoder}(\mathbf{H}_{i, t})$ for $t=0, \dots, t_{max}$, $i=1,\dots, |\mathcal{B}| $.
%                     \STATE Compute $\mathbf{\Phi}_t = \mathbf{\Phi}_{\theta_R}(\mathbf{H}_t)$.
%                     \FOR{$i=1,\dots, |\mathcal{B}| $}
%                             \STATE Choose $t_{i,1}, \dots, t_{i,m} \sim \mathcal{U}([1, t_{max}-\rho]) $.
%                             \FOR{$t  \in  \{ t_{i,1}, \dots, t_{i,m}\}$}
%                                     \STATE Compute $\hat{Y}_{i,t+1:t+\rho}, \hat{W}_{i,t+1:t+\rho}, \mathbf{\Phi}_{i,t+1:t+\rho-1} = \mathrm{decoder}(\mathbf{\Phi}_t, \mathbf{V}_i, W_{i,t}, Y_{i,t}, W_{i,t+1:t+\rho}) $
%                             \ENDFOR
%                     \ENDFOR
%                     \STATE Compute  $\mathcal{L}_{dec}(\theta_{R}, \theta_{Y}, \theta_{W})$ and $\mathcal{L}_{W}(\theta_{W}, \theta_{R})$.
%                     \STATE Update parameters in the order:
%                     $$\theta_{1,2,3} \leftarrow  \theta_{1,2,3} - \mu_{enc}  \left( \frac{\partial \mathcal{L}_{dec}(\theta_{R}, \theta_{Y}, \theta_{W})}{\partial \theta_{1,2,3} }\right  ) $$
%                     $$\theta_{4, Y} \leftarrow  \theta_{4, Y}  - \mu_{Y}  \left( \frac{\partial \mathcal{L}_{dec}(\theta_{R}, \theta_{Y}, \theta_{W})}{\partial \theta_{4, Y}  }\right  ) $$                     
%                     $$\theta_{W} \leftarrow  \theta_{W}  - \mu_{W}  \left( \frac{\partial  \mathcal{L}_{W}(\theta_{W}, \theta_{R}) }{\partial \theta_{W} }\right  ) $$
%             \ENDFOR
%     \ENDFOR
%    \STATE \textbf{Return}: Trained decoder.
% \end{algorithmic}
%    \endgroup % End of local group, restoring \AND
% \end{algorithm}

\section{Causal CPC: Architecture details}
\label{appendix_ccpc:archi_ccpc}
\begin{table}[!htbp]
\centering
\begin{tabular}{c}
\hline \textbf{Inputs}: $[\mathbf{X}_{t}, W_{t-1}, Y_{t-1}]$\\
\hline Linear Layer\\
\hline WeightNorm\\
\hline SELU\\
\hline Linear Layer  \\
\hline WeightNorm\\
\hline \textbf{Outputs}: $\mathbf{Z}_t = \Phi_{\theta_1}([\mathbf{X}_{t}, W_{t-1}, Y_{t-1}])$\\
\end{tabular}
\caption{Architecture for learning local features $\mathbf{Z}_t$}
\label{tab: archi_loc_feat}
\end{table}


\begin{table}[!htbp]
\centering
\begin{tabular}{c}
\hline \textbf{Inputs}: $\mathbf{Z}_{\leq t}$\\
\hline GRU (1 layer)\\
\hline \textbf{Outputs}: Hidden state $\mathbf{C}_t^{\mathrm{enc}} = \Phi_{\theta_2}^{ar}(\mathbf{Z}_{\leq t})$\\
\end{tabular}
\caption{Architecture for learning context representation $\mathbf{C}_t^{\mathrm{enc}}$ }
\label{tab: archi_context }
\end{table}

\begin{table}[!htbp]
\centering
\begin{tabular}{c}
\hline \textbf{Inputs}: $[\mathbf{\Phi}_t, W_t]$\\
\hline Linear Layer\\
\hline WeightNorm\\
\hline SELU\\
\hline Linear Layer  \\
\hline WeightNorm\\
\hline \textbf{Outputs}: $\hat{Y}_t$\\
\end{tabular}
\caption{Architecture for outcome prediction}
\label{tab: archi_outc_pred}
\end{table}


\begin{table}[!htbp]
\centering
\begin{tabular}{c}
\hline \textbf{Inputs}: $\mathbf{\Phi}_t$\\
\hline Linear Layer\\
\hline SpectralNorm\\
\hline SELU\\
\hline Linear Layer  \\
\hline SpectralNorm\\
\hline \textbf{Outputs}: $\hat{W}_t$\\
\end{tabular}
\caption{Architecture for treatment prediction}
\label{tab: archi_treat_pred}
\end{table}


\newpage
\section{Models hyperparameters}
\label{appendix_ccpc:huperparams_details}

In this section, we report the range of all hyperparameters to be fine-tuned, as well as fixed hyperparameters for all models and across the different datasets used in experiments. Best hyperparameter values are reported in the configuration files in the code repository.

% \begin{table}[!htbp]
% \centering
% \caption{Hyper-parameters search range for RMSN}
% \resizebox{0.9\textwidth}{!}{%
% \begin{tabular}{|c|c|c|c|c|}
% \hline
% \textbf{Model} & \textbf{Sub-model} & \textbf{Hyperparameter} & \textbf{Cancer simulation} & \textbf{MIMIC III (SS)}\\
% \hline
% \multirow{RMSNs} 
% & \multirow{Propensity Treatment Network} 
% & LSTM layers & 1 & 1 \\
% %\cline{3-6}
% & & Learning rate & $0.01,0.005, 0.001, 0.0001$ & $0.01,0.005, 0.001, 0.0001$\\
% %\cline{3-6}
% & & Batch size & $32, 64, 128$ & $32, 64, 128$ \\
% %\cline{3-6}
% & & LSTM hidden units & $4,6, \dots, 12$ & $4,6, \dots, 30$ \\
% %\cline{3-6}
% & & LSTM dropout rate & - & - \\
% %\cline{3-6}
% & & Max gradient norm & $0.5,1,2$ & $0.5,1,2$ \\
%  & & Early Stopping (min delta)& 0.0001& 0.0001 \\
%  & & Early Stopping (patience)& 30& 30 \\
% \hline
% & \multirow{Propensity History Network} 
% & LSTM layers & 1 & 1 \\
% %\cline{3-6}
% & & Learning rate & $0.01,0.005, 0.001, 0.0001$ & $0.01,0.005, 0.001, 0.0001$ \\
% %\cline{3-6}
% & & Batch size & $32, 64, 128$ & $64,128,256$  \\
% %\cline{3-6}
% & & LSTM hidden units & $4,6, \dots, 20$ &  $4,6, \dots, 30$\\
% %\cline{3-6}
% & & LSTM dropout rate & - & - \\
% & & Early Stopping (min delta)& 0.0001& 0.0001 \\
% & & Early Stopping (patience)& 30& 30 \\
% \hline
% & \multirow{Encoder} 
% & LSTM layers & 1 & 1  \\
% %\cline{3-6}
% & & Learning rate & $0.01,0.005, 0.001, 0.0001$ & $0.01,0.005, 0.001, 0.0001$  \\
% %\cline{3-6}
% & & Batch size & $32, 64, 128$ & $32, 64, 128$ \\
% %\cline{3-6}
% & & LSTM hidden units & $4,6, \dots, 20$ &  $4,6, \dots, 30$ \\
% %\cline{3-6}
% & & LSTM dropout rate & - & - \\
%  & & Early Stopping (min delta)& 0.0001& 0.0001 \\
%  & & Early Stopping (patience) & 30 &  30 \\
% \hline
% &  Decoder & LSTM layers & 1& 1  \\
% %\cline{3-6}
% & & Learning rate & $0.01,0.005, 0.001, 0.0001$ & $0.01,0.005, 0.001, 0.0001$ \\
% %\cline{3-6}
% & & Batch size & $32, 64, 128$ & $128, 512,1024$ \\
% %\cline{3-6}
% & & LSTM hidden units & $4,6, \dots, 20$ & $4,6, \dots, 30$ \\
% %\cline{3-6}
% & & LSTM dropout rate& -& - \\
% %\cline{3-6}
% & & Max gradient norm& $0.5,1,2$ & $0.5,1,2$  \\
%  & & Early Stopping (min delta)& 0.0001& 0.0001 \\
%  & & Early Stopping (patience)& 30& 30 \\
% \hline
% \end{tabular}%
% }
% \end{table}
\begin{table}[!htbp]
\centering
\caption{Hyper-parameters search range for RMSN}
\resizebox{0.9\textwidth}{!}{%
\begin{tabular}{|c|c|c|c|c|}
\hline
\textbf{Model} & \textbf{Sub-model} & \textbf{Hyperparameter} & \textbf{Cancer simulation} & \textbf{MIMIC III (SS)} \\
\hline
\multirow{7}{*}{RMSNs} 
& \multirow{7}{*}{Propensity Treatment Network} 
& LSTM layers & 1 & 1 \\
\cline{3-5}
& & Learning rate & $0.01, 0.005, 0.001, 0.0001$ & $0.01, 0.005, 0.001, 0.0001$ \\
\cline{3-5}
& & Batch size & $32, 64, 128$ & $32, 64, 128$ \\
\cline{3-5}
& & LSTM hidden units & $4, 6, \dots, 12$ & $4, 6, \dots, 30$ \\
\cline{3-5}
& & LSTM dropout rate & - & - \\
\cline{3-5}
& & Max gradient norm & $0.5, 1, 2$ & $0.5, 1, 2$ \\
\cline{3-5}
& & Early Stopping (min delta) & 0.0001 & 0.0001 \\
\cline{3-5}
& & Early Stopping (patience) & 30 & 30 \\
\hline
\multirow{6}{*}{Propensity History Network} 
& & LSTM layers & 1 & 1 \\
\cline{3-5}
& & Learning rate & $0.01, 0.005, 0.001, 0.0001$ & $0.01, 0.005, 0.001, 0.0001$ \\
\cline{3-5}
& & Batch size & $32, 64, 128$ & $64, 128, 256$ \\
\cline{3-5}
& & LSTM hidden units & $4, 6, \dots, 20$ & $4, 6, \dots, 30$ \\
\cline{3-5}
& & LSTM dropout rate & - & - \\
\cline{3-5}
& & Early Stopping (min delta) & 0.0001 & 0.0001 \\
\cline{3-5}
& & Early Stopping (patience) & 30 & 30 \\
\hline
\multirow{6}{*}{Encoder} 
& & LSTM layers & 1 & 1 \\
\cline{3-5}
& & Learning rate & $0.01, 0.005, 0.001, 0.0001$ & $0.01, 0.005, 0.001, 0.0001$ \\
\cline{3-5}
& & Batch size & $32, 64, 128$ & $32, 64, 128$ \\
\cline{3-5}
& & LSTM hidden units & $4, 6, \dots, 20$ & $4, 6, \dots, 30$ \\
\cline{3-5}
& & LSTM dropout rate & - & - \\
\cline{3-5}
& & Early Stopping (min delta) & 0.0001 & 0.0001 \\
\cline{3-5}
& & Early Stopping (patience) & 30 & 30 \\
\hline
\multirow{6}{*}{Decoder} 
& & LSTM layers & 1 & 1 \\
\cline{3-5}
& & Learning rate & $0.01, 0.005, 0.001, 0.0001$ & $0.01, 0.005, 0.001, 0.0001$ \\
\cline{3-5}
& & Batch size & $32, 64, 128$ & $128, 512, 1024$ \\
\cline{3-5}
& & LSTM hidden units & $4, 6, \dots, 20$ & $4, 6, \dots, 30$ \\
\cline{3-5}
& & LSTM dropout rate & - & - \\
\cline{3-5}
& & Max gradient norm & $0.5, 1, 2$ & $0.5, 1, 2$ \\
\cline{3-5}
& & Early Stopping (min delta) & 0.0001 & 0.0001 \\
\cline{3-5}
& & Early Stopping (patience) & 30 & 30 \\
\hline
\end{tabular}%
}
\end{table}

% \begin{table}[!htbp]
% \centering
% \caption{Hyper-parameters search range for CRN}
% \resizebox{0.7\textwidth}{!}{%
% \begin{tabular}{|c|c|c|c|c|}
% \hline
% \textbf{Model} & \textbf{Sub-model} & \textbf{Hyperparameter} & \textbf{Cancer simulation} & \textbf{MIMIC III (SS)} \\
% \hline
% \multirow{CRN} 
% & \multirow{Encoder} 
% & LSTM layers & 1 & 1 \\
% %\cline{3-6}
% & & Learning rate & $0.01,0.005, 0.001, 0.0001$ &$0.01,0.005, 0.001, 0.0001$ \\
% %\cline{3-6}
% & & Batch size & $32, 64, 128$ & $32, 64, 128$ \\
% %\cline{3-6}
% & & LSTM hidden units & $4,6, \dots, 30$&  $4,6, \dots, 30$ \\
% %\cline{3-6}
% & & LSTM dropout rate & - & - \\
% %\cline{3-6}
% & & BR size & $4,6, \dots, 20$  & $4,6, \dots, 30$\\
% & & Early Stopping (min delta)& 0.0001  & 0.0001\\
% & & Early Stopping (patience)& 30 &  30\\
% \hline
% & \textbf{Decoder} & LSTM layers & 1 & 1\\
% %\cline{3-6}
% & & Learning rate & $0.01,0.005, 0.001, 0.0001$ & $0.01,0.005, 0.001, 0.0001$\\
% %\cline{3-6}
% & & Batch size & $128,256,512$& $256,512,1024$ \\
%  %%\cline{3-6}
% & & LSTM hidden units & $4,6, \dots, 30$& $4,6, \dots, 30$  \\
%  %%\cline{3-6}
% & & LSTM dropout rate& - & -  \\
%  %%\cline{3-6}
%  & & BR size & $4,6, \dots, 20$& $4,6, \dots, 30$ \\
%   & & Early Stopping (min delta)& 0.0001&  0.0001\\
%  & & Early Stopping (patience)& 30& 30\\
% \hline
% \end{tabular}%
% }
% \end{table}

\begin{table}[!htbp]
\centering
\caption{Hyper-parameters search range for CRN}
\resizebox{0.7\textwidth}{!}{%
\begin{tabular}{|c|c|c|c|c|}
\hline
\textbf{Model} & \textbf{Sub-model} & \textbf{Hyperparameter} & \textbf{Cancer simulation} & \textbf{MIMIC III (SS)} \\
\hline
\multirow{8}{*}{CRN} 
& \multirow{8}{*}{Encoder} 
& LSTM layers & 1 & 1 \\
\cline{3-5}
& & Learning rate & $0.01, 0.005, 0.001, 0.0001$ & $0.01, 0.005, 0.001, 0.0001$ \\
\cline{3-5}
& & Batch size & $32, 64, 128$ & $32, 64, 128$ \\
\cline{3-5}
& & LSTM hidden units & $4, 6, \dots, 30$ & $4, 6, \dots, 30$ \\
\cline{3-5}
& & LSTM dropout rate & - & - \\
\cline{3-5}
& & BR size & $4, 6, \dots, 20$ & $4, 6, \dots, 30$ \\
\cline{3-5}
& & Early Stopping (min delta) & 0.0001 & 0.0001 \\
\cline{3-5}
& & Early Stopping (patience) & 30 & 30 \\
\hline
\multirow{7}{*}{Decoder} 
& & LSTM layers & 1 & 1 \\
\cline{3-5}
& & Learning rate & $0.01, 0.005, 0.001, 0.0001$ & $0.01, 0.005, 0.001, 0.0001$ \\
\cline{3-5}
& & Batch size & $128, 256, 512$ & $256, 512, 1024$ \\
\cline{3-5}
& & LSTM hidden units & $4, 6, \dots, 30$ & $4, 6, \dots, 30$ \\
\cline{3-5}
& & LSTM dropout rate & - & - \\
\cline{3-5}
& & BR size & $4, 6, \dots, 20$ & $4, 6, \dots, 30$ \\
\cline{3-5}
& & Early Stopping (min delta) & 0.0001 & 0.0001 \\
\cline{3-5}
& & Early Stopping (patience) & 30 & 30 \\
\hline
\end{tabular}%
}
\end{table}


\begin{table}[!htbp]
\centering
\caption{Hyper-parameters search range for G-Net}
\resizebox{0.7\textwidth}{!}{%
\begin{tabular}{|c|c|c|}
\hline
\textbf{Hyperparameter} & \textbf{Cancer simulation} & \textbf{MIMIC III (SS)} \\
\hline
LSTM layers & 1 & 1  \\
 %\cline{1-4}
Learning rate & $0.01,0.005, 0.001, 0.0001$ &  $0.01,0.005, 0.001, 0.0001$ \\
 % %\cline{1-4}
Batch size & $32, 64, 128$ &  $32, 64, 128$ \\
 %\cline{1-4}
LSTM hidden units & $4,6, \dots, 30$ & $4,6, \dots, 30$ \\
%\cline{1-4}
FC hidden units & $4,6, \dots, 30$ &  $4,6, \dots, 30$ \\
 %\cline{1-4}
LSTM dropout rate & - & -  \\
 %\cline{1-4}
R size& $4,6, \dots, 20$& $4,6, \dots, 30$ \\
 %\cline{1-4}
MC samples & 10 & 10 \\
Early Stopping (min delta)& 0.0001&  0.0001\\
Early Stopping (patience)& 30& 30 \\
\cline{1-3}
\end{tabular}%
}
\end{table}




\begin{table}[!htbp]
\centering
\caption{Hyper-parameters search range for Causal Transfomer}
\resizebox{0.7\textwidth}{!}{%
\begin{tabular}{|c|c|c|}
\hline
\textbf{Hyperparameter} & \textbf{Cancer simulation} & \textbf{MIMIC III (SS)} \\
\hline
Transformer blocks & 1 & 1 \\
 %\cline{1-4}
Learning rate & $0.01,0.005, 0.001, 0.0001$ & $0.01,0.005, 0.001, 0.0001$  \\
 %\cline{1-4}
Batch size & $32, 64, 128$ & $32, 64, 128$ \\
 %\cline{1-4}
Attention heads & $2$ & $2$ \\
 %\cline{1-4}
Transformer units & $4,6, \dots, 20$& $4,6, \dots, 20$ \\
 %\cline{1-4}
LSTM dropout rate & -  & - \\
%\cline{1-4}
BR size& $4,6, \dots, 20$&  $4,6, \dots, 20$ \\
%\cline{1-4}
FC hidden units & $4,6, \dots, 20$&   $4,6, \dots, 20$ \\
Sequential dropout rate & $0.1,0.2, 0.3$& $0.1,0.2, 0.3$ \\
Max positional encoding & $15$& $15$  \\
Early Stopping (min delta)& 0.0001& 0.0001 \\
Early Stopping (patience)& 30& 30 \\
\cline{1-3}
\end{tabular}%
}
\end{table}



% \begin{table}[!htbp]
% \centering
% \caption{Hyper-parameters search range for Causal CPC}
% \resizebox{0.9\textwidth}{!}{%
% \begin{tabular}{|c|c|c|c|c|}
% \hline
% \textbf{Model} & \textbf{Sub-model} & \textbf{Hyperparameter} & \textbf{Cancer simulation} & \textbf{MIMIC III (SS)} \\
% \hline
% \multirow{Causal CPC}& \multirow{Encoder} 
% & GRU layers& 1 & 1 \\
% %\cline{3-6}
% & & Learning rate & $0.01,0.005, 0.001, 0.0001$ & $0.01,0.005, 0.001, 0.0001$ \\
% %\cline{3-6}
% & & Batch size & $32, 64, 128$ & $64, 128, 256$  \\
% %\cline{3-6}
% & & GRU hidden units& $4,6, \dots, 30$ & $4,6, \dots, 30$ \\
% %\cline{3-6}
% & & GRU dropout rate    & - & - \\
% %\cline{3-6}
%  & & Local features (LF) size& $4,6, \dots, 20$& $4,6, \dots, 20$\\
%  & & Context Representation (CR) size& $4,6, \dots, 20$ & $4,6, \dots, 20$ \\
%  & & Early Stopping (min delta)& 0.001& 0.001\\
%  & & Early Stopping (patience)& 100&    100 \\
% \hline
% & \textbf{Decoder} & GRU layers& 1& 1 \\
% %\cline{3-6}
% & & Learning rate (decoder w/o treatment sub-network)& $0.01,0.005, 0.001, 0.0001$ & $0.01,0.005, 0.001, 0.0001$ \\
%  & & Learning rate (encoder fine-tuning) & $0.001,0.0005, 0.0001, 0.00005$ & $0.001,0.0005, 0.0001, 0.00005$ \\
%  & & Learning rate (treatment sub-network)& $0.05, 0.01, 0.005, 0.0001$ & $0.05, 0.01, 0.005, 0.0001$  \\
% %\cline{3-6}
% & & Batch size & $32, 64, 128$ & $32, 64, 128$  \\
%  %%\cline{3-6}
% & & GRU hidden units& CR size& CR size  \\
%  %%\cline{3-6}
% & & GRU dropout rate    & - & - \\
%  %%\cline{3-6}
% & & BR size& CR size& CR size   \\
% & & GRU layers (Treat Encoder)& 1& 1\\
% & & GRU hidden units (Treat Encoder)& 6& 6\\
% & &FC hidden units & $4,6, \dots, 20$ & $4,6, \dots, 20$ \\
% & & Random time indices (m) & 10\% & 10\% \\
%  & & Early Stopping (min delta)& 0.001&  0.001\\
%  & & Early Stopping (patience)& 50& 50\\
% \hline

% \end{tabular}%
% }
% \end{table}
\begin{table}[!htbp]
\centering
\caption{Hyper-parameters search range for Causal CPC}
\resizebox{0.9\textwidth}{!}{%
\begin{tabular}{|c|c|c|c|c|}
\hline
\textbf{Model} & \textbf{Sub-model} & \textbf{Hyperparameter} & \textbf{Cancer simulation} & \textbf{MIMIC III (SS)} \\
\hline
\multirow{9}{*}{Causal CPC} & \multirow{9}{*}{Encoder} 
& GRU layers & 1 & 1 \\
\cline{3-5}
& & Learning rate & $0.01, 0.005, 0.001, 0.0001$ & $0.01, 0.005, 0.001, 0.0001$ \\
\cline{3-5}
& & Batch size & $32, 64, 128$ & $64, 128, 256$ \\
\cline{3-5}
& & GRU hidden units & $4, 6, \dots, 30$ & $4, 6, \dots, 30$ \\
\cline{3-5}
& & GRU dropout rate & - & - \\
\cline{3-5}
& & Local features (LF) size & $4, 6, \dots, 20$ & $4, 6, \dots, 20$ \\
\cline{3-5}
& & Context Representation (CR) size & $4, 6, \dots, 20$ & $4, 6, \dots, 20$ \\
\cline{3-5}
& & Early Stopping (min delta) & 0.001 & 0.001 \\
\cline{3-5}
& & Early Stopping (patience) & 100 & 100 \\
\hline
\multirow{13}{*}{Decoder} & & GRU layers & 1 & 1 \\
\cline{3-5}
& & Learning rate (decoder w/o treatment sub-network) & $0.01, 0.005, 0.001, 0.0001$ & $0.01, 0.005, 0.001, 0.0001$ \\
\cline{3-5}
& & Learning rate (encoder fine-tuning) & $0.001, 0.0005, 0.0001, 0.00005$ & $0.001, 0.0005, 0.0001, 0.00005$ \\
\cline{3-5}
& & Learning rate (treatment sub-network) & $0.05, 0.01, 0.005, 0.0001$ & $0.05, 0.01, 0.005, 0.0001$ \\
\cline{3-5}
& & Batch size & $32, 64, 128$ & $32, 64, 128$ \\
\cline{3-5}
& & GRU hidden units & CR size & CR size \\
\cline{3-5}
& & GRU dropout rate & - & - \\
\cline{3-5}
& & BR size & CR size & CR size \\
\cline{3-5}
& & GRU layers (Treat Encoder) & 1 & 1 \\
\cline{3-5}
& & GRU hidden units (Treat Encoder) & 6 & 6 \\
\cline{3-5}
& & FC hidden units & $4, 6, \dots, 20$ & $4, 6, \dots, 20$ \\
\cline{3-5}
& & Random time indices (m) & 10\% & 10\% \\
\cline{3-5}
& & Early Stopping (min delta) & 0.001 & 0.001 \\
\cline{3-5}
& & Early Stopping (patience) & 50 & 50 \\
\hline
\end{tabular}%
}
\end{table}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


==> appendices/5.tex <==
\chapter{Appendix: Chapter \ref{chapter:crl}}

\section{Proofs}



\subsection{Background: Subspace detection in a deterministic model}
% Standard SSL problem 
% static points 
% projections on and coordinates 
% Convex hull and its radius 
% Dual point
% Dual directions
% Subspace incoherence
% THEOREM 2.5
\paragraph{Standard \gls{ssc} problem} In the setting of \citet{elhamifar2013sparse, geometrySSC2012}, we consider data points \(\mathbf{X} = [\mathbf{x}_{1},\dots,\mathbf{x}_{N}] \in \mathbb{R}^{n \times N}\) and we define the \gls{ssc} as 

\begin{equation}
\label{eq:ss_express_standard}
\min_{\mathbf{c}\in\mathbb{R}^N} \|\mathbf{c}\|_{1}
\quad\text{subject to}\quad
\mathbf{X}\,\mathbf{c} = \mathbf{x}_i
\quad\text{and}\quad
\mathbf c_i = 0.
\end{equation}

Let \(\mathbf{X}^{(m)}\in\mathbb{R}^{n\times N_m}\) be the matrix whose columns are the \(N_m\) points on subspace \(\mathcal S_m\). For each \(m=1,\dots,M\) and \(i=1,\dots,N_m\),  we define
\[
\mathbf{X}^{(m)}_{-i}
\;=\;
\bigl[\mathbf{x}^{(m)}_{1},\dots,\mathbf{x}^{(m)}_{i-1},\mathbf{x}^{(m)}_{i+1},\dots,\mathbf{x}^{(m)}_{N_m}\bigr]
\]
which is the matrix obtained by removing the \(i\)-th column from \(\mathbf{X}^{(m)}\).  We can therefore "absorb" the constrating equality \(\mathbf c_i = 0\) of Euation \ref{eq:ss_express_standard} in \(\mathbf{X}_{-i}\) and write 


\begin{equation}
\label{eq:ss_express_standard_X_i}
\min_{\mathbf{c}\in\mathbb{R}^N} \|\mathbf{c}\|_{1}
\quad\text{subject to}\quad
\mathbf{X}_{-i}\,\mathbf{c} = \mathbf{x}_i
\end{equation}

To understand when a solution of the optimization problem in \ref{eq:ss_express_standard_X_i}, we turn to the dual problem: 
\begin{equation}
\label{eq:dual_ss_express_standard_X_i}
\max_{\bm{\lambda} \in \mathbb{R}^n} \langle\bm{\lambda}, \mathbf x_i \rangle \quad \text{subject to} \quad \|\mathbf X_{-i}^\top\bm{\lambda}\|_{\infty} \leq 1
\end{equation}

Here, $\lambda \in \mathbb{R}^n$ is a vector in the ambient space whose purpose is to witness/certify the optimality and support of the primal solution. This lead us to the definition of a dual point:

\begin{definition}[Dual point]
\label{def:dual_point}
Consider a point \(\mathbf{x}_i \in \mathbb{R}^n\) , and let \(\mathcal{C}^*(\mathbf{x}_i, \mathbf X_{-i})\) be the set of optimal solutions to\ref{eq:dual_ss_express_standard_X_i}. The \emph{dual point} \(\bm{\lambda}(\mathbf{x}_i, \mathbf X_{-i})\) is defined as the element of \(\mathcal{C}^*(\mathbf{x}_i, \mathbf X_{-i})\) with the minimum Euclidean norm.
\end{definition}

\(\bm{\lambda}(\mathbf{x}_i, \mathbf X_{-i})\) represents the dual certificate for the sparsest code representing \( \mathbf{x}_i \) using atoms in \( \mathbf X_{-i} \).

Next, let \(\mathbf{U}^{(m)}\in\mathbb{R}^{n\times d_m}\) be any orthonormal basis of \(\mathcal S_m\). In this basis, we write
\[
\mathbf{X}^{(m)}
=
\mathbf{U}^{(m)}\,\mathbf{A}^{(m)},
\]
where
\[
\mathbf{A}^{(m)}
=
\bigl[\mathbf{a}_1^{(m)},\dots,\mathbf{a}_{N_m}^{(m)}\bigr]
\;\in\;\mathbb{R}^{d_m\times N_m}
\]
has unit‐norm columns \(\mathbf{a}_i^{(m)}\). The columns of \(\mathbf{A}^{(m)}\) are precisely the coordinates of each point in the orthonormal basis \(\mathbf{U}^{(m)}\).
\begin{definition}[Dual directions]
\label{dualdirectiondef}
For each subspace index \(m\) and data‐point index \(i\), define the \emph{dual direction} \(\mathbf{v}_i^{(m)} \in \mathbb{R}^n\), arranged as columns of the matrix
\[
\mathbf{V}^{(m)}
\;=\;
\bigl[\mathbf{v}_1^{(m)},\,\mathbf{v}_2^{(m)},\,\dots,\,\mathbf{v}_{N_m}^{(m)}\bigr].
\]
These vectors correspond to the dual points
\[
\bm{\lambda}_i^{(m)}
\;=\;
\bm{\lambda}\bigl(\mathbf{a}_i^{(m)},\,\mathbf{A}_{-i}^{(m)}\bigr)
\]
via
\[
\mathbf{v}_i^{(m)}
\;=\;
\mathbf{U}^{(m)} \,\frac{\bm{\lambda}_i^{(m)}}{\|\bm{\lambda}_i^{(m)}\|}.
\]
\end{definition}

The dual direction is nothing but a unit-norm projection of the dual point into the subspace of \(\mathbf{x}_i\) when \(\bm{\lambda}_i^{(m)}\) is the dual point's latent coordinates. Intuitively, it is direction in space that best aligns with \( x_i \), maximizing the inner product \( \langle \lambda, x_i \rangle \), while still respecting the dual constraint \(\| \mathbf X_{-i}^\top \bm{\lambda}\|_{\infty} \leq 1.\)

One of the utilities of dual directions is that it allows us to describe the \textbf{worst-case alignment} between any point from another subspace (i.e., not in $\mathcal{S}_{m}$) and the dual directions $\mathbf{V}^{(m)}$ of that subspace. 

\begin{definition}[Subspace incoherence]
\label{subspaceincoherence}
Let \(\mathcal{X} = \bigcup_{m=1}^M \mathcal{X}_m\) be a union of point sets, and let \(\mathbf{V}^{(m)}\) be the matrix of dual directions for \(\mathcal{X}_m\) as in Definition~\ref{dualdirectiondef}.  The \emph{subspace incoherence} of \(\mathcal{X}_m\) with respect to the other points is
\[
\mu\bigl(\mathcal{X}_m\bigr)
\;=\;
\max_{\mathbf{x}\,\in\,\mathcal{X}\setminus\mathcal{X}_m}
\;\bigl\|\mathbf{V}^{(m)\,T}\,\mathbf{x}\bigr\|_{\ell_\infty}.
\]
\end{definition}

Subspace incoherence quantifies how "confusable" or "close" the directions of external points are to those characterizing the subspace. If \( \mu\bigl(\mathcal{X}_m\bigr)\) is small then no out-of-subspace point aligns strongly with any dual direction of \( \mathcal S^{(m)} \). This helps prevent such points from leaking into the sparse representation of points from \( \mathcal S^{(m)} \).

Subspace incoherence plays a central role in theoretical guarantees in \gls{ssc} and support recovery, as shown in the following theorem of \citet{geometrySSC2012}: let's define
\[
\mathcal{P}(\mathbf{X})
\;\coloneqq\;
\mathrm{conv}\bigl\{\pm \mathbf{x}_1,\;\pm \mathbf{x}_2,\;\dots,\;\pm \mathbf{x}_N\bigr\},
\]
where 
\(\mathrm{conv}(S)\) denotes the convex hull of a set \(S\subseteq\mathbb{R}^n\), i.e.\ the smallest convex set containing \(S\),  and \(\{\pm\mathbf{x}_i\} = \{\mathbf{x}_i,\,-\mathbf{x}_i\}\). Then subspace detection property (\ref{eq:subspace_detect}) is guaranteed under a bounding of the maximum subspace incoherence: 
% Equivalently, one may write
% \[
% \mathcal{P}(\mathbf{X})
% \;=\;
% \Bigl\{\mathbf{y} \in \mathbb{R}^n : 
% \mathbf{y}
% = \sum_{i=1}^N \lambda_i \,\mathbf{x}_i
% - \sum_{i=1}^N \lambda_i' \,\mathbf{x}_i,\quad
% \lambda_i,\lambda_i' \ge 0,\quad 
% \sum_{i=1}^N \lambda_i \;+\;\sum_{i=1}^N \lambda_i' = 1
% \Bigr\}.
% \]
% This shows that every point in \(\mathcal{P}(\mathbf{X})\) can be realized as a convex combination of \(\pm \mathbf{x}_1,\dots,\pm \mathbf{x}_N\).

\begin{theoremBox}[\citet{geometrySSC2012}]
\label{thm:subspace_detect_determin_std}
Suppose that for each \(m = 1,\dots,M\),
\begin{equation}
\label{eq:geom_cond_incoherence}
\mu\bigl(\mathcal{X}_m\bigr)
<
\min_{\,i:\,\mathbf{x}_i\in\mathcal{X}_m}
r\bigl(\mathcal{P}^m_{-i}\bigr).
\end{equation}
Then the subspace‐detection property holds.  Moreover, if \ref{eq:geom_cond_incoherence} is satisfied for a fixed \(m\), then the \emph{local} subspace‐detection property holds in the following sense: for every \(\mathbf{x}_i\in\mathcal{X}_m\), the solution to \ref{eq:ss_express_standard_X_i} can have nonzero entries only at columns of \(\mathbf{X}\) that lie in the same subspace \(\mathcal{X}_m\).
\end{theoremBox}

\subsection{Proof of Theorem \ref{thm:equiv_hard_penalized_prob_j}}
Define Lagrangian for the problem \(\mathcal{P}_t\bigl(Df(\mathbf{Z}),C_{:,j}\bigr)\):
\[
  \mathcal{L}_t(C_{:,j},\lambda,\nu)
  = \|C_{:,j}\|_1
    + \lambda\bigl(\ell_j(C_{:,j})-t\bigr)
    + \nu\,C_{j,j},
  \quad
  \lambda\ge0,\;\nu\in\mathbb{R},
\]
where \(\lambda\) and \(\nu\) are the multipliers for the constraints \(\,\ell_j(C_{:,j})\le t\) and \(c_j=0\), respectively.

Since
\begin{itemize}
  \item \(\ell_j(\cdot)\) is continuous and convex (indeed strictly convex quadratic if \(\mathbb{E}_{\mathbf{Z}}\bigl[\,Df(\mathbf Z)^{\!\top}Df(\mathbf Z)\bigr]\) is positive definite),
  \item \(\|\cdot\|_1\) is convex,
  \item there exists a feasible solution \(C_{:,j}^\star\) to \(\mathcal{P}_t\bigl(Df(\mathbf{Z}),C_{:,j}\bigr)\), that is, with \(\ell_j(C_{:,j}^\star)<t\) and \(C_{j,j}^\star=0\) (e.g.\ \(C_{:,j}^\star=\mathbf 0\) if \(t>\ell_j(\mathbf 0)\)), 
\end{itemize}
Slater’s condition holds (one inequality plus one equality), so strong duality applies. 

Let  $C_{:,j}^{\mathrm{LS}} = \arg \min_{C_{:,j} \in \mathbb R^{d_x} \quad C_{j,j}=0} \ell_j(C_{:,j})$, the solutions exists and is unique by strict convexity of \(\ell_j(\cdot)\).

\textbf{KKT system}

A triple \((C_{:,j}^*,\lambda^*,\nu^*)\) solves \(\mathcal{P}_t\bigl(Df(\mathbf{Z}),C_{:,j}\bigr)\) if and only if it satisfies the following KKT conditions:

\begin{align*}
  &\text{Primal feasibility:}
    &&\ell_j(C_{:,j}^*) \le t,\quad C_{j,j}^*= 0,
    &&\quad (K1)\\
  &\text{Dual feasibility:}
    &&\lambda^* \ge 0,
    &&\quad (K2)\\
  &\text{Complementary slackness:}
    &&\lambda^* \bigl(\ell_j(C_{:,j}^*) - t\bigr) = 0,
    &&\quad (K3)\\
  &\text{Stationarity:}
    &&0 \;\in\; \partial\|C_{:,j}^*\|_1 \;+\;\lambda^*\,\nabla \ell_j(C_{:,j}^*) \;+\;\nu^*\,\mathbf e_j,
    &&\quad (K4)
\end{align*}

Here \(\mathbf e_j\) denotes the \(j\)-th standard basis vector in \(\mathbb{R}^{d_x}\).

Because \(\ell_j\) it is strictly convex and there is only a single equality constraint \(C_{j,j}=0\), the stationarity condition (K4) uniquely determines \((C_{:,j}^*,\nu^*)\) it once \(\lambda^*\) is fixed.  Moreover, complementary slackness (K3) forces \(\lambda^*>0\) whenever \(\ell_j(C_{:,j}^*)<t\) is impossible—i.e.\ for all \(t>\ell_j(C_{:,j}^{\mathrm{LS}})\).  


Consider now the penalized problem  \(\mathcal{P}_{\lambda}(Df(\mathbf{Z}), C_{:,j})\), whose Lagrangian is
\begin{equation}\label{eq:LL}
\mathcal{L}_{\lambda}(C_{:,j},\nu)
= \ell_j(C_{:,j}) \;+\; \lambda\,\|C_{:,j}\|_1 \;+\; \nu\,C_{j,j},
\qquad
\nu\in\mathbb{R}.
\end{equation}
Its first‐order optimality (stationarity) condition reads
\begin{equation}\label{eq:stationarity_L}
\mathbf 0 \;\in\; \nabla \ell_j(C_{:,j}^*)
  \;+\;\lambda\,\partial\|C_{:,j}^*\|_1
  \;+\;\nu^*\, \mathbf e_j.
\end{equation}
Comparing \eqref{eq:stationarity_L} with (K4) shows that any \((C_{:,j}^*,\lambda^*,\nu^*)\) satisfying the KKT system for \(\mathcal{P}_t\bigl(Df(\mathbf{Z}),C_{:,j}\bigr)\) also satisfies \eqref{eq:stationarity_L} with \(\lambda=\lambda^*\).  Together with the common constraint \(c_j^*=0\), we obtain: If \(c^*\) solves \(\mathcal{P}_t\bigl(Df(\mathbf{Z}),C_{:,j}\bigr)\) with multipliers \((\lambda^*,\nu^*)\), then \(C_{:,j}^*\) also solves  \(\mathcal{P}_{\lambda}(Df(\mathbf{Z}), C_{:,j})\) under the constraint \(C_{j,j}=0\).


\textbf{Bijection between \(\lambda\) and \(t\)} Define the penalized‐solution path (respecting \(c_j=0\)):
\begin{equation}
    \label{eq:sol_path_penalized}
      C_{:,j}^*(\lambda)
  := \arg\min_{\substack{C_{:,j}\in\mathbb{R}^{d_x}\\C_{j,j}=0}}
     \bigl\{\,\ell_j(C_{:,j}) + \lambda\,\|C_{:,j}\|_1\bigr\}.
\end{equation}
By strict convexity of \(\ell_j\), convexity of \(\|\cdot\|_1\), and the affine constraint \(C_{j,j}=0\), the minimiser \(C_{:,j}^*(\lambda)\) is unique.  Now set
\[
  t_j(\lambda)
  := \ell_j\bigl(C_{:,j}^*(\lambda)\bigr).
\]
$\lambda \longrightarrow t_j(\lambda)$ is continuous and piecewise linear (Proposition 1 \citep{rosset2007piecewiseLassoPath}) and  strictly decreasing; its limit values are the following

As \(\lambda\to0^+\), the penalty vanishes and \(C_{:,j}^*(\lambda)\to C_{:,j}^{\mathrm{LS}}\)   Thus
\[
  \lim_{ \lambda\to0^+}t_j(\lambda)=\ell_j\bigl(C_{:,j}^{\mathrm{LS}}\bigr).
\]

As \(\lambda\to\infty\), the \(\lambda\|C_{:,j}\|_1\) term dominates in Equation \ref{eq:sol_path_penalized}, forcing \(C_{:,j}^*(\lambda)\to \mathbf 0\); hence
\[
\lim_{ \lambda\to \infty}  t_j(\lambda)=\ell_j(\mathbf 0).
\]

Therefore
\[
  t\colon (0,\infty)\;\longrightarrow\;\bigl[\,\ell_j\bigl(C_{:,j}^{\mathrm{LS}}\bigr),\,\ell_j(\mathbf 0)\bigr)
\]
is a continuous bijection. Note that since we assume self-expressiveness \ref{assp:self_expression} \(\ell_j\bigl(C_{:,j}^{\mathrm{LS}}\bigr) = 0\)

Given any 
\[
  t_j^\star \;\in\;\bigl[\,\ell_j\bigl(C_{:,j}^{\mathrm{LS}}\bigr),\,\ell_j(\mathbf 0)\bigr),
\]
continuity and bijectivity of \(t_j(\cdot)\) guarantee a unique \(\lambda_j \ge 0\) such that 
\[
  t_j(\lambda_j) =  t_j^\star.
\]
At that \(\lambda_j\), the solution \(C_{:,j}^*(\lambda_j)\) of \(\mathcal{P}_{\lambda}(Df(\mathbf{Z}), C_{:,j})\) satisfies 
\[
  \ell_j\bigl(C_{:,j}^*(\lambda)\bigr) = t_j^\star
  \quad\text{and}\quad
  \mathbf 0\;\in\;\nabla \ell_j(C_{:,j}^*(\lambda_j)) + \lambda_j\,\partial\|C_{:,j}^*(\lambda_j)\|_1 + \nu^*\,\mathbf e_j,
\]
which matches the stationarity KKT condition (K4) for \(\mathcal{P}_t\bigl(Df(\mathbf{Z}),C_{:,j}\bigr)\).  Hence \(C_{:,j}^*(\lambda_j)\) is also the minimizer of \(\mathcal{P}_t\bigl(Df(\mathbf{Z}),C_{:,j}\bigr)\).  This establishes a one-to-one correspondence \(\lambda\) and \(t\).

\subsection{High-Probability Guarantee for Subspace Detection}
\label{proof:subspace_detect_whp}
We provide in this section the proof of Theorem  \ref{thm:subspace_detect_whp}. We recall that \( \mathbf{Z} \in \mathrm{subG}_{d_z}(K) \) (Definition \ref{def:Z_subgauss_vector}) and the smoothness assumption (\ref{assp:smooth_f}) over \(f\): the decoder \( f \in \mathcal{C}^2(\mathbb{R}^{d_z}; \mathbb{R}^{d_x}) \) is twice continuously differentiable, with uniformly bounded curvature. That is, for each output coordinate \( f_i \), the Hessian satisfies
\[
\sup_{\mathbf{z} \in \mathbb{R}^{d_z}} \| D^2 f_i(\mathbf{z}) \|_{\mathrm{op}} \le L, \quad \text{for all } i \in \llbracket 1, d_x \rrbracket.
\]
Define the gradient vectors:
\[
P_i(\mathbf{Z}) := \nabla f_i(\mathbf{Z}) \in \mathbb{R}^{d_z}, \quad i = 1, \dots, d_x,
\]
and let the symmetric convex polytope \( \mathcal{K}(\mathbf{Z}) \subset \mathbb{R}^{d_z} \) be given by:
\[
\mathcal{K}(\mathbf{Z}) := \mathrm{conv}\left(\pm P_1(\mathbf{Z}), \dots, \pm P_{d_x}(\mathbf{Z})\right).
\]
Let the in-radius of \( \mathcal{K}(\mathbf{Z}) \) be defined by:
\[
r(\mathbf{Z}) := r(\mathcal{K}(\mathbf{Z})) = \min_{\mathbf{u} \in \mathbb{S}^{d_z-1}} \max_{1 \le i \le d_x} |\langle P_i(\mathbf{Z}), \mathbf{u} \rangle|.
\]
\begin{lemma}[Concentration of the in-radius of the Gradient Polytope]
\label{lemma:concentration_r(K)}
The in-radius of \( \mathcal{K}(\mathbf{Z}) \) has the concentration inequality:
\[
\mathbb{P}\left( \left| r(\mathbf{Z}) - \mathbb{E} r(\mathbf{Z}) \right| \ge t \right) \le 2 \exp\left( -\frac{t^2}{2K^2L^2} \right).
\]
Moreover, the expected in-radius is bounded by:
\[
\mathbb{E} \, r(\mathbf{Z}) \le \Lambda_1 \, K \, L \, \sqrt{ \frac{\log(d_x/d_z)}{d_z} },
\]
for a universal constant \( \Lambda _1> 0 \).
In particular, we have the one-sided, lower tail bound over the in-radius: 
\begin{equation}
    \label{eq:inradius_lower_tail_bnd}
    \mathbb{P} \Bigl\{r(\mathbf{Z})<\,\Lambda_1\,K\,L\,\sqrt{\tfrac{\log d_x}{d_z}}\Bigr\}
\;\le\;
\exp\!\Bigl(-\tfrac{\Lambda_1^2\,\log(d_x)}{2\,d_z}\Bigr).
\end{equation}
\end{lemma}

%\begin{proof}
\begin{proof} 
\textbf{In-radius Concentration}
Since  \( \|D^2 f_i(\mathbf{z})\|_{\mathrm{op}} \le L \) for all \( i \in [d_x] \) and \( \mathbf{z} \in \mathbb{R}^{d_z} \), the gradient map \( z \mapsto P_i(\mathbf{z}) = \nabla f_i(\mathbf{z}) \in \mathbb{R}^{d_z} \) is \(L\)-Lipschitz for each \(i\), i.e.,
\[
\|P_i(\mathbf{z}) - P_i(\mathbf{z}')\| \le L \|\mathbf{z} - \mathbf{z}'\|.
\]
For any fixed unit vector \( \mathbf{u} \in \mathbb{S}^{d_z-1} \), define the support function:
\[
\phi_{\mathbf{u}}(\mathbf{Z}) := \max_{1 \le i \le d_x} |\langle P_i(\mathbf{Z}), \mathbf{u} \rangle|.
\]
Since each \( P_i \) is \(L\)-Lipschitz, it follows that \( \phi_{\mathbf{u}}(\mathbf{Z}) \) is also \(L\)-Lipschitz. Moreover, the in-radius
\[
r(\mathbf{Z}) := \inf_{\mathbf{u} \in \mathbb{S}^{d_z-1}} \phi_{\mathbf{u}}(\mathbf{Z})
\]
is also \(L\)-Lipschitz as an infimum over a uniformly Lipschitz family. Therefore,
\[
|r(\mathbf{Z}) - r(\mathbf{Z}')| \le L \|\mathbf{Z} - \mathbf{Z}'\| \quad \text{for all } \mathbf{Z}, \mathbf{Z}' \in \mathbb{R}^{d_z}.
\]
Since \( \mathbf{Z} \) is sub-Gaussian with constant \( K \), applying standard concentration for Lipschitz functions of sub-Gaussian variables \citep{vershynin2018HDProba} gives:
\[
\mathbb{P}\left( \left| r(\mathbf{Z}) - \mathbb{E} r(\mathbf{Z}) \right| \ge t \right)
\le 2 \exp\left( - \frac{t^2}{2 K^2 L^2} \right),
\]
which proves the first part.

\textbf{Bound on the Expected in-radius.}
We now estimate the mean value \( \mathbb{E} r(\mathbf{Z}) \). Since
\[
r(\mathbf{Z}) = \inf_{u \in \mathbb{S}^{d_z-1}} \max_{1 \le i \le d_x} |\langle P_i(\mathbf{Z}), \mathbf{u} \rangle| = \inf_{u \in \mathbb{S}^{d_z-1}} \max_{1 \le i \le d_x} X_{i,\mathbf{u}}(\mathbf{Z}),
\]
we define the stochastic process:
\[
X_{i,\mathbf{u}}(\mathbf{Z}) :=|\langle P_i(\mathbf{Z}), \mathbf{u} \rangle|.
\]
Each map \( \mathbf{Z} \mapsto X_{i,\mathbf{u}}(\mathbf{Z}) \) is \(L\)-Lipschitz and hence sub-Gaussian with norm at most \( K L \). Furthermore, for any pairs \( (i,\mathbf{u}), (j,\mathbf{v}) \in  \llbracket 1, d_x \rrbracket \times \mathbb{S}^{d_z-1} \),
\[
|X_{i,\mathbf{u}}(\mathbf{Z}) - X_{j,\mathbf{v}}(\mathbf{Z}')| \le L \|\mathbf{Z} -\mathbf{Z}'\|(1 + \|\mathbf{u} - \mathbf{v}\|),
\]
implying the variance proxy:
\[
\rho((i,\mathbf{u}), (j,\mathbf{v})) := K L \left( \mathbf{1}_{i \ne j} + \|\mathbf{u} - \mathbf{v}\| \right).
\]
Hence, the collection \( \{X_{i,\mathbf{u}}(\mathbf{Z})\} \) is a \( \rho \)-sub-Gaussian process over the index set \( T =  \llbracket 1, d_x \rrbracket \times \mathbb{S}^{d_z-1} \).

By Dudley's entropy integral bound for sub-Gaussian processes:
\[
\mathbb{E} \sup_{(i,\mathbf{u}) \in T} X_{i,\mathbf{u}}(\mathbf{Z})
\le C \int_0^{\mathrm{diam}(T)} \sqrt{ \log N(T, \rho; \varepsilon) } \, d\varepsilon,
\]
where \( N(T, \rho; \varepsilon) \) is the \( \varepsilon \)-covering number of \( T \) under \( \rho \), and \( \mathrm{diam}(T) \le K L (2 + \pi) \).

To bound the covering number: The discrete index set \( \llbracket 1, d_x \rrbracket\) contributes a factor of \( d_x \). The unit sphere \( \mathbb{S}^{d_z-1} \) has \( \varepsilon \)-covering number at most \( (3 / \delta)^{d_z} \) in Euclidean norm, where \( \delta = \varepsilon / (K L) \). Thus,
    \[
    N(T, \rho; \varepsilon) \le d_x \left( \frac{3 K L}{\varepsilon} \right)^{d_z}.
    \]
Plugging into Dudley’s integral gives:
\[
\mathbb{E} \sup_{(i,\mathbf{u})} X_{i,\mathbf{u}}(\mathbf{Z})
\le \Lambda_1 K L \int_0^{2 K L} \sqrt{ \log d_x + d_z \log(3 K L / \varepsilon) } \, d_z\varepsilon
\lesssim K L \sqrt{ \frac{\log d_x}{d_z} },
\]
where the last step follows from standard integral splitting and evaluation \citep{ledoux2001concentration}.

Since \( r(\mathbf{Z}) = \inf_{\mathbf{u} \in \mathbb{S}^{d_z-1}} \max_{1 \le i \le d_x}  X_{i,\mathbf{u}}(\mathbf{Z}) \le \sup_{(i,\mathbf{u})}  X_{i,\mathbf{u}}(\mathbf{Z}) \), it follows that:
\[
\mathbb{E} r(\mathbf{Z}) \le \mathbb{E} \sup_{(i,\mathbf{u})} X_{i,\mathbf{u}}(\mathbf{Z}) \lesssim K L \sqrt{ \frac{\log d_x}{d_z} }.
\]

\textbf{In-radius lower tail bound} Since for each \(t > 0\)
\[
\mathbb{P}\left( \left| r(\mathbf{Z}) - \mathbb{E} r(\mathbf{Z}) \right| \ge t \right) \le 2 \exp\left( -\frac{t^2}{2K^2L^2} \right),
\]
and given \(\mathbb{E}[r(\mathbf{Z})]\le \Lambda_1 \,K\,L\,\sqrt{\tfrac{\log(d_x)}{d_z}}\), then setting \(t=\tfrac12\,\mathbb{E}[r(\mathbf Z)]\) yields
\[
\mathbb{P} \Bigl\{r(\mathbf{Z})<\tfrac12\,\Lambda_1\,K\,L\,\sqrt{\tfrac{\log d_x}{d_z}}\Bigr\}
\;\le\;
2 \exp\!\Bigl(-\tfrac{\Lambda_1^2\,\log(d_x)}{8\,d_z}\Bigr),
\]

or equivalently
\[
\mathbb{P} \Bigl\{r(\mathbf{Z})<\,\Lambda_1\,K\,L\,\sqrt{\tfrac{\log d_x}{d_z}}\Bigr\}
\;\le\;
\exp\!\Bigl(-\tfrac{\Lambda_1^2\,\log(d_x)}{2\,d_z}\Bigr).
\]
\end{proof}


\begin{lemma}[Frobenius-Norm Tail and Expectation Bounds]
\label{lemma:bound_norm_max}
Let
\[
\mathbf{A} = [\mathbf{a}_1, \dots, \mathbf{a}_{N_1}] \in \mathbb{R}^{d_1 \times N_1}, \quad
\mathbf{a}_i \overset{\mathrm{iid}}{\sim} \mathrm{Unif}(\mathbb{S}^{d_1 - 1}),
\]
and let \(\Sigma \in \mathbb{R}^{d_1 \times d_2}\) be deterministic, and \(\lambda \overset{\mathrm{iid}}{\sim} \mathrm{Unif}(\mathbb{S}^{d_2 - 1})\) independent of \(\mathbf{A}\). Define
\[
X_i := \langle \mathbf{a}_i, \Sigma \lambda \rangle, \qquad
\sigma_i^2 := Var(X_i \mid \mathbf{a}_i) = \frac{\| \Sigma^\top \mathbf{a}_i \|_2^2}{d_2}, \qquad
\sigma_{\max} := \max_{1 \le i \le N_1} \sigma_i.
\]
Then there exist universal constants \(\Lambda_2 > 0\) such that, for all \(t > 0\),
\begin{enumerate}
  \item[(i)] \emph{High-Probability Tail Bound.}
  \[
    \mathbb{P}\left\{
      \max_{1 \le i \le N_1} |X_i| > \mathbb{E} \left[ \max_i |X_i| \right] + t
    \right\}
    \le
    2 \exp\left( -\,\,\frac{d_2\,t^2}{2\|\Sigma\|_F^2} \right).
  \]
  \item[(ii)] \emph{Expectation Bound.}
  \[
    \mathbb{E} \left[ \max_{1 \le i \le N_1} |X_i| \right]
    \le
    \Lambda_2\,\frac{\|\Sigma\|_F}{\sqrt{d_2}} \, \sqrt{ \log(N_1 + 1) }.
  \]
\end{enumerate}
In particular, we have the one-sided tail bound:
\begin{equation}
\label{eq:bound_norm_max_lower_tail_bnd}
\mathbb{P}\left\{
\max_{1 \le i \le N_1} |X_i|
\leq (1 + \Lambda_2) \frac{\|\Sigma\|_F}{\sqrt{d_2}} \sqrt{\log(N_1 + 1)}
\right\}
\geq
 1 - \frac{2}{\sqrt{N_1 + 1}}.
\end{equation}
\end{lemma}

\begin{proof}
\textbf{Step 1: Concentration of individual terms.}  
For each fixed \( \mathbf{a}_i \), the function \( \lambda \mapsto X_i(\lambda) = \langle \mathbf{a}_i, \Sigma \lambda \rangle \) is \( \|\Sigma^\top \mathbf{a}_i\|_2 \)-Lipschitz on the sphere \( \mathbb{S}^{d_2 - 1} \). By Lévy’s lemma on the sphere (see \cite{ledoux2001concentration,vershynin2018HDProba}), for all \( \epsilon > 0 \),
\[
\mathbb{P}\left\{ \left| X_i - \mathbb{E}[X_i \mid \mathbf{a}_i] \right| \ge \epsilon \;\middle|\; \mathbf{a}_i \right\}
\le
2 \exp\left( -\,\,\frac{d_2\,\epsilon^2}{2\| \Sigma^\top \mathbf{a}_i \|_2^2} \right).
\]
Since \( \mathbb{E}[X_i \mid \mathbf{a}_i] = 0 \), we conclude \( X_i \mid \mathbf{a}_i \) is sub-Gaussian with proxy \( \sigma_i = \|\Sigma^\top \mathbf{a}_i\|_2 / \sqrt{d_2} \).

\textbf{Step 2: Concentration of the maximum.}  
Define
\[
F(\lambda) := \max_{1 \le i \le N_1} |X_i(\lambda)|.
\]
Conditioned on \(\mathbf{A}\), each \(X_i\) is fixed and \(F(\lambda)\) is \( \sigma_{\max} \)-Lipschitz over \( \mathbb{S}^{d_2 - 1} \). Applying Lévy’s lemma \citep{milman1986asymptotic} gives
\[
\mathbb{P}\left\{
  F(\lambda) - \mathbb{E}[F(\lambda) \mid \mathbf{A}] > t \;\middle|\; \mathbf{A}
\right\}
\le
2 \exp\left( -\,c\,\frac{d_2\,t^2}{\sigma_{\max}^2} \right)
\le
2 \exp\left( -\,c\,\frac{d_2\,t^2}{\|\Sigma\|_F^2} \right),
\]
where the final inequality uses \( \sigma_{\max} \leq \frac{\|\Sigma\|_F}{\sqrt{d_2}} \). Averaging over \(\mathbf{A}\) completes the proof of part (i).

\textbf{Step 3: Expectation via Dudley’s entropy integral.}  
Conditioned on \(\mathbf{A}\), the collection \( \{X_i\}_{i=1}^{N_1} \) forms a finite sub-Gaussian process indexed by \( \{1, \dots, N_1\} \). Dudley’s theorem implies \citep{talagrand2005generic}
\[
\mathbb{E}[F(\lambda) \mid \mathbf{A}]
\le
\Lambda_2 \int_{0}^{\sigma_{\max}} \sqrt{ \log N_1 } \, d\varepsilon
= \Lambda_2 \, \sigma_{\max} \sqrt{ \log N_1 }.
\]
Since \( \sigma_{\max} \leq \frac{\|\Sigma\|_F}{\sqrt{d_2}} \), we conclude
\[
\mathbb{E} \left[ \max_{1 \le i \le N_1} |X_i| \right]
= \mathbb{E}[F(\lambda)]
\le
\Lambda_2\, \frac{\|\Sigma\|_F}{\sqrt{d_2}} \, \sqrt{ \log(N_1 + 1) },
\]
completing part (ii).

\textbf{Step 4: One-sided tail bound.} Since
  \[
    \mathbb{P}\left\{
      \max_{1 \le i \le N_1} |X_i| > \mathbb{E} \left[ \max_i |X_i| \right] + t
    \right\}
    \le
    2 \exp\left( -\,\,\frac{d_2\,t^2}{2\|\Sigma\|_F^2} \right),
  \]
and given the expectation bound
  \[
    \mathbb{E} \left[ \max_{1 \le i \le N_1} |X_i| \right]
    \le
    \Lambda_2 \frac{\|\Sigma\|_F}{\sqrt{d_2}} \, \sqrt{ \log(N_1 + 1) },
  \]
  then choosing \(t =  \frac{\|\Sigma\|_F}{\sqrt{d_2}} \, \sqrt{ \log(N_1 + 1) } \)  yield

\[
\mathbb{P}\left\{
  \max_{1 \le i \le N_1} |X_i|
  \leq (1 + \Lambda_2) \frac{\|\Sigma\|_F}{\sqrt{d_2}} \sqrt{\log(N_1 + 1)}
\right\}
\geq
1 - 2 \exp\left( -\frac{1}{2} \log(N_1 + 1) \right)
= 1 - \frac{2}{\sqrt{N_1 + 1}}.
\]
\end{proof}
Let \(\mathcal{P}^m_{-i} \coloneqq \mathcal{P}(\mathbf{X}_{-i}^m)\), then application of Lemma \ref{lemma:concentration_r(K)} yields  
\begin{equation}
\label{eq:boundonrad}
\qquad \mathbb{P} \biggl\{
\Lambda_1\,K\,L\,\sqrt{\tfrac{\log n_m}{d_m}}
\le r \bigl(
\mathcal{P}^m_{-i} \bigr) \mbox{ for all pairs } (m,i)
\biggr\} 
\ge 
1-\sum_{m=1}^M  n_m
\exp\!\Bigl(-\tfrac{\Lambda_1^2\,\log(n_m)}{2\,d_m}\Bigr).
\end{equation}

On the other hand, by noticing that 
\begin{equation}
\label{eq:contmu}
\begin{aligned}
\left\| \mathbf{X}^{(k)^\top} \mathbf{V}^{(\ell)} \right\|_{\ell_\infty}
&= \max_{i = 1, \ldots, N_\ell} \left\| \mathbf{X}^{(k)^\top} \mathbf{v}_i^{(\ell)} \right\|_{\ell_\infty} \\
&= \max_{i = 1, \ldots, N_\ell} \left\| \mathbf{A}^{(k)^\top} \mathbf{U}^{(k)^\top} \mathbf{U}^{(\ell)} \frac{\boldsymbol{\lambda}_i^{(\ell)}}{\|\boldsymbol{\lambda}_i^{(\ell)}\|_2} \right\|_{\ell_\infty},
\end{aligned}
\end{equation}

and that \(\operatorname{aff}(\mathcal{S}_k, \mathcal{S}_m) =  \|\mathbf{U}^{(k)^\top} \mathbf{U}^{(m)} \|_F \) \citep{geometrySSC2012}, an application of \ref{lemma:bound_norm_max} to Equation \ref{eq:contmu} yields 

\[
\mathbb{P}\left\{
  \left\| \mathbf{X}^{(k)^\top} \mathbf{V}^{(m)} \right\|_{\ell_\infty}
  \leq (1 + \Lambda_2) \frac{\operatorname{aff}(\mathcal{S}_k, \mathcal{S}_m)}{\sqrt{d_2}} \sqrt{\log(n_m + 1)}
\right\}
\geq
 1 - \frac{2}{\sqrt{n_m + 1}}.
\]
 and therefore 
 \begin{equation}
\label{eq:unfbound}
\begin{aligned}
\mathbb{P}\biggl\{\,%
  \bigl\| \mathbf{X}^{(k)\top}\mathbf{V}^{(m)} \bigr\|_{\ell_\infty}
  &\le (1+\Lambda_2)\,\frac{\operatorname{aff}\bigl(\mathcal{S}_k, \mathcal{S}_m\bigr)}{\sqrt{d_2}}\,
        \sqrt{\log(n_m + 1)}\\[-0.5ex]
  &\quad \text{for all } (m, k)\ \text{with } m \ne k
\biggr\}
\;\ge\;
1 - \sum_{1 \le k \ne m \le M} \frac{2}{\sqrt{n_m + 1}}\\[-0.5ex]
&= 1 - \sum_{m=1}^M \frac{2(M-1)}{\sqrt{n_m + 1}}.
\end{aligned}
\end{equation}


As a consequence of Equations \ref{eq:unfbound}  and\ref{eq:boundonrad}, if we impose the condition 

\[
\max_{k \neq m} \Lambda_2' \, \operatorname{aff}(\mathcal{S}_k, \mathcal{S}_m) \frac{\sqrt{\log(n_k + 1)}}{\sqrt{d_m}} 
\leq \Lambda_1\,K\,L\,\sqrt{\frac{\log n_m}{d_m}},
\]
which is equivalent to saying
\begin{equation}
    \label{eq:incherence_con}
    \max_{k \neq m} \operatorname{aff}(\mathcal{S}_k, \mathcal{S}_m) \sqrt{\log(n_k + 1)} 
\leq \Lambda\,K\,L\,\sqrt{\log n_m}, \quad \text{with } \Lambda = \frac{\Lambda_1}{\Lambda_2'},
\end{equation}
then the subspace detection property holds with probability
\[
1 - \sum_{m=1}^M n_m \exp\!\left(-\frac{\Lambda_1^2 \log(n_m)}{2 d_m}\right) 
- \frac{2(M - 1)}{\sqrt{n_m + 1}}.
\]
The condition of Equation \ref{eq:incherence_con} is exactly that of Theorem \ref{thm:subspace_detect_whp}.


\subsection{Recovery of Feature Clusters via Spectral Clustering}
We now prove Proposition \ref{prop:recovery_nonoverlap_spec_cltsr}. We show that spectral clustering on the affinity matrix
\[
A = |C^*| + |C^*|^\top
\]
recovers with high probability the connected components of the feature graph $G_F$ under standard \gls{ssc} assumptions. Since we assume the incoherence gap of Theorem \ref{thm:subspace_detect_whp} holds, then by the same theorem, the subspace detection property holds, and therefore classical results on subspace clustering apply with high probability. In the following, we detail the arguments for cluster recovery with spectral clustering; we omit the expression "with high probability" for better readability.

\paragraph{Union-of-Subspaces from Latent Structure}
Let feature $i$ have latent-parent set $\mathrm{Pa}(i) \subseteq [d_z]$. Then the Jacobian row can be written as
\[
Df_{i,:}(\mathbf{Z}) = \nabla_{\mathbf{z}} f_i(\mathbf{Z})^\top = \sum_{j \in \mathrm{Pa}(i)} \alpha_{i,j}(\mathbf{Z})\, \mathbf{e}_j^\top,
\]
so each $Df_{i,:}(\mathbf{Z})$ lies in a union of low-dimensional subspaces spanned by subsets of $\{\mathbf{e}_j\}$. This corresponds to a union-of-subspaces model \citep{geometrySSC2012}.

\paragraph{\gls{ssc} Self-Expression Recovers Graph Structure}
We solve the population Lasso problem:
\[
\mathbf{C}^* = \arg\min_{\substack{\mathbf{C} \in \mathbb{R}^{d_x \times d_x} \\ \operatorname{diag}(\mathbf{C}) = 0}} \; \mathbb{E}_{\mathbf{Z}} \left[ \|Df(\mathbf{Z}) - \mathbf{C} Df(\mathbf{Z})\|_F^2 \right] + \lambda \|\mathbf{C}\|_1.
\]
Under standard \gls{ssc} conditions, such as subspace incoherence and low-noise \citep{elhamifar2013sparse}, we have:
\[
\mathbf{C}^*_{ii'} \ne 0 \quad \Leftrightarrow \quad \mathrm{Pa}(i) \cap \mathrm{Pa}(i') \ne \varnothing.
\]
Define the affinity matrix $\mathbf{A} = |\mathbf{C}^*| + |\mathbf{C}^*|^\top$. Then the support of $\mathbf{A}$ corresponds exactly to the edge set of the feature graph $G_F$.

\paragraph{Connected Components from Laplacian Nullspace}
Let $\mathbf{D} = \operatorname{diag}(\mathbf{A}\mathbf{1})$ and form the symmetric normalized Laplacian
\[
\mathbf{L}_{\mathrm{sym}} = \mathbf{I} - \mathbf{D}^{-1/2} \mathbf{A} \mathbf{D}^{-1/2}.
\]
It is well known \citep{von2007tutorialSpectrCls} that the multiplicity of the zero eigenvalue of $\mathbf{L}_{\mathrm{sym}}$ equals the number of connected components in $G_F$, and its nullspace is spanned by indicator vectors of those components.

\paragraph{Recovery via Spectral Clustering}
Spectral clustering (e.g., Ng–Jordan–Weiss variant) computes the first $k$ eigenvectors of $\mathbf{L}_{\mathrm{sym}}$, stacks them into a matrix $\mathbf{U} \in \mathbb{R}^{d_x \times k}$, and applies $k$-means to its rows. In the exact block-diagonal case, these rows are standard basis vectors corresponding to the true partition, so clustering achieves zero error \citep{ng2001spectral}.

\subsection{Guarantees of features grouping via clustering techniques}
We now prove Theorem~\ref{thm:overlap_cluster_recovery}. We break the argument into six main steps:
\begin{enumerate}[label=\textbf{\arabic*.}, wide, labelwidth=!, labelsep=1em, leftmargin=*]
    \item \textbf{Concentration of Gram entries (Step 1)} we show that with high probability
    \[
    \|\widehat\Sigma-\Sigma\|_\infty
    \]
    is of order \(O(KL\sqrt{d_x\log(d_x^2/\varepsilon)})\).

    \item \textbf{Restricted strong convexity (Step 2)} we prove that the population and empirical Lasso risks are strongly convex on \(s\)‑sparse rows, guaranteeing a unique minimizer.

    \item \textbf{Support recovery via primal–dual witness (Step 3 \& 4)} uses mutual incoherence and dominance to show that all off‑support coefficients vanish and that in‑group coefficients are large.

    \item \textbf{Affinity block bounds (Step 5)} translates the coefficient bounds into lower and upper bounds on the entries of the affinity matrix \(A^*\).

    \item \textbf{Spectral perturbation and rounding (Step 6)} we control the eigenspace deviation \(O(\|E\|_2/\Delta)\) and show that both SAAC and SymNMF recover the true (possibly overlapping) clusters up to the stated error rate.
\end{enumerate}

\subsection*{Step 1: Concentration of Inner-Product Entries}

We begin by controlling the entries of the empirical Gram matrix \(\widehat{\bm\Sigma}\), whose \((i,i')\)–th entry is
\[
g_{ii'}(\bm Z)
=\bigl\langle \partial_i f(\bm Z),\,\partial_{i'}f(\bm Z)\bigr\rangle.
\]
This uniform control is essential for later bounding the population Lasso risk.

First, the vector mean–value theorem tells us that for any \(\bm z,\bm z'\in\mathbb R^{d_z}\),
\[
\nabla f_i(\bm z)-\nabla f_i(\bm z')
=\int_{0}^{1}
D^2f_i\bigl(\bm z + t(\bm z'-\bm z)\bigr)\,(\bm z'-\bm z)\,dt.
\]
Since \(\|D^2f_i\|_{\mathrm{op}}\le L\) by Assumption \ref{assp:smooth_f}, it follows immediately that
\[
\|\nabla f_i(\bm z)-\nabla f_i(\bm z')\|
\le L\,\|\bm z'-\bm z\|,
\]
so each coordinate gradient \(\partial_i f(\bm z)\) is \(L\)–Lipschitz in \(\bm z\).

Turning next to the inner‐product function itself, differentiation yields
\[
\nabla g_{ii'}(\bm z)
=\sum_{\ell\in\{i,i'\}}
D^2f_\ell(\bm z)\,\partial_{\ell'}f(\bm z).
\]
Again, using \(\|D^2f_\ell\|_{\mathrm{op}}\le L\) together with the bounded‐Jacobian condition \(\sup_{\bm z}\|Df(\bm z)\|_F = \sqrt{d_x}\), we deduce
\[
\|\nabla g_{ii'}(\bm z)\|
\le 2\,L\, \sqrt{d_x},
\]
so \(g_{ii'}\) is \(2L\sqrt{d_x}\)–Lipschitz.

Because \(\bm Z\) is \(K\)–sub‐Gaussian, the Borell–Tsirelson–Ibragimov–Sudakov inequality \citep{SudakovTsirelson1978} applies to any \(2L\sqrt{d_x}\)–Lipschitz function of \(\bm Z\).  In particular, for each pair \((i,i')\) and any \(t>0\),
\[
\Pr\bigl(|g_{ii'}(\bm Z)-\mathbb E_{\bm Z}\,g_{ii'}(\bm Z)|\ge t\bigr)
\le 2\exp\!\Bigl(-\frac{t^2}{2K^2L^2d_x}\Bigr).
\]
A union bound over the \(\binom{d_x}{2}\) entries then shows that for any \(\varepsilon\in(0,1)\), with probability at least \(1-\varepsilon/3\),
\[
\|\widehat{\bm\Sigma} - \bm\Sigma\|_{\infty}
= \max_{i,i'}\bigl|g_{ii'}(\bm Z)-\mathbb E_{\bm Z}\,g_{ii'}(\bm Z)\bigr|
\le c_2\,K\,L\;\sqrt{d_x\log\!\bigl(d_x^2/\varepsilon\bigr)},
\]
where \(c_2>0\) is an absolute constant.  We denote this event by \(E_1\).  Establishing \(E_1\) completes our concentration argument for the inner‐product entries and sets the stage for analyzing the population Lasso estimator.  

\subsection*{Step 2: Primal–Dual Witness for the Population Lasso}

Building on the Gram‐matrix control from the previous section, we now analyze the population‐level Lasso problem.  Recall the population Gram
\[
\bm{\Sigma} \;=\;\mathbb{E}_{\bm{Z}}\bigl[Df(\bm{Z})\,Df(\bm{Z})^\top\bigr],
\]
and consider the estimator
\[
\min_{C\in\mathbb{R}^{d_x\times d_x}}
\;\mathbb{E}_{\bm{Z}}\bigl\lVert Df(\bm{Z}) - C\,Df(\bm{Z})\bigr\rVert_F^2
\;+\;\lambda\|C\|_1.
\]
\noindent\emph{Restricted strong convexity.}
By Assumption \ref{assp:restrict_eigenval}, the population Gram satisfies
\[
\bm{v}^\top\bm{\Sigma}\,\bm{v}
\;\ge\;
\kappa\,\|\bm{v}\|_2^2
\quad\text{whenever }\|\bm{v}\|_0\le s.
\tag{3.1a}
\]
Hence, the smooth part of the objective has the Hessian
\[
\,D^2Q(C)[\Delta C,\Delta C]
=2\sum_{i}(\Delta C)_{i,:}\,\bm{\Sigma}\,(\Delta C)_{i,:}^\top
\ge2\kappa\|\Delta C\|_F^2,
\]
so \(Q(C)\) is \(2\kappa\)–strongly convex on all row‑wise \(s\)–sparse directions, implying a unique minimizer \(C^*\).

\noindent \emph{Sample curvature.}
In practice, we replace \(\Sigma\) by its sample version \(\widehat\Sigma=\tfrac1N\sum_tDf(Z^{(t)})Df(Z^{(t)})^\top\). \cite{raskutti10a} shows that if \(N\gtrsim s\log d_z\), then with probability greater than \(1-\varepsilon/3\),
\[
\bm{v}^\top\widehat\Sigma\,\bm{v}
\;\ge\;
(\kappa/2)\|\bm{v}\|_2^2
\quad\forall\,\|\bm{v}\|_0\le s.
\tag{3.1b}
\]
Thus, the empirical risk is also strongly convex with high probability, again guaranteeing a unique minimizer over \(s\)–sparse rows. % (lemma 1 in raskutti10a)

\noindent\emph{Dual feasibility and setting \(\lambda\).}
Let \(S\) denote the true support of \(C^*\).  The KKT conditions on the complement \(S^c\) read
\[
\nabla_{S^c}\,\mathbb{E}\|Df - C\,Df\|_F^2\big|_{C=C^*}
\;+\;\lambda\,U_{S^c}
\;=\;0,
\]
with \(U_{S^c}\in[-1,1]^{|S^c|}\).  Enforcing the primal–dual witness \(C^*_{S^c}=0\) yields
\[
2\,\bm{\Sigma}_{S^c,S}\,C^*_{S} + \lambda\,U_{S^c} = 0
\quad\Longrightarrow\quad
\|\bm{\Sigma}_{S^c,S}C^*_{S}\|_\infty<\lambda.
\]
By mutual incoherence, \(\|\Sigma_{S^c,S}\Sigma_{S,S}^{-1}\|_\infty\le1-\gamma\), and dominance ensures \(\|\Sigma_{S,S}C^*_{S}\|_\infty\approx m_{\max}\), so deterministically \(\|\Sigma_{S^c,S}C^*_{S}\|_\infty\le(1-\gamma)m_{\max}\). Meanwhile, the high‑probability event \(E_1\) controls random fluctuations by \(\delta_{\rm rand}=c_2KL\sqrt{d_x\log(d_x^2/\varepsilon)}\).  Thus, choosing
\[
\lambda
=\Bigl(1-\tfrac\gamma2\Bigr)\,m_{\max}
\;+\;
c_2\,K\,L\;\sqrt{d_x\log\!\bigl(d_x^2/\varepsilon\bigr)}
\]
strictly exceeds \((1-\gamma)m_{\max}+\delta_{\rm rand}\), forcing \(C^*_{S^c}=0\).

\noindent At this point, we have shown that under \(E_1\) and the RE event, the population Lasso solution \(C^*\) recovers the correct support with high probability.  In the next section, we translate these coefficient bounds into affinity‐matrix guarantees and, ultimately, into clustering accuracy.

\subsection*{Step 3: Sign Consistency \& In‑Group Recovery}

Next, we show that any two features \(i,i'\), $i \neq i'$, in the same latent group \(G_j\) obtain a large positive self‑expression coefficient
\[
C^*_{ii'} 
\;=\;
\arg\min_{c\in\mathbb R}\;
\mathbb E_{\bm Z}\bigl\|\partial_i f(\bm Z)-c\,\partial_{i'} f(\bm Z)\bigr\|_2^2,
\]
and in particular 
\[
C^*_{ii'}\;\ge\;1 - (\delta+\mu)\;-\;\frac{c_2\,K\,L\,\sqrt{d_x}\,\log(d_x^2/\varepsilon)}{m_j}.
\]

To see this, note first that on the true one‑dimensional support \(S=\{(i,i')\}\), the \(\ell_1\) penalty drops out and \(C^*_{ii'}\) solves the simple least‑squares problem
\[
\min_{c\in\mathbb R}\;\mathbb E_{\bm Z}\bigl\|\partial_i f(\bm Z)-c\,\partial_{i'} f(\bm Z)\bigr\|_2^2.
\]
Differentiating under the expectation and setting to zero gives the closed‑form
\[
C^*_{ii'}
=\frac{\mathbb E_{\bm Z}\langle \partial_i f(\bm Z),\;\partial_{i'}f(\bm Z)\rangle}
       {\mathbb E_{\bm Z}\|\partial_{i'}f(\bm Z)\|_2^2}.
\]
We now bound the numerator and denominator in turn.  By Dominance \ref{assp:dominance_partial}, the key partial \(\partial f_i/\partial z_j\) satisfies
\[
\mathbb E_{\bm Z}\Bigl|\frac{\partial f_i}{\partial \bm  z_j}(\bm  Z)\Bigr|
\ge(1-\delta)\,\sqrt{\mathbb E_{\bm Z}\|\nabla_{\bm z} f_i(\bm Z)\|^2}
=(1-\delta)\sqrt{m_j}.
\]
Moreover, Mutual Incoherence ensures that cross‑terms contribute at most \(\mu\,\sqrt{m_j^2}\), so altogether
\[
\mathbb E_{\bm Z}\langle \partial_i f(\bm Z),\;\partial_{i'}f(\bm Z)\rangle
\;\ge\;(1-\delta-\mu)\,m_j.
\]

On the other hand, from the uniform deviation event \(E_1\) we know each entry of the empirical Gram deviates by at most \(\Delta:=c_2\,K\,L\sqrt{d_x\log(d_x^2/\varepsilon)}\).  In particular,
\[
\bigl|\|\partial_{i'}f(\bm Z)\|_2^2 - \mathbb E_{}\|\partial_{i'}f(\bm Z)\|_2^2\bigr|
\le\Delta,
\]
and since \(\mathbb E_{\bm Z}\|\partial_{i'}f(\bm Z)\|_2^2=m_j\), we have
\[
\mathbb E_{\bm Z}\|\partial_{i'}f(\bm Z)\|_2^2
\;\le\;
m_j + \Delta.
\]

Putting these together,
\[
C^*_{ii'}
=\frac{\mathbb E_{\bm Z}\langle \partial_i f(\bm Z),\partial_{i'}f(\bm Z)\rangle}{\mathbb E_{\bm Z}\|\partial_{i'}f(\bm Z)\|_2^2}
\;\ge\;
\frac{(1-\delta-\mu)\,m_j}{\,m_j+\Delta\,}
\;\ge\;
1 - (\delta+\mu) - \frac{\Delta}{m_j},
\]
which is the stated bound 
\[
\displaystyle
C^*_{ii'}\ge1 - (\delta+\mu) - \tfrac{c_2KL\sqrt{d_x}\,\log(d_x^2/\varepsilon)}{m_j}.
\]
\subsection*{Step 4: Affinity Matrix \& Block Bounds}

With the support recovery and coefficient bounds in place, define the induced affinity
\[
A^*_{ii'} \;=\; |C^*_{ii'}| \;+\; |C^*_{i'i}|.
\]
On the intersection of our two high‑probability events \(E_1\) (uniform deviation of \(\widehat\Sigma\)) and \(E_2\) (empirical RE), we obtain sharp “block” estimates separating in‑group from cross‑group affinities.

\vspace{0.5em}
\emph{Intra‑cluster bound.}
If \(i,i'\in Ch(j)\), then by the sign‑consistency argument, each of \(C^*_{ii'}\) and \(C^*_{i'i}\) obeys
\[
C^*_{\bullet\,\bullet}\;\ge\;1 - (\delta+\mu)
\;-\;\frac{c_2\,K\,L\,\sqrt{d_x\,\log(d_x^2/\varepsilon)}}{m_j},
\]
so summing yields
\[
A^*_{ii'}
\;\ge\;
2\Bigl(1 - (\delta+\mu)\Bigr)
\;-\;\frac{2\,c_2\,K\,L\,\sqrt{d_x\,\log(d_x^2/\varepsilon)}}{m_j}.
\]
Absorbing constants into \(C_3=2c_2\) and re‑scaling by \(m_j\) gives the clean form
\[
A^*_{ii'} 
\;\ge\;
\bigl(1 - \delta - \mu\bigr)\,m_j
\;-\;
C_3\,K\,L\,\sqrt{d_x\,\log\!\bigl(\tfrac{d_x^2}{\varepsilon}}\bigr).
\]

\vspace{0.5em}
\emph{Inter‑cluster bound.}
If \(i\in Ch(j)\) and \(i'\in Ch(k)\) with \(k\neq j\), then dual‑feasibility forces \(C^*_{ii'}=0\) on the population level, and concentration adds at most \(c_2KL\sqrt{d_x\log(d_x^2/\varepsilon)}\) to each coefficient.  Hence
\[
A^*_{ii'}
\;\le\;
\Bigl|\mathbb E_{\bm Z}\langle\partial_i f(\bm Z),\partial_{i'} f(\bm Z)\rangle\Bigr|
\;+\;
C_3\,K\,L\,\sqrt{d_x\,\log\!\bigl(\tfrac{d_x^2}{\varepsilon}\bigr)}
\;\le\;
\mu\,\sqrt{m_jm_k}
\;+\;
C_3\,K\,L\,\sqrt{d_x}\,\log\!\bigl(\tfrac{d_x^2}{\varepsilon}\bigr),
\]
which in the symmetric‐affinity form becomes
\[
A^*_{ii'} 
\;\le\;
\mu\,m_j\,m_k
\;+\;
C_3\,K\,L\,\sqrt{d_x\,\log\!\bigl(\tfrac{d_x^2}{\varepsilon}\bigr)}.
\]

These two inequalities reveal a gap between “strong” in‑group affinities and “weak” cross‑group affinities—precisely the structure needed for the subsequent spectral perturbation and clustering steps.  

\subsection*{Step 5: Spectral Perturbation \& Eigenspace Deviation}

To transition from coefficient bounds to clustering, we compare the observed affinity \(A^*\) with the ideal block matrix 
\[
H=\sum_{j}m_{j}\,1_{G_j}1_{G_j}^\top,
\]
and let the perturbation be 
\[
E = A^* - H.
\]
Our goal is to show that \(E\) is small in operator norm and thus the leading eigenspaces of \(A^*\) and \(H\) remain close.

Gershgorin’s circle \citep{horn2012matrix} theorem first controls the size of \(E\).  Since each row of \(E\) has at most \(d_x\) nonzero entries, each is bounded in magnitude by 
\[
C_3\,K\,L\,\sqrt{d_x\,\log\!\bigl(d_x^2/\varepsilon\bigr)},
\]
we obtain
\[
\|E\|_2\;\le\;\|E\|_{1,\infty}
\;\le\;d_x\,C_3\,K\,L\,\sqrt{d_x\,\log\!\bigl(d_x^2/\varepsilon\bigr)}.
\]

Next, Weyl’s inequality for symmetric matrices \citep{horn2012matrix} implies that every eigenvalue of \(A^*\) deviates from its counterpart in \(H\) by at most \(\|E\|_2\):
\[
\bigl|\lambda_i(A^*)-\lambda_i(H)\bigr|\;\le\;\|E\|_2
\quad\forall\,i.
\]

We then define the critical eigengap
\[
\Delta
=\min_j m_j \;-\;\mu\max_{k\ne j}\sqrt{m_jm_k}
\;-\;2\|E\|_2.
\]
Whenever \(\Delta>0\), the Davis–Kahan sin \(\Theta\) theorem \citep{davis1970rotation} guarantees that the distance between the top-\(d_z\) eigenspaces of \(H\) and \(A^*\) is controlled by
\[
\|\sin\Theta(\widehat U,U)\|_2
\;\le\;\frac{\|E\|_2}{\Delta},
\]
and in particular, each eigenvector satisfies
\[
\|\widehat u_i - u_i\|_2
\;\le\;\frac{\|E\|_2}{\Delta}.
\]
Thus, under the gap condition \(\Delta>0\), the spectral embeddings produced by \(A^*\) remain within a small radius of the ideal block‑model embeddings—paving the way for accurate rounding in the clustering step.  

\subsection*{Step 6.1: SAAC Rounding}

After forming the affinity matrix \(A^*\), SAAC \citep{panov2017SAAC} extracts its top \(d_z\) eigenvectors 
\[
\widehat U = \bigl[\hat u^1,\dots,\hat u^{d_z}\bigr]\in\mathbb R^{d_x\times d_z},
\]
and then fits a binary membership matrix \(Z\in\{0,1\}^{d_x\times d_z}\) alongside a prototype matrix \(X\in\mathbb R^{d_z\times d_z}\) by minimizing 
\[
\|\widehat U - Z\,X\|_F^2
\quad\text{subject to }Z_{i,\cdot}\neq0\ \forall i,
\]
so that each feature \(i\) is assigned to at least one cluster and \(\widehat U\approx ZX\).

In practice, SAAC alternates between  
\[
X \;=\;\arg\min_X\|\widehat U - Z\,X\|_F^2 
\;=\;(Z^\top Z)^{-1}Z^\top\widehat U
\]
and, for each \(i\),
\[
Z_i \;=\;\arg\min_{z\in\{0,1\}^{d_z}\setminus\{0\}}\|\widehat U_i - z\,X\|_2^2
\;=\;\begin{cases}
1 &\text{at }j=\arg\min_k\|\widehat U_i - X_k\|_2,\\
0 &\text{otherwise},
\end{cases}
\]
i.e.\ each feature picks the single prototype \(X_j\) closest in Euclidean distance to its embedding \(\widehat U_i\).  These two updates are repeated until convergence.  

The success of this \emph{nearest‑neighbor rounding} follows from our perturbation bounds: with probability \(\ge 1-\varepsilon\),  
\[
\|\widehat U_i - U_i\|_2\;\le\;\frac{\|E\|_2}{\Delta},
\]
where \(U_i\) is the ideal block‑model embedding and \(\Delta\) the eigengap.  In the noiseless block model \(H=\sum_jm_j1_{G_j}1_{G_j}^\top\), the normalized indicator eigenvectors \(\{u_j\}\) satisfy  
\[
\|u_j - u_{j'}\|_2\;\ge\;2,\quad j\neq j'.
\]
Hence if 
\[
\frac{\|E\|_2}{\Delta}<\tfrac12,
\]
then each \(\widehat U_i\) lies within \(1/2\) of its true \(U_i\) and farther from any other \(u_{j'}\).  Nearest‑neighbor rounding therefore selects the correct cluster(s), and when overlaps occur, features lie near intersections of the relevant \(\{u_j\}\), still recovered as long as the intersection angles exceed the noise radius.  Combining these facts yields the misclassification rate
\[
\max\limits_{ 1 \leq j \leq d_z} \frac{|\widehat G_j\triangle G_j|}{|G_j|}
=\mathcal O\!\Bigl(\delta + \tfrac{\mu}{\gamma} + \tfrac{K\,L\,\;\sqrt{d_x\log(d_x^2/\varepsilon)}}{\min\limits_{ 1 \leq j \leq d_z} m_j}\Bigr).
\]
as claimed in the Theorem \ref{thm:overlap_cluster_recovery}.  

\subsection*{Step 6.2: SymNMF Rounding}

SymNMF \citep{Kuang2015SymNMF} replaces the binary assignment of SAAC with a nonnegative factorization.  We fit
\[
\min_{Y\ge0}\;F(Y)\;=\;\bigl\|A^*-Y\,Y^\top\bigr\|_F^2,
\]
where each row \(Y_i\) encodes soft memberships of feature \(i\).  The classic multiplicative update of  \citet{Kuang2015SymNMF}),
\[
Y_{ij}\;\leftarrow\;Y_{ij}\;\times\;
\frac{[\,A^*Y\,]_{ij}}{[\,Y\,Y^\top Y\,]_{ij}},
\]
preserves nonnegativity and drives \(F(Y)\) downward until a stationary point \(Y^*\) is reached.

Once converged, we normalize each row,
\[
T_i = Y^*_i \bigl/\|Y^*_i\|_1\;\in\;\Delta^{d_z-1},
\]
and then “round” by hard‐thresholding:
\[
Z_{i,j} =
\begin{cases}
1, & j = \displaystyle\arg\max_k\,T_{i,k},\\[1ex]
0, & \text{otherwise}.
\end{cases}
\]
In practice, when several entries tie within a small tolerance, all corresponding clusters may be assigned to \(i\), capturing overlaps.

Under the same eigenspace perturbation bound \(\|\widehat U - U\|_{2\to\infty}\!\le\!\|E\|_2/\Delta\), the ideal block‑model solution \(Y=U\Lambda^{1/2}\) (with rows proportional to the indicator eigenvectors) is perturbed only slightly.  A perturbation smaller than half the gap between the top two coordinates of each ideal row cannot change the index of the largest entry, so hard‐thresholding recovers the exact cluster memberships.  Allowing ties yields overlap‐aware assignments.  Hence, SymNMF achieves the same misclassification rate,
\[
\max_j\frac{|\widehat G_j\triangle G_j|}{|G_j|}
=O\!\Bigl(\delta + \tfrac\mu\gamma + \tfrac{KL\sqrt{d_x\log(d_x^2/\varepsilon)}}{\min_jm_j}\Bigr),
\]
completing the proof of the theorem \ref{thm:overlap_cluster_recovery}.  


\subsection{Generalization and Stability Under the Self-Expression Problem}

\paragraph{Proof of Theorem \ref{thm:genetalization_SExprLoss}}
We aim to control the uniform generalization gap:
\[
\Delta :=
\sup_{C \in \mathcal{C}_\lambda}
\left| \mathbb{E}_{\mathbf{x} \sim p_{data}}[\bar{\ell}(C, f; \mathbf{x}) ] - \frac{1}{N} \sum_{i=1}^N \bar{\ell}(C, f; \mathbf{x})  \right|,
\quad \text{where} \quad
\bar{\ell}(C, f; \mathbf{x}) = \left\| (I - C)\bar{J}_f(\mathbf{x}; q_\phi) \right\|_F^2.
\]
\subparagraph{Step 1: Symmetrization.}
By the standard symmetrization inequality (see \cite[Theorem 3.1]{bartlett2002rademacher}), we have:
\[
\mathbb{E}_{\mathbf{X}_{1:N}}[\Delta]
\le
2\,\mathbb{E}_{\mathbf{x}_{1:N},\,\sigma_{1:N}}
\left[ \sup_{C \in \mathcal{C}_\lambda}
\frac{1}{N} \sum_{i=1}^N \sigma_i\,\ell(C; \mathbf{x}_i) \right],
\]
where \( \sigma_i \in \{ \pm 1 \} \) are  Rademacher variables which are independent.

\subparagraph{Step 2: Contraction via Ledoux–Talagrand.}
Fix \(\mathbf{x} \in \mathcal{X} \subset \mathbb{R}^{d_x} \). Since \( \|\bar{J}_f(\mathbf{x}; q_\phi)\|_F \le M_\phi \), appplying the contraction inequality \citep{ledoux2001concentration} gives:
\[
\mathbb{E}_\sigma \left[
\sup_{C \in \mathcal{C}_\lambda}
\frac{1}{N} \sum_{i=1}^N \sigma_i \| \bar{\ell}(C, f; \mathbf{x}_i) \|_F^2
\right]
\le
4M \cdot \mathbb{E}_\sigma \left[
\sup_{C \in \mathcal{C}_\lambda}
\frac{1}{N} \sum_{i=1}^N \sigma_i \langle \bar{\ell}(C, f; \mathbf{x}_i) , E \rangle_F
\right],
\]
%, the function \( h \mapsto \|h\|_F^2 \) is \( 2M \)-Lipschitz on the ball of radius \( M \). 
where \( E \in \mathbb{R}^{n \times d} \) is an auxiliary matrix (a “ghost sample”) used in the contraction argument.

\subparagraph{Step 3: Reduction to linear class.}
Since
\[
\langle \bar{\ell}(C, f; \mathbf{x}_i) , E \rangle_F = \langle \bar{J}_f(\mathbf{x}_i; q_\phi), E \rangle_F - \langle C \bar{J}_f(\mathbf{x}_i; q_\phi), E \rangle_F,
\]
and the first term is independent of \( C \), we reduce to bounding:
\[
\mathbb{E}_\sigma \left[
\sup_{C \in \mathcal{C}_\lambda}
\frac{1}{N} \sum_{i=1}^N \langle C \bar{J}_f(\mathbf{x}_i; q_\phi), \sigma_i \rangle_F
\right].
\]

\subparagraph{Step 4: Bounding the Rademacher complexity.}
Define the class of self-expressive tangent maps:
\[
\mathcal{H}_{\lambda,f} := \left\{ \mathbf{x} \mapsto C \bar{J}_f(\mathbf{x}; q_\phi) \;\middle|\; C \in \mathbb{R}^{d_x \times d_x},\; \mathrm{diag}(C) = 0,\; \|C\|_1 \le \lambda \right\}.
\]
Using the duality \( \sup\limits_{\|C\|_1 \le \lambda} \langle C, A \rangle = \lambda \|A\|_\infty \), the Rademacher complexity \(\mathfrak{R}_N(\mathcal{H}_{\lambda,f})\) of \(\mathcal{H}_{\lambda,f}\) is bounded:
\[
\mathfrak{R}_N(\mathcal{H}_{\lambda,f})
\le
\frac{\lambda}{N} \mathbb{E}_\sigma \left\| \sum_{i=1}^N \sigma_i \bar{J}_f(\mathbf{x}_i; q_\phi)^\top \right\|_\infty.
\]
Since \( \|\bar{J}_f(\mathbf{x}_i; q_\phi)\|_F \le M_{\phi} \) implies \( \|\bar{J}_f(\mathbf{x}_i; q_\phi)\|_{\rm op} \le M_\phi \), classical matrix concentration \citep{tropp2012user} gives:
\[
\mathbb{E}_\sigma \left\| \sum_{i=1}^N \sigma_i \bar{J}_f(\mathbf{x}_i; q_\phi)^\top \right\|_\infty
\le
M_{\phi} \sqrt{2 N \log d_x},
\]
thus:
\[
\mathfrak{R}_N(\mathcal{H}_{\lambda,f})
\le
\lambda M_{\phi} \sqrt{ \frac{2 \log d_x}{N} }.
\]
\subparagraph{Step 5: Final bound via McDiarmid’s inequality.}
Combining the above gives:
\[
\mathbb{E}_{\mathbf{X}_{1:N}}[\Delta]
\le
8 \lambda M_\phi^2 \sqrt{ \frac{2 \log d_x}{N} }.
\]
To lift this to a high-probability bound, we apply McDiarmid’s inequality \citep{ShalevShwartzBenDavid2014}: with probability at least \( 1 - \delta \) we finally obtain
\[
\Delta
\le
8 \lambda M_\phi^2 \sqrt{ \frac{2 \log d_x}{N} }
+ M_\phi^2 \sqrt{ \frac{2 \log(1/\delta)}{N} }.
\]
% or a standard concentration result for empirical Rademacher processes

\paragraph{Proof of Proposition~\ref{prop:jacobian-perturbation}} 
Write \(A = \tilde{\mathrm{D}}f(\mathbf{Z})\), \(E = E(\mathbf{Z})\), and \(\Delta = I - C^*\). Then:
\[
\|\mathrm{D}f(\mathbf{Z})- \mathrm{D}f(\mathbf{Z})C^*\|_F^2
= \|(\tilde{\mathrm{D}}f(\mathbf{Z}) + E(\mathbf{Z}))\Delta\|_F^2
= \|\tilde{\mathrm{D}}f(\mathbf{Z})\Delta\|_F^2
+ 2\langle \tilde{\mathrm{D}}f(\mathbf{Z})\Delta, E(\mathbf{Z})\Delta\rangle_F
+ \|E(\mathbf{Z})\Delta\|_F^2.
\]
Thus, the deviation satisfies:
\[
\left| \|\mathrm{D}f(\mathbf{Z})- \mathrm{D}f(\mathbf{Z})C^*\|_F^2 - \|\tilde{\mathrm{D}}f(\mathbf{Z}) - \tilde{\mathrm{D}}f(\mathbf{Z})C^*\|_F^2 \right|
= \left| 2\langle \tilde{\mathrm{D}}f(\mathbf{Z})\Delta, E(\mathbf{Z})\Delta\rangle_F + \|E(\mathbf{Z})\Delta\|_F^2 \right|.
\]

\subparagraph{Step 1: Bounding \(\|E(\mathbf{Z})\Delta\|_F\).}
We have \(\|E(\mathbf{Z})\Delta\|_F \le \|E(\mathbf{Z})\|_F \|\Delta\|_{\mathrm{op}}\). Since \(E\) has \(d_x\) independent sub-Gaussian columns, by vector concentration \cite[Proposition 3.3.7]{vershynin2018HDProba}, there exists \(\Lambda_1 > 0\) such that for any \(\delta \in (0,1)\),
\[
\mathbb{P}\left\{ \|E(\mathbf{Z})\|_F > \Lambda_1 \varepsilon \sqrt{d_z d_x} + \varepsilon \sqrt{2d_z \ln(2d_x/\delta)} \right\} \le \delta.
\]
Thus, with probability at least \(1-\delta\),
\[
\|E(\mathbf{Z})\Delta\|_F \le \|\Delta\|_{\mathrm{op}} \left( \Lambda_1 \varepsilon \sqrt{d_z d_x} + \varepsilon \sqrt{2d_z \ln\tfrac{2d_x}{\delta}} \right).
\]

\subparagraph{Step 2: Bounding the cross term.}
By Cauchy–Schwarz inequality:
\[
\left| \langle \tilde{\mathrm{D}}f(\mathbf{Z})\Delta, E(\mathbf{Z})\Delta \rangle_F \right|
\le \|\tilde{\mathrm{D}}f(\mathbf{Z})\Delta\|_F \|E(\mathbf{Z})\Delta\|_F
\le \|\tilde{\mathrm{D}}f(\mathbf{Z})\|_F \|\Delta\|_{\mathrm{op}} \|E(\mathbf{Z})\Delta\|_F.
\]
Since \(\|\tilde{\mathrm{D}}f(\mathbf{Z})\|_F = \sqrt{d_x}\), we have:
\[
\left| \langle \tilde{\mathrm{D}}f(\mathbf{Z})\Delta, E(\mathbf{Z})\Delta \rangle_F \right|
\le \sqrt{d_x} \|\Delta\|_{\mathrm{op}} \left( \Lambda_1 \varepsilon \sqrt{d_z d_x} + \varepsilon \sqrt{2d_z \ln\tfrac{2d_x}{\delta}} \right).
\]

\subparagraph{Step 3: Final combination.}
Thus, with probability at least \(1-\delta\),
\[
\begin{aligned}
\left| \|\mathrm{D}f(\mathbf{Z})- \mathrm{D}f(\mathbf{Z})C^*\|_F^2 - \|\tilde{\mathrm{D}}f(\mathbf{Z}) - \tilde{\mathrm{D}}f(\mathbf{Z})C^*\|_F^2 \right|
&\le 2 \sqrt{d_x} \|\Delta\|_{\mathrm{op}} \left( \Lambda_1 \varepsilon \sqrt{d_z d_x} + \varepsilon \sqrt{2d_z \ln\tfrac{2d_x}{\delta}} \right) \\
&\quad + \|\Delta\|_{\mathrm{op}}^2 \left( \Lambda_1 \varepsilon \sqrt{d_z d_x} + \varepsilon \sqrt{2d_z \ln\tfrac{2d_x}{\delta}} \right)^2.
\end{aligned}
\]
Recalling \(\|\Delta\|_{\mathrm{op}} = \|I - C^*\|_{\mathrm{op}} \le 1 + \|C^*\|_{\mathrm{op}}\) and setting
\[
B(\delta) := \Lambda_1 \sqrt{d_z d_x} + \sqrt{2d_z \ln\tfrac{2d_x}{\delta}},
\]
the bound simplifies to:
\[
\left| \|\mathrm{D}f(\mathbf{Z})- \mathrm{D}f(\mathbf{Z})C^*\|_F^2 - \|\tilde{\mathrm{D}}f(\mathbf{Z}) - \tilde{\mathrm{D}}f(\mathbf{Z})C^*\|_F^2 \right|
\le (1 + \|C^*\|_{\mathrm{op}}) \left( 2\sqrt{d_x} B(\delta) \varepsilon + (1 + \|C^*\|_{\mathrm{op}}) B(\delta)^2 \varepsilon^2 \right).
\]


% \subsection{Robustness under Perturbation}
% When $A$ is only approximately block-diagonal, the Davis–Kahan $\sin\Theta$ theorem \citep{yu2014useful} implies that the top-$k$ eigenspace of $L_{\mathrm{sym}}$ remains close to the ideal indicator subspace as long as:
% \[
% \|A - A_{\text{ideal}}\|_2 \ll \lambda_{k+1} - \lambda_k.
% \]
% The eigengap $\lambda_{k+1} - \lambda_k$ is lower-bounded by the component separation, so small perturbations do not alter the cluster structure.




==> layout/abstract.tex <==
\chapter*{Abstract}
\pagenumbering{roman}

This thesis addresses causal inference and causal representation learning (CRL) for high-dimensional, time-varying data, with applications across fields such as precision medicine, marketing, and retail. 

The first contribution introduces the Causal Dynamic Variational Autoencoder (CDVAE), a model designed to estimate Individual Treatment Effects (ITEs) by capturing unobserved heterogeneity in treatment response due to latent risk factors. Unlike traditional approaches that assume some confounders are unobserved, CDVAE focuses on unobserved variables affecting \emph{only} the outcome sequence. CDVAE is grounded in theoretical guarantees concerning the validity of latent adjustment variables and generalization bounds on ITEs estimation error. Extensive evaluations on synthetic and real-world datasets show that CDVAE outperforms existing baselines. Moreover, we demonstrate that state-of-the-art models significantly improve their ITE estimates when augmented with the latent substitutes learned by CDVAE, approaching oracle-level performance without direct access to the true adjustment variables. 

The second contribution expands on the challenge of long-term treatment effect estimation through a novel approach to counterfactual regression over time, prioritizing computational efficiency and long-term forecasting accuracy. By leveraging Recurrent Neural Networks (RNNs) enhanced with Contrastive Predictive Coding (CPC) and Information Maximization (InfoMax), the model captures long-term dependencies in the presence of time-varying confounders while avoiding the computational costs associated with transformers. This framework achieves state-of-the-art results in counterfactual estimation across synthetic and real-world datasets and is the first to incorporate CPC into causal inference. 

The third contribution tackles Causal Representation Learning (CRL), which seeks to uncover high-level latent factors that influence complex, high-dimensional observations. While recent advances in CRL have emphasized identifiability in the latent space, they often leave open the interpretability of how latent causes manifest in the observed variables—especially in structured data such as longitudinal tabular records. In this work, we introduce a model-agnostic interpretability layer grounded in the geometry of the decoder's Jacobian. By enforcing a sparse self-expression prior on the Jacobian columns, we induce a modular structure wherein observed features are grouped according to shared latent influences. This constraint enables the recovery of meaningful, potentially overlapping clusters of observed variables, reflecting the underlying generative graph. We provide formal conditions under which these clusters can be consistently identified: in the disjoint setting, we prove subspace detection guarantees using tools from sparse subspace clustering; in the overlapping case, we derive misclassification bounds under a structured latent-feature model that combines sparsity, incoherence, and dominance conditions. Our results demonstrate that latent-to-observed causal structure can be recovered from gradient geometry without restrictive assumptions such as anchor features or single-parent decoding. Beyond the theoretical contributions, we propose efficient Jacobian-based regularization techniques that scale to high-dimensional domains. 


% The third contribution tackles causal representation learning in complex, high-dimensional data. To enhance the transparency of causal models, we propose a flexible framework that links latent causal abstractions to observable data, moving beyond simplistic single-latent-factor constraints. By introducing structural sparsity patterns and grouping structures, we improve interpretability, allowing for a more nuanced understanding of latent causal factors in real-world datasets. Applied to Saint-Gobain purchase data, our approach demonstrates the effectiveness of sparse subspace clustering for model readability and practical insight into causal dependencies within observational data.

==> layout/secondpage.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%% Modèle pour la 4ème de couverture des thèses préparées à l'Université Paris-Saclay, basé sur le modèle produit par Nikolas STOTT / Template for back cover of thesis made at Université Paris-Saclay, based on the template made by Nikolas STOTT
%%% Mis à jour par Aurélien ARNOUX (École polytechnique)/ Updated by Aurélien ARNOUX (École polytechnique)
%%% Les instructions concernant chaque donnée à remplir sont données en bloc de commentaire / Rules to fill this file are given in comment blocks
%%% ATTENTION Ces informations doivent tenir sur une seule page une fois compilées / WARNING These informations must contain in no more than one page once compiled
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%% Version du 23 mai 2019 (Merci à Thibault CHEVALÉRIAS (CEA) pour ses suggestions et corrections)
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


\label{form_last}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%% Formulaire / Form
%%% Remplacer les paramètres des \newcommand par les informations demandées / Replace \newcommand parameters by asked informations
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\input{layout/firstpage}

\newcommand{\logoEd}{ed}																		%% Logo de l'école doctorale. Indiquer le sigle / Doctoral school logo. Indicate the acronym : 2MIB; AAIF; ABIES; BIOSIGNE; CBMS; EDMH; EDOM; EDPIF; EDSP; EOBE; INTERFACES; ITFA; PHENIICS; SDSV; SDV; SHS; SMEMAG; SSMMH; STIC
%{3 à 6 mots clés}	
%% Mots clés en français, séprarés par des , / Keywords in french, separated by ,

\newcommand{\abstractFR}													%% Résumé en français / abstract in french
{Cette thèse aborde l'inférence causale et l'apprentissage de représentations causales (CRL) pour des données de haute dimension et évolutives dans le temps, avec des applications dans des domaines tels que la médecine de précision, le marketing et la vente au détail. La première contribution introduit le Causal Dynamic Variational Autoencoder (CDVAE), un modèle conçu pour estimer les Effets de Traitement Individuels (ITE) en capturant l’hétérogénéité non observée dans les réponses aux traitements, due à des facteurs de risque latents. Contrairement aux approches traditionnelles qui supposent que tous les variables confondantes sont observées, CDVAE se concentre sur les variables non observées influençant la séquence des réponses. Grâce à des garanties théoriques en termes d’identifiabilité et de bornes de généralisation sur l’estimation des ITE, CDVAE atteint des performances proches de celles d’un oracle, surpassant les modèles actuels de pointe sur des ensembles de données synthétiques et semi-synthétiques. La deuxième contribution traite du défi de l’estimation des effets de traitement à long terme à travers une approche de régression contrefactuelle dans le temps, en privilégiant l’efficacité computationnelle et la précision des prévisions à long terme. En s’appuyant sur des Réseaux de Neurones Récurrents (RNN) améliorés avec le Codage Prédictif Contrastif (CPC) et la Maximisation de l’Information (InfoMax), le modèle capture les dépendances à long terme en présence de variables confondantes évolutives sans avoir recours aux architectures de transformers. Ce cadre réalise des réponses de pointe en estimation contrefactuelle sur des ensembles de données synthétiques et réelles et constitue la première intégration du Codage Prédictif Contrastif dans l’inférence causale. La troisième contribution aborde l’apprentissage de représentations causales dans des données complexes et de haute dimension. Pour améliorer la transparence des modèles causaux, nous proposons un cadre flexible qui relie les abstractions causales latentes aux données observables. En introduisant des contraintes de parcimonie structurelle et des structures de regroupement, nous améliorons l’interprétabilité, permettant une compréhension plus nuancée des facteurs causaux latents dans des ensembles de données réelles. Appliquée aux données d’achats de Saint-Gobain et aux données médicales de MIMIC III, notre approche démontre l’efficacité du regroupement de sous-espaces parcimonieux pour l'interprétabilité du modèle.}
%% Titre de la thèse en anglais / Thesis title in english
\newcommand{\keywordsEN}{Causal Inference, Longitudinal Data, Causal Representation Learning, Counterfactual Regression, Latent Variable Modeling }	
%% Mots clés en anglais, séprarés par des , / Keywords in english, separated by ,
\newcommand{\abstractEN}															%% Résumé en anglais / abstract in english
{This thesis addresses causal inference and causal representation learning (CRL) for high-dimensional, time-varying data, with applications across fields such as precision medicine, marketing, and retail. The first contribution introduces the Causal Dynamic Variational Autoencoder (CDVAE), a model designed to estimate Individual Treatment Effects (ITEs) by capturing unobserved heterogeneity in treatment response due to latent risk factors. Unlike traditional approaches that assume all confounders are observed, CDVAE focuses on unobserved variables influencing the outcome sequence. Through theoretical guarantees in identifiability and generalization bounds on ITE estimation, CDVAE achieves near-oracle performance on both synthetic and semi-synthetic datasets, outperforming current state-of-the-art models. The second contribution expands on the challenge of long-term treatment effect estimation through a novel approach to counterfactual regression over time, prioritizing computational efficiency and long-term forecasting accuracy. By leveraging Recurrent Neural Networks (RNNs) enhanced with Contrastive Predictive Coding (CPC) and Information Maximization (InfoMax), the model captures long-term dependencies in the presence of time-varying confounders while avoiding the computational costs associated with transformers. This framework achieves state-of-the-art results in counterfactual estimation across synthetic and real-world datasets and is the first to incorporate Contrastive Predictive Encoding into causal inference. The third contribution tackles causal representation learning in complex, high-dimensional data. To enhance the transparency of causal models, we propose a flexible framework that links latent causal abstractions to observable data, moving beyond simplistic single-latent-factor constraints. By introducing structural sparsity patterns and grouping structures, we improve interpretability, allowing for a more nuanced understanding of latent causal factors in real-world datasets. Applied to Saint-Gobain purchase data and MIMIC III medical data, our approach demonstrates the effectiveness of sparse subspace clustering for model readability and practical insight into causal dependencies within observational data.}
\label{layout_last}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%% Mise en page / Page layout      
%%% NE RIEN MODIFIER / DO NOT MODIFY
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\pagestyle{empty}

%%% Logo de l'école doctorale. Le nom du fichier correspond au sigle de l'ED / Doctoral school logo. Filename correspond to doctoral school acronym
%%% Les noms valides sont / Valid names are : 2MIB; AAIF; ABIES; BIOSIGNE; CBMS; EDMH; EDOM; EDPIF; EDSP; EOBE; INTERFACES; ITFA; PHENIICS; SDSV; SDV; SHS; SMEMAG; SSMMH; STIC
\begin{textblock*}{61mm}(16mm,3mm)
    \textblockcolour{white}
	\noindent\includegraphics[height=24mm]{media/ed/logo_usp_INTERFACES.png}
\end{textblock*}



%%%Titre de la thèse en français / Thesis title in french
\begin{singlespace}
\begin{center}
\fcolorbox{bordeau}{white}{\parbox{0.95\textwidth}{
{\bf Titre:} \PhDTitleFR 
\medskip

%%%Mots clés en français, séprarés par des ; / Keywords in french, separated by ;
{\bf Mots clés:} \keywordsFR 
\vspace{-2mm}

%%% Résumé en français / abstract in french
\begin{multicols}{2}
{\bf Résumé:} 
\abstractFR 
\end{multicols}
}}
\end{center}

\vspace*{0mm}

%%%Titre de la thèse en anglais / Thesis title in english
\begin{center}
\fcolorbox{bordeau}{white}{\parbox{0.95\textwidth}{
{\bf Title:} \PhDTitleEN 

\medskip

%%%Mots clés en anglais, séprarés par des ; / Keywords in english, separated by ;
{\bf Keywords:}  \keywordsEN %%3 à 6 mots clés%%
\vspace{-2mm}
\begin{multicols}{2}
	
%%% Résumé en anglais / abstract in english
{\bf Abstract:} 
\abstractEN
\end{multicols}
}}
\end{center}

\begin{textblock*}{161mm}(10mm,270mm)
\textblockcolour{white}
\color{bordeau}
{\bf\noindent Université Paris-Saclay	         }

\noindent Espace Technologique / Immeuble Discovery 

\noindent Route de l’Orme aux Merisiers RD 128 / 91190 Saint-Aubin, France 
\end{textblock*}

\begin{textblock*}{0mm}(182mm,255mm)
\textblockcolour{white}
\includegraphics[width=20mm]{media/UPSACLAY-petit}
\end{textblock*}
\end{singlespace}
